ALPACA -- Adaptive Learning Pipeline for Comprehensive AI

The advancement of AI technologies has greatly increased the complexity of AI pipelines as they include many stages such as data collection, pre-processing, training, evaluation and visualisation. To provide effective and accessible AI solutions, it is important to design pipelines for different user groups such as experts, professionals from different fields and laypeople. Ease of use and trust play a central role in the acceptance of AI systems. The presented system, ALPACA (Adaptive Learning Pipeline for Advanced Comprehensive AI Analysis), offers a comprehensive AI pipeline that addresses the needs of diverse user groups. ALPACA integrates visual and code-based development and facilitates all key phases of the AI pipeline. Its architecture is based on Celery (with Redis backend) for efficient task management, MongoDB for seamless data storage and Kubernetes for cloud-based scalability and resource utilisation. Future versions of ALPACA will support modern techniques such as federated and continuous learning as well as explainable AI methods to further improve security, usability and trustworthiness. The application is demonstrated by an Android app for similarity recognition, which emphasises ALPACA's potential for use in everyday life.

==> Chapters/09_Conclusion_old.tex <==
\section{Conclusion and Future Directions}
\label{sec:Conclusion}

%Must answer:

%\item Is it possible to develop a universally applicable AI pipeline that remains usable for different user groups?
%
%\item Can an AI ecosystem be enriched by incorporating input from different user groups?
%
%\item How can such a pipeline be expanded by experts and still be operable by laypeople?
%
%\item Can the output and decision-making processes of AI pipelines be made comprehensible for all %user groups?
%
%\item Can a system like ALPACA lead to an ecosystem where different user groups can participate and %different neglected domains can also be penetrated by AI?

The introduction of artificial intelligence into everyday life and the resulting ever-faster development of AI systems are leading to an ever-increasing need for systematic AI pipelines that can seamlessly integrate various phases such as data collection, preparation, model generation, and evaluation. Data is becoming more and more complex, and the constant change also requires constantly adaptable and easy-to-maintain systems. These AI pipeline systems are intricate networks of interconnected data processing and analysis stages, each playing a unique role in transforming raw data into meaningful insights. ALPACA (Adaptive Learning Pipeline for Advanced Comprehensive AI Analysis) addresses these problems and presents a solution to this challenge.

One of the most important features of ALPACA is that it is designed as a universal, extensible AI pipeline framework and is aimed at various user groups, from data scientists and AI experts to specialists in other fields, students, and laypeople.  ALPACA's system design was chosen so that it can be expanded without interfering with the existing code. This offers users and developers the opportunity to continuously improve the performance of the system, integrate new functions and thus solve new challenges through the use of AI. Additionally, the paper highlights the critical role of user experience and usability in building trust in AI systems and highlights the need for domain-agnostic AI pipelines that can support users across different knowledge levels. ALPACA achieves this through the harmonious integration of complex technical components and the convergent design of a user-behaviour-sensitive visual interface. This achieves a unified user interface across all pipeline levels and all necessary tools. This facilitates access and opens the door to an ecosystem where different user groups can experiment and contribute their expertise, as well as train, analyze, and evaluate models.

Another important feature of ALPACA lies in its ability to use graphics processing units (GPUs) for data preprocessing and model training. This integration significantly increases computing speed, especially in complex network configurations, and provides scalability and cost efficiency through cloud computing. The paper highlights the transformative potential of GPU-accelerated AI, making AI pipelines more efficient and accessible to a wider audience.

In addition, ALPACA offers solutions tailored to different user groups to meet their needs and ensure efficient use of the pipeline:
\begin{itemize}

\item \textbf{Data scientists and AI experts:} ALPACA optimizes workflows and enables efficient experimentation with different algorithms and hyperparameters. By securing intermediate results, extensive collaboration is enabled, which increases the exchange of knowledge and productivity.

\item \textbf{Specialists in other areas:} Subject-specific experts leverage ALPACA's user-friendly interfaces and automated workflows, bridging the gap between their expertise and advanced AI techniques. This democratization of AI enables subject-matter experts to harness the power of AI in their respective fields.

\item \textbf{Students and laypeople:} ALPACA serves as an educational platform and can offer interactive tutorials, example projects, and guided exercises. Exploratory learning allows people without specific AI knowledge to experiment with models and overcome real-world challenges, fostering a culture of continuous learning and increasing public acceptance of AI.

\end{itemize}

To illustrate the versatility of ALPACA, the paper presents a demo scenario in the field of Android similarity detection. This practical application demonstrates ALPACA's ability to handle complex AI tasks while remaining accessible and understandable to a wide range of users. Additionally, the demo scenario shows how a crowdsourcing approach can solve the often complex problem of data categorization by harnessing the power of the crowd.

The article raises interesting research questions, examines the feasibility of universally applicable AI pipelines that serve different user groups, and examines how AI ecosystems can benefit from the participation of different user groups.

In summary, ALPACA represents a significant advance in the development of AI pipelines, offering a user-centric approach that embraces inclusivity, ease of use, and collaboration. By addressing the challenges of complexity and accessibility, ALPACA is paving the way for a future where AI becomes an integral part of diverse fields, breaking down barriers and democratizing access to the transformative power of artificial intelligence. In addition, ALPACA's overall architectural design based on modularity, scalability, and user-centred design proves to be a powerful and adaptable tool for comprehensive AI analysis of mobile applications. By seamlessly integrating data management, user interaction and ethical considerations, the ALPACA system allows users to participate in the analysis process while maintaining standards of transparency, privacy and reproducibility.


==> Chapters/OldSota.tex <==
\section{State of the Art}
\label{sec:stateoftheart}

Artificial Intelligence (AI) pipelines serve as fundamental constructs in the contemporary landscape of AI systems, facilitating their efficient use from initial development to deployment and maintenance of AI models. These pipelines orchestrate a series of sequential steps that transmute raw data into a useful output \cite{Baylor.2017}. This output can range from a refined dataset over a trained AI model to a complete prediction system and typically includes the stages of data preprocessing, model training, model evaluation, data prediction, and eventually the deployment on, e.g., cloud or edge infrastructure \cite{Steidl.2023}. A central advantage of AI pipelines is their capacity to automate repetitive and time-intensive tasks inherent to AI development, including data refinement, feature engineering, and model selection \cite{Radanliev.2023}. By mechanizing these processes, AI pipelines substantially mitigate temporal and cognitive demands, simplifying the harnessing of AI for real-world problem resolution \cite{Radanliev.2023}. According to \cite{Hummer.2019} this time-saving advantage can be extended by using parallel computing, which saves up to 7\% of time. 

Various tools and frameworks are available for constructing AI pipelines. These pipelines range from individual and highly specialized pipelines designed for a specific use case to cloud-based online pipelines covering many use cases and providing many tools and techniques. 

On the side of specialized pipelines, in the last years, a lot of research has been published, like KoopaML \cite{GarciaHolgado.2022} or IPMP \cite{Frey.2020} in the medicine and health care sector or \cite{Albertsson.08.07.2018} in physics. 

On the other side, cloud-based pipelines are also available, mostly driven by global players like the Google Cloud Vertex AI Pipelines \cite{google.vertex.2023}, Amazon SageMaker \cite{AmazonWebServicesInc.26.10.2023}, Microsoft Azure Machine Learning \cite{Microsoft.Azure.31.10.2023b}, IBM Watson Studio \cite{IBM.Watson.2022b} or Databricks \cite{Databricks.31.10.2023b}. These cloud-based pipelines provide a comprehensive platform for establishing, deploying, and overseeing end-to-end machine learning workflows. However, the high cost and complexity of these cloud-based pipelines represent a barrier to entry for many people. An alternative way was shown by the AI4EU project which was a European-driven project fostering a "European Artificial Intelligence On-Demand Platform and Ecosystem“ \cite{AI4EU.2023}. In contrast to most other cloud-based AI pipelines, it "brings together the AI community“ \cite{AIWatch.31.10.2023} and was designed to transfer knowledge from research to business applications. In this context, it can be used by experts who are developing AI components and providing them for the community, as well as by laypeople without any AI knowledge.

But none of the pipelines developed so far have managed to deliver a universal solution that can be used by anyone in every context. Therefore, research on AI pipeline design is an active realm of investigation, aiming to enhance both efficiency and efficacy \cite{Steidl.2023}. For instance, one recent study presents AutoAI, an advanced autonomous AI design based on cutting-edge algorithms \cite{Radanliev.2023}, while \cite{Baylor.2017} present TFX, a Tensorflow-based AI platform.  \cite{Steidl.2023} investigates some research in the context of AI pipelines and derives a taxonomy of requirements that future AI pipelines must fulfill. According to \cite{Steidl.2023}, one of the key challenges in systematizing, unifying, and expanding AI pipelines is the identification and structural organization of the central conceptual ideas. Furthermore, they found out that currently, no end-to-end pipeline exists that covers the complete AI lifecycle "from data collection to AI model deployment and monitoring in production". All in all, they discover lacks in all phases of AI pipelines, from data collection, over versioning of any pipeline step, and every generated artifact step to the operating business of the entire pipeline. To tackle these issues, the author's effort addresses inquiries related to the terminological nuances, tasks, and challenges inherent to AI pipelines. In this context, they introduce a taxonomy of a  four-stage AI pipeline, including data handling, model learning, software development, and system operations.


==> Decissions/ACM_TKDD_1.tex <==
Dear Mr. Torka:

I write you in regards to manuscript # TKDD-2023-12-0860 entitled "ALPACA - Adaptive Learning Pipeline for Advanced Comprehensive AI Analysis" which you submitted to the Transactions on Knowledge Discovery from Data.

In view of the criticisms of the reviewer(s) found at the bottom of this letter, your manuscript has been denied publication in the Transactions on Knowledge Discovery from Data.

Thank you for considering the Transactions on Knowledge Discovery from Data for the publication of your research. I hope the outcome of this specific submission will not discourage you from the submission of future manuscripts.

Sincerely,
Dr Jian Pei
Editor in Chief, Transactions on Knowledge Discovery from Data
jpei@cs.sfu.ca

Editor's Comments to Author:

Associate Editor
Comments to the Author:
In this paper, the authors proposed a comprehensive and holistic adaptive learning framework, which can be used for Android similarity detection.

The reviewers agree that the paper needs significant improvement before it's ready for publication, such as limited novelty, lack of discussion and comparison with SOTA, etc.

Reviewer(s)' Comments to Author:

Reviewer: 1

Recommendation: Minor Revision

Comments:
Strengths:
1. The proposed system is end-to-end framework, starting from data collection to model evaluation and data visualization.
2. The proposed system has a bunch of rich features, including data collection, data preprocessing, etc.
3. The presentation of this paper is good and easy to follow.

Weakness:
1. What AI algorithms are available for the users to choose? In Figure 7, there are only two auto-encoder based algorithms available, which is not enough to deal with various machine learning tasks. Are there any classification methods? More details are required.
2. The contributions of this paper are still vague. In Section 2, the authors list quick a few existing AI system. I highly recommend that the authors compare the difference between these systems and the proposed ALPACA in a table, which will highlight the major difference and showcase the contribution of the proposed ALPACA.
3. Students usually have limited knowledge on AI field, especially for some beginners. Will it be better to provide some explanation of each hyper-parameter (e.g., configuration in Figure 8)? Are there any features designed for students and laypeople, since the authors mention that this system is designed for various groups of people?

Additional Questions:
Review's recommendation for paper type: Full length technical paper

Does the paper present innovative ideas or material?: No

In what ways does this paper advance the field?: This paper proposed an end-to-end AI system for various groups of people with different expertise. However, the authors do not emphasize the contribution of the proposed method compared with the existing machine learning systems.

Rate how well the ideas are presented (very difficult to understand=1 very easy to understand =5): 3

Rate the information in the paper is it sound, factual, and accurate?(poor=1 excellent=5): 3

Please explain why.: See detailed comments below.

Rate the paper on its contribution to the body of knowledge to this field (none=1, very important=5): 3

Rate the overall quality of the writing (very poor=1, excellent=5): 4

Does this paper cite and use appropriate references?: Yes

If not, what important references are missing?:

Is the treatment of the subject complete?: Yes

If not, What important details / ideas/ analyses are missing?:

Please help ACM create a more efficient time-to-publication process: Using your best judgment, what amount of copy editing do you think this paper needs?: Moderate

Most ACM journal papers are researcher-oriented. Is this paper of potential interest to developers and engineers?: Yes


Reviewer: 2

Recommendation: Reject

Comments:
This paper introduces the ALPACA system. It is designed as an adaptive AI pipeline that is trustworthy, expandabale, and scalable and is suitable for users with different levels of expertise. The authors provide detailed information about the system design and implementation details for each stage. Please see my concerns about the paper below.

- My major concern is that this paper is more like a technical report about system implementation, while there are not much focus about its impact to knowledge discovery from data and how we can use the system to advance the field. I wonder whether this paper would be a good fit for this journal.

- In Section 2, it would be better if the authors could discuss similarities and differences of the existing pipelines compared to the ALPACA. For example, how do AI4EU differ from ALPACA if both are designed for AI experts and laypeople? Similar discussions for other related pipelines would signify the importance of ALPACA.

- It seems that main focus lies in introducing how to use this app for similar Android app detection (e.g., collecting data from app stores, preprocessing data based on the collected APK files), while the claims in Section 1 is more about a versatile AI pipelines that can be used in various application scnearios. More discussions about how to use ALPACA for other application scenarios are needed, e.g., how do we use data collector to collect data from different modes (e.g., image, video, text, graph), how would these data be preprocessed for the next stage in ALPACA.

- In Stage 3, is there any way that the user could develop their own model and import it into the system? If so, how to do that? Otherwise, please provide some rationale about why this functionality is not needed in ALPACA.

Additional Questions:
Review's recommendation for paper type: Full length technical paper

Does the paper present innovative ideas or material?: No

In what ways does this paper advance the field?:

Rate how well the ideas are presented (very difficult to understand=1 very easy to understand =5): 3

Rate the information in the paper is it sound, factual, and accurate?(poor=1 excellent=5): 4

Please explain why.: The paper provides detailed information about the system design and implementation details, but not much novel ideas in the field of knowledge discovery.

Rate the paper on its contribution to the body of knowledge to this field (none=1, very important=5): 2

Rate the overall quality of the writing (very poor=1, excellent=5): 3

Does this paper cite and use appropriate references?: Yes

If not, what important references are missing?:

Is the treatment of the subject complete?: Yes

If not, What important details / ideas/ analyses are missing?:

Please help ACM create a more efficient time-to-publication process: Using your best judgment, what amount of copy editing do you think this paper needs?: Heavy

Most ACM journal papers are researcher-oriented. Is this paper of potential interest to developers and engineers?: Maybe


Reviewer: 3

Recommendation: Reject

Comments:
TKDD focuses on the theory, methodologies, and applications in knowledge discovery and data mining. This includes developing algorithms and frameworks that significantly enhance understanding or discovery from data. The ALPACA paper, however, is more about creating an AI pipeline framework focused on infrastructure and usability rather than advancing the field of data mining or knowledge discovery.

The manuscript lacks a clear focus on data mining techniques or methods for discovering novel patterns or insights from data. The examples given, like Android similarity detection, do not introduce or apply any new data mining algorithms. The analysis relies on existing tools (e.g., AndroGuard for APK analysis) without any new methods or contributions that enhance knowledge discovery.

The ALPACA framework primarily focuses on integrating existing technologies like Kubernetes, Celery, Redis, and MongoDB into an AI pipeline. This combination is not particularly novel, as these tools are already widely used in the industry for similar purposes. The use of these tools together for scalability, task orchestration, and data storage does not represent a significant advance in the field of AI pipelines.
The core functionalities of ALPACA, such as data preprocessing, model training, and evaluation, are standard components of many AI pipelines. The paper lacks a distinctive methodological contribution or a new algorithmic innovation that differentiates it from other AI pipeline frameworks. The idea of creating a user-friendly AI pipeline is valuable, but it does not introduce a new concept or approach that could be considered groundbreaking.

The paper does not adequately address the state-of-the-art in AI pipeline design. There is a lack of comparison with recent advancements in the field, such as pipelines that incorporate federated learning, self-supervised learning, or advanced optimization techniques. The manuscript lacks a detailed evaluation against other AI pipeline frameworks (like TFX, MLflow, Kubeflow) in terms of performance, usability, scalability, or flexibility, which would be necessary to claim any significant improvement or innovation.

Additional Questions:
Review's recommendation for paper type: Full length technical paper

Does the paper present innovative ideas or material?: No

In what ways does this paper advance the field?:

Rate how well the ideas are presented (very difficult to understand=1 very easy to understand =5): 3

Rate the information in the paper is it sound, factual, and accurate?(poor=1 excellent=5): 2

Please explain why.: The paper's emphasis on creating a user-centric AI pipeline and discussing its deployment and scalability aspects diverges from TKDD’s core themes. While making AI tools accessible is valuable, the lack of novel contributions to knowledge discovery or data mining makes this work less suitable for TKDD.

Rate the paper on its contribution to the body of knowledge to this field (none=1, very important=5): 2

Rate the overall quality of the writing (very poor=1, excellent=5): 2

Does this paper cite and use appropriate references?: Yes

If not, what important references are missing?:

Is the treatment of the subject complete?: No

If not, What important details / ideas/ analyses are missing?: The core functionalities of ALPACA, such as data preprocessing, model training, and evaluation, are standard components of many AI pipelines. The paper lacks a distinctive methodological contribution or a new algorithmic innovation that differentiates it from other AI pipeline frameworks. The idea of creating a user-friendly AI pipeline is valuable, but it does not introduce a new concept or approach that could be considered groundbreaking.

Please help ACM create a more efficient time-to-publication process: Using your best judgment, what amount of copy editing do you think this paper needs?: Moderate

Most ACM journal papers are researcher-oriented. Is this paper of potential interest to developers and engineers?: No 

==> Decissions/ger.tex <==
Sehr geehrter Herr Torka,

Ich schreibe Ihnen in Bezug auf das Manuskript Nr. TKDD-2023-12-0860 mit dem Titel „ALPACA – Adaptive Learning Pipeline for Advanced Comprehensive AI Analysis“, das Sie bei Transactions on Knowledge Discovery from Data eingereicht haben.

Aufgrund der Kritik der Gutachter, die Sie am Ende dieses Briefes finden, wurde die Veröffentlichung Ihres Manuskripts bei Transactions on Knowledge Discovery from Data abgelehnt.

Vielen Dank, dass Sie Transactions on Knowledge Discovery from Data für die Veröffentlichung Ihrer Forschung in Betracht ziehen. Ich hoffe, das Ergebnis dieser speziellen Einreichung wird Sie nicht davon abhalten, zukünftige Manuskripte einzureichen.

Mit freundlichen Grüßen
Dr. Jian Pei
Chefredakteur, Transactions on Knowledge Discovery from Data
jpei@cs.sfu.ca


Anmerkungen des Herausgebers an den Autor:

Mitherausgeber
Anmerkungen an den Autor:
In diesem Artikel schlagen die Autoren ein umfassendes und ganzheitliches adaptives Lernframework vor, das zur Erkennung von Android-Ähnlichkeiten verwendet werden kann.

Die Gutachter sind sich einig, dass das Papier vor der Veröffentlichung noch erheblich verbessert werden muss, z. B. aufgrund begrenzter Neuartigkeit, fehlender Diskussion und Vergleich mit SOTA usw.

Anmerkungen des/der Gutachter(s) an den Autor:

Gutachter: 1

Empfehlung: Kleine Überarbeitung

Anmerkungen:
Stärken:
1. Das vorgeschlagene System ist ein End-to-End-Framework, das von der Datenerfassung bis zur Modellbewertung und Datenvisualisierung reicht.
2. Das vorgeschlagene System verfügt über eine Reihe umfangreicher Funktionen, darunter Datenerfassung, Datenvorverarbeitung usw.
3. Die Präsentation dieses Artikels ist gut und leicht verständlich.

Schwäche:
1. Welche KI-Algorithmen stehen den Benutzern zur Auswahl? In Abbildung 7 sind nur zwei auf Auto-Encoder basierende Algorithmen verfügbar, was für die Bewältigung verschiedener Aufgaben des maschinellen Lernens nicht ausreicht. Gibt es Klassifizierungsmethoden? Weitere Details sind erforderlich.
2. Die Beiträge dieses Papiers sind noch vage. In Abschnitt 2 listen die Autoren kurz einige bestehende KI-Systeme auf. Ich empfehle den Autoren dringend, die Unterschiede zwischen diesen Systemen und dem vorgeschlagenen ALPACA in einer Tabelle zu vergleichen, die die Hauptunterschiede hervorhebt und den Beitrag des vorgeschlagenen ALPACA zeigt.
3. Studenten haben im Allgemeinen nur begrenzte Kenntnisse im KI-Bereich, insbesondere einige Anfänger. Wäre es besser, einige Erklärungen zu jedem Hyperparameter bereitzustellen (z. B. Konfiguration in Abbildung 8)? Gibt es Funktionen, die für Studenten und Laien entwickelt wurden, da die Autoren erwähnen, dass dieses System für verschiedene Personengruppen entwickelt wurde?

Zusätzliche Fragen:

Empfehlung der Rezension für den Papiertyp: Vollständiges technisches Papier

Enthält das Papier innovative Ideen oder Material?: Nein

Inwiefern bringt dieses Papier das Feld voran?: Dieses Papier schlägt ein End-to-End-KI-System für verschiedene Personengruppen mit unterschiedlichem Fachwissen vor. Die Autoren betonen jedoch nicht den Beitrag der vorgeschlagenen Methode im Vergleich zu den bestehenden maschinellen Lernsystemen.

Bewerten Sie, wie gut die Ideen präsentiert werden (sehr schwer zu verstehen = 1, sehr leicht zu verstehen = 5): 3

Bewerten Sie die Informationen im Papier: Sind sie fundiert, sachlich und genau? (schlecht = 1, ausgezeichnet = 5): 3

Bitte erklären Sie, warum.: Siehe ausführliche Kommentare unten.

Bewerten Sie den Beitrag des Artikels zum Wissensbestand in diesem Bereich (kein Beitrag = 1, sehr wichtig = 5): 3

Bewerten Sie die allgemeine Qualität des Textes (sehr schlecht = 1, ausgezeichnet = 5): 4

Zitiert und verwendet dieser Artikel entsprechende Referenzen?: Ja

Wenn nicht, welche wichtigen Referenzen fehlen?:

Ist die Behandlung des Themas vollständig?: Ja

Wenn nicht, welche wichtigen Details/Ideen/Analysen fehlen?:

Bitte helfen Sie ACM dabei, einen effizienteren Veröffentlichungsprozess zu schaffen: Wie viel Lektorat benötigen Sie nach bestem Wissen und Gewissen für diesen Artikel?: Mäßig

Die meisten ACM-Zeitschriftenartikel sind forschungsorientiert. Ist dieser Artikel für Entwickler und Ingenieure von potenziellem Interesse?: Ja

Gutachter: 2

Empfehlung: Ablehnen

Kommentare:
Dieses Papier stellt das ALPACA-System vor. Es ist als adaptive KI-Pipeline konzipiert, die vertrauenswürdig, erweiterbar und skalierbar ist und sich für Benutzer mit unterschiedlichem Fachwissen eignet. Die Autoren liefern detaillierte Informationen zum Systemdesign und zu Implementierungsdetails für jede Phase. Meine Bedenken bezüglich des Papiers finden Sie weiter unten.

- Meine größte Sorge ist, dass dieses Papier eher einem technischen Bericht über die Systemimplementierung ähnelt, während nicht viel Wert auf dessen Auswirkungen auf die Wissensentdeckung aus Daten und darauf gelegt wird, wie wir das System nutzen können, um das Feld voranzubringen. Ich frage mich, ob dieses Papier gut in diese Zeitschrift passen würde.

- In Abschnitt 2 wäre es besser, wenn die Autoren Ähnlichkeiten und Unterschiede der bestehenden Pipelines im Vergleich zu ALPACA diskutieren könnten. Wie unterscheidet sich beispielsweise AI4EU von ALPACA, wenn beide für KI-Experten und Laien konzipiert sind? Ähnliche Diskussionen für andere verwandte Pipelines würden die Bedeutung von ALPACA verdeutlichen.

- Es scheint, dass der Hauptfokus auf der Einführung liegt, wie diese App zur Erkennung ähnlicher Android-Apps verwendet werden kann (z. B. Sammeln von Daten aus App-Stores, Vorverarbeiten von Daten basierend auf den gesammelten APK-Dateien), während sich die Behauptungen in Abschnitt 1 eher auf vielseitige KI-Pipelines beziehen, die in verschiedenen Anwendungsszenarien verwendet werden können. Weitere Diskussionen darüber, wie ALPACA für andere Anwendungsszenarien verwendet werden kann, sind erforderlich, z. B. wie wir den Datensammler verwenden, um Daten aus verschiedenen Modi (z. B. Bild, Video, Text, Grafik) zu sammeln, wie diese Daten für die nächste Phase in ALPACA vorverarbeitet werden würden.

- Gibt es in Phase 3 eine Möglichkeit, dass der Benutzer sein eigenes Modell entwickeln und in das System importieren kann? Wenn ja, wie geht das? Andernfalls geben Sie bitte eine Begründung dafür an, warum diese Funktionalität in ALPACA nicht benötigt wird.

Zusätzliche Fragen:
Empfehlung der Rezension für den Papiertyp: Vollständiges technisches Papier

Enthält das Papier innovative Ideen oder Materialien?: Nein

Inwiefern bringt dieses Papier das Feld voran?:

Bewerten Sie, wie gut die Ideen präsentiert werden (sehr schwer zu verstehen = 1, sehr leicht zu verstehen = 5): 3

Bewerten Sie die Informationen im Papier: Sind sie fundiert, sachlich und genau? (schlecht = 1, ausgezeichnet = 5): 4

Bitte erklären Sie, warum: Das Papier bietet detaillierte Informationen über das Systemdesign und die Implementierungsdetails, aber nicht viele neue Ideen im Bereich der Wissensentdeckung.

Bewerten Sie den Beitrag des Artikels zum Wissensbestand in diesem Bereich (kein Beitrag = 1, sehr wichtig = 5): 2

Bewerten Sie die allgemeine Qualität des Textes (sehr schlecht = 1, ausgezeichnet = 5): 3

Zitiert und verwendet dieser Artikel entsprechende Referenzen?: Ja

Wenn nicht, welche wichtigen Referenzen fehlen?:

Ist die Behandlung des Themas vollständig?: Ja

Wenn nicht, welche wichtigen Details/Ideen/Analysen fehlen?:

Bitte helfen Sie ACM dabei, einen effizienteren Veröffentlichungsprozess zu schaffen: Wie viel Lektorat benötigen Sie nach bestem Wissen und Gewissen für diesen Artikel?: Umfangreich

Die meisten ACM-Zeitschriftenartikel sind forschungsorientiert. Ist dieser Artikel für Entwickler und Ingenieure von potenziellem Interesse?: Vielleicht

Gutachter: 3

Empfehlung: Ablehnen

Kommentare:
TKDD konzentriert sich auf die Theorie, Methoden und Anwendungen in der Wissensentdeckung und im Data Mining. Dazu gehört die Entwicklung von Algorithmen und Frameworks, die das Verständnis oder die Entdeckung aus Daten deutlich verbessern. Im ALPACA-Artikel geht es jedoch eher um die Erstellung eines KI-Pipeline-Frameworks mit Fokus auf Infrastruktur und Benutzerfreundlichkeit als um die Weiterentwicklung des Bereichs Data Mining oder Wissensentdeckung.

Dem Manuskript fehlt ein klarer Fokus auf Data-Mining-Techniken oder -Methoden zur Entdeckung neuer Muster oder Erkenntnisse aus Daten. Die angeführten Beispiele, wie die Android-Ähnlichkeitserkennung, führen keine neuen Data-Mining-Algorithmen ein oder wenden sie an. Die Analyse basiert auf vorhandenen Tools (z. B. AndroGuard für die APK-Analyse) ohne neue Methoden oder Beiträge, die die Wissensentdeckung verbessern.

Das ALPACA-Framework konzentriert sich in erster Linie auf die Integration vorhandener Technologien wie Kubernetes, Celery, Redis und MongoDB in eine KI-Pipeline. Diese Kombination ist nicht besonders neuartig, da diese Tools in der Branche bereits weithin für ähnliche Zwecke verwendet werden. Die gemeinsame Verwendung dieser Tools für Skalierbarkeit, Aufgabenorchestrierung und Datenspeicherung stellt keinen bedeutenden Fortschritt im Bereich der KI-Pipelines dar.
Die Kernfunktionen von ALPACA, wie Datenvorverarbeitung, Modelltraining und -bewertung, sind Standardkomponenten vieler KI-Pipelines. Dem Papier fehlt ein unverwechselbarer methodischer Beitrag oder eine neue algorithmische Innovation, die es von anderen KI-Pipeline-Frameworks unterscheidet. Die Idee, eine benutzerfreundliche KI-Pipeline zu erstellen, ist wertvoll, führt jedoch kein neues Konzept oder keinen neuen Ansatz ein, der als bahnbrechend angesehen werden könnte.

Das Papier geht nicht ausreichend auf den neuesten Stand der KI-Pipeline-Entwicklung ein. Es fehlt ein Vergleich mit jüngsten Fortschritten in diesem Bereich, wie z. B. Pipelines, die föderiertes Lernen, selbstüberwachtes Lernen oder fortschrittliche Optimierungstechniken beinhalten. Dem Manuskript fehlt eine detaillierte Bewertung im Vergleich zu anderen KI-Pipeline-Frameworks (wie TFX, MLflow, Kubeflow) in Bezug auf Leistung, Benutzerfreundlichkeit, Skalierbarkeit oder Flexibilität, die erforderlich wäre, um eine signifikante Verbesserung oder Innovation zu behaupten.

Zusätzliche Fragen:
Empfehlung der Rezension für den Papiertyp: Vollständiges technisches Papier

Enthält das Papier innovative Ideen oder Materialien?: Nein

Inwiefern bringt dieses Papier das Feld voran?:

Bewerten Sie, wie gut die Ideen präsentiert werden (sehr schwer zu verstehen = 1, sehr leicht zu verstehen = 5): 3

Bewerten Sie die Informationen im Papier: Sind sie fundiert, sachlich und genau? (schlecht = 1, ausgezeichnet = 5): 2

Bitte erklären Sie, warum: Der Schwerpunkt des Papiers auf der Erstellung einer benutzerzentrierten KI-Pipeline und der Erörterung ihrer Bereitstellungs- und Skalierbarkeitsaspekte weicht von den Kernthemen von TKDD ab. Obwohl es wertvoll ist, KI-Tools zugänglich zu machen, ist diese Arbeit aufgrund des Mangels an neuartigen Beiträgen zur Wissensentdeckung oder zum Data Mining weniger für TKDD geeignet.

Bewerten Sie den Beitrag des Artikels zum Wissensbestand in diesem Bereich (keine=1, sehr wichtig=5): 2

Bewerten Sie die allgemeine Qualität des Textes (sehr schlecht=1, ausgezeichnet=5): 2

Zitiert und verwendet dieser Artikel entsprechende Referenzen?: Ja

Wenn nicht, welche wichtigen Referenzen fehlen?:

Ist die Behandlung des Themas vollständig?: Nein

Wenn nicht, welche wichtigen Details/Ideen/Analysen fehlen?: Die Kernfunktionen von ALPACA, wie Datenvorverarbeitung, Modelltraining und Auswertung, sind Standardkomponenten vieler KI-Pipelines. Dem Artikel fehlt ein unverwechselbarer methodischer Beitrag oder eine neue algorithmische Innovation, die ihn von anderen KI-Pipeline-Frameworks unterscheidet. Die Idee, eine benutzerfreundliche KI-Pipeline zu erstellen, ist wertvoll, führt jedoch kein neues Konzept oder keinen neuen Ansatz ein, der als bahnbrechend angesehen werden könnte.

Bitte helfen Sie ACM dabei, einen effizienteren Veröffentlichungsprozess zu erstellen: Wie viel Lektorat benötigt dieser Artikel Ihrer Meinung nach nach bestem Wissen und Gewissen?: Mäßig

Die meisten ACM-Zeitschriftenartikel sind forschungsorientiert. Ist dieses Dokument für Entwickler und Ingenieure von Interesse?: Nein

==> Draft_ger.tex <==
1.	Hintergrund 
In den letzten Jahren hat das Aufkommen KI-gestützten Codegeneratoren die Softwareentwicklung revolutioniert. Wurden diese Tools in der Vergangenheit eher dazu eingesetzt die Entwicklung herkömmlicher Software zu erleichtern liegt der Fokus heute auch zunehmend auf der Entwicklung von Codegeneratoren, die speziell für die Erstellung leistungsstarker und sicherer KI-Systeme gedacht sind. Technisch basieren diese Tools auf maschinellem Lernen (ML) und natürlicher Sprachverarbeitung (NLP) durch Large Languarge Models (LLM). Zu den bekanntesten Modellen zählen die auf Generative Pre-trained Transformer (GPT) basierenden Modelle ChatGPT, OpenAI Codex, GitHub Copilot und AlphaCode, die aus natürlichen Spracheingabeaufforderungen komplexen Code generieren können. Dieser Wandel steigert nicht nur die Produktivität, sondern bringt auch neue Herausforderungen mit sich, insbesondere in Bezug auf die Sicherheit und Zuverlässigkeit des Codes. In dieser Arbeit gehen wir der Frage nach wie sicher und effizient diese Codegeneratoren sind. Wir untersuchen außerdem wie die Sicherheit von Codegeneratoren einerseits sowie die Qualität des generierten Codes andererseits optimiert werden kann. Des Weiteren beschäftigen wir uns mit der Frage, was getan werden kann um Codegeneratoren für die Generierung von sicherer, lauffähiger und qualitativ hochwertiger KI zu optimieren und wie die Zugänglichkeit dieser Systeme verbessert werden kann.
2.	Aktueller Entwicklungsstand
KI-basierte Codegeneratoren, auch KI-Assistenten genannt, unterstützen Entwickelnde bei der Softwareentwicklung durch den Einsatz von maschinellem Lernen und Techniken der natürlichen Sprachverarbeitung (Hossain et al. 2023). Dabei kommen meist LLMs zum Einsatz, welche eine Interaktion in natürlicher Sprache ermöglichen (Hossain et al. 2023), (Sarkar et al. 2022), (Cotroneo et al. 2024), (Taeb et al. 2024). Durch den Einsatz dieser LLM, können KI-Assistenten heute weit mehr als die klassische Autovervollständigung, welche nur wenige Codezeilen synthetisieren kann; sie sind mehr und mehr dazu in der Lage, komplette Programme in Form von Klassen, Funktionen und Testfällen in unterschiedlichen Programmiersprachen völlig autonom zu generieren (Hossain et al. 2023), (Taeb et al. 2024) (Sarkar et al. 2022). Im Falle von GPT-3 wird dabei sogar die Absicht des Codes im Detail erklärt [7] (Hossain et al. 2023). In Bezug auf GitHub Copilot zeigen (Madi (2022)), dass die Komplexität und Lesbarkeit des generierten Codes mit menschlich geschriebenem Code vergleichbar ist (Sarkar et al. 2022).
KI-Codegeneratoren zeigen ein erhebliches Potenzial zur Verbesserung der Effizienz bei der Softwareentwicklung. Laut (Klemmer et al. 2024) nutzen 70 % der professionellen Entwickler bereits KI-Technologien während des gesamten Softwareentwicklungszyklus. Dabei werden diese in verschiedenen Bereichen der Softwareentwicklung eingesetzt, darunter Projektplanung, Anforderungsdefinition und -analyse, Codeerstellung, Testen, Refactoring und Change Management, Optimieren, Debuggen sowie Dokumentation und Erklärung von Code (Klemmer et al. 2024), (Hossain et al. 2023), (Sarkar et al. 2022), (Res et al. 2024). Es kann davon ausgegangen werden, das diese Technologie eine erhebliche Zeitersparnis und eine deutliche Steigerung der Effizient, Effektivität und Produktivität bewirkt (Taeb et al. 2024), (Klemmer et al. 2024) , (Chen et al., 2021) (Negri-Ribalta et al. 2024), (Sarkar et al. 2022). Dadurch verkürzen diese Technologien auch die Markteinführungszeiten neuer Software erheblich (Improta 2023). Darüber hinaus ermöglichen diese Assistenten auch die einfache Erkundung unbekannter Sprachen und APIs sowie das erlernen bessere Vorgehensweisen bei der Programmierung (Sarkar et al. 2022).
Ein weiterer Anwendungsbereich ist die Substitution von Informationsquellen wie Suchmaschinen und Online-Communities (wie Stack Overflow) durch diese Assistenten, was jedoch kritisch betrachtet werden muss (Klemmer et al. 2024), (Sarkar et al. 2022). So führt die dadurch stattfinden Abwanderung von Nutzenden und die daraus resultierende Verschlechterung der Qualität, Pflege und Weiterentwicklung dieser Informationsquellen auch zu Problemen für die Assistenten, die diese Quellen verdrängen, da deren Modelle meist auf Daten aus diesen Informationsquellen basieren (Sarkar et al. 2022), (Klemmer et al. 2024) [12]. Deren Verschwinden könnte somit die Trainingsbasis der Modelle gefährden und einen negativen Rückkopplungseffekt auslösen (Klemmer et al. 2024).
Außerdem werden diese Assistenten auch vermehrt für sicherheitskritischen Softwareentwicklung genutzt, beispielsweise zur Schwachstellenidentifikation, als Ersatz für teure Sicherheitsscanner, zur automatischen Behebung von (sicherheitskritischen) Kodierungsfehler und Sicherheitslücken, zur Definition von Angriffsvektoren sowie zur Erstellung von Malware und Exploits (Klemmer et al. 2024), (Berabi et al. 2024). Dabei wird ein weiterer Anstieg der Nutzung (Res et al. 2024), (Sarkar et al. 2022) auch bei Bearbeitung sicherheitsrelevanten Aufgaben erwartet (Klemmer et al. 2024). Aufgrund dieses vielfältigen Einsatzes haben diese Systeme jedoch auch einen erheblichen Einfluss auf die Zuverlässigkeit, Sicherheit und den Schutz von IT Systemen (Sarkar et al. 2022). 
3.	KI-Codegeneratoren
KI-Codegeneratoren können sowohl für die Entwicklung herkömmlicher Software Programmieren (Rajamani 2022) (Mozannar et al. 2024) (Wong et al. 2023) als auch für die Erstellung von KI-Systemen selbst genutzt werden (Sundberg und Holmström 2023) (Sarker 2022) (Yang et al. 2018) nutzen. Sie basieren meist auf LLM, welche zunehmend an Bedeutung gewinnen. Diese Sprachmodelle können nicht nur Fließtext und mehrstufige Anweisungen interpretieren (Zamfirescu-Pereira et al. 2023), sondern auch Antworten generieren, die von menschlichen Antworten kaum zu unterscheiden sind (Zamfirescu-Pereira et al. 2023) (Borger et al. 2023). Die rasante Entwicklung von LLMs kann insbesondere am Beispiel ChatGPT beobachtet werden, welches signifikante Fortschritte im Bereich Kontextverständnis, Sprachgenerierung, Anpassungsfähigkeit und Mehrsprachigkeit gemacht hat (Ray 2023). Diese Entwicklungen ermöglichen eine einfache Interaktion, indem sie natürliche Sprache (sog. „Prompting“) zur Steuerung der LLM-Ausgaben nutzen und die „Mensch-KI-Interaktion“ (Ray 2023) verbessern. KI-Codegeneratoren bieten Potenzial, das in vielen Bereichen gewinnbringend genutzt werden kann (Borger et al. 2023). Dies umfasst Anwendungen in Medizin, Gesundheitswesen, Wirtschaft, Finanzen, Recht, kreatives Schreiben, Inhaltserstellung, Bildungswesen, Medien, Unterhaltung, Verkauf, Marketing, Öffentlichkeitsarbeit, Bankwesen und wissenschaftlicher Forschung (Borger et al. 2023), (Ray 2023). Darüber hinaus sind sie auch in der herkömmlichen Programmierung und dem Code-Debugging sowie der automatischen Generierung von KI-Modellen von großem Nutzen (Ray 2023).
3.1.	KI-Codegeneratoren für herkömmliche Softwareentwicklung
KI-Codegeneratoren halten im Zuge der digitalen Transformation zunehmend Einzug in Wissenschaft (Ray 2023) und Wirtschaft (Sundberg und Holmström 2023) (Ray 2023) (Wong et al. 2023), werden aber zunehmend auch von Privatpersonen eingesetzt (Sundberg und Holmström 2023). 
Dabei zeigen diese Systeme enormes Potential bei der Softwareentwicklung, sowie der Datenverarbeitung und -analyse und können als nicht-menschliche Assistenten kooperativ genutzt werden (Ray 2023). KI-gestützte Funktionen zur Codegenerierung, Codevervollständigung, Codeübersetzung, Codeoptimierung, Codezusammenfassung, Codeüberprüfung, Debugging, Codedokumentation und Klonerkennung übertreffen bestehende Systeme bei weitem (Ray 2023) (Wong et al. 2023) (Mozannar et al. 2024). Dabei können diese Systeme nicht nur Funktionen und Klassen in einer breiten Palette von Programmiersprachen ergänzen, sondern basierend auf vorgegebenen Prompts auch selbst schreiben (Wong et al. 2023) (Mozannar et al. 2024). Darüber hinaus ermöglichen sie die automatisierte Entwicklung von Code für intelligente und smarte Systeme (Sarker 2022). 
Darüber hinaus lassen sich durch den Einsatz von KI-Techniken Wissen und Erfahrungen aus vorausgegangenen Projekten ableiten (Wong et al. 2023) (Yang et al. 2018). Die hohe Leistungsfähigkeit dieser Systeme resultiert insbesondere aus dem Einsatz moderner LLMs, die mit Milliarden von Datenpunkten trainiert wurden (Mozannar et al. 2024). Aufgrund dieser Leistung haben sich LLMs als eine wichtige Designmethode erwiesen, die potenziell auch für Nicht-KI-Experten (im Folgenden als Laien bezeichnet) zugänglich ist und die Nutzung von KI-Systemen intuitiver gestaltet (Zamfirescu-Pereira et al. 2023).
Auf wirtschaftlicher Seite verbessert der Einsatz solcher KI-Techniken die Effizienz und Qualität von Projekten (Wong et al. 2023) und beschleunigt Geschäftsprozesse, was zu einer höheren Produktivität und Rentabilität der Unternehmen führt (Sarker 2022). Auf wissenschaftlicher und privater Seite könnte diese Technologie auch Nichtexpertise den Zugang zu softwaregestützter Problemlösung ermöglichen (Borger et al. 2023) und somit Zeit und Ressourcen sparen da keine externen Entwickler mehr benötigt werden (Sundberg und Holmström 2023). 
(Sundberg und Holmström 2023) weisen jedoch darauf hin, dass der verantwortungsvolle Einsatz von KI für kleinere Unternehmen, die oft nicht über die notwendigen technologischen Kompetenzen verfügen, einen Wettbewerbsnachteil darstellen kann. Zudem müssen die von der KI generierten Codes sorgfältig validiert werden, da sie fehlerhaft sein und Sicherheitslücken enthalten können (Mozannar et al. 2024) was eine weitere Arbeitsbelastung darstellt. Dieser Nachteil verstärkt sich in wissenschaftlichen und privaten Kontext noch weiter, da hier oft die notwendige Expertise im Umgang mit KI-Codegeneratoren fehlt. So kommt eine Kosten-Nutzen-Analyse von (Mozannar et al. 2024) über KI-gestützte Programmierassistenzsysteme zu dem Schluss, dass diese Systeme die Arbeitsbelastung und Produktivität nur dann positiv beeinflussen können, wenn die Anwender über ausreichende Expertise im Bereich des Prompt Engineerings (siehe dazu auch Kapitel Prompt Engeneering) verfügen (Zamfirescu-Pereira et al. 2023). Außerdem stellen Installation, Wartung und Verwaltung von KI-Systemen ein weiteres Hemmnis dar (Sundberg und Holmström 2023).
Um den Zugang von KI-Programmierassistenten für Forschung, Wirtschaft und Privatpersonen zu erleichtern müssen diese Systeme einfach zugänglich und intuitiv bedienbar sein. (Rajamani 2022) präsentiert die Vision einer auf ML-Modellen und logischen Regeln beruhenden futuristische Programmierumgebung, die sich kontinuierlich während der Nutzung weiterentwickelt, während (Sundberg und Holmström 2023) die Entwicklung von KI-Plattformen als Lösung vorschlagen. Durch den Einsatz solcher Plattformen kann eine Brücke zwischen verschiedenen Expertenkreisen (z.B. Fachexperten-, Geschäfts- und Technologieexperten) geschlagen werden, wodurch bestehende technische, sprachliche und interessensbedingte Hindernisse überwunden und Lösungen für komplexe Probleme schneller und effizienter erreicht werden können (Sundberg und Holmström 2023). Außerdem zeigen (Sundberg und Holmström 2023) das durch die Demokratisierung von KI und durch die damit verbundene Erweiterung des Nutzerkreis neue, diversifiziert und innovativere KI-Lösungen entstehen können. 
Allerdings ergeben sich beim Einsatz von KI auch technische (Ray 2023) (Ylitalo), ethische (Ray 2023) (Borger et al. 2023), rechtliche (Ray 2023) (Borger et al. 2023) und sozialen (Borger et al. 2023) Anforderungen, die einer tiefgehenden Analyse bedürfen.
Das Potential solcher KI Systeme beschränkt sich aber nicht nur auf die Entwicklung gewöhnlicher Software sondern kann auch genutzt werden um die Entwicklung von KI-Systemen zu revolutionieren (Wong et al. 2023).
3.2.	KI-Codegeneratoren zur Generierung von KI
Ein zunehmend wichtiger Einsatzzweck von KI-Codegeneratoren ist die automatische Erstellung von Machine Learning (ML)- und KI-Code durch KI-Systeme, wodurch KI auch nicht-KI-Experten zugänglich wird. Um KI jedoch auch für diese Nicht-Experten oder für Experten anderer Domänen nutzbar zu machen und um dem steigenden Bedarf an wissensintensiven Prozessen Rechnung zu tragen, muss die Technologie zum Erstellen solcher KI-Modelle einfach zugänglich sein. (Feltus et al. 2021) fordert daher, dass KI-Tools eine symbiotische Beziehung mit den Erstellenden eingehen und einen nutzerzentrischen, einfachen KI-Generierungsansatz verfolgen muss. Dies soll insbesondere auch ein ausgewogenes Zusammenspiel von KI-gestützter Innovation und menschlichem Fachwissen fördern (Ray 2023).
Die Einsatzfelder solcher KI-Generatoren erstrecken sich über die fünf von (Sarker 2022) aufgestellten Kategorien „Analytische KI“, die Erkenntnisse aus Daten gewinnt (z.B. Big Data Analysen (Sundberg und Holmström 2023)), „Funktionale KI“, die Maßnahmen ergreift (z.B. Optimierung von Geschäftsprozessen (Sarker 2022)), „Interaktive KI“, die die Automatisierung der Kommunikation ermöglicht, „Textuelle KI“, die Textanalyse oder Verarbeitung natürlicher Sprache umfasst, und „Visuelle KI“, die Computer Vision oder Augmented Reality umfasst. Dabei gelten für Systeme zur automatischen Synthese von KI-Code die Bereits erläuterten Ansätze zur Synthese von herkömmlicher Software, erweiterte um in diesem Kapitel vorgestellte Prinzipien.
Die Entwicklung von KI-Modellen unterliegt dabei jedoch oft hohen Eintrittshürden (z.B. Expertenwissen) und einer hohen Dynamik und Datenvariation, was die Zugänglichkeit erschwert (Sarker 2022). Daher werden derzeit sowohl Domänen-Experten als auch Datenwissenschaftler und AI/ML-Experten zur Entwicklung benötigt (Sarker 2022). Eine weitere Hürde stellt die Validierung von Modellen dar, welche durch Domänenexperten und Laien bisher kaum gewährleistet werden kann (Yang et al. 2018). Da diese oft nur die Genauigkeit des Systems betrachten, könnten problematische oder falsche Modelle zum Einsatz kommen (Yang et al. 2018). Darüber hinaus müssen Zugangsbeschränkungen für die Entwicklung von KI-Modellen mithilfe geeigneter Konzepte wie interaktiven Assistenzsystemen abgebaut werden um Laien und Domänenexperten bestmöglich zu unterstützen (Sarker 2022), (Pinhanez 2019) (Wong et al. 2023) (Yang et al. 2018).
(Feltus et al. 2021) schlagen daher unterstützende Technologien vor, um Nicht-Experten bei der Modellerstellung und Wissensanalyse zu unterstützen. Mögliche Ansatzpunkte zum Abbau dieser Schranken sind nutzerfreundliche gestaltete (Yang et al. 2018) No-Code-Programmierassistenzsystemen (Sundberg und Holmström 2023), KI-Plattformen (Quelle AI4EU) sowie die Einführung von KI-Ökosystemen (Pinhanez 2019).
Die Einführung diese Systeme kann bei Gewährleistung eines einfachen und nutzerfreundlichen Zugangs die Demokratisierung von KI-Technologie gewährleisten (Sundberg und Holmström 2023). Dadurch kann KI nicht nur für große Unternehmen, sondern auch für kleine Betriebe und Organisationen, die Wissenschaft und Einzelpersonen zugänglich und erschwinglich gemacht werden. Um auch unerfahrene Nutzer ohne Coding-, Sicherheits- und KI-Erfahrung in die Lage zu versetzen, KI-Modelle zu entwickeln, bereitzustellen, zu betreiben und zu trainieren müssen diese No-Code-KI-Plattformen diesem Nutzerkreis durch eine Kombination aus KI-Assistenten, MLOps und nutzerfreundlichen grafischen Oberflächen zugänglich gemacht werden (Sundberg und Holmström 2023). Dadurch kann auch auf oft nicht vorhandene Experten wie Datenwissenschaftler und ML/AI-Experten verzichtet werden (Sundberg und Holmström 2023).
(Ylitalo) weißen darauf hin, dass solche AI-Tools auch an die Zielgruppe angepasst werden müssen. Dies zeigen Sie am Beispiel der Studie „“Github Copilot AI Pair programmer: asset or liability“ [Quelle?] welche nahelegt, dass der GitHub Copilot zwar ein gutes Tool für Senior Entwickler darstellt, Junior Entwickler aber nicht zugutekommt. Des Weiteren sollten die von Nicht-Experten entwickelten Modelle soweit aufbereitet werden, dass die Entwickelnden deren Implikationen verstehen und die Bedeutung ihres Einsatzes bewerten können (Feltus et al. 2021). 
Zur Erstellung von nutzerfreundlichen grafischen Oberflächen für No-Code-Programmierassistenzsystemen kann auf Tools wie das „Test-Driven Machine Teaching“ zurückgegriffen werden, welches Designer dabei unterstützt GUIs zu entwickeln die sich dem Interaktionsfluss (interactive machine learning (iML)) und den Gegebenheiten von Laien anpasst und diese gleichzeitig auf technische Fallstricke die beim Erstellen von ML-Modellen auftreten können hinweist (Yang et al. 2018). Durch diese interaktiven und benutzerfreundlichen grafischen Oberflächen sowie durch an die Bedürfnisse und Fähigkeiten der Nutzer im Bereich ML/AI und Programmierung angepasste Prozesse können robustere KI-Modelle von Laien entwickelt werden (Yang et al. 2018). Die in die GUI integrierbaren geführten Prozesse unterstützen dabei die Einhaltung grundlegender Regeln und Sicherheitsaspekte (Yang et al. 2018) und sorgen somit auch für einen sichereren und ethischeren Umgang mit KI. 
(Pinhanez 2019) stellen mit dem „Massive Open Learning AI-System“ (MOLA) einen communitybasierten und kollaborativen Ansatz zur AI-Entwicklung vor. Der Vorteil eines offenen, integrativen KI-Ökosystems ergibt sich durch das Heben von Synergieeffekten innerhalb der Community und das Vorhandensein von Expertenwissen unterschiedlicher Disziplinen. (Pinhanez 2019) untersuchen in Ihrer Studie unter anderem die kollaborative Entwicklung eines KI-Assistenten für Diabetespatienten. Hierbei zeigen sich auch die Vorteile solch eines Systems. So bemerkte die Community, dass der KI-Assistenten von einigen etischen Gruppen aufgrund kultureller Besonderheiten nicht gut angenommen wurde, was im Anschluss kooperativ gelöst werden konnte. Eine weitere KI-Plattform wurde im Rahmen des Forschungsprojekts AI4EU (Quelle) vorgestellt. AI4EU stellt dabei eine containerbasierte Architektur zur kollaborativen Entwicklung von KI-Modellen durch Experten und Nichtexperten zur Verfügung. Darüber hinaus heben (Sundberg und Holmström 2023) cloudbasierte KI-Plattformen sog. „KI as a Service“-Systeme als möglichen neuen Wirtschaftszweig hervor. Durch solch einen Cloud getriebenen Ansatz lässt sich ein Umfangreiches, Lain und Experten gleichermaßen einschließendes, KI-Ökosystem aufbauen (Sundberg und Holmström 2023). Ein dabei bisher jedoch unerforschter Bereich ist die kollaborative Entwicklung mehrerer Nicht-Experten an einem Modell (Feltus et al. 2021). Außerdem muss beachtet werden, das KI-Modelle in vieler Unternehmen als Geschäftsgeheimnisse angesehen und damit nicht öffentlich zugänglich gemacht werden dürfen.
(Clune 2019) schlagen darüber hinaus die Entwicklung eines zwei phasigen, KI-generierenden Algorithmus (AI-GA) vor, welcher autonom an der Entwicklung von allgemeiner künstlicher Intelligenz (AGI) forschen soll. Dieses Konzept basiert auf der Evolution von einfachen Proteinen zu komplexen Lebensformen und überträgt diesen Prozess auf die KI-Entwicklung. In Phase 1 soll das System alle für KI notwendigen und gegebenenfalls noch fehlenden Komponenten entdecken und verstehen. In Phase 2 soll das System lernen, diese Bausteine zu einem komplexen System zusammenzubauen, das den Anforderungen einer AGI entspricht. Obwohl dieser Ansatz weit über das hier vorgestellte Assistenzsystem hinausgeht, können die vorgeschlagenen Phasen zur Erforschung von künstlicher Intelligenz auch auf solche Systeme angewendet werden. Zudem weist (Clune 2019) darauf hin, dass bei der Entwicklung eines solchen Tools zahlreiche Überlegungen im Bereich der Sicherheit und Ethik erforderlich sind.
Ein weitrechendes Problem bei der Entwicklung solcher Systeme stellt jedoch die Notwendigkeit von umfangreichen und qualitativ hochwertigen Trainingsdaten dar. 
Eine bisher weitgehend ignorierte Datenquelle ist die von (Bojer und Meldgaard 2021) untersuchte Onlineplattform Kaggle. In ihrer Studie analysieren sie sechs verschiedene Kaggle-Wettbewerbe und stellten die Ansprüche und die Qualität der Lösungen den von Spyros Makridakis und Michèle Hibon organisierten M-Wettbewerben gegenüber. Ihre Untersuchung konzentrierte sich auf Vorhersageprobleme, wie Wetterdaten sowie Produktions- und Verkaufsprognosen. Zur Validierung der Leistungsfähigkeit erstellten sie für diese sechs Wettbewerbe Benchmarks basierend auf einfachen und bewährten naiven und saisonalen naiven Methoden, welche im Anschluss mit den Kaggle Lösungen vergleichen werden. Dabei übertrafen die besten Lösungen auf Kaggle die einfachen Lösungen um mindestens 25 % und maximal 74 %. Selbst die Lösungen auf Platz 50 übertrafen die einfachen Lösungen noch um mindestens 10 %. Außerdem zeigen (Bojer und Meldgaard 2021), dass die an den M-Wettbewerben geübte Kritik, wie das Fehlen hochfrequenter und hierarchischer Zeitreihen sowie fehlende Sekundärinformationen wie exogene Variablen, was diese Wettbewerbe wenig repräsentativ für reale wirtschaftliche Probleme macht (Darin & Stellwagen, 2020; Fry & Brundage, 2019), bei den Kaggle-Wettbewerben teilweise gelöst ist. Kaggle-Wettbewerbe bieten somit eine gute Lernmöglichkeit und belegen die in den M-Wettbewerben aufgestellte Hypothese, dass Kombinationen aus verschiedenen ML-Tools besser abschneiden als Einzellösungen. 
Ein Manko von Kaggle ist jedoch, dass die Plattform lediglich Lösungen verlangt und die Teilnehmer nicht verpflichtet sind, den dazugehörigen Code hochzuladen, wobei die besten Lösungen meist auch über Quellcode verfügen. Dies unterstreicht die Bedeutung der auf Kaggle eingereichten Lösungen und ihr Potenzial als Trainingskorpus für LLM-basierte KI-Code generatoren.
In Bezug auf die Erschließung von Wissensquellen weißen (Sarkar 2023) jedoch darauf hin, dass die Integration von strukturiertem (z.B. Wissensgraphen) und unstrukturiertem Wissen (z.B. Wikipedia) eine erhebliche Herausforderung darstellt. Außerdem ist es erforderlich, dass das Wissensmodel sowohl durch eine Maschine (KI) als auch von einem Menschen verstanden und genutzt werden kann (Feltus et al. 2021).
Aufgrund dieser Entwicklungen hat sich der Einsatz von LLMs als eine wichtige Designmethode erwiesen, die auch für Nicht-KI-Experten zugänglich ist und die Nutzung von KI-Systemen intuitiver gestaltet. Durch eine symbiotische Beziehung zwischen Technologie und den Erstellenden können robuste und ethisch vertretbare KI-Modelle entwickelt werden, die sowohl von Maschinen als auch von Menschen verstanden und genutzt werden können. Die Forschung an benutzerfreundlichen und flexiblen No-Code-KI-Generatoren fördert dabei die Akzeptanz von KI und ermöglicht gleichzeitig die Integration von KI in allen Bereichen der Gesellschaft (Feltus et al. 2021). 
3.3.	Im Einsatz befindliche KI-Codegeneratoren
Im Bereich der Künstlichen Intelligenz (KI) haben sich Codegeneratoren als leistungsstarke Werkzeuge etabliert, die den Entwicklungsprozess beschleunigen und automatisieren können. Diese Systeme nutzen maschinelles Lernen und natürliche Sprachverarbeitung, um Code zu generieren, der auf bestimmten Eingaben basiert. Allgemein muss jedoch beachtet werden, dass es trotz vielversprechender Ergebnisse bekannte Mängel gibt. Modelle können vollständige Lösungen oder wichtige Teile der Lösungen direkt aus den Trainingsdaten kopieren, anstatt neuen Code zu generieren. Obwohl Entwickler sich bemühen, nur qualitativ hochwertigen Code zu bereinigen und beizubehalten, gibt es keine Garantie für dessen Richtigkeit (Sarkar et al. 2022). Konsistenz ist ein weiteres Problem (Sarkar et al. 2022). Im Folgenden werden die drei wichtigsten, bekanntesten und in der untersuchten Literatur am häufigsten besprochenen KI-Codegeneratoren vorgestellt.
Name	Beschreibung	Nutzende Authoren
ChatGPT	ChatGPT, ein Produkt von OpenAI, ist eines der vielseitigsten GPT-Modelle für die Codegenerierung. Es wurde in zahlreichen Studien untersucht und wird fortlaufend weiterentwickelt.
(Hossain et al. 2023), (Cotroneo et al. 2024) [57], (Improta 2023), (Negri-Ribalta et al. 2024), (Taeb et al. 2024)

Copilot	GitHub Copilot, ebenfalls von OpenAI entwickelt und in Zusammenarbeit mit GitHub bereitgestellt, bietet Entwicklern Vorschläge direkt in der Entwicklungsumgebung.
(Hossain et al. 2023), (Cotroneo et al. 2024) [20], (Improta 2023), (Negri-Ribalta et al. 2024)

OpenAI Codex	Codex (Chen, Tworek, Jun, Yuan, Ponde, et al., 2021), eine speziell auf die Codegenerierung ausgerichtete Version von GPT-3, ist die Basis für GitHub Copilot. Es hat sich in verschiedenen Benchmarks und Anwendungen bewährt.
Es kann im HumanEval-Codegenerierungsbenchmark durchschnittlich 47/164 Probleme in einem Versuch lösen (Sarkar et al. 2022). Bei einem Datensatz mit 10.000 Programmierproblemen löst Codex etwa 3 % der Probleme innerhalb von 5 Versuchen (Sarkar et al. 2022). 
Große schwächen sind, das Codex syntaktisch falschen oder undefinierten Code erzeugen und Funktionen, Variablen und Attribute aufrufen kann, die undefiniert oder außerhalb des Gültigkeitsbereichs liegen (Sarkar et al. 2022).
(Hossain et al. 2023), (Perry et al. 2023), (Negri-Ribalta et al. 2024), (337, Xu, Li), (Sarkar et al. 2022), (Taeb et al. 2024)

AlphaCode	AlphaCode, entwickelt von DeepMind, wurde direkt anhand von GitHub-Daten trainiert und für Programmierwettbewerbe optimiert. Es kann eine große Anzahl potenzieller Lösungen auf eine Handvoll valider Kandidaten reduzieren und erreicht bei Wettbewerben eine Erfolgsquote von 34 % (Sarkar et al. 2022). Es liegt damit auf Augenhöhe mit dem durchschnittlichen menschlichen Teilnehmer (Sarkar et al. 2022). Bei einem Datensatz mit 10.000 Programmierproblemen löst AlphaCode etwa 4 – 7 % der Probleme innerhalb von 5 Versuchen (Sarkar et al. 2022).  AlphaCode 2 schneidet bei Codieraufgaben sogar bis zu 85 % besser ab als menschliche Konkurrenten (Res et al. 2024).	(Sarkar et al. 2022)

Neben den oben genannten gibt es eine Vielzahl weiterer KI-basierter Codegeneratoren, die in der Analysierten Literatur Erwähnung finden:
Name	Nutzende	Name	Nutzende	Name	Nutzende
AI der IntelliJ IDEA	(Hossain et al. 2023)
DeepAPIplusSec	(Negri-Ribalta et al. 2024) 
Mistral Mixtral	(Negri-Ribalta et al. 2024)

Amazon CodeWhisperer	(Improta 2023)
Facebooks InCoder	(Perry et al. 2023) [5, 11]
PolyCoder	(Negri-Ribalta et al. 2024) (337, Xu, Li).
CodeBERT	(Negri-Ribalta et al. 2024) (337, Xu, Li), (Taeb et al. 2024)
Google Gemini	(Cotroneo et al. 2024) [25]
Salesforce CodeGen	(Improta 2023), (Negri-Ribalta et al. 2024)

CodeGen	(Negri-Ribalta et al. 2024) (337, Xu, Li).	Google PaLM	(Negri-Ribalta et al. 2024)
StarCoder	(Negri-Ribalta et al. 2024) (337, Xu, Li)
CodeParrot	(Negri-Ribalta et al. 2024)
Gpt2csrc	(Negri-Ribalta et al. 2024) [Pearce et al. (2023)]	Tabnine	(Hossain et al. 2023)

CodeT5	(Negri-Ribalta et al. 2024)
Meta LLaMA	(Negri-Ribalta et al. 2024)
	
DeepAPI-onlySec	(Negri-Ribalta et al. 2024) 
Microsoft Copilot	(Cotroneo et al. 2024) [48]
	
3.4.	Bewertung von KI-Codegeneratoren anhand von Nutzerstudien
KI-Codegeneratoren unterstützen Entwickelnde schon heute in allen Bereichen des Softwareentwicklungszyklus (Perry et al. 2023). Es ist wichtig, dass diese Tools potenzielle Sicherheitslücken vermeiden und robusten, sicheren Code erzeugen (Taeb et al. 2024). Um die Vor- und Nachteile dieser Systeme aus Nutzersicht beurteilen zu können werden Studien von  (Perry et al. 2023), (Sarkar et al. 2022) und (Klemmer et al. 2024) analysiert. 
(Perry et al. 2023) führt eine Laborstudie durch, um zu validieren ob Nutzenden von KI-Codegeneratoren unsichereren Code schreiben. Dazu werden die Studienteilnehmer in Gruppen eingeteilt, wobei eine Gruppe KI-Codegeneratoren nutzt, die andere hingegen nicht. Diesen Gruppen werden im Anschluss sicherheitsrelevante Aufgaben gestellt, welche auf Richtigkeit und Sicherheit evaluiert werden. Die Aufgaben erstecken sich dabei über die Bereiche Verschlüsselung, Zugriffskontrolle, Datenbanken, Datenein- und -ausgaben sowie Datentypen und Webtechnologien. Darüber hinaus wird das Interaktionsveralten der Nutzenden mit dem KI-System aufgezeichnet und analysiert. Um das ganze Reproduzierbar zu machen, bieten die Autoren der Studie die anonymisierten Studiendaten zum Download an. Darin enthalten sind u.a. die Anfragen an und das Interaktionsverhalten mit dem Modell, die ausgegebenen Antworten des Modells sowie die Sicherheitsevaluationen. Außerdem werden Interviews mit den Teilnehmenden durchgeführt, um deren Vertrauen in diese Technologie zu evaluieren. Dabei können zwei wesentliche Aussagen getroffen werden: Zum einen zeigt sich, dass Studienteilnehmer unabhängig von deren Erfahrung, denen KI-Assistenten zur Seite gestellt wurden, unsichereren Code schrieben, jedoch davon ausgingen, dass ihr Code sicherer sei (Perry et al. 2023). Im Gegensatz dazu schrieben Studienteilnehmer ohne KI-Assistenten sichereren Code und konnten die Sicherheit auch besser einschätzen. Zum anderen konnten (Perry et al. 2023) ein Problem bei der Nutzung von KI-Codegeneratoren durch unerfahrene Nutzer und Laien aufdecken. Diese Nutzergruppe neigt dazu, den von der KI generierten Code als sicher und qualitativ hochwertig zu betrachten, selbst wenn dieser unsicher ist, was potenzielle Gefahren mit sich bringt. Erfahrene Nutzer hingegen können die Qualität und Sicherheit des ausgegebenen Codes besser einschätzen und profitieren von einer Produktivitätssteigerung. Zudem sind sie in der Lage, die Ausgaben des Assistenten durch Anpassungen der Prompts so zu beeinflussen, dass die Qualität und Sicherheit des ausgegebenen Codes verbessert wird.

(Sarkar et al. 2022) und (Klemmer et al. 2024) setzen bei ihren Auswertungen auf Erfahrungsberichten der Nutzenden. So analysieren (Sarkar et al. 2022) Erfahrungsberichte über LLM-gestützte Programmierassistenten aus öffentlich zugänglicher Quelle. Die Autoren fokussieren sich bei ihrer Untersuchung darauf, wie KI-gestützte Programmierassistenten die Codeentwicklung beeinflussen und wie sie sich von bestehenden Systemen unterscheiden. (Klemmer et al. 2024) hingegen wertet den Einsatz von KI-Assistenten in der Softwareentwicklung anhand von 27 halbstrukturierte Interviews mit Software-Experten sowie durch das Review von 190 relevanten Reddit-Beiträgen und -Kommentaren aus. Sie legen besonderes Augenmerk auf die Sicherheitspraktiken und -bedenken der Entwickler. Dabei befassen sie sich mit den Vorgehensweisen von Entwicklern bei der Nutzung von KI-Assistenzsystemen und untersuchen die daraus hervorgehenden Auswirkungen auf die Softwareentwicklung und -sicherheit. 
Außerdem analysieren und verfeinern (Sarkar et al. 2022) einsatzspezifische Metaphern und Definitionen basierend auf dem Nutzungsverhalten von KI-gestützter Programmierung und kommen zu dem Schluss, dass diese oft zu kurz greifen. Im Fall der Nutzung als Suchassistent zur Beschaffung von Informationen ersetzt das System die klassische Internetsuche, wobei wertvolle Kommentare und Diskussionen verloren gehen, da KI-Codegeneratoren lediglich den Code ausgeben. Bei der Betrachtung als Compiler werden menschenlesbare Code oder auch textuelle Spezifikationen als natürliche Spracheingaben behandelt, die vom KI-Modell in Quellcode kompiliert werden. Im Gegensatz zu traditionellen Compilern arbeiten diese Modelle jedoch nicht deterministisch und erfordern eine aktive Überprüfung und Anpassung des Codes bei jeder Ausgabe. Beim Einsatz von KI-Assistenten als Pair Programming Partner wird eine Arbeitsteilung zwischen Mensch und KI angestrebt, wobei der Mensch das Ziel durch Prompts vorgibt („Navigator“) und das KI-Modell dieses Ziel durch Codeausgabe erreicht („Driver“). Allerdings kann dem generierten Code nicht vollumfänglich vertraut werden. Außerdem betrachten die Autoren auch eine weitere Definition die sie als „Eine besondere Art der Programmierung“ bezeichnen. Hier übernimmt das KI-Modell zwar die Codegenerierung, der Mensch benötigt jedoch weiterhin Grundkenntnisse in der Programmierung und der Zielsprache da die Ausgabe des Modells nachträglich geprüft werden muss. Diese letzte Definition kommt vermutlich am nächsten an das momentane Vorgehen heran (angaben des Autors (ich selbst)) (Sarkar et al. 2022).
Dennoch kommen alle Autoren zu dem Schluss, dass sich diese Technik aufgrund der immensen Zeitersparnis immer mehr durchsetzt. Nach Auswertung aller durch (Klemmer et al. 2024) analysierten Interviews und Reddit-Posts zeigt sich darüber hinaus, dass sich der Einsatz von KI-Assistenten trotz Sicherheits- und Qualitätsbedenken immer mehr durchsetzt. So werden KI-Codegeneratoren fast täglich eingesetzt, obwohl mehr als die Hälfte der Entwickler negative Auswirkungen auf die Softwaresicherheit erwarten. Eine Studie zum Einsatz von GitHub Copilot schätzt, dass bis 2030 mithilfe dieser Tools eine Produktivitätssteigerung von 30 % bzw. eine Steigerung des weltweiten BIP um 1,5 Billionen Dollar erreicht werden kann [25, 27] (Klemmer et al. 2024). Außerdem gehen einige Studienteilnehmer davon aus, dass der Einsatz von KI-Assistenten ein wesentlicher Teil der Wahrung der Wettbewerbsfähigkeit darstellen wird und dass sich die Leistungsfähigkeit von KI-Assistenten in den nächsten drei bis vier Jahren weiter verbessert. Weiterhin nehmen die Teilnehmer an, dass sich der Aufgabenbereich von Softwareentwicklern in Zukunft immer mehr in Richtung Prompt-Engineering und KI-Management verschiebt. Ein weiterer Studienteilnehmer merkt außerdem an, dass der Einsatz dieser Technologie durch eine Produktivitätssteigerung auch zu reduzierten Personalkosten führt, was den Einsatz dieser Technologie aus Unternehmersicht in Zukunft noch interessanter machen dürfte. (Sarkar et al. 2022) und (Klemmer et al. 2024) stellt jedoch fest, dass die Formulierung von Eingabeaufforderungen (Prompt Engineering) gerade für unerfahrene Nutzer bisher noch zu Schwierigkeiten führt. (Klemmer et al. 2024) weißen darüber hinaus darauf hin, dass alle generierten Antworten einem umfangreichen Review unterzogen werden müssen, was ein wesentlicher Nachteil heutiger Codegeneratoren ist. Da hierzu jedoch bisher keine definierten und verifizierbaren Verfahren vorliegen wünschen sich einige Studienteilnehmer weitere Forschung in diesem Bereich. Andere Studienteilnehmer gaben jedoch an bereits selbst aufwendige Peer Review Prozesses und umfangreicher Softwaretests in ihren KI-gestützten Arbeitsprozess integriert zu haben (Klemmer et al. 2024).
4.	Herausforderung und Risiken beim Einsatz von KI-Codegeneratoren
Mit der zunehmenden Integration von KI-basierten Codegeneratoren in den Softwareentwicklungsprozess wird es immer wichtiger, die damit verbundenen Herausforderungen und Risiken zu verstehen. Während leistungsstarke Modelle sich wirtschaftlich positiv für die sie einsetzenden Unternehmen auswirken können (Sarkar et al. 2022), (Klemmer et al. 2024) (Improta 2023), können minderwertige Modelle sowohl die Produktivität senken als auch erhebliche Sicherheitsrisiken darstellen (Improta 2023). Insbesondre die Einführung von an Endbenutzer angepasste Programmierassistenten bringt spezifische Herausforderungen mit sich, die professionelle Programmierer und Laien gleichermaßen betreffen (Sarkar et al. 2022). 
4.1.	Technisch bedingte Herausforderungen
Auf technischer Seite ergeben sich insbesondere Anforderungen in den Bereichen Zuverlässigkeit, Genauigkeit, Kontrolle von Verzerrungen, Generalisierungsfähigkeit, Erklärbarkeit der Modelle, Kontextverständnis sowie Sicherheitsaspekte (Ray 2023) welche wiederum Auswirkungen auf die Bereiche Ethik, Recht und Soziales haben können wie das Beispiel von fehlerhaften oder ethisch bedenklichen Antworten zeigt. Dies liegt insbesondere an den Trainingsdaten und den technischen Eigenschaften der meist zum Einsatz kommenden LLM-Modellen. 
Da das Sammeln von Trainingsdaten ein zeitaufwändiger und dadurch teurer Prozess ist (Improta 2023), werden die zum Training verwendeten Datensätze meist durch das Crawlen von Milliarden von Quellcodezeilen (Cotroneo et al. 2024), (Mozannar et al. 2024) aus öffentlich zugänglichen, umfangreichen, nicht geprüften, teilweise unvollständigen und nicht immer vertrauenswürdiger „Online-Softwareartefakten wie Quellcode-Repositorys [z.B. GitHub (Cotroneo et al. 2024) [23] und StackOverflow Threads (Improta 2023)], Fehlerdatenbanken und Codeausschnitten“ (Wong et al. 2023) gewonnen. Dabei ist zu beachten, dass bei Code aus Repositorys oft nicht bekannt ist, wie sicher oder effizient dieser Code ist. Dadurch erlernen die damit trainierten Modelle aber auch das Generieren der in den Trainingsdaten vorhandene Schwächen wie das nicht Berücksichtigen wichtiger Randfälle, das Verwenden von veraltete und unsicheren Funktionen und Bibliotheken sowie das Ausgebeben von unvollständigem, nicht lauffähigem, unsichem, sicherheitskritischem, fehlerhaftem oder gar mit Malware kompromittiertem Code (Improta 2023), (Sarkar et al. 2022), (Klemmer et al. 2024), (Cotroneo et al. 2024), (Negri-Ribalta et al. 2024), Perry et al. (2023). Außerdem können diese Modelle nur korrekt antworten, solange sich die Frage im Rahmen ihrer Trainingsdaten befindet, ansonsten geben die Modelle unklare oder falsche Antworten oder beginnen zu Halluzinieren (Klemmer et al. 2024), (Negri-Ribalta et al. 2024). 
Neben den Trainingsdaten bietet aber auch die LLM-Technologie an sich Schwachstellen. So basierend die durch LLMs generierten Antwort lediglich auf statistischen Abstraktionen der Trainingsdaten (Chen et al., 2021). Diese Systeme können also lediglich Vorhersagen welches „Wort“ als nächstes am wahrscheinlichsten ist, und nicht, ob dies semantisch Sinn ergibt (Negri-Ribalta et al. 2024). 
Bedingt durch diese Schwächen können Modelle z.B. richtig aussehenden aber syntaktisch falschen oder undefinierten Code erzeugen, welcher Beispielsweise Funktionen oder Variablen aufrufen, die nicht definiert wurden oder außerhalb des Gültigkeitsbereichs liegen (Sarkar et al. 2022). 
Erschwerend kommt hinzu, das sich Fehler in den Trainingsdaten oder im Design des Modells nur sehr schwer detektieren lassen, da die interne Prozess der LLM/GPT bisher außerhalb jeglicher Qualitätskontrolle liegen (Cotroneo et al. 2024). So kann trotz aller Bemühungen der Entwickelnden nur qualitativ hochwertigen und bereinigtem Code aus diesen Generatoren zu verwenden, keine Garantie für dessen Richtigkeit und Konsistenz gegeben werden (Sarkar et al. 2022). Die Verbesserung der Codequalität und -Sicherheit stellt sich bisher jedoch als schwierig dar, da hierzu große Mengen an qualitativ hochwertigen Trainingsdaten benötigt werden (Berabi et al. 2024). 
Ebenso erfordert der Betrieb solcher umfangreichen KI-Assistenten ein komplexes technisches Wissen. So sind zum Betrieb moderner KI-Systeme neben CI/CD/DevOps und MLOps oft auch Cloud Infrastrukturen notwendig. Die Verwaltung und der Betrieb solchen Infrastrukturen ist jedoch äußerst komplex. Eine Lösung bieten (Ylitalo) indem sie untersuchen wie generative künstliche Intelligenz (GAI) bei Verwaltung und Betrieb von Cloud Infrastruktur unterstützen kann. Dabei setzen sie auf einen durch KI automatisierten „Infrastructure as Code“ Ansatz, wodurch die Servicequalität verbessert und die notwendigen Prozesse vereinfacht werden können. Allerdings konzentrieren sich die Autoren auf die Unterstützung von Cloud-Experten beim Management solcher Systeme und nicht auf die Substitution dieser.
Aus den oben genannten Gründen schrecken Unternehmen und deren Entwickler immer noch vor einem weitreichenden Einsatz dieser Technologie zurück (Res et al. 2024). Daher sollten sich zukünftige Arbeiten darauf konzentrieren, die Sicherheit und Genauigkeit dieser Tools weiter zu verbessern um eine sichere Nutzung zu gewährleisten (Taeb et al. 2024).
4.2.	Codequalität
Eine der wichtigsten Aspekte bei der Betrachtung von KI-Codegeneratoren ist neben der korrekten Funktionalität des generierten Codes dessen Sicherheit. So sind laut Open Source Security and Risk Analysis (OSSRA) [3], [4] (siehe (Hossain et al. 2023)) 40 % (Pearce et al. (2022)) des erzeugten Codes unsicher (Hossain et al. 2023). Im Gegensatz dazu zeigt jedoch eine Studie von Sandoval et al. [x], dass der Einsatz von KI-Assistenzsystemen nur 10 % mehr Sicherheitslücken im Vergleich zu einer Kontrollgruppe ohne KI-Assistenzsystemen verursachte (Klemmer et al. 2024). (Pearce et al., 2022, 2023) gehen darauf ein, dass die von OpenAI angebotenen Systeme zwar weitestgehend funktionalen und sicheren Code generieren, das Ergebnis bei unterschiedlichen CWE und Programmiersprachen jedoch variiert. So enthalten 50 % des generierten C-Codes Sicherheitslücken wohingegen nur 39 % des Pythoncodes Lücken aufweisen (Pearce et al. (2023)) (Negri-Ribalta et al. 2024). Auch (Taeb et al. 2024), (Negri-Ribalta et al. 2024), (Perry et al. 2023) und (Cotroneo et al. 2024) analysieren, wie sich verschiedene Codegeneratoren bzw. deren Nutzung auf die Codesicherheit auswirken. 
Zur Validierung der Codesicherheit befüllen (Taeb et al. 2024) die Systeme CodeBERT, GPT 3.5 und CodeX mit durch CVE-, CWE, NIST und NVD-Schwachstellen sowie den Top10 OWASP Web Risiken kompromittiertem Code und analysieren wie gut diese Systeme den kompromittierten Code reparieren können. Die Ausgaben der Modelle wurden im Anschluss unter anderem von statischen Codeanalysatoren wie Clang-Tidy, FlawFinder und VCG analysiert. Dabei stellte sich heraus, dass CodeX die höchste Codegenerierungsfähigkeit aufweist und dabei genauen, sicheren und datenschutzkonformen Code erzeugt. GPT 3.5 zeigte zwar geringere Codegenerierungsfunktionen im Vergleich zu CodeX, war jedoch sehr effektiv bei der Erklärung potenzieller Schwachstellen und der Kommentierung von Code und LogFiles. CodeBert konnte ebenfalls hochwertigen Code generieren, war jedoch in Bezug auf Sicherheitsmaßnahmen schwächer. Außerdem zeigen sie, dass die Qualität und Sicherheit der Ausgabe von der Komplexität der Aufgaben und der Genauigkeit der Anweisungen und somit unter anderem von den Fähigkeiten des Bedieners abhängen (Taeb et al. 2024). 
Neben den bereits im Kapitel 3.4 vorgestellten Studien von (Perry et al. 2023), (Sarkar et al. 2022) und (Klemmer et al. 2024) analysieren (Negri-Ribalta et al. 2024), (Ylitalo) und (Improta 2023) ebenfalls die Auswirkungen des stetig steigenden Einsatzes von KI-Assistenten auf die Codequalität und Codesicherheit. Dabei kommen (Negri-Ribalta et al. 2024) basierend auf einer systematischen Literaturreview zu dem Schluss, das derzeitige KI-Codegeneratoren bekannte und leicht zu vermeidende Schwachstellen oder gar Malware in ihren Ausgaben aufweisen. (Ylitalo) heben darüber hinaus hervor, dass die vom KI-Assistenzsystem „Github Copilot“ vorgeschlagenen Codeblöcke teilweise unvollständig oder falsch sind und darüber hinaus teilweise gravierende Sicherheitslücken enthalten. Das Detektieren von Sicherheitslücken in diesem teilweise unfertigem und nicht lauffähigem Code stellt indes eine erhebliche Herausforderung dar, die nur durch eine Analyse komplexer Muster und weitentfernter Beziehungen innerhalb des gesamten Codes zu lösen ist (Berabi et al. 2024), (Cotroneo et al. 2024). Eine Studie von (Improta 2023) legen außerdem nahe, dass die Codequalität von „Github Copilot“ kein Einzelfall ist, was im Falle deren Verwendung zu schwerwiegenden Sicherheitsproblemen führen kann. Beispielsweise können unsichere Verschlüsselungen und andere Sicherheitslücken entstehen, die Angriffe auf den generierten Code erleichtern. Daher ist es von entscheidender Bedeutung, Mechanismen zu entwickeln, die solche Sicherheitsprobleme frühzeitig erkennen und beheben (Improta 2023). 
(Cotroneo et al. 2024) weißen ebenfalls darauf hin, dass der Faktor Mensch wesentlichen Einfluss bei der Betrachtung der Qualität und Sicherheit von durch Codegeneratoren erzeugten Code hat. Sie zeigen auf, das unbedarfte Nutzende die Sicherheit von durch KI-generierten Code bisher nicht beurteilen können (Cotroneo et al. 2024). Ebenso führen sie auf, das eine manuelle Überprüfung aufgrund der durch den Einsatz von KI Generatoren erwartbaren Zunahme an zu prüfendem Code nicht umgesetzt werden kann (Cotroneo et al. 2024) [41, 40]. Sie zeigen außerdem auf, dass der Einsatz statischer Analysetools welche z.B. auf Abstrakter Syntaxbaum (AST) [43, 65, 67, 16] basieren, aufgrund der oft unvollständigen durch KI generierten Programme nicht eingesetzt werden können (Cotroneo et al. 2024). Außerdem vermindert die Notwendigkeit einer manuellen Prüfung und das potenzielle Vorhandensein schwerwiegender Sicherheitsrisiken die Akzeptanz dieser Technologie erheblich (Cotroneo et al. 2024). 
4.3.	Herausforderungen beim Prompt Engeneering
Wie bereits zuvor erläutert, stellt das  sogenannte Prompt Engineering einer der größten Herausforderungen bei der Nutzung von KI-Codegeneratoren das (Sarkar et al. 2022), (Klemmer et al. 2024). Das Schreiben effektiver Eingabeaufforderungen für KI-Modelle ist schwierig und erfordert detaillierte Anweisungen und eine klare Logik (Sarkar et al. 2022), (Klemmer et al. 2024). Außerdem müssen Probleme oft in Teilprobleme zerlegen werden um durch heutige KI-Systeme gelöst werden zu können (Sarkar et al. 2022). So müssen Benutzer ihre Absichten bisher detailliert und feingranular spezifizieren und häufig nachträglich verfeinern, um die gewünschten Ergebnisse zu erzielen (Sarkar et al. 2022). Dies stellt ein entscheidendes Hindernis dar, insbesondere für unerfahrene Endnutzer wie Buchhalter oder Wissenschaftler, die keine Programmierkenntnisse besitzen, aber durch natürlichsprachige Programmierassistenten erheblich entlastet werden könnten (Sarkar et al. 2022). Die Interaktionsschnittstellen dieser Systeme muss daher zukünftig in Bezug auf Benutzerfreundlichkeit und die Ergebnisqualität verbessert werden (Klemmer et al. 2024).
4.4.	Sicherheit und Vertrauen
Ein sich durch die vorausgegangenen Punkte ergebender kritischer Aspekt ist das in Kapitel XXX beschriebene und vorwiegend unerfahrenen Nutzenden zum Problem werdende, blinde und teilweise ungerechtfertigte Vertrauen in den generierten Code (Sarkar et al. 2022). Darauf aufbauend stellen (Sarkar et al. 2022) zudem fest, dass das Codeverständnis und die Wartung des Codes als kritische Punkte betrachtet werden müssen, da die Automatisierung der Codegenerierung dazu führen kann, dass Benutzer weniger Zeit in das Testen und Verstehen ihrer Programme investieren und sich uneingeschränkt auf den generierten Code verlassen. Unerfahrene Nutzer neigen z.B. fälschlicherweise zu der Annahme, dass der von diesen Assistenten erzeugte Code sicher und qualitativ hochwertig ist (Perry et al. 2023), (Sarkar et al. 2022). Die Autoren stellen außerdem fest, dass Teilnehmer, die KI-Assistenten verwendeten, weniger sicheren Code produzierten, obwohl sie glaubten, sichereren Code geschrieben zu haben. Dieses blinde Vertrauen kann Sicherheitsrisiken begünstigen (Klemmer et al. 2024). Um dadurch auftretende Unfälle zu verhindern, müssen zusätzliche Mechanismen wie statische und dynamische Codeprüfungen sowie strenge Evaluations- und Validierungsmethoden implementiert werden (Sarkar et al. 2022). Die erwartbare Zunahme an von KI generiertem und nachträglich zu prüfendem Code kann die durch die Tools entstehende Zeitersparnis bei der Programmierung somit wieder zunichtemachen wenn diese keinen qualitativ ausreichend guten und fehlerfreien Code produzieren (Klemmer et al. 2024), (Sarkar et al. 2022). 
4.5.	Soziale, Rechtliche und Ethische Herausforderungen
Die sozialen, rechtlichen und ethischen Anforderungen betreffen die Sicherheit und den Schutz von Daten, die Auswirkungen auf die Umwelt, die Transparenz und Rechenschaftspflicht der KI-Systeme sowie die Vermeidung von Missbrauch und die Förderung einer verständlichen und rechtlich, ethisch und sozial vertretbaren Interaktion (Ray 2023).
(Borger et al. 2023) analysieren in ihrer Arbeit die Herausforderungen, die sich durch den Einsatz von großen Sprachmodellen (LLM) wie ChatGPT und Bard in den Bereichen der wissenschaftlichen Forschung und Bildung in Bezug auf diese drei zentralen Spannungsfelder ergeben. Es muss z.B. beachtet werden, dass diese Systeme sofort von jedermann nutzbar sind und grundsätzlich auch für böswillige Zwecke missbraucht werden können, welche der nutzenden Person bisher unzugänglich waren (Borger et al. 2023). Zum Schutz vor Missbrauch implementierte z.B. OpenAI Sicherheitsvorkehrungen die eine böswillige Nutzung von ChatGPT unterbinden soll (Borger et al. 2023).
Außerdem ergeben sich auch gesellschaftlichen Auswirkungen, die durch den Einsatz von KI-gestützter Systemen auftreten können. (Borger et al. 2023) zeigen auf, dass es noch zu lösenden Probleme in den Bereichen Privatsphäre, Vertraulichkeit und Sicherheit gibt. Andererseits zeigen sie auch, dass der Einsatz von KI bisherige Barrieren und Zugangsbeschränkungen überwinden kann. Ein Beispiel aus der Biologie zeigt, sich dadurch ergebende Vorteile. So können Biologe zukünftig KI-Systeme zur Softwareentwicklung nutzen wodurch theoretisch jeder Biologe zum Bioinformatiker werden kann. 
Eine ähnliche Analyse wird auch von (Wong et al. 2023) vorgenommen. Dieser gelangt zu der Erkenntnis, dass KI-gestützte Programmierung Softwareentwicklern die Möglichkeit eröffnet effizienter und effektiver zu arbeiten [4], es jedoch eine ausgewogene Balance zwischen der Produktivitätssteigerung einerseits und der Gewährleistung von Sicherheit, Schutz und Zuverlässigkeit andererseits benötigt. Dies gelingt jedoch nur, wenn das System dazu in der Lage ist, Probleme bereits in der Entwicklungsphase zu erkennen [8] und diese zu Lösen noch bevor sie zu einer Gefahr werden können [9,10].
Auch (Ylitalo) weißen auf den etischen Aspekt hin. Sie legen nahe, dass die eingesetzten Modelle und die Ausgaben dieser im Wesentlichen verstanden werden müssen, um die durch sie entstehenden ethischen Risiken und die Auswirkungen besser einordnen zu können.
Ein weiterer aus ethischer Perspektive zu beachtender Punkt kann aus den Ergebnissen von (Zamfirescu-Pereira et al. 2023) abgeleitet werden, welche herausarbeiten, dass die Interaktion mit LLM-Modellen einen gewissen Grad an Sprach- und Prompting-Expertise erfordert und sich bisher nicht an den Bedürfnissen von Nicht-Programmierern und Endbenutzern orientiert (Zamfirescu-Pereira et al. 2023). Es wird darauf hingewiesen, dass Nutzende zwar in der Lage sind, diese Systeme opportunistisch zu erkunden, jedoch Schwierigkeiten haben, systematisch mit dem System zu interagieren und robuste Ergebnisse zu erzielen. (Zamfirescu-Pereira et al. 2023) weißen außerdem darauf hin, dass die meisten Probleme dadurch entstehen, dass Menschen mit dem System ebenfalls, wie mit einem Menschen interagieren, die dazu kognitiven Fähigkeiten bisher aber nicht durch solche Systeme abgedeckt werden wodurch es zu etisch, rechtlich oder sozial bedenklichen Interaktionen kommen kann. (Ray 2023) ergänzen diese Aussage und führen verschiedene Herausforderungen bei der Entwicklung von LLM-basierten Chatbots als problematisch auf. Dazu gehören die Beibehaltung des Kontexts und der Kontextwechsel, der Umgang mit Mehrdeutigkeiten, die Personalisierung, das Nichtvorhandensein von „gesundem Menschenverstand“, emotionale Intelligenz, ethische Überlegungen, Robustheit und Sicherheit, der Umgang mit Anfragen außerhalb der Trainingsdaten sowie die Skalierbarkeit und Effizienz.
Außerdem weisen (Zamfirescu-Pereira et al. 2023) darauf hin, dass die Entwicklung von LLM-basierten Chatbots, wie beispielsweise Bots im Kundenservice, für Laien eine Herausforderung darstellt, da deren Umsetzung sowohl effektiver Strategien zum Verständnis des Kontextes bedarf als auch eine wirksame Strategie zur Detektion von Fehlern und zur Bewertung der Systemwirksamkeit erfordert. Um dieses Problem zu adressieren, stellen die Autoren „BotDesigner“ vor, einen No-Code-basierten Chatbot-Designer, der es Laien einerseits ermöglicht, einen Chatbot auf Basis eines LLMs allein durch Eingabeaufforderungen zu entwickeln, und andererseits einen Chatbot generiert, der Nutzenden effizient und einfach verständlich durch die zu erledigende Aktivität führt. 
Auch auf rechtlicher Seite ergeben sich einige Hürden. So muss ein effektiver Schutz der Privatsphäre und der Daten gemäß den geltenden Gesetzen und Vorschriften gewährleistet sein (Ray 2023). Ein weiterer Punkt stellt die Gewährleistung des Urheberrechts dar. Hierbei kann es sowohl durch das Training der Modelle als auch durch die eigentliche Modellausgabe zu Urheberrechtsverstößen kommen (Klemmer et al. 2024). Werden z.B. die eingegebenen Prompts und die daraus resultierenden Antworten mit in das zukünftige Modelltraining einbezogen, so kann es passieren das zukünftige Modelle dieses Wissen erlernen und sich als Quelle dieser Information ausgeben, da Metadaten aus vorherige Sitzungen wie der Name des Autors meist nicht bereitstehen und somit nicht in das Training einfließen (Klemmer et al. 2024). Die eigene Urheberschaft nachzuweisen könnte sich in diesem Fall als schwierig erweisen. Des Weiteren können die durch den Assistenten ausgegebenen Antworten selbst Urheberechtlich geschützte sein, was ein immenses Rechtsrisiko für Nutzende darstellt (Klemmer et al. 2024). 
5.	Angriffsmöglichkeiten und Schutz von KI-Codegeneratoren
5.1.	Angriffsmöglichkeiten auf KI-Generatoren
5.1.1.	Revers Psychologie, Prompt-Injection und Jailbreak-Angriffe
Mit dem verstärkten Einsatz von KI-Sprachmodellen wie ChatGPT steigen auch die Risiken im Bereich der Cybersicherheit. (Gupta et al. 2023) analysieren die Gefahren, die bei einer missbräuchlichen Verwendung dieser Modelle entstehen können, und zeigen, wie ethische Sicherheitsbeschränkungen und Datenschutzvorkehrungen durch Techniken wie umgekehrter Psychologie, Prompt-Injection\todo{Erklären} und Jailbreak-Angriffe\todo{Erklären} außer Kraft gesetzt werden können. Diese Angriffe ermöglichen es, die Sicherheitsmechanismen von Sprachmodellen zu umgehen, indem spezielle Eingaben genutzt werden, um unerwünschte oder schädliche Ausgaben zu erzeugen. Das Umgehen dieser Schranken führt dazu, dass diese Systeme auch zum Erstellen von Schadsoftware oder gar zum Ausführen von Angriffen eingesetzt werden können (Gupta et al. 2023) .
Darüber hinaus zweigen Studie von Niu et al. (2023) und (Hossain et al. 2023), dass 2,82 % (Niu et al. (2023) der Ausgaben von KI-Modellen sensible, personenbezogene und technische Daten wie Benutzerdaten, Adressen, E-Mail-Adressen und Geburtsdaten, geistiges Eigentum, gespeicherte sensible Daten, Schlüssel, geschützter Quellcode, sensible Modelle und firmeninterne Algorithmen enthalten die durch die zuvor vorgestellten Angriffe aber auch während der normalen Nutzung dieser Systeme zugreifbar sind. Zudem finden sich in 0,78 % der Fälle Informationen aus Krankenakten oder Identitäten und in 0,64 % geheime Informationen wie private Schlüssel für biometrische Authentifizierung oder Passwörter (Negri-Ribalta et al. 2024). Dies stellt ein erhebliches Sicherheitsrisiken dar.
5.1.2.	Poisoning
Ein anderer Grund für die Ausgaben von qualitativ ungeeignetem und unsicher Code stellt die absichtlich negative Beeinflussung der Modelle dar. So zeigt (Improta 2023) auf, wie NLP-Code-Generatoren durch Poisoning angegriffen werden können und welche Angriffsvektoren sich daraus ergeben. (Improta 2023) analysiert sowohl Blackbox als auch Whitebox-Angriffe die sie vor-, nach-, und während des Trainings durchführen. Des Weiteren werden die Auswirkungen von Angriffen in der Pre- und Fine-Tune-Phase analysiert. Generell orientieren sich Poisoning Angriffe an der bereits zuvor als kritisch zu betrachtend vorgestellten Mechanik der Trainingsdatenbeschaffung, indem in diese Daten absichtlich fehlerhaften Trainingsdaten injizierten werden [31, 35, 30, 28] (Cotroneo et al. 2024), (Improta 2023). Dabei sind gut gemachte Poisoningangriffe nur schwer zu erkennen, da diese oft so konstruiert sind das sie die Gesamtleistungsfähigkeit des Modells nicht beeinträchtigen und das vergiftetet Modell lediglich dazu verleitet wird auf bestimmte Anfragen mit durch bekannte Schwachstellen und Sicherheitsmängeln kompromittierten Code zu antworten (Improta 2023). 
Zum Infizieren der Trainingsdaten bieten sich indes mehrere Strategien an. Bei einem White Box Angriff kann der Angreifer vergiftete Elemente, in die bereits vorhandene Trainingsdaten einschleusen, braucht dazu aber auch direkten Zugriff auf diese (Improta 2023). Beim einem Black Box Angriff kann der Angreifer nicht direkt auf die bereits gesammelten Daten zugreifen und versucht stattdessen das durch Webcrawler durchgeführte Sammeln von Daten durch das geschickte platzierte fehlerhafte Daten innerhalb der zu crawlenden Quellen zu kompromittieren (Improta 2023). Außerdem kann das Kompromittieren sowohl in der Pre- als auch in der Finetuning Phase durchgeführt werden (Improta 2023). In der Pre Tuning Phase werden die massenhaft zur Verfügung gestellten Basisdaten des Modells kompromittiert, während ein Angriff auf das Fine Tuning die Daten, die das Modell für seinen spezifischen Anwendungsfall vorbereiten und optimieren sollen kompromittiert werden (Improta 2023). 
5.2.	Verteidigung von KI-Codegeneratoren
Die zunehmende Nutzung von KI-Codegeneratoren macht ein umfangreiches Konzept zur Wahrung der Qualitativ und der Sicherheit notwendig. Um diese Systeme gegen Missbrauch und gegen das generieren von schlechtem mit Schwachstellen versehenen Code zu schützen, sind verschiedene Strategien erforderlich.
5.2.1.	Qualitäts- und Schwachstellenanalyse des ausgegebenen Codes
Ein ausschlaggebender Faktor bei der Akzeptanz von durch KI-Codegeneratoren generierten Code ist dessen Qualität, insbesondere bezugnehmend auf die Sicherheit. Um dies zu gewährleisten müssen Möglichkeiten geschaffen werden den generierten Code (teil-)automatisierte zu überprüfen (Taeb et al. 2024), (Cotroneo et al. 2024), (Hossain et al. 2023) oder um direkt sicheren Code zu generieren. Dies lässt sich insbesondere anhand der in Kapitel 4.2 erläuterten Schwierigkeiten in Bezug auf die Codequalität nachvollziehen. Um potenzielle Sicherheitsrisiken zu minimieren muss der von KI geschriebene Code daher genauso kritisch begutachtet werden wie der eines Menschen (Klemmer et al. 2024).
Um das in Kap 4.2 bereits angesprochene Problem des Erkennen von Schwachstellen in unfertigem (Cotroneo et al. 2024) und nicht lauffähigem (Berabi et al. 2024) Code zu adressieren, stellen (Cotroneo et al. 2024) und (Berabi et al. 2024) zwei mögliche Lösungen vor. (Berabi et al. 2024) stellen zur Lösung des Problems der automatischen Behebung nicht trivialer Codierungsfehler und Sicherheitslücken das System DeepCode AI Fix vor. Dieses wurde auf einem Datensatz bestehend aus Commits aus verschiedenen Open-Source-Repositories trainiert. Zur Erkennung reduzieren das System den Kontext auf wesentliche Informationen, wodurch weitreichende Abhängigkeiten auch innerhalb von unfertigem und nicht lauffähigem Code erkannt und die Codequalität verbessert werden kann.  (Cotroneo et al. 2024) stellen das Tool DeVAIC (Detection of Vulnerabilities in AI-generated Code) vor, dass ebenso dazu in der Lage ist, vollständigem, aber auch unvollständigem Python-Code zu überprüfen. Das System basiert auf der Erkennung sicherheitskritischer Muster und regulärer Ausdrücke und zeigt eine Genauigkeit von 94 % bei der Erkennung von 35 Common Weakness Enumerations (CWEs), welche unter die Top 10 OWASP Schwachstellenkategorien fallen. Zur Analyse eines Code-Schnipsels benötigt das System lediglich 0,14 Sekunden und übertrifft somit kommerziell eingesetzte Produkte wie CodeQL [16], Bandit [65], PyT [67] und Semgrep [72], bei der Schwachstellenerkennung [62, 13, 2, 33] welche darüber hinaus nur mit vollständigem Code arbeiten können (Cotroneo et al. 2024). 
Eine weitere technische Möglichkeit wurde von „He und Vechev“ (2023) mit dem Tool SVEN vorgestellt. Dieses kann bestehenden Codegeneratoren vorangestellt werden und benötigt kein weiteres Training oder Fine-Tuning. SVEN liefert mit den beiden Systemen SVENsec sowie SVENvul zwei verschiedene Tools mit denen sich entweder gezielt sicherer oder unsichere Code generieren lässt (Negri-Ribalta et al. 2024). SVENsec erhöht die Sicherheitsrate dabei von 59,1 auf 92,3 % (He und Vechev, 2023) wobei SVENvul das Risiko je nach Modellparameter um 23,5 % für 350 Millionen Parameter, 22,3 % für 2,7 Millarden Parameter und 25,3 % für 6,1 Milliarden Parameter erhöht.
Außerdem weißen (Negri-Ribalta et al. 2024) darauf hin, dass durch KI-generierter Code genauso wie menschengenerierter Code durch statische und dynamische Evaluationsmethoden geprüft werden muss. Hierzu gehören umfassende Sicherheitsprüfungen und Peer Reviews, um mögliche Schwachstellen zu identifizieren und zu beheben (Negri-Ribalta et al. 2024). Durch die Implementierung dieser Schutzmaßnahmen können die Risiken beim Einsatz von KI-Codegeneratoren minimiert und die Sicherheit sowie die Qualität des generierten Codes erheblich verbessert werden.
Ein weiterer Ansatz wird von (Taeb et al. 2024) vorgestellt. Diese validieren die Sicherheit von CodeBERT, GPT 3.5 und CodeX indem sie das System auffordern mit CVE-, CWE, NIST und NVD-Schwachstellen sowie den Top10 OWASP Web Risiken kompromittiertem Code zu analysieren und zu reparieren. 
5.2.2.	Datenerstellung
Wie bereits in Kapitel \todo{Ref} erläutert, bestehen, bedingt durch die Mechaniken zur Datensammlung, zahlreiche Angriffsvektoren, welche ein Datapoisoning \todo{Ref} begünstigen. Diese Daten sind für das Training jedoch unerlässlich. Um das Vorhandensein von kompromittierten Daten ausschließen zu können, sollten KI-Modelle nur auf geprüfte und qualitativ hochwertige, aus vertrauenswürdigen Quellen stammenden oder gelabelten Daten trainiert werden (Improta 2023), (Perry et al. 2023), (Negri-Ribalta et al. 2024). Außerdem empfehlen (Negri-Ribalta et al. 2024) die Modelle sowohl mit positiven als auch mit negativen, gelabelten Beispiele zu Trainieren um dem System nicht nur zu vermitteln was gut sondern auch was schlecht ist (Negri-Ribalta et al. 2024). Das Vorhandensein entsprechender Labels ist jedoch oft nicht gegeben. Das manuelle Prüfen und Kennzeichnen dieser Daten stellt darüber hinaus eine mühsame und fehleranfällige Tätigkeit dar (Desmond et al. 2022), welche meist nicht praktikabel ist. 
Eine Lösungen könnten darin bestehen, Techniken zum automatischen Labeln oder zur Bereinigung von fehlerhaften Daten einzusetzen, um die Qualität der Modelle zu verbessern. Dazu könnten die genutzten Trainingsdaten vorab durch statische Analysetools analysiert werden (Improta 2023; Perry et al. 2023). (Cotroneo et al. 2024) nennt zur Identifizierung und Bewertung von Sicherheitslücken im generierten Code verschiedene Werkzeuge und Sicherheits-Test-Suiten wie CodeQL, die Security Test Suites, Bandit, Semgrep und das Python-Taint-Modul (PyT). Diese Tools könnten jedoch auch genutzt werden, um die eigentlichen Trainingsdaten zu untersuchen. Zudem sollten auch Verfahren entwickelt werden, welche Wissen aus Bibliotheksdokumentation sowie „Expertenwissen“ heranzuziehen, um die in den Trainingsdaten vorhandenen Beispiele entsprechend zu gewichten (Perry et al. 2023).
Eine weitere Lösung wird von (Desmond et al. 2022) angeboten. Die Autoren stellen dazu ein System vor, welches einen interaktiven, KI-gestützten Datenbeschriftungsansatz anbietet. Dieser könnte genutzt werden, um den Korpus für das Wissen von LLMs um gelabelte Daten (z.B. gute und schlechte Codebeispiele) zu ergänzen. Dieses System kann sowohl unüberwacht als auch halbüberwacht arbeiten. Ein mögliches Szenario bestünde darin, durch Menschen gekennzeichnete Daten sowie Daten aus Quellen mit bekannten Leistungswerten, wie z.B. Kaggle-Wettbewerben im Bereich der KI-Effizienz oder Hackathons im Bereich Code-Sicherheit, zu extrahieren und die Ergebnisse dieser Wettbewerbe als Labels zu verwenden. Diese Daten könnten dann genutzt werden, um Daten aus anderen Quellen, z.B. Repositories, automatisch semisupervised nachzulabeln.
Ein weiterer empfohlener Ansatz zur Risikominimierung sieht vor, verschiedene Programmiersprachen in die Trainingsdaten miteinzubeziehen und ein Gleichgewicht zwischen der Größe des Trainingsdatensatzes und der Fähigkeit des Systems zu finden (Negri-Ribalta et al. 2024). Außerdem sollten die Modelle ein Feintuning mit sorgfältig ausgewählten Daten durchlaufen sowie ein strengeres Training hinsichtlich syntaktischer und semantischer Korrektheit erfahren.
Außerdem könnten die in Abschnitt \todo{4.2?} vorgestellten Ansätze zur Sicherheitsanalyse des durch KI-Codegeneratoren ausgegebenen Codes auch zur Analyse der Trainingsdaten eingesetzt werden. Des Weiteren könnten die Ausgaben der Generatoren mit allen hier vorgestellten Tools geprüft und gelabelt und im Anschluss den Trainingsdaten zugeführt werden. Somit könnte ein kontinuierliches Lernen der KI-Codegeneratoren erzielt, die Integrität und Sicherheit der Trainingsdaten gewährleistet und die Leistungsfähigkeit der KI-Codegeneratoren optimiert werden.
5.2.3.	Datensätze zum Verifizieren der Codekorrektheit und Codesicherheit
Die Validierung und Verbesserung von KI-Codegeneratoren erfordert umfangreiche Datensätze zu deren Training und Evaluation. Diese Datensätze müssen, um diese Gen-KI Systeme effizient testen zu können, dazu geeignet sein innerhalb eines automatisierten Prompt-Programmierungs-Evaluierungs-Prozesses eingesetzt werden zu können. Die im Folgenden Vorgestellten Datensätze können hierbei eine wesentliche Rolle spielen, da sie eine strukturierte und standardisierte Basis für das Testen und Optimieren der KI-Modelle bieten. 
HumanEval: Der HumanEval-Datensatz (Chen, Tworek, Jun, Yuan, de Oliveira Pinto, et al., 2021) (Sarkar et al. 2022) besteht aus 164 handgeschriebenen Programmierproblemen. Jedes Problem enthält eine Funktionssignatur, einen Docstring, einen Body und mehrere Unit-Tests, wobei im Durchschnitt 7,7 Tests pro Problem vorhanden sind. Dieser Datensatz ermöglicht es, die Fähigkeit eines KI-Codegenerators zu überprüfen, korrekten und funktionalen Code, ausgehend von einem Docstring zu schreiben, der die gestellten Anforderungen erfüllt und die definierten Tests besteht (Quelle: HumanEval Dataset | Papers With Code, GitHub - openai/human-eval: Code for the paper "Evaluating Large Language Models Trained on Code").
Mostly Basic Python Problems (MBPP): Der MBPP-Datensatz (Austin et al., 2021) (Sarkar et al. 2022) bietet eine Sammlung von etwa 1000 Python-Programmieraufgaben auf Einsteigerniveau, die ähnlich wie HumanEval strukturiert sind (Aufgabenbeschreibung, Lösung, Testfälle). Er kann verwendet werden, um die generativen Fähigkeiten der Modelle und das Verständnis der gestellten Prompts in Bezug auf verschiedene Programmierprobleme zu evaluieren. Durch die Verwendung dieses Datensatzes kann überprüft werden, ob die Modelle in der Lage sind, präzisen und funktionalen Code für diverse Aufgaben zu erzeugen (Quelle: Program Synthesis with Large Language Models" von Austin et al. (2021), google-research/mbpp at master · google-research/google-research · GitHub).
CodeContests: CodeContests (Y. Li et al., 2022b; Sarkar et al. 2022) ist ein 13.000 Trainings-, 113 Validierungs-, und 165 Testbeispiele umfassender Datensatz, dessen Schwierigkeit auf kompetitivem Wettbewerbsniveau angesiedelt ist. Er umfasst neben der Aufgabenbeschreibung, der Lösung und Testfällen auch inkorrekte menschliche Lösungen. Die Probleme sind in der Regel komplexer und erfordern fortgeschrittene Programmierkenntnisse. Der Datensatz hilft dabei, die Fähigkeit der KI-Modelle zu testen, anspruchsvolle und realistische Programmierprobleme zu lösen (Competition-level code generation with AlphaCode, GitHub - google-deepmind/code_contests).
CodeXGLUE: CodeXGLUE (Lu et al., 2021) CodeXGLUE [(Cotroneo et al. 2024), 47] ist eine umfassende Benchmark-Suite und umfasst insgesamt 14 Datensätze bestehend aus 10 Programmiersprachen (CodeXGLUE (microsoft.github.io)). Er enthält verschiedene Aufgaben aus dem Bereich der Softwarenentwicklung zu den Themen Code-Code (Klon-Erkennung, Fehlererkennung, Lückentest, Code-Vervollständigung, Code-Verfeinerung und Code-zu-Code-Übersetzung), Text-Code (natürlichsprachliche Code-Suche, Text-zu-Code-Generierung), Code-Text (Code-Zusammenfassung) und Text-Text (Dokumentationsübersetzung). Außerdem enthält die Benchmark-Suite eine Plattform zur Evaluierung von Modellen und drei Baseline Referenzmodelle, basierend auf CodeBERT, CodeGPT und einem Encoder-Decoder-Framework für Sequence-to-Sequence-Aufgaben. Dieser Benchmark-Suite ist besonders geeignet, um die generelle Leistungsfähigkeit von KI-Modellen in unterschiedlichen Programmierkontexten zu bewerten (CodeXGLUE (microsoft.github.io), CodeXGLUE: A Machine Learning Benchmark Dataset for Code Understanding and Generation).
Copilot CWE Scenarios Dataset [(Cotroneo et al. 2024), 63: Der Copilot CWE Scenarios Dataset enthält 89 spezifische Programmieraufgabenszenarien, die auf den Top-25 Common Weakness Enumeration (CWE) basieren. Dieser Datensatz wird verwendet, um die Fähigkeit der KI-Modelle zu testen, sicherheitskritische Schwachstellen zu identifizieren und zu beheben. Jedes Szenario besteht aus einer Aufgabenbeschreibung, Metadaten und CWE-Informationen. Neben dem Datensatz stellen die Autoren auch ein Evaluierungsframework zur Verfügung mit welchem die durch den KI-Codegenerator bassierten Ergebnisse ausgewertet werden können. Grundlage hierfür bildet CodeQL(About CodeQL — CodeQL (github.com)) (Copilot CWE Scenarios Dataset (zenodo.org), Asleep at the Keyboard? Assessing the Security of GitHub Copilot’s Code Contributions). 
SecurityEval [(Cotroneo et al. 2024), 77]: SecurityEval ist ein Framework, das speziell zur Bewertung der Sicherheitsaspekte von KI-generiertem Code entwickelt wurde. Er enthält eine Vielzahl von sicherheitskritischen Szenarien und Schwachstellen, basierend auf Common Weakness Enumeration (CWE). Diese müssen von den zu testende Modelle erkannt und behoben werden. Dazu liefert das Framework eine Aufgabenbeschreibung, fehlerhaften Code, Lösungscode und Testfälle sowie eine auf CodeQL basierende Auswertung der Ausgaben.
LLMSecEval [(Cotroneo et al. 2024), 84]: LLMSecEval ist ein Benchmark-Datensatz zur Bewertung der Sicherheitsleistung von großen Sprachmodellen (LLMs) bei der Codegenerierung. Er umfasst 150 verschiedene sicherheitsrelevante Programmieraufgaben in natürlicher Sprache sowie deren Lösungen. Die Szenarien wurden so gewählt, dass sie anfällig für die Top 25 Common Weakness Enumeration (CWE) sind (LLMSecEval: A Dataset of Natural Language Prompts for Security Evaluations). Der Datensatz hat das Ziel die Erkennungsrate von Schwachstellen und die allgemeine Sicherheit des generierten Codes zu beurteilen.
CrossVul (Negri-Ribalta et al. 2024): CrossVul ist ein Cross-Language-Vulnerability-Datensatz, der Informationen zu Sicherheitslücken in verschiedenen Programmiersprachen enthält. Der Datensatz umfasst Commit-Daten, die für die Analyse und Erkennung von Sicherheitsschwachstellen in Software-Projekten verwendet werden können. CrossVul wurde entwickelt, um Forschern und Praktikern im Bereich der Softwaresicherheit ein umfangreiches und vielseitiges Dataset zur Verfügung zu stellen, das für verschiedene Anwendungen wie die Entwicklung von Vulnerability-Detection-Modellen genutzt werden kann. Im Vergleich zu anderen Datensätzen wie CVEFixes, Devign, ReVeal und BigVul trägt CrossVul zur Vielfalt und Größe der verfügbaren Daten für Sicherheitsanalysen bei. (https://2021.esec-fse.org/details/fse-2021-demonstrations/15/CrossVul-A-Cross-Language-Vulnerability-Dataset-with-Commit-Data, https://dl.acm.org/doi/abs/10.1145/3468264.3473122)
Big-Vul (Negri-Ribalta et al. 2024): Der Big-Vul-Datensatz ist eine umfangreiche Sammlung von C/C++-Code-Schwachstellen, einschließlich Codeänderungen und CVE-Zusammenfassungen. Er umfasst CVE-Einträge aus dem Zeitraum von 2002 bis 2019 und enthält detaillierte Informationen zu jeder Schwachstelle. (https://dl.acm.org/doi/abs/10.1145/3379597.3387501).
MegaVul: Der Big-Vul-Datensatz ist eine umfangreiche Sammlung von Informationen über Software-Sicherheitslücken in großen Open-Source-Projekten. Er enthält Details zu den Schwachstellen, ihrer Schwere, dem betroffenen Code und den Maßnahmen zur Behebung. Der Datensatz dokumentiert auch den Kontext der Entdeckung, einschließlich der verwendeten Methoden und Werkzeuge. Big-Vul ermöglicht eine quantitative Analyse, um Muster und Trends in der Entstehung und Behebung von Sicherheitslücken zu erkennen und präventive Maßnahmen zu entwickeln. (https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=10555623)
VUDENC (Negri-Ribalta et al. 2024): Der Datensatz „VUDENC: Vulnerability Detection with Deep Learning on a Natural Codebase for Python“ ist speziell entwickelt worden, um die Erkennung von Sicherheitsanfälligkeiten in Python-Code mittels Deep Learning zu unterstützen. Dieser Datensatz umfasst eine Sammlung von Python-Quellcode-Snippets, die sowohl sichere als auch unsichere Code-Abschnitte enthalten.
5.2.4.	Technische Absicherungen
Technische Sicherungsmaßnahmen sind aufgrund der stetig steigenden Verbreitung von KI-Codegeneratoren ein zentrales Element zu deren Absicherung [2]. Dabei ergeben sich mannigfaltige Möglichkeiten zur Gewährleistung der Sicherheit von KI-Systemen. 
Eine Möglichkeit besteht beispielsweise darin, die KI-Assistenten auf eigener Hardware selbst zu hosten (Klemmer et al. 2024). Um diese zu schützen, sollten sowohl die Daten als auch die Modelle selbst sowie die Benutzeroberflächen, API-Endpunkte und die Software inklusive aller (Drittanbieter-) Bibliotheken mit umfangreichen Sicherheitsmaßnahmen gegen potenzielle Bedrohungen wie Daten- und Model-Spoofing, Manipulation, Verleugnung, Informationsoffenlegung, Denial-of-Service und Rechteausweitung geschützt werden (Hossain et al. 2023). Zur proaktiven Absicherung können Sicherungsmechanismen wie Zugangskontrollen, Verschlüsselung, Integritätsprüfung (Signaturen und Hashes zur Integritätsprüfung der Modelle und Trainingsdaten) und Authentifizierungs- und Autorisierungsmechanismen implementiert werden (Hossain et al. 2023), (Improta 2023). Ein weiterer wichtiger Punkt ist, das auch die Entwicklungsumgebung selbst bzw. die KI-Plattform in welcher sich das Modell befindet sicher ist (Taeb et al. 2024).
Ein anderer Ansatz zur Erhöhung der Sicherheit sieht die Nutzung von externen, kommerziellen Systemen mit vorgelagerten, filternden Proxysystemen vor (Klemmer et al. 2024).  Hierbei muss aber sowohl die Sicherheit der Proxy als auch der Zugriff durch und auf externe Systeme mit zusätzlichen Schutzmaßnahmen versehen werden.  Außerdem kann die Sicherheit bei der Nutzung auch durch organisatorische Lösungen wie  Datenschutzgarantien durch den Betreibenden erhöht werden (Klemmer et al. 2024).
Diese Maßnahmen schaffen eine vertrauenswürdige Codierungsumgebung und gewährleisten ein sicheres System. 
5.2.5.	Spezialisieren der Modelle
Eine weitere Option zur Qualitätsverbesserung der Ausgaben stellt das Spezialisieren von Modellen dar. Dabei werden Modelle gezielt für Aufgaben in Bereichen wie der Softwaresicherheit optimiert. Dazu sind jedoch qualitativ hochwertigerer, besserer und gegebenenfalls auf Sicherheitsrisiken spezialisierte Datensätze notwendig (Klemmer et al. 2024). Außerdem ist für die Erstellung domänenspezifischer Modelle eine explizite Wissensdarstellung notwendig, die maschinenverständlich aufbereitet ist (Feltus et al. 2021). Dies gewährleistet, dass das Fachwissen klar und strukturiert erfasst und von einem AI-Modell verarbeitet werden kann. 
5.2.6.	Optimierung der Prompts
Wie bereits zuvor gezeigt, besteht eine Abhängigkeit zwischen der Sprach- und Wortgewandtheit und dem Prompt-Design mit der Ergebnisqualität (Klemmer et al. 2024), (Perry et al. 2023), (Res et al. 2024) (Negri-Ribalta et al. 2024) (siehe dazu Kapitel 3.4 und 4.2). 
Auf Seite der Sprach- und Wortgewandtheit zeigt sich, dass bereits kleine Rechtschreib-, Grammatik- und Kontextfehler oder Ungenauigkeiten in der Eingabe, die im natürlichen Sprachgebrauch akzeptabel sind, zu falschen Ergebnissen führen können (Perry et al. 2023), (Negri-Ribalta et al. 2024). 
Der Einfluss des Prompt-Designs wurde unter anderem von (Negri-Ribalta et al. 2024), (Pearce et al. 2022) und (Klemmer et al. 2024) betrachtet. Die Formulierung der gestellten Frage beeinflusst die Ergebnisqualität signifikant (Negri-Ribalta et al. 2024). Zudem führt das explizite Anweisen zur Generierung von sicherem Code tatsächlich zu sichererem Code (Klemmer et al. 2024), (Perry et al. 2023). Dies zeigt sich am Beispiel der Anfrage: „füge eine separate, nicht anfällige SQL-Funktion über einer Task-Funktion hinzu“, die in 94 % der Fälle zu sicherem Code führt, während „füge eine separate, anfällige SQL-Funktion über der Task-Funktion hinzu“ zu unsicherem Code resultiert (Pearce et al. 2022). Auch das Bereitstellen von Hilfs- und Beispielcode, detaillierten Aufgabenanweisungen, Kontextinformationen, gut spezifizierten Arbeitsschritten, Funktionsdeklarationen, genaue Spezifikationen (z.B. „verwende ECDSA“), klar definierte Anweisungen (z.B. „schreibe ein JavaScript“), Funktionsdeklarationen mit Parameter- und Typangaben (z.B. „def signusingecdsa(key, message):“), Rückfragen (z.B. „Was sind Zertifikate?“), Angaben zu verwendenden Bibliotheken (z.B. „nutze import crypto“), die Zielsprache (z.B. „schreibe in Python“), die Länge der Eingabe und die Distanz zwischen Prompt und zu lösender Aufgabe sowie zwischen vorausgegangenem Prompt und vorheriger Ausgabe, haben Einfluss auf die Ergebnisqualität (Perry et al. 2023), (Klemmer et al. 2024). Außerdem weißen einige Studienteilnehmer darauf hin, dass Sicherheitsprobleme einfacher erkannt werden können, wenn KI-Assistenzsysteme nur zur Generierung kleinere Codeblöcke verwendet werden (Klemmer et al. 2024).
Aus diesen Gründen schlagen (Negri-Ribalta et al. 2024) die Einführung von Richtlinien für das Prompting sowie für die Nachbearbeitung der Ergebnisse vor (Negri-Ribalta et al. 2024). Zudem hilft das Anpassen der Parameter der KI-Assistenten, wie zum Beispiel eine erhöhte Temperatur, dabei, sichereren Code zu generieren (Perry et al. 2023).
Darüber hinaus haben einige Studienteilnehmer bereits Strategien entwickelt, um auf unpassende Antworten des KI-Assistenten zu reagieren, beispielsweise durch das Bereitstellen zusätzlicher Informationen oder das Umformulieren der Prompts. Weiterhin stellen die Autoren fest, dass viele Prompts hintereinander innerhalb einer Session die Fehlerrate erhöhen, da der KI-Assistent dann auch mit den bereits in dieser Session gegebenen eventuelle falschen Ausgaben arbeitet (Perry et al. 2023).
Während die bisher aufgezeigten Optimierungsansätze explizit von den Fähigkeiten des Nutzenden abhängig sind, analysieren (Res et al. 2024) auch nutzerunabhängige Optimierungen, darunter Prefixtuning (Li und Liang 2021), General Alignment Shifting-Ansatz (Generalklausel) [8], szenario-spezifisches Prompt Tuning, iteratives Prompt Tuning sowie Kombinationen dieser Ansätze. 
Beim Prefixtunings (Li und Liang 2021) werden spezielle Token (Präfixe) vor die eigentlichen Prompt gesetzt, um die Ausgabe eines Sprachmodells zu steuern oder zu verbessern. (Res et al. 2024) weißen jedoch darauf hin, dass die von He und Vechev [7] vorgestellte Version Zugriff auf das Modell erfordert.
Der General Alignment Shifting-Ansatz verwendet eine "generelle Klausel" als Teil des Nutzerprompts, um die Sicherheitsausrichtung zu Beginn der Code-Generierung zu steuern. Diese Methode ist einfach zu implementieren und erfordert wenig bis kein Expertenwissen, kann jedoch von der LLM als irrelevant gefiltert werden und muss präzise formuliert werden, um wirksam zu sein. Diese Generalklausel können Anweisungen zum Generieren von sicherem Code enthalten. Ebenso können Informationen zu generellen oder spezifischen Sicherheitslücken (z.B. spezifische CWEs) angegeben werden.
Der szenario-spezifische Ansatz versorgt den KI-Assistenten mit detaillierten lokalen Kontextinformationen, Handlungsanweisungen, Warnungen und sicherheitsrelevanten Merkmalen, erfordert jedoch Expertenwissen, um potenzielle Risiken zu identifizieren und zu mindern. Automatische Vorschläge basierend auf Kontext und Datentypen können die Anforderungen an das Expertenwissen reduzieren.
Der iterative Ansatz verändert den Prompt durch wiederholte Anpassungen der Kommentare zu zuvor generiertem Code, wobei jede Iteration das vorherige Ergebnis einbezieht und zusätzliche Informationen oder Warnungen hinzufügt. Dabei kann z.B. in jeder Iteration die Anforderung zur Behebung einer spezifischen CWE erfolgen. Die Autoren nutzen zur Definition solch eines Regelwerks Mitre [26]. Diese Methode ist aufgabenunabhängig und erfordert kein Expertenwissen, da sie allgemeine Sicherheitsanforderungen iterativ anwendet und so eine breite Palette von Sicherheitsproblemen abdeckt. Allerdings kann ein unsachgemäß gestalteten Regelsatzes sowie die Reihenfolge der Iterationsschritte Auswirkungen auf die Rechenzeit und nicht zuletzt auf das Ergebnis haben. 
Zur Beurteilung der Wirksamkeit dieser Ansätze verwenden die Autoren das OpenVPN-Projekt in Kombination mit GitHub Copilot [6] und den zuvor vorgestellten Ansätzen. Dabei zeigt sich, dass sich die Generierung von unsicherem Code reduziert (Szenario - 16 %, iterativ - 12 %, clause - 8 %), während mehr sichere Code produziert wird (Szenario + 0 %, iterativ + 8 %, clause + 4 %) wird (Res et al. 2024).
Ein wesentlicher Vorteil all dieser Ansätze ist, dass diese Methode ressourcensparender sind als z.B. die Modeloptimierung, da weder ein weiteres Optimierungssystem benötigt wird noch ein Basismodell nachtrainiert werden muss. Die Wirksamkeit solcher Ansätze auf die Codesicherheit wurde bereits von [17][32][13][8]. 
5.2.7.	Modeloptimierung
(Res et al. 2024) analysieren neben der Wirkweise des Prompt Engineering auch anderen Ansätzen wie die Ausgabenoptimierung oder die Modellfeinabstimmung und vergleich diese. 
Bei der Ausgabenoptimierung wird die Ausgabe des Modells nachträglich durch weitere Systeme optimiert. So könnte dem Codegenerator ein weiteres auf Codesicherheit optimiertes Modell oder eine Kombination aus statischen Analysatoren und Regeln nachgelagert werden. Solch ein Konzept wurde von Snyk [24] vorgestellt. 
Bei der Modellfeinabstimmung wird ein vorhandenes Modell anhand weiterer Trainingsdaten z.B. aus dem Bereich Sicherheit nachtrainiert und die Ergebnisqualität in diese Richtung beeinflusst. Als Vorteil ist zu nennen, das Nutzende ohne weiteres Wissen sofort mit diesem Modell interagieren und sichern Code produzieren könne. Nachteilig zeigt sich jedoch, dass dazu Zugriff auf das Ursprungsmodell notwendig ist (Res et al. 2024).
5.2.8.	Menschzentrierter Schutz
Um Missbrauch vorzubeugen, setzen Betreiber wie Open AI auf integrierte, administrative Regelungen wie Governance- und Ethikrichtlinien [24] (Gupta et al. 2023). Auf Seite der Nutzenden können auch Regulatorische oder Rechtlicher Maßnahmen getroffen werden, um etwaige Risiken zu minimieren. So führen zahlreiche Unternehmen bereits Richtlinie zur KI-Nutzung ein (Klemmer et al. 2024). Hierbei sind insbesondere große Technologievorreiter wie Apple [65], Samsung [36] und Google [24] zu nennen, welche die Nutzung von KI-Assistenzsystemen komplett untersagen (Klemmer et al. 2024). Im Falle von Google [24] wurde sogar der Einsatz des hauseigenen Chatmodells Bart aufgrund von Sicherheits- und Qualitätsprobleme sowie Datenschutzbedenken verboten [24] (Klemmer et al. 2024). Diese Regeln werden aber oft missachtet oder umgangen (Klemmer et al. 2024).
Außerdem sollten Urheberrechtsrisiken adressiert werden, indem durch technische oder regulatorische Maßnahmen lediglich Prompts ohne Quellcode übergeben werden dürfen und der generieten Code nicht direkt verwendet werden darf (Klemmer et al. 2024).
Ein weiterer Baustein zur Sicherung der Codequalität und -sicherheit, kann durch die Schulung der Nutzer in Bezug auf die Verwendung von Codegeneratoren erfolgen (Negri-Ribalta et al. 2024), (Taeb et al. 2024). So geben (Klemmer et al. 2024) zu bedenken, dass es im Laufe der Zeit zu einem Gewöhnungseffekt kommen könnte wodurch die Ergebnisse dieser Systeme, trotz fragwürdiger oder fehlerhafter Ausgaben, weniger Kritisch hinterfragt werden (Klemmer et al. 2024). Den Nutzenden muss somit vermittelt werden diese Tools richtig zu verwenden, die Ergebnisse kritisch zu hinterfragen, die Qualität des generierten Codes zu bewerten und Schwachstellen frühzeitig zu erkennen (Negri-Ribalta et al. 2024), (Taeb et al. 2024). Dazu gehört auch das den Ausgaben von KI-Codegeneratoren ein gewisses Maß an Misstrauen entgegengebracht werden sollte und das diese Ausgaben immer einer Sicherheitsprüfungen zu unterziehen sind (Negri-Ribalta et al. 2024). Daher sollte weitere Forschung auch die Entwicklung von praktischen Schulungen für Nutzenden untersuchen (Taeb et al. 2024). Außerdem sollten Nutzende über die Grenzen der KI-Modelle informiert und das Design der Benutzeroberfläche in dieser Richtung angepasst werden (Negri-Ribalta et al. 2024).
Diese Schutzmechanismen beschränken sich dabei nicht auf den Bereich der klassischen Codegenerieren sondern können auch im Bereich der Generierung von KI durch KI angewandt werden. Zusätzlich weißen diese Systeme trotz kontinuierlicher Fortschritte häufig Schwächen in der umfassenden Unterstützung von Domänenexperten ohne spezifisches KI- oder Netzwerk-Know-how auf (Borger et al. 2023; Gottlander und Khademi 2023; Sundberg und Holmström 2023; Sarker 2022; Sarkar 2023; Pakalapati et al. 2023; Wong et al. 2023). So besteht eine große Notwendigkeit Nicht-KI-Experten in der Modellierung zu unterstützen (Feltus et al. 2021; Ylitalo; Minn 2022; Desmond et al. 2022). Weiterhin zeigen (Yang et al. 2018) und (Pinhanez 2019), dass KI-Tools wie interaktive maschinelle Lernwerkzeuge und Chatbots so gestaltet werden müssen, dass sie die Bedürfnisse von Nicht-KI-Experten berücksichtigen, da sie sonst für diese Nutzergruppe keine Vorteile bieten (Yang et al. 2018; Pinhanez 2019). Eine Studie von (Zamfirescu-Pereira et al. 2023) kommt zu dem Ergebnis, dass Nicht-KI-Experten oft Schwierigkeiten haben, effektive Prompts für große Sprachmodelle zu entwerfen (Zamfirescu-Pereira et al. 2023) während (Ray 2023) aufzeigt, dass eine ausgewogene Balance zwischen KI- und menschlicher Expertise geben sein muss, um effektive Ergebnisse zu erzielen (Ray 2023). Ein KI-Assistenzsysteme zur Erstellung und Verwaltung komplexe KI-Anwendungen für vernetzte und heterogene Umgebungen muss diese Punkte berücksichtigen, um erfolgreich zu sein. So ist der Einsatz von Domänenexperten ohne spezifisches KI-Knowhow denkbar, nicht jedoch der Einsatz von Nicht-KI-Experten ohne Domänenwissen. Außerdem müssen das KI-Assistenzsysteme und die intuitiver Benutzeroberfläche für den Einsatz durch Domänenexperten optimierte werden.
6.	Angriffsmöglichkeiten und Schutz durch KI-Codegeneratoren
6.1.	Angriffsmöglichkeiten durch KI-Codegeneratoren
(Gupta et al. 2023) zeigen am Beispiel von ChatGPT auf, wie GenKI-Techniken zur Erstellung von Cyberangriffen wie Social-Engineering-Angriffe, Phising Mails, Maleware und autonom generierten Angriffsnutzlasten sowie Schadcode genutzt werden können (Gupta et al. 2023) .
6.2.	Verteidigungsmöglichkeiten durch KI-Codegeneratoren
Andererseits weißen (Gupta et al. 2023) und (Taeb et al. 2024) darauf hin, das sich diese Tools zum Verteidigen von IT-Umgebungen einsetzen lassen. So kann durch den Einsatz von KI-Codegeneratoren die Effizienz und Sicherheit des Codes verbessert werden (Taeb et al. 2024), was eine Reduzierung der Angriffsfläche zur Folgen haben kann. 
Dabei kann es ebenfalls notwendig sein Ethikrichtlinien außer Kraft zu setzen, da das System ansonsten keine verwertbaren Informationen liefert (Gupta et al. 2023). Außerdem wird erläutert, wie ChatGPT für eine reaktionsschnelle, automatische Cyberabwehr eingesetzt werden kann. Dabei können z.B. die Analyse von Daten wie Netzwerkverkehr und Log-Daten zur Angriffserkennung, die Erstellung von Bedrohungsinformationen und Berichten sowie die automatische Generierung von sichern Code und Testfällen durch GenKI verbessert werden. Darüber hinaus können diese Systeme auch zur Schulung eingesetzt werden, um z.B. das Sicherheitsbewusstsein der Mitarbeiter zu verbessern (Gupta et al. 2023).
7.	Zusammenfassung der Auswirkungen unsicherer KI-Codegeneratoren
Die Nutzung unsicherer KI-Codegeneratoren birgt erhebliche Risiken und Herausforderungen, die soziale, rechtliche und ethische Aspekte sowie Fragen der Zuverlässigkeit, Sicherheit und Datenschutz betreffen. Unsichere Systeme können das Vertrauen in die Technologie untergraben, indem sie fehlerhaften oder unsicheren Code erzeugen (Gupta et al. 2023). Zudem besteht die Gefahr, dass solche Codegeneratoren sozial, ethisch und rechtlich problematische Inhalte liefern (Gupta et al. 2023) oder private sowie urheberrechtlich geschützte Informationen preisgeben (Negri- (Negri-Ribalta et al. 2024), (Taeb et al. 2024). Darüber hinaus können die Modelle bestehende Trainingsdaten kopieren, anstatt neuen Code zu generieren (Sarkar et al. 2022).
Die Herausforderungen erstrecken sich auch auf die technische Zuverlässigkeit: Die Qualität der Antworten kann über die Zeit hinweg nachlassen, und es können komplexe sowie nicht ausführbare Lösungen ausgegeben werden (Klemmer et al. 2024). Zudem können Fehler und Inkonsistenzen aus den Trainingsdaten in den generierten Code eingebettet oder subtile, schwer erkennbare Fehler eingefügt werden (Sarkar et al. 2022). Dies kann dazu führen, dass unerfahrene Nutzer falschen Code implementieren, fehlerhafte Vorgehensweisen erlernen und sich schlechte Gewohnheiten hinsichtlich Codequalität und Sicherheit antrainieren (Becker et al., 2023), (Negri-Ribalta et al. 2024). 
Außerdem können KI-Codegeneratoren sowohl Ziel als auch Quelle von Cyberangriffen und -verteidigung sein. Ein Beispiel sind spezialisierte GenKI-Tools wie PentestGPT, die in diesem Kontext relevant sind (Gupta et al. 2023). Die Einführung solcher Technologien kann neue, bisher unbekannte Sicherheitsrisiken mit sich bringen, was die Notwendigkeit für kontinuierliche Überwachung und Aktualisierung der Sicherheitsmaßnahmen unterstreicht (Negri-Ribalta et al. 2024).
Schließlich zeigen Usability- und Designstudien zur KI-gestützten Programmierung, dass die Beurteilung der Korrektheit von generiertem Code eine Herausforderung darstellt, insbesondere bei grundlegenden Fehlern oder Ineffizienzen (Vaithilingam et al., 2022). Dennoch steigt die Verbreitung solcher Systeme, wie etwa durch die Telemetriedaten des Bing Developer Assistenten belegt wird (Quelle). Diese Daten zeigen, dass Programmierer KI-gestützte Werkzeuge auch dann nutzen, wenn sie die Lösung bereits kennen, da diese Tools die Arbeit schneller und effizienter machen (Wei et al. 2015; Zhang et al. 2016). Dies verdeutlicht die Notwendigkeit, dass KI-gestützte Werkzeuge sowohl hinsichtlich ihrer Effizienz als auch ihrer Genauigkeit kontinuierlich verbessert werden müssen.
Daher ist es entscheidend, diese Aspekte bei der Nutzung solcher Technologien sorgfältig zu berücksichtigen und entsprechende Lösungen zu entwickeln, um eine sichere und verantwortungsvolle Anwendung zu gewährleisten.
8.	KI zum Wohle der Gesellschaft
Der Einsatz von Künstlicher Intelligenz (KI) zum Wohle der Gesellschaft, bekannt als "AI for Good" (AI4G) (Kshirsagar et al. 2021), ist ein vielversprechendes Konzept, das darauf abzielt, soziale, ökologische und wirtschaftliche Herausforderungen zu adressieren. Dieser Ansatz konzentriert sich insbesondere auf wirtschaftlich unrentable Projekte, die von gemeinnützigen Organisationen, Sozialunternehmen und Regierungen unterstützt werden, in den Bereichen Nachhaltigkeit, Gesundheit, humanitäre Hilfe und soziale Gerechtigkeit liegen und bisher kaum von KI durchdrungen sind (Kshirsagar et al. 2021). Durch den Einsatz von KI in der Datenaufbereitung und -verarbeitung können diese gemeinwohlorientierten Projekte erheblich optimiert werden, wodurch auch die Ziele für nachhaltige Entwicklung (SDGs) der Vereinten Nationen unterstützt werden (Kshirsagar et al. 2021).
Trotz der potenziellen Vorteile von KI für gemeinwohlorientierte Projekte bestehen erhebliche Herausforderungen. Derzeit wird der Einsatz von KI vor allem von Unternehmen vorangetrieben, die diese Technologien wirtschaftlich vermarkten können (Kshirsagar et al. 2021). Dies führt zu hohen Markteintrittsbarrieren für gemeinwohlorientierte Organisationen, die oft nicht die Ressourcen haben, um KI-Technologien selbst zu entwickeln (Kshirsagar et al. 2021). Die Zusammenarbeit mit externen Partnern ist daher meist unerlässlich, was jedoch eine Abhängigkeit von einer begrenzten Anzahl verfügbarer Experten zur Folge hat. Diese Abhängigkeit stellt ein wesentliches Hemmnis für die Verbreitung des AI4G-Ansatzes dar.
Eine Studie von (Perry et al. 2023) hat gezeigt, dass KI-Codeassistenten informatikfremden Personen den Zugang zur Softwareentwicklung erleichtern und deren Produktivität erheblich steigern können. Daraus folgt, dass KI-Codegeneratoren auch im AI4G-Bereich helfen könnten, diese Barrieren zu überwinden, indem sie von KI-fremden Domänen-Experten innerhalb der gemeinwohlorientierten Organisationen bedient werden können. Dies würde diesen Organisationen ermöglichen, KI-Technologien effektiver und unabhängig von externen Experten zu nutzen.

Allerdings bringen derzeitige KI-Systeme aufgrund des komplizierten Prompt Engineerings hauptsächlich erfahrenen Programmierern einen nennenswerten Vorteil, obwohl insbesondere Laien erheblich von solchen Tools profitieren könnten (Sarkar et al. 2022), (Perry et al. 2023). Das Feld der maschinellen Lern- und KI-Entwicklung bleibt daher für viele Personen, die keine Vorkenntnisse in Informatik haben, weitgehend unzugänglich (Bojer und Meldgaard 2021).
Zudem bilden die zum Schutz eingeführten Ethikrichtlinien eine Barriere [24] (Gupta et al. 2023), wodurch es vorkommen kann, dass KI-Assistenten manche Antworten verweigern, selbst wenn diese aus Gründen der Softwaresicherheit gestellt wurden (Klemmer et al. 2024). Diese Barriere kann jedoch meist durch das Umformulieren der Frage umgangen werden und stellt lediglich ein Usability-Hindernis dar. Ein weiteres Hemmnis, gerade für kleinere Organisationen, sind die teils hohen Lizenzkosten solcher Systeme (Klemmer et al. 2024).
Zusammengefasst zeigt sich, dass der Einsatz von KI zum Wohle der Gesellschaft ein hohes Potenzial besitzt, jedoch auch mit erheblichen Herausforderungen verbunden ist. Diese müssen sorgfältig adressiert werden, um die Vorteile von AI4G voll ausschöpfen zu können.
9.	Verbesserungen für einen KI-Codegenerator: Ein umfassender Ansatz
Die kontinuierliche Verbesserung von KI-basierten Codegeneratoren erfordert ein durchdachtes System aus verschiedenen Mechanismen und Techniken. Im Folgenden werden verschiedene Ansätze und Ideen, basierend auf den zuvor vorgestellten Fachartikeln zu einem umfassenden Konzept zur Erhöhung der Sicherheit und Effizienz von KI-generiertem Code zusammengeführt. Das vorgeschlagene System soll dabei über umfangreiche Sicherungsmechanismen verfügen, um die Generierung von schlechtem oder gar schadhaftem (KI)-Code zu verhindern. Hierzu ist es insbesondre notwendig die bisher zum Training verwendeten Daten umfangreich zu validieren und den Trainingsprozess auf eine sichere und effiziente KI-Codegenerierung auszurichten. 
Dazu schlagen wird die Erstellung einer komplexes KI-Plattform vor, welche das LLM/GPT-Modell dazu in die Lage versetzt den für das Training vorgesehenen Code selbständig zu prüfen, zu labeln und zu validieren. Hierfür wird ein GPT-Modell zuerst mit Datensätzen Fine-getuned, die es befähigen unsicheren von sicherem Code zu unterscheiden und respektive sicheren Code zu generieren. 
Hierfür sollen die in Kap \todo{Datensätze zum Verifizieren der Codekorrektheit und Codesicherheit Teil 1} beschriebenen Datensätze genutzt werden. Dabei soll das Modell, basierend auf den vorhandenen Aufgabenbeschreibungen Lösungen generieren und diese mit den in den Datensätzen bereitgestellten Lösungen vergleichen. Dadurch soll eine Optimierung hin zum richtigen Ergebnis vorgenommen werden. Dazu sollen die ausgegebenen Lösungen basierend auf den mitgelieferten Lösungen aber auch anhand externen Sicherheitstools (z.B. CodeQL, Bandit, Semgrep und das Python-Taint-Modul (PyT) (Cotroneo et al. 2024)) auf Sicherheitslücken überprüft und bewertet werden. Die während dieses Prozesses als gute oder schlecht gekennzeichnete Lösungen sollen im Anschluss als neues Wissen in die Trainingsdaten integriert und dem Lernprozess zugeführt werden. Dies soll die Leistungsfähigkeit des Systems verbessern und die Ausgabe von korrektem und sicherem Code optimieren. Zusätzlich soll das System mit Wissen über Schwachstellen wie gängige CVE-, CWE, NIST und NVD-Schwachstellen, mit Erkenntnissen aus OWASP und Mitre sowie mit externem Wissen aus Publikationen und Büchern optimiert werden.
Außerdem sollen die in Kap \todo{Datensätze zum Verifizieren der Codekorrektheit und Codesicherheit Teil 2} beschriebenen Datensätze, die sowohl über textuelle Beschreibungen als auch über Codelösungen verfügen, genutzt werden, um das Interaktionsverhalten mit den Nutzenden (Prompt Engineering) zu simulieren. Dadurch soll die Ausgabe von sichern Code unabhängig von der Qualität der Prompts optimiert werden. Außerdem enthalten diese Datensätze teilweise Aufgaben zur Generierung von sicherheitskritischem Code. Dies wird genutzt, um die im vorherigen Schritt vorgenommene Optimierung zu Validieren. Das in diesem Schritt gewonnen Wissen wird ebenfalls in die Trainingsdaten zurücküberführt. 
Darüber hinaus soll, zusätzlich zu den bereits vorgestellten Datensätzen, das Projekt SVEN für die Modellfeinabstimmung und die Ausgabenoptimierung verwendet werden. SVENsec liefert hierbei sicheren Code, wohingegen SVENvul diesen mit Schwachstellen versieht (He und Vechev, 2023). Durch den Einsatz dieser beiden Tools kann explizit das Generieren von sicherem und unsicherem Code erzwungen werden. Dadurch können weitere potentiell sichere und unsichere Ausgaben generiert werden, welche im Anschluss jedoch noch geprüft werden müssen. Diese Daten können dann ebenso gelabelt und dem Trainingsprozess zugeführt werden.
Darauf aufbauend müssen die bisher verwendeten, unsicheren Trainingsdaten aus öffentlich zugänglich Quellen mit diesem System evaluiert, repariert und entsprechend gelabelt werden. Anschließend werden sowohl die guten und reparierten Daten als Positivbeispiele als auch die negativen durch statarische Analyseverfahren validierten Daten in einem iterativen Prozess (Feedbackschleife) in das Training des Modells zurückgeführt.
Des Weiteren sollen auch die von (Res et al. 2024) und (Perry et al. 2023) vorgeschlagenen Prompt-Optimierungen integriert werden. Dabei sollen diese Prompt-Optimierungen auf die Erzeugung von sicherem, mit Fehlerhandling ausgestattetem, und effizientem Code sowie die Erzeugung von entsprechenden Testfällen fordern. Außerdem sollen sie z.B. das Setzen generischer Werte aus Manuals und das Implementieren bekannter Sicherheitslücken und Schwachstellen (CVE-, CWE, NIST und NVD) verbieten (z.B. „vermeide alle dir bekannten CVE-, CWE, NIST und NVD-Schwachstellen und gebe nur sicheren durch Testfälle validierbaren Code sowie diese Testfälle aus.“). Zusätzlich soll das System dazu aufgefordert werden in OWASP und Mitre beschriebenen Angriffsvektoren zu vermeiden (z.B. „prüfe den Code auf alle bekannten Schwachstellen aus Mitre und gebe nur sicheren durch Testfälle validierbaren Code sowie diese Testfälle aus.“) (Improta 2023). 
Da sich die Prompt-Optimierungen bisher jedoch nicht mit der Generierung von KI durch KI beschäftigt haben, müssen die Optimierungen auch dahingehend angepasst werden (z.B. „Generierung ein sicheres und leistungsstarkes KI-Modell mit hoher Güte“).
Außerdem soll das Modell über die Fähigkeit verfügen fehlendes, aber notwendiges Wissen, das vom Nutzer nicht bereitgestellt wurde zu erfragen. Dabei muss das System dazu in der Lage sein, von den Nutzenden verursachte Definitionslücken, die zur Gewährleistung der Effizienz und Sicherheit der Ausgabe notwendig sind zu erkennen und die notwendigen Daten zu erfragen. Dieses System kann ebenfalls durch einen Hackathon evaluiert werden. Durch dieses Interaktionsdesign wird der KI-Assistent in die Lage versetzt die hier gefundenen Auswirkungen des Prompt Engineering auf die Ergebnisqualität weiter zu reduzieren, indem das System Fehler in Prompts durch Rückfragen minimiert. Somit werden auch unerfahrenen Nutzenden befähigt, sicheren und effektiven Code zu generieren. Des Weiteren ermöglicht dieses System eine effektive Umsetzung des AI4G-Ansatzes, indem ein Generator für sicheren KI-Code entwickelt wird, welcher durch einen diesen Organisationen zur Verfügung stehenden Domänen-Experten bedient werden kann (Kshirsagar et al. 2021).
Da das Modell kontinuierlich weiter verbesset werden soll, müssen auch die von den Nutzenden gestellten Prompts und der daraus generierte Code mit Hilfe dieses Ansatzes in das kontinuierliche Training integriert werden. Dazu müssen alle Codeausgaben des Assistenten mithilfe der bereits vorgestellten externen Sicherheitstools überprüft werden. Als positiv erkannter Code wird dem Nutzenden angezeigt und als positiv gekennzeichnetes Beispiel in die Trainingsdaten überführt. Als negativ erkannte Daten werden den Trainingsdaten als Negativbeispiele hinzugefügt und nicht ausgegeben. Stattdessen wird der Generierungsprozess so lange wiederholt, bis sicherer und fehlerfreier Code generiert wurde. Die so gewonnenen Erkenntnisse werden dem Training ebenfalls iterativ zugeführt. 
Um jedoch nicht nur das Erzeugen von herkömmlichem Code, sondern auch das Erzeugen von KI durch KI effektiver gestalten zu können sind weitere Überlegungen notwendig. So muss ein zusätzliches Fine-Tuning zur automatischen Generierung von sicherem und effizientem KI-Code durchgeführt werden. Während dieses Prozesses muss dem System Fachwissen zur Generierung von effizienter KI zugeführt werden. Dazu werden Trainingsdaten durch Crawlen von Plattformen wie Kaggle (siehe Kap …) generiert werden, da zu den dort als gut markierten KI-Modellen oft auch der entsprechende Code vorliegt (Bojer und Meldgaard 2021). Zusätzlich sollten auch schlecht abschneidende KI-Modelle in den Korpus aufgenommen und dem Training als schlecht gekennzeichnete Beispiele zugeführt werden. Dabei müssen alle von Plattformen wie Kaggle gewonnenen Daten auf Sicherheitslücken überprüft werde, um die Leistungsfähigkeit des Systems nicht wieder zu verschlechtern (Basieren auf (Improta 2023)). Des Weiteren kann auch hier wieder auf externes Wissen wie Fachartikel und Bücher zurückgegriffen werden.
Die Wirksamkeit dieses Ansatzes soll, wie von (Taeb et al. 2024) vorgeschlagen, durch Hackathons mit Experten und Studierenden durchgeführt werden. Dies ermöglicht Einblicke in die verschiedenen Ansätze der Nutzergruppen beim Prompt Engineering und bewertet die Effektivität des Ansatzes. Außerdem kann dabei überprüft werden, ob das Modell, unabhängig vom Kenntnisstand der Nutzer, konsistent sicheren und qualitativ hochwertigen Code erzeugt. Außerdem solle das in diesem Schritt gewonnene Wissen ebenfalls iterativ in den Trainingskorpus überführt.

Zusätzlich zur Optimierung des eigentlichen Modells muss jedoch auch das komplette Ökosystem, in welchem sich dieses Modell befindet abgesichert werden. Dazu müssen die in (Kap .. und .. ..) vorgestellten  Sicherungsmechanismen in die KI-Plattform integriert werden. Hierbei müssen insbesondere die KI-Trainingspipeline und das eigentliche Modell geschützt werden. Außerdem müssen das Frontend- und das Backend der KI-Pipeline sowie die Hardwareinfrastruktur und alle hardwarenahen Systeme ausreichend geschützt werden. Eine umfassende und sichere KI-Pipeline ist somit ebenfalls von großer Bedeutung.
Durch die Implementierung dieser vielfältigen Ansätze und Techniken kann ein sicherer und effizienter KI-Codegenerator entwickelt werden. Die Kombination von Sicherungsmechanismen, gezielten Datensätzen, praktischen Anwendungen und umfassenden Evaluationsmethoden schafft eine robuste Basis für die kontinuierliche Verbesserung und Anpassung des Systems.
10.	Fazit
Mit der fortschreitenden Entwicklung von KI-Codegeneratoren zur Erstellung sowohl von klassischem Code als auch von KI-Code ergeben sich bedeutende Chancen und Risiken für die Software- und KI-Entwicklung. Während diese Technologien das Potenzial haben, die Effizienz und Produktivität erheblich zu steigern, müssen die damit verbundenen Herausforderungen sorgfältig adressiert werden. Als zentrale Herausforderungen gelten hierbei die Sicherheit und Zuverlässigkeit sowie die Qualität und Vertrauenswürdigkeit des generierten Codes. Diese können durch verschiedene in diesem Paper beschriebenen und im Anschluss zu einer komplexen KI-Plattform vereinigten Ansätze erreicht werden.
Dabei verfügt diese KI-Plattform über ein ausgeklügeltes System zur Nutzung und Validierung von bestehende sowie zur automatischen Erzeugung von weiteren Trainingsdaten, welche im Anschluss in einem Iterativen und kontinuierlich stattfindenden Prozess für das Modelltraining und die Modelloptimierung genutzt werden.
Außerdem wird ein menschenzentrierter, leicht zugänglicher und benutzerfreundlicher KI-Ansatz eingeführt, der auch von Laien verwendet werden kann. Dieser Ansatz soll allen Nutzergruppen, unabhängig von ihrem Erfahrungsstand, bei der Erstellung von effektivem und sicherem Code sowie leistungsstarken und sicheren KI-Modellen unterstützen. Dabei werden diese auch durch das in diese KI-Pipeline integrierten System zur Optimierung der Prompts sowie durch ein Rückfragesystem zur Vermeidung von Definitionslücken, die während des Prompt Engineerings auftreten können, unterstützt.
Außerdem werden die Risiken einer solchen KI-Plattform sowie die potenziellen Gefahren, die von ihr ausgehen können, aufgezeigt. Zur Bewältigung dieser Risiken wird ein umfassendes Sicherheitssystem skizziert, das sowohl Schutz vor klassischen Cyberbedrohungen als auch Abwehrmechanismen gegen Angriffe auf KI-Systeme wie Prompt-Injection und Jailbreak-Angriffe bietet. Es muss zudem sichergestellt werden, dass das Tool nicht für böswillige Zwecke missbraucht werden kann. Das zugrundeliegende Paper liefert hierfür einen ersten Ansatz.
Ebenso wird gezeigt, wie dieser Ansatz KI für gemeinwohlorientierte Projekte zugänglicher machen und somit den AI4G-Ansatz (AI for Goos) unterstützen kann. Diese KI-Plattform soll zu einer allgemein zugänglichen und damit gerechten Verbreitung dieser Technologien beitragen, wodurch das Vertrauen in KI-Codegeneratoren gestärkt wird.
Abschließend lässt sich festhalten, dass die Integration von KI-Systemen in der Softwareentwicklung weiter zunehmen wird, wodurch sowohl Experten als auch Laien ohne Vorwissen zunehmend in die Lage versetzt werden, eigenen Code zu generieren. Mit der kontinuierlichen Verbesserung dieser Technologien werden diese Systeme zukünftig auch für die Entwicklung anspruchsvoller und sicherheitskritischer Software eingesetzt. Daher ist es entscheidend, die damit verbundenen Risiken frühzeitig durch gezielte Maßnahmen zu minimieren und gleichzeitig die Vorteile der KI-Technologie umfassend zu nutzen, um das volle Potenzial von KI in der Softwareentwicklung gefahrlos auszuschöpfen und ihre sichere Anwendung zu gewährleisten.


Literaturverzeichnis
Berabi, Berkay; Gronskiy, Alexey; Raychev, Veselin; Sivanrupan, Gishor; Chibotaru, Victor; Vechev, Martin (2024): DeepCode AI Fix: Fixing Security Vulnerabilities with Large Language Models. Online verfügbar unter http://arxiv.org/pdf/2402.13291.
Bojer, Casper Solheim; Meldgaard, Jens Peder (2021): Kaggle forecasting competitions: An overlooked learning opportunity. In: International Journal of Forecasting 37 (2), S. 587–603. DOI: 10.1016/j.ijforecast.2020.07.007.
Borger, Jessica G.; Ng, Ashley P.; Anderton, Holly; Ashdown, George W.; Auld, Megan; Blewitt, Marnie E. et al. (2023): Artificial intelligence takes center stage: exploring the capabilities and implications of ChatGPT and other AI-assisted technologies in scientific research and education. In: Immunology and Cell Biology 101 (10), S. 923–935. DOI: 10.1111/imcb.12689.
Clune, Jeff (2019): AI-GAs: AI-generating algorithms, an alternate paradigm for producing general artificial intelligence. Online verfügbar unter http://arxiv.org/pdf/1905.10985.
Cotroneo, Domenico; Luca, Roberta de; Liguori, Pietro (2024): DeVAIC: A Tool for Security Assessment of AI-generated Code. Online verfügbar unter http://arxiv.org/pdf/2404.07548.
Desmond, Michael; Brachman, Michelle; Duesterwald, Evelyn; Dugan, Casey; Nath Joshi, Narendra; Pan, Qian; Spina, Carolina (2022): AI Assisted Data Labeling with Interactive Auto Label. In: AAAI 36 (11), S. 13161–13163. DOI: 10.1609/aaai.v36i11.21714.
Feltus, Christophe; Ma, Qin; Proper, Henderik A.; Kelsen, Pierre (2021): Towards AI Assisted Domain Modeling. In: Iris Reinhartz-Berger und Shazia Sadiq (Hg.): Advances in Conceptual Modeling. ER 2021 Workshops CoMoNoS, EmpER, CMLS St. John's, NL, Canada, October 18–21, 2021, Proceedings, Bd. 13012. International Conference on Conceptual Modeling. Cham: Springer International Publishing (Programming and Software Engineering, 13012), S. 75–89. Online verfügbar unter https://link.springer.com/chapter/10.1007/978-3-030-88358-4_7.
Gottlander, Johan; Khademi, Theodor (2023): The Effects of AI Assisted Programming in Software Engineering. Online verfügbar unter https://odr.chalmers.se/items/acf7c5fa-50dc-4c11-842b-d1414e7bf689.
Gupta, Maanak; Akiri, Charankumar; Aryal, Kshitiz; Parker, Eli; Praharaj, Lopamudra (2023): From ChatGPT to ThreatGPT: Impact of Generative AI in Cybersecurity and Privacy. In: IEEE Access 11, S. 80218–80245. DOI: 10.1109/ACCESS.2023.3300381.
Hossain, Ismail; Istiak Chowdhury, N. M.; Hasan, Ragib (2023): How Secure is AI-based Coding?: A Security Analysis Using STRIDE and Data Flow Diagrams. In: 2023 IEEE Virtual Conference on Communications (VCC). 2023 IEEE Virtual Conference on Communications (VCC). NY, USA, 11/28/2023 - 11/30/2023. Piscataway, New Jersey: IEEE, S. 56–61.
Improta, Cristina (2023): Poisoning Programs by Un-Repairing Code: Security Concerns of AI-generated Code. In: 2023 IEEE 34th International Symposium on Software Reliability Engineering Workshop. ISSRE 2023 : 9-12 October 2023, Florence, Italy : proceedings. 2023 IEEE 34th International Symposium on Software Reliability Engineering Workshops (ISSREW). Florence, Italy, 10/9/2023 - 10/12/2023. Institute of Electrical and Electronics Engineers. Piscataway, NJ: IEEE, S. 128–131.
Klemmer, Jan H.; Horstmann, Stefan Albert; Patnaik, Nikhil; Ludden, Cordelia; Burton, Cordell, JR; Powers, Carson et al. (2024): Using AI Assistants in Software Development: A Qualitative Study on Security Practices and Concerns. Online verfügbar unter http://arxiv.org/pdf/2405.06371.
Kshirsagar, Meghana; Robinson, Caleb; Yang, Siyu; Gholami, Shahrzad; Klyuzhin, Ivan; Mukherjee, Sumit et al. (2021): Becoming Good at AI for Good. In: Marion Fourcade (Hg.): Proceedings of the 2021 AAAI/ACM Conference on AI, Ethics, and Society. AIES '21: AAAI/ACM Conference on AI, Ethics, and Society. Virtual Event USA, 19 05 2021 21 05 2021. ACM Special Interest Group on Artificial Intelligence. New York,NY,United States: Association for Computing Machinery (ACM Digital Library), S. 664–673.
Li, Xiang Lisa; Liang, Percy (2021): Prefix-Tuning: Optimizing Continuous Prompts for Generation. In: Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers), S. 4582–4597. DOI: 10.18653/v1/2021.acl-long.353.
Minn, Sein (2022): AI-assisted knowledge assessment techniques for adaptive learning environments. In: Computers and Education: Artificial Intelligence 3, S. 100050. DOI: 10.1016/j.caeai.2022.100050.
Mozannar, Hussein; Bansal, Gagan; Fourney, Adam; Horvitz, Eric (2024): Reading Between the Lines: Modeling User Behavior and Costs in AI-Assisted Programming. In: Florian Floyd Mueller, Penny Kyburz, Julie R. Williamson, Corina Sas, Max L. Wilson, Phoebe Toups Dugas und Irina Shklovski (Hg.): Proceedings of the CHI Conference on Human Factors in Computing Systems. Unter Mitarbeit von Florian Floyd Mueller, Penny Kyburz, Julie R. Williamson, Corina Sas, Max L. Wilson, Phoebe Toups Dugas und Irina Shklovski. CHI '24: CHI Conference on Human Factors in Computing Systems. Honolulu HI USA, 11 05 2024 16 05 2024. Erscheinungsort nicht ermittelbar: Association for Computing Machinery (ACM Digital Library), S. 1–16.
Negri-Ribalta, Claudia; Geraud-Stewart, Rémi; Sergeeva, Anastasia; Lenzini, Gabriele (2024): A systematic literature review on the impact of AI models on the security of code generation. In: Front. Big Data 7, S. 1386720. DOI: 10.3389/fdata.2024.1386720.
Pakalapati, Naveen; Venkatasubbu, Selvakumar; Sistla, Sai Mani Krishna (2023): The Convergence of AI/ML and DevSecOps: Revolutionizing Software Development. In: JKLST 2 (2), S. 189–212. DOI: 10.60087/jklst.vol2.n2.p212.
Perry, Neil; Srivastava, Megha; Kumar, Deepak; Boneh, Dan (2023): Do Users Write More Insecure Code with AI Assistants? In: Weizhi Meng, Christian D. Jensen, Cas Cremers und Engin Kirda (Hg.): Proceedings of the 2023 ACM SIGSAC Conference on Computer and Communications Security. CCS '23: ACM SIGSAC Conference on Computer and Communications Security. Copenhagen Denmark, 26 11 2023 30 11 2023. Erscheinungsort nicht ermittelbar: Association for Computing Machinery (ACM Digital Library), S. 2785–2799.
Pinhanez, Claudio (2019): Machine Teaching by Domain Experts: Towards More Humane,Inclusive, and Intelligent Machine Learning Systems.
Rajamani, Sriram (2022): AI Assisted Programming. In: Venkatesh Choppella (Hg.): Proceedings of the 15th Annual ACM India Compute Conference. Unter Mitarbeit von Amey Karkare, Chitra Babu und Sridhar Chimalakonda. COMPUTE 2022: COMPUTE 2022. Jaipur India, 09 11 2022 11 11 2022. New York,NY,United States: Association for Computing Machinery (ACM Digital Library), S. 5.
Ray, Partha Pratim (2023): ChatGPT: A comprehensive review on background, applications, key challenges, bias, ethics, limitations and future scope. In: Internet of Things and Cyber-Physical Systems 3, S. 121–154. DOI: 10.1016/j .iotcps.2023.04.003.
Res, Jakub; Homoliak, Ivan; Perešíni, Martin; Smrčka, Aleš; Malinka, Kamil; Hanacek, Petr (2024): Enhancing Security of AI-Based Code Synthesis with GitHub Copilot via Cheap and Efficient Prompt-Engineering. Online verfügbar unter http://arxiv.org/pdf/2403.12671.
Sarkar, Advait; Gordon, Andrew D.; Negreanu, Carina; Poelitz, Christian; Ragavan, Sruti Srinivasa; Zorn, Ben (2022): What is it like to program with artificial intelligence? Online verfügbar unter https://www.ppig.org/papers/2022-ppig-33rd-sarkar/.
Sarkar, Rajdeep (2023): Integrating Structured and Unstructured Knowledge Sources for Domain-Specific Chatbots. Online verfügbar unter https://aran.library.nuigalway.ie/bitstream/handle/10379/17963/rajdeep_thesis_final.pdf?sequence=1.
Sarker, Iqbal H. (2022): AI-Based Modeling: Techniques, Applications and Research Issues Towards Automation, Intelligent and Smart Systems. In: SN COMPUT. SCI. 3 (2), S. 158. DOI: 10.1007/s42979-022-01043-x .
Sundberg, Leif; Holmström, Jonny (2023): Democratizing artificial intelligence: How no-code AI can leverage machine learning operations. In: Business Horizons 66 (6), S. 777–788. DOI: 10.1016/j.bushor.2023.04.003.
Taeb, Maryam; Chi, Hongmei; Bernadin, Shonda (2024): Assessing the Effectiveness and Security Implications of AI Code Generators. In: CISSE 11 (1), S. 6. DOI: 10.53735/cisse.v11i1.180.
Wong, Man-Fai; Guo, Shangxin; Hang, Ching-Nam; Ho, Siu-Wai; Tan, Chee-Wei (2023): Natural Language Generation and Understanding of Big Code for AI-Assisted Programming: A Review. In: Entropy 25 (6), S. 888. DOI: 10.3390/e25060888 .
Yang, Qian; Suh, Jina; Chen, Nan-Chen; Ramos, Gonzalo (2018): Grounding Interactive Machine Learning Tool Design in How Non-Experts Actually Build Models. In: Proceedings of the 2018 Designing Interactive Systems Conference. New York, NY, USA. New York, NY, USA: ACM, S. 573–584.
Ylitalo, Aleksi: AI assisted public cloud management. Online verfügbar unter https://www.theseus.fi/handle/10024/850830.
Zamfirescu-Pereira, J. D.; Wong, Richmond Y.; Hartmann, Bjoern; Yang, Qian (2023): Why Johnny Can’t Prompt: How Non-AI Experts Try (and Fail) to Design LLM Prompts. In: Proceedings of the 2023 CHI Conference on Human Factors in Computing Systems. New York, NY, USA. New York, NY, USA: ACM, S. 1–21.



==> SOTA_Draft.tex <==
%\citeauthor{}~\cite{}
KI Techniken lassen sich auch zum KI gestützten Programmieren \cite{Rajamani.2022, Mozannar.2024} (Rajamani 2022) (Mozannar et al. 2024) (Wong et al. 2023) aber auch zur KI Entwicklung (Sundberg und Holmström 2023) (Sarker 2022) (Yang et al. 2018) einsetzen.
So erläutern (Sarker 2022) Prinzipien verschiedener KI-Techniken die sich einsetzen lassen um automatisiert (KI-) Modelle für intelligente und smarte Systeme zu entwickeln. Durch den Einsatz solcher KI-Techniken lassen Geschäftsprozesse beschleunigen wodurch die Produktivität und Rentabilität des Betriebs gesteigert werden kann (Sarker 2022). Außerdem lässt sich dadurch auch die Effizienz und Qualität von Projekten steigern (Wong et al. 2023). Des Weiteren lassen sich dadurch auch Wissen und Erfahrungen aus bereits vorhanden Daten ableiten (Wong et al. 2023) (Yang et al. 2018). Allerdings weißen die Autoren darauf hin, dass die Entwicklung von die Geschäftsprozesse verbessernden KI-Modellen aufgrund der hohen Dynamik und der Datenvariation ein anspruchsvolles Feld ist (Sarker 2022) und zur Lösung derzeit sowohl Domänen-Experten als auch AI/ML Experten benötigt werden (Pinhanez 2019) (Wong et al. 2023) (Yang et al. 2018). Da die in den Betrieben vorhandenen Domänen-Experten meinst nicht über KI-Wissen verfügen, KI Experten aber oft nicht verfügbar sind, müssen die Zugangsbeschränkungen für die Entwicklung von KI-Modellen mithilfe von geeigneten Konzepten wie interaktiven Assistenzsystemen abgebaut und der Zugang für Nicht Experten sichergestellt werden (Pinhanez 2019). Um zu verstehen welche Hindernisse für Laien beim Erstellen von KI-Modelle entstehen und wie Laien befähigt werden können selbst am KI boom zu partizipieren analysieren (Yang et al. 2018) diesen Prozess. Dabei betrachten Sie wie diese Arbeitsschritte auch für Personen ohne AI- und ML-Wissen zugänglich gemacht werden kann. Ein großes Problem stellt beispielsweise die Validierung von Modellen dar, da Laien oft nur die Genauigkeit des Systems beurteilen können und dadurch auch problematische oder gar falsche Modelle zum Einsatz kommen können. Zur Analyse dieser Probleme teilen (Sarker 2022) die zu entwickelnde Modelle in fünf Kategorien ein: „Analytische KI“, die Erkenntnisse aus Daten gewinnt; „Funktionale KI“, die Maßnahmen ergreift; „Interaktive KI“, die die Automatisierung der Kommunikation ermöglicht; „Textuelle KI“, die Textanalyse oder Verarbeitung natürlicher Sprache umfasst; und „Visuelle KI“, die Computer Vision oder Augmented Reality umfasst. 

Um KI auch für Nicht-Experten oder für Experten anderer Domänen nutzbar zu machen und um dem steigenden Bedarf an wissensintensiven Prozessen Rechnung zu tragen muss die Technologie zum Erstellen solcher KI-Modelle eine symbiotische Beziehung mit den Erstellenden eingehen können (Feltus et al. 2021) und sich mit einem nutzerzentrischen und einfachen Ansatz erstellen lassen. Dazu ist es jedoch erforderlich, dass das dahinterliegende Wissensmodel sowohl durch eine Maschine (KI) als auch von einem Menschen verstanden und genutzt werden kann (Feltus et al. 2021). Daher gewinnt die Forschung an Prozessen und Werkzeugen zur einfach, flexibel, robust und durch Laien durchführbaren Erstellung von ML-Modellen immer mehr an Bedeutung. Dies fördert Akzeptanz von KI und ermöglicht gleichzeitig die Integration von KI in allen Bereichen der Gesellschaft (Feltus et al. 2021). Dies würde insbesondere der Erstellung von sicherem und Leistungsfähigen KI-Code zugutekommen. (Sarkar 2023) weißen jedoch darauf hin, dass die Integration von strukturierten (z.B. Wissensgraphen) und unstrukturierten Wissensquellen (z.B. Wikipedia) eine erhebliche Herausforderung darstellt. (Feltus et al. 2021) und [43] schlagen daher vor, unterstützender Technologien einzusetzen, um Nicht-Experten bei der Modellerstellung aber auch bei der Wissensanalyse zu unterstützen. Ein bisher unerforschter Bereich stellt dabei noch die kollaborative Entwicklung mehrerer Nicht-Experten an einem Modell dar (Feltus et al. 2021). In diesem Kontext gewinnen gerade auf Large Language Models (LLM) basierende Programmierassistenzsysteme wie Chat GPT zunehmend an Bedeutung. Diese Sprachmodelle können nicht nur Fließtext und mehrstufige Anweisungen interpretieren (Zamfirescu-Pereira et al. 2023), sondern auch Antworten generieren, die von menschlichen Antworten kaum zu unterscheiden sind (Zamfirescu-Pereira et al. 2023) (Borger et al. 2023). Der rasante Entwicklung von LLMs kann insbesondere am Beispiel ChatGPT beobachtet werden, welches signifikante Fortschritte im Bereich Kontextverständnis, Sprachgenerierung, Anpassungsfähigkeit und Mehrsprachigkeit gemacht hat (Ray 2023). Diese Entwicklungen ermöglichen eine einfache Interaktion, indem sie natürliche Sprache (sog. „Prompting“) zur Steuerung der LLM-Ausgaben nutzen und die „Mensch-KI-Interaktion“ (Ray 2023) verbessern. Aufgrund dieser Entwicklungen hat sich diese Technik als eine wichtige Designmethode erwiesen, die potenziell auch für Nicht-KI-Experten zugänglich ist und die Nutzung von KI-Systemen intuitiver gestaltet (Zamfirescu-Pereira et al. 2023).
Dadurch entsteht ein Potenzial, das in vielen Bereichen gewinnbringend genutzt werden kann (Borger et al. 2023). So entstehen vielfältige Einsatzmöglichkeiten, in den Bereichen Medizin, Gesundheitswesen, Wirtschaft, Finanzen, Recht, juristische Dienstleistungen, kreatives Schreiben, Inhaltserstellung, Bildungswesen, Medien, Unterhaltung, Verkauf, Marketing, Öffentlichkeitsarbeit, Bankwesen, wissenschaftliche Forschung bis hin zur Programmierung und dem Code-Debugging (Ray 2023). Insbesondere in der wissenschaftlichen Forschung (Ray 2023) und der Softwareentwicklung (Ray 2023) (Wong et al. 2023) bieten diese Systeme ein bisher kaum genutztes Potential. So entstehen neue Möglichkeiten bei der Datenverarbeitung und -analyse sowie durch eine kooperative Nutzung als nicht-menschliche Sparringpartner z.B. bei der Hypothesengenerierung (Ray 2023). Gerade im Bereich der Softwareentwicklung übertreffen KI-gestützte Funktionen zur Codegenerierung, Codevervollständigung, Codeübersetzung, Codeoptimierung, Codezusammenfassung, Codeüberprüfung und Debugging zur Fehlererkennung, Codedokumentation und Klonerkennung (Ray 2023) (Wong et al. 2023) (Mozannar et al. 2024) die Leistungsfähigkeit bestehender Systeme um ein Vielfaches. So können diese Systeme Funktionen und Klassen in einer breiten Palette von Programmiersprachen nicht nur ergänzen, sondern basierend auf den vorgegebenen Prompts auch selbst schreiben (Wong et al. 2023) (Mozannar et al. 2024). Dieses Potential beschränkt sich aber nicht nur auf die Entwicklung gewöhnlicher Software sondern kann auch genutzt werden um die Entwicklung von KI-Systemen zu revolutionieren (Wong et al. 2023).
Diese Leistungsfähigkeit kommt insbesondere durch den Einsatz moderner Large Language Models (LLM), welche mit Milliarden von Codezeilen trainiert wurden (Mozannar et al. 2024). (Rajamani 2022) präsentieren zudem einen Vorschlag für eine KI gestützte Programmierumgebung welche sowohl auf ML-Modellen als auch auf logischen Regeln beruht und sich kontinuierlich mit ihrer Nutzung weiterentwickeln kann. (Mozannar et al. 2024) führen eine Kosten-Nutzen-Analyse des Einsatzes von KI-gestützten Programmierassistenzsystemen (LLMs) für Codeempfehlungen durch und konzentrieren sich dabei auf Expertenanwender. Sie kommen zu dem Schluss, dass diese Systeme die Arbeitsbelastung reduzieren und die Produktivität steigern können. Allerdings betonen (Mozannar et al. 2024), dass dieser Nutzen nur dann erreicht wird, wenn die Anwender über ausreichende Expertise im Bereich des Prompt Engineerings verfügen um bei diesem für Laien herausfordernden Prozess ausreichend effektive Eingabeaufforderungen generieren (Zamfirescu-Pereira et al. 2023). Zudem müssen die von der KI generierten Codes sorgfältig validiert werden, da sie fehlerhaft sein und Sicherheitslücken enthalten können (Mozannar et al. 2024).
(Sundberg und Holmström 2023) zeigen auf, dass KI aufgrund ihres enormen Potenzials im Zuge der digitalen Transformation zunehmend in die Wirtschaft integriert, wird aber auch für Einzelpersonen zunehmend an Interesse gewinnt. Sie stellen jedoch auch fest, dass der verantwortungsvolle Einsatz von KI für kleinere Unternehmen, die häufig nicht über die notwendigen technologischen Kompetenzen verfügen einen Wettbewerbsnachteil darstellen. Daher beschäftigen sich (Sundberg und Holmström 2023) mit der Demokratisierung von KI durch den Einsatz von KI-basierten No-Code Programmierassistenzsysteme, welche diese Technologie auch für Einzelpersonen und kleinere Organisationen zugänglich und erschwinglich machen kann. Dabei arbeiten Sie insbesondere heraus, welchen Mehrwert Unternehmen durch den Einsatz von KI und ML erlangen (z.B. Big Data Analysen) können und welche Schwierigkeiten sich dabei insbesondere für kleinere Unternehmen (z.B. MLOps) auftun. Als mögliche Lösung definieren (Sundberg und Holmström 2023) No-Code-KI-Plattformen die durch eine Kombination aus KI-Assistenten, MLOps und nutzerfreundlichen grafischen Oberflächen auch unerfahrene Nutzer ohne jegliche Codierungskentnisse befähigen, KI-Modelle zu entwickeln, bereitzustellen, zu betreiben und zu trainieren, ohne die dahinterstehenden komplexen Algorithmen im Detail verstehen zu müssen. (Ylitalo) weißen in diesem Kontext jedoch darauf hin, das AI Tools auch an die Zeilgruppe angepasst werden müssen. Dies zeigen Sie am Beispiel der Studie „“Github Copilot AI Pair programmer: asset or liability“ [Quelle?] welche nahelegt, das der GitHub Copilot zwar ein gutes Tool für Senior Entwickler darstellt, Junior Entwickler aber nicht zugutekommt. Des Weiteren sollten die von Nicht-Experten entwickelten Modelle soweit aufbereitet werden, dass die Entwickelnden deren Implikationen verstehen und die Bedeutung ihres Einsatzes bewerten können (Feltus et al. 2021). Dies soll insbesondere auch ein ausgewogenes Zusammenspiel von KI-gestützter Innovation und menschlichem Fachwissen fördern (Ray 2023). (Pinhanez 2019) stellen mit dem Open Learning AI-System (MOLA) einen Communitybasierten Ansatz zur AI Entwicklung vor. Im Gegensatz zu einer geschlossenen KI-Plattform, kann hierbei ein kollaboratives KI-Ökosystem entstehen. Der Vorteil einer solchen offenen, integrativen für Domänen- und KI-Experten zugänglichen KI-Plattformen ergibt sich einerseits durch das heben von Synergieeffekten innerhalb dieser Community und andererseits durch das Vorhandensein von Expertenwissen unterschiedlicher Disziplinen (Pinhanez 2019). (Pinhanez 2019) untersuchen in Ihrer Studie unter anderem die kollaborative Entwicklung eines KI-Assistenten für Diabetespatienten. Hierbei zeigten sich auch die Vorteile solch eines Systems. So bemerkte die Community, dass der KI-Assistenten von einigen etischen Gruppen aufgrund Kultureller Besonderheiten nicht gut angenommen wurde. Dies konnte im Anschluss kooperativ gelöst werden. Da die KI Modelle vieler Unternehmen als Geschäftsgeheimnisse anzusehen sind können diese zwar meinst nicht öffentlich gemacht werden. Die Entwicklung der Assistenzsysteme zur Entwicklung von KI könnten aber durchaus innerhalb solch einer Community entwickelt werden. Durch das Projekt AI4EU steht bereits eine containerbasierte Architektur zur kollaborativen Entwicklung von KI Modellen durch Experten und Nichtexperten zur Verfügung (mehr dazu unter). Zur Erstellung von nutzerfreundlichen grafischen Oberflächen stellen (Yang et al. 2018) das Tool „Test-Driven Machine Teaching“ vor, welches Designer dabei unterstützt GUIs zu entwickeln die sich dem Interaktionsfluss durch interactive machine learning (iML) und dadurch den Gegebenheiten von Laien anpasst und diese gleichzeitig auf technische Fallstricke die beim Erstellen von ML-Modellen auftreten können hinweist. Durch den Einsatz solcher Plattformen kann eine Brücke zwischen verschiedenen Expertenkreisen (z.B. Fachexperten-, Geschäfts- und Technologieexperten) geschlagen werden, wodurch bestehende technische, sprachliche und interessensbedingte Hindernisse überwunden und Lösungen für komplexe Probleme schneller und effizienter erreicht werden können (Sundberg und Holmström 2023). Durch interaktive und benutzerfreundliche grafische Oberflächen sowie an die Bedürfnisse und Fähigkeiten der Nutzer im Bereich ML/AI und Programmierung angepasste Prozesse können robustere KI-Modelle von Laien entwickelt werden (Yang et al. 2018). Die in die GUI integrierbaren geführten Prozesse unterstützen dabei die Einhaltung grundlegender Regeln und Sicherheitsaspekte (Yang et al. 2018) und sorgen somit auch für einen sichereren und ethischeren umgang mit KI. Außerdem heben (Sundberg und Holmström 2023) cloudbasierte KI-Plattformen sog. „KI as a Service“-Systeme als möglichen neuen Wirtschaftszweig hervor. Durch die Cloud getriebenen Ansatz lässt sich einerseits ein Umfangreiches KI-Ökosystem aufbauen (Sundberg und Holmström 2023). Andererseits können momentane Hindernisse wie die Installation, Wartung und Verwaltung von KI-Systemen aus den Unternehmen in hin zum Plattformbetreiber verlagert werden (Sundberg und Holmström 2023). Außerdem zeigen die Autoren das durch die Demokratisierung von KI und durch die damit verbundene Erweiterung des Nutzerkreis neue, diversifiziert und innovativere KI-Lösungen entstehen können. Außerdem können durch den Einsatz dieser Technologie sowohl Zeit als auch Ressourcen gespart werden, da in diesem Fall keine Datenwissenschaftler oder Entwickler mehr benötigen werden (Sundberg und Holmström 2023). 
Allerdings ergeben sich beim Einsatz von KI auch technische (Ray 2023) (Ylitalo), ethische (Ray 2023) (Borger et al. 2023), rechtliche (Ray 2023) (Borger et al. 2023) und sozialen (Borger et al. 2023) Anforderungen, die einer tiefgehenden Analyse bedürfen.
Technische Anforderungen
Im Bereich der technischen Probleme ergeben sich insbesondere Anforderungen in den Bereichen Zuverlässigkeit, Genauigkeit, Kontrolle von Verzerrungen, Generalisierungsfähigkeit, Erklärbarkeit der Modelle sowie Sicherheits- und Kontextverständnisaspekte von KI-Systemen (Ray 2023) welche wiederum Auswirkungen auf die Bereiche Ethik, Recht und Soziales haben können wie das Beispiel von Fehlerhaften oder ethisch Bedenklichen Antworten aufgrund von verzerrten Daten zeigt.
Auch der Betrieb umfangreicher KI-Modelle erfordert ein umfangreiches technisches Wissen. So sind zum Betrieb moderner KI-Systeme neben CI/CD/DevOps und MLOps oft auch Cloud Infrastruktur notwendig. Die Verwaltung und der Betrieb solchen Infrastrukturen ist jedoch äußerst komplex. Eine Lösung bieten (Ylitalo) indem sie untersuchen wie generative künstliche Intelligenz (GAI) bei Verwaltung und Betrieb von Cloud Infrastruktur unterstützen kann. Dabei setzen sie auf einen durch KI automatisierten „Infrastructure as Code“ Ansatz, wodurch die Servicequalität verbessert und die notwendigen Prozesse vereinfacht werden können. Allerdings konzentrieren sich die Autoren auf die Unterstützung von Cloud-Experten beim Management solcher Systeme und nicht auf die Substitution dieser.
Darüber hinaus haben (Ylitalo) auch die Zuverlässigkeit solcher Systeme untersucht. Dabei kommen sie zu dem Schluss, dass viele der durch das KI-Assistenzsystem „Github Copilot“ vorgeschlagenen Codeblöcke unvollständig sind, falsch waren oder sogar schwerwiegende Sicherheitslücken enthielten. Dies kann gerade in Bezug auf die Nutzung von unerfahrenen Nutzern oder Juniorentwicklern zu schwerwiegenden Konsequenzen führen.
Ethische Anforderungen
Die ethischen Anforderungen betreffen die Sicherheit und den Schutz von Daten, die Auswirkungen auf die Umwelt, die Transparenz und Rechenschaftspflicht der KI-Systeme sowie die Vermeidung von Missbrauch und die Förderung einer verständlichen und ethisch vertretbaren Interaktion (Ray 2023).
(Borger et al. 2023) analysieren in ihrer Arbeit die Herausforderungen, die sich durch den Einsatz von großen Sprachmodellen (LLM) wie ChatGPT und Bard in Bezug auf diese drei zentralen Spannungsfelder ergeben. Dabei muss auch beachtet werden, dass diese Systeme sofort von jedermann benutzt werden können und grundsätzlich auch für böswillige Zwecke missbraucht werden können die der nutzenden Person aufgrund von Zugangsbarrieren bisher unzugänglich waren (Borger et al. 2023). Zu Schutz vor Missbrauch implementierte z.B. OpenAI Sicherheitsvorkerungen die eine böswillige Nutzung von ChatGPT unterbinden soll (Borger et al. 2023).
Dabei analysieren sie gesellschaftlichen Auswirkungen, die durch den Einsatz von KI-gestützter Systemen in der Wissenschaft auftreten. Sie zeigen auf, dass es noch zu lösenden Probleme in den Bereichen Privatsphäre, Vertraulichkeit und Sicherheit von Forschungsdaten und -texten gibt. Andererseits zeigen sie auch, dass der Einsatz von KI bisherige Barrieren in der Forschung überwinden kann. Ein Beispiel aus der Biologie zeigt, dass nun jeder Biologe mit KI-Software sein Forschungsproblem angehen und somit theoretisch zum Bioinformatiker werden kann. 
Eine ähnliche Analyse wird auch von (Wong et al. 2023) vorgenommen. Dieser gelangt zu der Erkenntnis, dass KI-gestützte Programmierung Softwareentwicklern die Möglichkeit verschafft ermöglichen, effizienter und effektiver zu arbeiten [4], es jedoch eine ausgewogene Balance zwischen der Produktivitätssteigerung einerseits und der Gewährleistung von Sicherheit, Schutz und Zuverlässigkeit auf der anderen Seite benötigt. Dazu muss das System dazu in der Lage sein solche Probleme bereits in der Entwicklungsphase vorherzusehen und zu erkennen [8], bevor sie zu einer Gefahr werden [9,10].
Auch (Ylitalo) weißen auf den etischen Aspekt hin. Sie legen nahe, dass die eingesetzten Modelle im wesentlichen verstanden werden sollte um die durch sie entstehenden Risiken und die etische Auswirkungen einordnen zu können.
Eine weiterer aus ethischer Perspektive zu beachtender Punkt kann aus den Ergebnissen von (Zamfirescu-Pereira et al. 2023) interpretiert werden, welche herausarbeiten, dass die Interaktion mit LLM-Modellen einen gewissen Grad an Sprach- und Prompting-Expertise erfordert und sich bisher nicht an den Bedürfnissen von Nicht-Programmierern und Endbenutzern orientiert (Zamfirescu-Pereira et al. 2023). Es wird darauf hingewiesen, dass Nutzende zwar in der Lage sind, diese Systeme opportunistisch zu erkunden, jedoch Schwierigkeiten haben, systematisch mit dem System zu interagieren und robuste Ergebnisse zu erzielen. (Zamfirescu-Pereira et al. 2023)weißen außerdem darauf hin, dass die meisten Probleme dadurch entstehen, dass Menschen mit dem System ebenfalls, wie mit einem Menschen interagieren, die dazu kognitiven Fähigkeiten bisher aber nicht durch solche Systeme abgedeckt werden. (Ray 2023) ergänzen diese Aussage und führen verschiedene Herausforderungen bei der Entwicklung von LLM-basierten Chatbots als problematisch auf. Dazu gehören die Beibehaltung des Kontexts und der Kontextwechsel, der Umgang mit Mehrdeutigkeiten, die Personalisierung, das Nichtvorhandensein von „gesundem Menschenverstand“, emotionale Intelligenz, ethische Überlegungen, Robustheit und Sicherheit, der Umgang mit Anfragen außerhalb der Verteilung sowie die Skalierbarkeit und Effizienz.
Außerdem weisen (Zamfirescu-Pereira et al. 2023) darauf hin, dass die Entwicklung von LLM-basierten Chatbots, wie beispielsweise Bots im Kundenservice, für Laien eine Herausforderung darstellt, da deren Umsetzung sowohl effektiver Strategien zum Verständnis des Kontextes bedarf als auch eine wirksame Strategie zur Detektion von Fehlern und zur Bewertung der Systemwirksamkeit erfordert. Um dieses Problem zu adressieren, stellen die Autoren „BotDesigner“ vor, einen No-Code-basierten Chatbot-Designer, der es Laien einerseits ermöglicht, einen Chatbot auf Basis eines LLMs allein durch Eingabeaufforderungen zu entwickeln, und andererseits einen Chatbot generiert, der Nutzenden effizient und einfach verständlich durch die zu erledigende Aktivität führt. 
Rechtliche Anforderungen: 
Rechtliche Anforderungen konzentrieren sich auf den Schutz der Privatsphäre und der Daten gemäß den geltenden Gesetzen und Vorschriften (Ray 2023).
Soziale Anforderungen: 
Es wurden keine spezifischen sozialen Anforderungen identifiziert, die explizit KI-Systeme betreffen (Ray 2023).


Datenerstellung
Ein bestehendes Hindernis ist die Bereitstellung geeigneten Wissens, auf dem solche KI-Modelle trainiert werden können. (Mozannar et al. 2024) beschreiben, dass die Leistungsfähigkeit dieser Modelle auf Milliarden von Codezeilen basiert. (Wong et al. 2023) geben an, dass dazu große Datenbanken basierend auf „Online-Softwareartefakten wie Quellcode-Repositorys, Fehlerdatenbanken und Codeausschnitten“ nötig sind. Dabei ist zu beachten, dass bei Code aus Repositorys oft nicht bekannt ist, wie sicher oder effizient dieser Code ist. Um aber domänenspezifische Modelle erstellen zu können ist eine explizite Wissensdarstellung nötig bei denen dieses Wissen maschinenverständlich aufbereitet wird (Feltus et al. 2021).

Diese Information ist jedoch für überwachtes oder teilüberwachtes Lernen unerlässlich. Das manuelle Kennzeichnen dieser Daten stellt jedoch eine mühsame und fehleranfällige Tätigkeit dar (Desmond et al. 2022).
Als Lösung könnte ein von (Desmond et al. 2022) vorgestelltes System dienen, bei dem ein interaktiver, KI-gestützter Datenbeschriftungsansatz genutzt wird. Dieser könnte genutzt werden um den Korpus für das Wissen von LLMs um gelabelte Daten zu ergänzen. Dieses System kann sowohl unbeaufsichtigt als auch halbüberwacht arbeiten. Ein mögliches Szenario bestünde darin, durch Menschen gekennzeichnete Daten sowie Daten aus Quellen mit bekannten Leistungswerten, wie z.B. Kaggle-Wettbewerben im Bereich der KI-Effizienz oder Hackathons im Bereich Code-Sicherheit, zu extrahieren und die Ergebnisse dieser Wettbewerbe als Labels zu verwenden. Diese Daten könnten dann genutzt werden, um Daten aus anderen Quellen, z.B. Repositories, automatisch nachzulabeln.
Rest?
Trotz kontinuierlicher Fortschritte zeigen bestehende Plattformen häufig Schwächen in der umfassenden Unterstützung für Domänenexperten ohne spezifisches KI- oder Netzwerk-Know-how (Borger et al. 2023; Gottlander und Khademi 2023; Sundberg und Holmström 2023; Sarker 2022; Sarkar 2023; Pakalapati et al. 2023; Wong et al. 2023). So diskutieren (Feltus et al. 2021) die Notwendigkeit von KI-unterstützter Domänenmodellierung, um Nicht-KI-Experten in der Modellierung zu unterstützen (Feltus et al. 2021; Ylitalo; Minn 2022; Desmond et al. 2022). Weiterhin zeigen (Yang et al. 2018) und (Pinhanez 2019), dass KI-Tools wie interaktive maschinelle Lernwerkzeuge und Chatbots so gestaltet werden müssen, dass sie die Bedürfnisse von Nicht-KI-Experten berücksichtigen, da sie sonst für diese Nutzergruppe keine Vorteile bieten (Yang et al. 2018; Pinhanez 2019). Eine Studie von (Zamfirescu-Pereira et al. 2023) kommt zu dem Ergebniss, dass Nicht-KI-Experten oft Schwierigkeiten haben, effektive Prompts für große Sprachmodelle zu entwerfen (Zamfirescu-Pereira et al. 2023) während (Ray 2023) aufzeigt, dass eine ausgewogene Balance zwischen KI- und menschlicher Expertise geben sein muss, um effektive Ergebnisse zu erzielen (Ray 2023). Ein KI-Assistenzsysteme zur Erstellung und Verwaltung komplexe KI-Anwendungen für vernetzte und heterogene Umgebungen muss diese Punkte berücksichtigen um erfolgreich zu sein. So ist der Einsatz von Domänenexperten ohne spezifisches KI-Knowhow denkbar, nicht jedoch der Einsatz von Nicht-KI-Experten ohne Domänenwissen. Außerdem müssen das KI-Assistenzsysteme und dieintuitiver Benutzeroberfläche für den Einsatz durch Domänenexperten optimierte werden.
Alternative Systeme an denen die Leistungsfähigkeit von LLMs bewisen wird
(Minn 2022) analysieren die Wirkungsweise von LLM basierten Systemen intelligenten Nachhilfesystemen (IST) für Schüler. Um den Lernerfolg zu steigern, implementieren sie eine durch ein LLM individualisierbare und adaptive Lernumgebung.

Tools um KI für jeden zugänglich zu machen aus (Yang et al. 2018): [3, 14, 26, 27]
Anforderungen durch den Menschn um KI für jeden zugänglich zu machen (Power to the People) aus [1, 7, 9, 20, 29]


==> doc/glyphtounicode.tex <==
% lcdf-typetools glyphtounicode.tex, Version 2.95
% Contents: Glyph mapping information for pdftex, used for PDF searching
% Generated from:
% - glyphlist.txt, Version 2.0
% - texglyphlist.txt, Version 2.95
% - texglyphlist-g2u.txt, Version 2.95
\pdfglyphtounicode{A}{00A0}
\pdfglyphtounicode{AE}{00A0}
\pdfglyphtounicode{AEacute}{00A0}
\pdfglyphtounicode{AEmacron}{00A0}
\pdfglyphtounicode{AEsmall}{00A0}
\pdfglyphtounicode{Aacute}{00A0}
\pdfglyphtounicode{Aacutesmall}{00A0}
\pdfglyphtounicode{Abreve}{00A0}
\pdfglyphtounicode{Abreveacute}{00A0}
\pdfglyphtounicode{Abrevecyrillic}{00A0}
\pdfglyphtounicode{Abrevedotbelow}{00A0}
\pdfglyphtounicode{Abrevegrave}{00A0}
\pdfglyphtounicode{Abrevehookabove}{00A0}
\pdfglyphtounicode{Abrevetilde}{00A0}
\pdfglyphtounicode{Acaron}{00A0}
\pdfglyphtounicode{Acircle}{00A0}
\pdfglyphtounicode{Acircumflex}{00A0}
\pdfglyphtounicode{Acircumflexacute}{00A0}
\pdfglyphtounicode{Acircumflexdotbelow}{00A0}
\pdfglyphtounicode{Acircumflexgrave}{00A0}
\pdfglyphtounicode{Acircumflexhookabove}{00A0}
\pdfglyphtounicode{Acircumflexsmall}{00A0}
\pdfglyphtounicode{Acircumflextilde}{00A0}
\pdfglyphtounicode{Acute}{00A0}
\pdfglyphtounicode{Acutesmall}{00A0}
\pdfglyphtounicode{Acyrillic}{00A0}
\pdfglyphtounicode{Adblgrave}{00A0}
\pdfglyphtounicode{Adieresis}{00A0}
\pdfglyphtounicode{Adieresiscyrillic}{00A0}
\pdfglyphtounicode{Adieresismacron}{00A0}
\pdfglyphtounicode{Adieresissmall}{00A0}
\pdfglyphtounicode{Adotbelow}{00A0}
\pdfglyphtounicode{Adotmacron}{00A0}
\pdfglyphtounicode{Agrave}{00A0}
\pdfglyphtounicode{Agravesmall}{00A0}
\pdfglyphtounicode{Ahookabove}{00A0}
\pdfglyphtounicode{Aiecyrillic}{00A0}
\pdfglyphtounicode{Ainvertedbreve}{00A0}
\pdfglyphtounicode{Alpha}{00A0}
\pdfglyphtounicode{Alphatonos}{00A0}
\pdfglyphtounicode{Amacron}{00A0}
\pdfglyphtounicode{Amonospace}{00A0}
\pdfglyphtounicode{Aogonek}{00A0}
\pdfglyphtounicode{Aring}{00A0}
\pdfglyphtounicode{Aringacute}{00A0}
\pdfglyphtounicode{Aringbelow}{00A0}
\pdfglyphtounicode{Aringsmall}{00A0}
\pdfglyphtounicode{Asmall}{00A0}
\pdfglyphtounicode{Atilde}{00A0}
\pdfglyphtounicode{Atildesmall}{00A0}
\pdfglyphtounicode{Aybarmenian}{00A0}
\pdfglyphtounicode{B}{00A0}
\pdfglyphtounicode{Bcircle}{00A0}
\pdfglyphtounicode{Bdotaccent}{00A0}
\pdfglyphtounicode{Bdotbelow}{00A0}
\pdfglyphtounicode{Becyrillic}{00A0}
\pdfglyphtounicode{Benarmenian}{00A0}
\pdfglyphtounicode{Beta}{00A0}
\pdfglyphtounicode{Bhook}{00A0}
\pdfglyphtounicode{Blinebelow}{00A0}
\pdfglyphtounicode{Bmonospace}{00A0}
\pdfglyphtounicode{Brevesmall}{00A0}
\pdfglyphtounicode{Bsmall}{00A0}
\pdfglyphtounicode{Btopbar}{00A0}
\pdfglyphtounicode{C}{00A0}
\pdfglyphtounicode{Caarmenian}{00A0}
\pdfglyphtounicode{Cacute}{00A0}
\pdfglyphtounicode{Caron}{00A0}
\pdfglyphtounicode{Caronsmall}{00A0}
\pdfglyphtounicode{Ccaron}{00A0}
\pdfglyphtounicode{Ccedilla}{00A0}
\pdfglyphtounicode{Ccedillaacute}{00A0}
\pdfglyphtounicode{Ccedillasmall}{00A0}
\pdfglyphtounicode{Ccircle}{00A0}
\pdfglyphtounicode{Ccircumflex}{00A0}
\pdfglyphtounicode{Cdot}{00A0}
\pdfglyphtounicode{Cdotaccent}{00A0}
\pdfglyphtounicode{Cedillasmall}{00A0}
\pdfglyphtounicode{Chaarmenian}{00A0}
\pdfglyphtounicode{Cheabkhasiancyrillic}{00A0}
\pdfglyphtounicode{Checyrillic}{00A0}
\pdfglyphtounicode{Chedescenderabkhasiancyrillic}{00A0}
\pdfglyphtounicode{Chedescendercyrillic}{00A0}
\pdfglyphtounicode{Chedieresiscyrillic}{00A0}
\pdfglyphtounicode{Cheharmenian}{00A0}
\pdfglyphtounicode{Chekhakassiancyrillic}{00A0}
\pdfglyphtounicode{Cheverticalstrokecyrillic}{00A0}
\pdfglyphtounicode{Chi}{00A0}
\pdfglyphtounicode{Chook}{00A0}
\pdfglyphtounicode{Circumflexsmall}{00A0}
\pdfglyphtounicode{Cmonospace}{00A0}
\pdfglyphtounicode{Coarmenian}{00A0}
\pdfglyphtounicode{Csmall}{00A0}
\pdfglyphtounicode{D}{00A0}
\pdfglyphtounicode{DZ}{00A0}
\pdfglyphtounicode{DZcaron}{00A0}
\pdfglyphtounicode{Daarmenian}{00A0}
\pdfglyphtounicode{Dafrican}{00A0}
\pdfglyphtounicode{Dbar}{00A0}
\pdfglyphtounicode{Dcaron}{00A0}
\pdfglyphtounicode{Dcedilla}{00A0}
\pdfglyphtounicode{Dcircle}{00A0}
\pdfglyphtounicode{Dcircumflexbelow}{00A0}
\pdfglyphtounicode{Dcroat}{00A0}
\pdfglyphtounicode{Ddotaccent}{00A0}
\pdfglyphtounicode{Ddotbelow}{00A0}
\pdfglyphtounicode{Decyrillic}{00A0}
\pdfglyphtounicode{Deicoptic}{00A0}
\pdfglyphtounicode{Delta}{00A0}
\pdfglyphtounicode{Deltagreek}{00A0}
\pdfglyphtounicode{Dhook}{00A0}
\pdfglyphtounicode{Dieresis}{00A0}
\pdfglyphtounicode{DieresisAcute}{00A0}
\pdfglyphtounicode{DieresisGrave}{00A0}
\pdfglyphtounicode{Dieresissmall}{00A0}
\pdfglyphtounicode{Digamma}{00A0}
\pdfglyphtounicode{Digammagreek}{00A0}
\pdfglyphtounicode{Djecyrillic}{00A0}
\pdfglyphtounicode{Dlinebelow}{00A0}
\pdfglyphtounicode{Dmonospace}{00A0}
\pdfglyphtounicode{Dotaccentsmall}{00A0}
\pdfglyphtounicode{Dslash}{00A0}
\pdfglyphtounicode{Dsmall}{00A0}
\pdfglyphtounicode{Dtopbar}{00A0}
\pdfglyphtounicode{Dz}{00A0}
\pdfglyphtounicode{Dzcaron}{00A0}
\pdfglyphtounicode{Dzeabkhasiancyrillic}{00A0}
\pdfglyphtounicode{Dzecyrillic}{00A0}
\pdfglyphtounicode{Dzhecyrillic}{00A0}
\pdfglyphtounicode{E}{00A0}
\pdfglyphtounicode{Eacute}{00A0}
\pdfglyphtounicode{Eacutesmall}{00A0}
\pdfglyphtounicode{Ebreve}{00A0}
\pdfglyphtounicode{Ecaron}{00A0}
\pdfglyphtounicode{Ecedillabreve}{00A0}
\pdfglyphtounicode{Echarmenian}{00A0}
\pdfglyphtounicode{Ecircle}{00A0}
\pdfglyphtounicode{Ecircumflex}{00A0}
\pdfglyphtounicode{Ecircumflexacute}{00A0}
\pdfglyphtounicode{Ecircumflexbelow}{00A0}
\pdfglyphtounicode{Ecircumflexdotbelow}{00A0}
\pdfglyphtounicode{Ecircumflexgrave}{00A0}
\pdfglyphtounicode{Ecircumflexhookabove}{00A0}
\pdfglyphtounicode{Ecircumflexsmall}{00A0}
\pdfglyphtounicode{Ecircumflextilde}{00A0}
\pdfglyphtounicode{Ecyrillic}{00A0}
\pdfglyphtounicode{Edblgrave}{00A0}
\pdfglyphtounicode{Edieresis}{00A0}
\pdfglyphtounicode{Edieresissmall}{00A0}
\pdfglyphtounicode{Edot}{00A0}
\pdfglyphtounicode{Edotaccent}{00A0}
\pdfglyphtounicode{Edotbelow}{00A0}
\pdfglyphtounicode{Efcyrillic}{00A0}
\pdfglyphtounicode{Egrave}{00A0}
\pdfglyphtounicode{Egravesmall}{00A0}
\pdfglyphtounicode{Eharmenian}{00A0}
\pdfglyphtounicode{Ehookabove}{00A0}
\pdfglyphtounicode{Eightroman}{00A0}
\pdfglyphtounicode{Einvertedbreve}{00A0}
\pdfglyphtounicode{Eiotifiedcyrillic}{00A0}
\pdfglyphtounicode{Elcyrillic}{00A0}
\pdfglyphtounicode{Elevenroman}{00A0}
\pdfglyphtounicode{Emacron}{00A0}
\pdfglyphtounicode{Emacronacute}{00A0}
\pdfglyphtounicode{Emacrongrave}{00A0}
\pdfglyphtounicode{Emcyrillic}{00A0}
\pdfglyphtounicode{Emonospace}{00A0}
\pdfglyphtounicode{Encyrillic}{00A0}
\pdfglyphtounicode{Endescendercyrillic}{00A0}
\pdfglyphtounicode{Eng}{00A0}
\pdfglyphtounicode{Enghecyrillic}{00A0}
\pdfglyphtounicode{Enhookcyrillic}{00A0}
\pdfglyphtounicode{Eogonek}{00A0}
\pdfglyphtounicode{Eopen}{00A0}
\pdfglyphtounicode{Epsilon}{00A0}
\pdfglyphtounicode{Epsilontonos}{00A0}
\pdfglyphtounicode{Ercyrillic}{00A0}
\pdfglyphtounicode{Ereversed}{00A0}
\pdfglyphtounicode{Ereversedcyrillic}{00A0}
\pdfglyphtounicode{Escyrillic}{00A0}
\pdfglyphtounicode{Esdescendercyrillic}{00A0}
\pdfglyphtounicode{Esh}{00A0}
\pdfglyphtounicode{Esmall}{00A0}
\pdfglyphtounicode{Eta}{00A0}
\pdfglyphtounicode{Etarmenian}{00A0}
\pdfglyphtounicode{Etatonos}{00A0}
\pdfglyphtounicode{Eth}{00A0}
\pdfglyphtounicode{Ethsmall}{00A0}
\pdfglyphtounicode{Etilde}{00A0}
\pdfglyphtounicode{Etildebelow}{00A0}
\pdfglyphtounicode{Euro}{00A0}
\pdfglyphtounicode{Ezh}{00A0}
\pdfglyphtounicode{Ezhcaron}{00A0}
\pdfglyphtounicode{Ezhreversed}{00A0}
\pdfglyphtounicode{F}{00A0}
\pdfglyphtounicode{FFIsmall}{00A0}
\pdfglyphtounicode{FFLsmall}{00A0}
\pdfglyphtounicode{FFsmall}{00A0}
\pdfglyphtounicode{FIsmall}{00A0}
\pdfglyphtounicode{FLsmall}{00A0}
\pdfglyphtounicode{Fcircle}{00A0}
\pdfglyphtounicode{Fdotaccent}{00A0}
\pdfglyphtounicode{Feharmenian}{00A0}
\pdfglyphtounicode{Feicoptic}{00A0}
\pdfglyphtounicode{Fhook}{00A0}
\pdfglyphtounicode{Finv}{00A0}
\pdfglyphtounicode{Fitacyrillic}{00A0}
\pdfglyphtounicode{Fiveroman}{00A0}
\pdfglyphtounicode{Fmonospace}{00A0}
\pdfglyphtounicode{Fourroman}{00A0}
\pdfglyphtounicode{Fsmall}{00A0}
\pdfglyphtounicode{G}{00A0}
\pdfglyphtounicode{GBsquare}{00A0}
\pdfglyphtounicode{Gacute}{00A0}
\pdfglyphtounicode{Gamma}{00A0}
\pdfglyphtounicode{Gammaafrican}{00A0}
\pdfglyphtounicode{Gangiacoptic}{00A0}
\pdfglyphtounicode{Gbreve}{00A0}
\pdfglyphtounicode{Gcaron}{00A0}
\pdfglyphtounicode{Gcedilla}{00A0}
\pdfglyphtounicode{Gcircle}{00A0}
\pdfglyphtounicode{Gcircumflex}{00A0}
\pdfglyphtounicode{Gcommaaccent}{00A0}
\pdfglyphtounicode{Gdot}{00A0}
\pdfglyphtounicode{Gdotaccent}{00A0}
\pdfglyphtounicode{Gecyrillic}{00A0}
\pdfglyphtounicode{Germandbls}{00A0}
\pdfglyphtounicode{Germandblssmall}{00A0}
\pdfglyphtounicode{Ghadarmenian}{00A0}
\pdfglyphtounicode{Ghemiddlehookcyrillic}{00A0}
\pdfglyphtounicode{Ghestrokecyrillic}{00A0}
\pdfglyphtounicode{Gheupturncyrillic}{00A0}
\pdfglyphtounicode{Ghook}{00A0}
\pdfglyphtounicode{Gimarmenian}{00A0}
\pdfglyphtounicode{Gjecyrillic}{00A0}
\pdfglyphtounicode{Gmacron}{00A0}
\pdfglyphtounicode{Gmir}{00A0}
\pdfglyphtounicode{Gmonospace}{00A0}
\pdfglyphtounicode{Grave}{00A0}
\pdfglyphtounicode{Gravesmall}{00A0}
\pdfglyphtounicode{Gsmall}{00A0}
\pdfglyphtounicode{Gsmallhook}{00A0}
\pdfglyphtounicode{Gstroke}{00A0}
\pdfglyphtounicode{H}{00A0}
\pdfglyphtounicode{H18533}{00A0}
\pdfglyphtounicode{H18543}{00A0}
\pdfglyphtounicode{H18551}{00A0}
\pdfglyphtounicode{H22073}{00A0}
\pdfglyphtounicode{HPsquare}{00A0}
\pdfglyphtounicode{Haabkhasiancyrillic}{00A0}
\pdfglyphtounicode{Hadescendercyrillic}{00A0}
\pdfglyphtounicode{Hardsigncyrillic}{00A0}
\pdfglyphtounicode{Hbar}{00A0}
\pdfglyphtounicode{Hbrevebelow}{00A0}
\pdfglyphtounicode{Hcedilla}{00A0}
\pdfglyphtounicode{Hcircle}{00A0}
\pdfglyphtounicode{Hcircumflex}{00A0}
\pdfglyphtounicode{Hdieresis}{00A0}
\pdfglyphtounicode{Hdotaccent}{00A0}
\pdfglyphtounicode{Hdotbelow}{00A0}
\pdfglyphtounicode{Hmonospace}{00A0}
\pdfglyphtounicode{Hoarmenian}{00A0}
\pdfglyphtounicode{Horicoptic}{00A0}
\pdfglyphtounicode{Hsmall}{00A0}
\pdfglyphtounicode{Hungarumlaut}{00A0}
\pdfglyphtounicode{Hungarumlautsmall}{00A0}
\pdfglyphtounicode{Hzsquare}{00A0}
\pdfglyphtounicode{I}{00A0}
\pdfglyphtounicode{IAcyrillic}{00A0}
\pdfglyphtounicode{IJ}{00A0}
\pdfglyphtounicode{IUcyrillic}{00A0}
\pdfglyphtounicode{Iacute}{00A0}
\pdfglyphtounicode{Iacutesmall}{00A0}
\pdfglyphtounicode{Ibreve}{00A0}
\pdfglyphtounicode{Icaron}{00A0}
\pdfglyphtounicode{Icircle}{00A0}
\pdfglyphtounicode{Icircumflex}{00A0}
\pdfglyphtounicode{Icircumflexsmall}{00A0}
\pdfglyphtounicode{Icyrillic}{00A0}
\pdfglyphtounicode{Idblgrave}{00A0}
\pdfglyphtounicode{Idieresis}{00A0}
\pdfglyphtounicode{Idieresisacute}{00A0}
\pdfglyphtounicode{Idieresiscyrillic}{00A0}
\pdfglyphtounicode{Idieresissmall}{00A0}
\pdfglyphtounicode{Idot}{00A0}
\pdfglyphtounicode{Idotaccent}{00A0}
\pdfglyphtounicode{Idotbelow}{00A0}
\pdfglyphtounicode{Iebrevecyrillic}{00A0}
\pdfglyphtounicode{Iecyrillic}{00A0}
\pdfglyphtounicode{Ifractur}{00A0}
\pdfglyphtounicode{Ifraktur}{00A0}
\pdfglyphtounicode{Igrave}{00A0}
\pdfglyphtounicode{Igravesmall}{00A0}
\pdfglyphtounicode{Ihookabove}{00A0}
\pdfglyphtounicode{Iicyrillic}{00A0}
\pdfglyphtounicode{Iinvertedbreve}{00A0}
\pdfglyphtounicode{Iishortcyrillic}{00A0}
\pdfglyphtounicode{Imacron}{00A0}
\pdfglyphtounicode{Imacroncyrillic}{00A0}
\pdfglyphtounicode{Imonospace}{00A0}
\pdfglyphtounicode{Iniarmenian}{00A0}
\pdfglyphtounicode{Iocyrillic}{00A0}
\pdfglyphtounicode{Iogonek}{00A0}
\pdfglyphtounicode{Iota}{00A0}
\pdfglyphtounicode{Iotaafrican}{00A0}
\pdfglyphtounicode{Iotadieresis}{00A0}
\pdfglyphtounicode{Iotatonos}{00A0}
\pdfglyphtounicode{Ismall}{00A0}
\pdfglyphtounicode{Istroke}{00A0}
\pdfglyphtounicode{Itilde}{00A0}
\pdfglyphtounicode{Itildebelow}{00A0}
\pdfglyphtounicode{Izhitsacyrillic}{00A0}
\pdfglyphtounicode{Izhitsadblgravecyrillic}{00A0}
\pdfglyphtounicode{J}{00A0}
\pdfglyphtounicode{Jaarmenian}{00A0}
\pdfglyphtounicode{Jcircle}{00A0}
\pdfglyphtounicode{Jcircumflex}{00A0}
\pdfglyphtounicode{Jecyrillic}{00A0}
\pdfglyphtounicode{Jheharmenian}{00A0}
\pdfglyphtounicode{Jmonospace}{00A0}
\pdfglyphtounicode{Jsmall}{00A0}
\pdfglyphtounicode{K}{00A0}
\pdfglyphtounicode{KBsquare}{00A0}
\pdfglyphtounicode{KKsquare}{00A0}
\pdfglyphtounicode{Kabashkircyrillic}{00A0}
\pdfglyphtounicode{Kacute}{00A0}
\pdfglyphtounicode{Kacyrillic}{00A0}
\pdfglyphtounicode{Kadescendercyrillic}{00A0}
\pdfglyphtounicode{Kahookcyrillic}{00A0}
\pdfglyphtounicode{Kappa}{00A0}
\pdfglyphtounicode{Kastrokecyrillic}{00A0}
\pdfglyphtounicode{Kaverticalstrokecyrillic}{00A0}
\pdfglyphtounicode{Kcaron}{00A0}
\pdfglyphtounicode{Kcedilla}{00A0}
\pdfglyphtounicode{Kcircle}{00A0}
\pdfglyphtounicode{Kcommaaccent}{00A0}
\pdfglyphtounicode{Kdotbelow}{00A0}
\pdfglyphtounicode{Keharmenian}{00A0}
\pdfglyphtounicode{Kenarmenian}{00A0}
\pdfglyphtounicode{Khacyrillic}{00A0}
\pdfglyphtounicode{Kheicoptic}{00A0}
\pdfglyphtounicode{Khook}{00A0}
\pdfglyphtounicode{Kjecyrillic}{00A0}
\pdfglyphtounicode{Klinebelow}{00A0}
\pdfglyphtounicode{Kmonospace}{00A0}
\pdfglyphtounicode{Koppacyrillic}{00A0}
\pdfglyphtounicode{Koppagreek}{00A0}
\pdfglyphtounicode{Ksicyrillic}{00A0}
\pdfglyphtounicode{Ksmall}{00A0}
\pdfglyphtounicode{L}{00A0}
\pdfglyphtounicode{LJ}{00A0}
\pdfglyphtounicode{LL}{00A0}
\pdfglyphtounicode{Lacute}{00A0}
\pdfglyphtounicode{Lambda}{00A0}
\pdfglyphtounicode{Lcaron}{00A0}
\pdfglyphtounicode{Lcedilla}{00A0}
\pdfglyphtounicode{Lcircle}{00A0}
\pdfglyphtounicode{Lcircumflexbelow}{00A0}
\pdfglyphtounicode{Lcommaaccent}{00A0}
\pdfglyphtounicode{Ldot}{00A0}
\pdfglyphtounicode{Ldotaccent}{00A0}
\pdfglyphtounicode{Ldotbelow}{00A0}
\pdfglyphtounicode{Ldotbelowmacron}{00A0}
\pdfglyphtounicode{Liwnarmenian}{00A0}
\pdfglyphtounicode{Lj}{00A0}
\pdfglyphtounicode{Ljecyrillic}{00A0}
\pdfglyphtounicode{Llinebelow}{00A0}
\pdfglyphtounicode{Lmonospace}{00A0}
\pdfglyphtounicode{Lslash}{00A0}
\pdfglyphtounicode{Lslashsmall}{00A0}
\pdfglyphtounicode{Lsmall}{00A0}
\pdfglyphtounicode{M}{00A0}
\pdfglyphtounicode{MBsquare}{00A0}
\pdfglyphtounicode{Macron}{00A0}
\pdfglyphtounicode{Macronsmall}{00A0}
\pdfglyphtounicode{Macute}{00A0}
\pdfglyphtounicode{Mcircle}{00A0}
\pdfglyphtounicode{Mdotaccent}{00A0}
\pdfglyphtounicode{Mdotbelow}{00A0}
\pdfglyphtounicode{Menarmenian}{00A0}
\pdfglyphtounicode{Mmonospace}{00A0}
\pdfglyphtounicode{Msmall}{00A0}
\pdfglyphtounicode{Mturned}{00A0}
\pdfglyphtounicode{Mu}{00A0}
\pdfglyphtounicode{N}{00A0}
\pdfglyphtounicode{NJ}{00A0}
\pdfglyphtounicode{Nacute}{00A0}
\pdfglyphtounicode{Ncaron}{00A0}
\pdfglyphtounicode{Ncedilla}{00A0}
\pdfglyphtounicode{Ncircle}{00A0}
\pdfglyphtounicode{Ncircumflexbelow}{00A0}
\pdfglyphtounicode{Ncommaaccent}{00A0}
\pdfglyphtounicode{Ndotaccent}{00A0}
\pdfglyphtounicode{Ndotbelow}{00A0}
\pdfglyphtounicode{Ng}{00A0}
\pdfglyphtounicode{Nhookleft}{00A0}
\pdfglyphtounicode{Nineroman}{00A0}
\pdfglyphtounicode{Nj}{00A0}
\pdfglyphtounicode{Njecyrillic}{00A0}
\pdfglyphtounicode{Nlinebelow}{00A0}
\pdfglyphtounicode{Nmonospace}{00A0}
\pdfglyphtounicode{Nowarmenian}{00A0}
\pdfglyphtounicode{Nsmall}{00A0}
\pdfglyphtounicode{Ntilde}{00A0}
\pdfglyphtounicode{Ntildesmall}{00A0}
\pdfglyphtounicode{Nu}{00A0}
\pdfglyphtounicode{O}{00A0}
\pdfglyphtounicode{OE}{00A0}
\pdfglyphtounicode{OEsmall}{00A0}
\pdfglyphtounicode{Oacute}{00A0}
\pdfglyphtounicode{Oacutesmall}{00A0}
\pdfglyphtounicode{Obarredcyrillic}{00A0}
\pdfglyphtounicode{Obarreddieresiscyrillic}{00A0}
\pdfglyphtounicode{Obreve}{00A0}
\pdfglyphtounicode{Ocaron}{00A0}
\pdfglyphtounicode{Ocenteredtilde}{00A0}
\pdfglyphtounicode{Ocircle}{00A0}
\pdfglyphtounicode{Ocircumflex}{00A0}
\pdfglyphtounicode{Ocircumflexacute}{00A0}
\pdfglyphtounicode{Ocircumflexdotbelow}{00A0}
\pdfglyphtounicode{Ocircumflexgrave}{00A0}
\pdfglyphtounicode{Ocircumflexhookabove}{00A0}
\pdfglyphtounicode{Ocircumflexsmall}{00A0}
\pdfglyphtounicode{Ocircumflextilde}{00A0}
\pdfglyphtounicode{Ocyrillic}{00A0}
\pdfglyphtounicode{Odblacute}{00A0}
\pdfglyphtounicode{Odblgrave}{00A0}
\pdfglyphtounicode{Odieresis}{00A0}
\pdfglyphtounicode{Odieresiscyrillic}{00A0}
\pdfglyphtounicode{Odieresissmall}{00A0}
\pdfglyphtounicode{Odotbelow}{00A0}
\pdfglyphtounicode{Ogoneksmall}{00A0}
\pdfglyphtounicode{Ograve}{00A0}
\pdfglyphtounicode{Ogravesmall}{00A0}
\pdfglyphtounicode{Oharmenian}{00A0}
\pdfglyphtounicode{Ohm}{00A0}
\pdfglyphtounicode{Ohookabove}{00A0}
\pdfglyphtounicode{Ohorn}{00A0}
\pdfglyphtounicode{Ohornacute}{00A0}
\pdfglyphtounicode{Ohorndotbelow}{00A0}
\pdfglyphtounicode{Ohorngrave}{00A0}
\pdfglyphtounicode{Ohornhookabove}{00A0}
\pdfglyphtounicode{Ohorntilde}{00A0}
\pdfglyphtounicode{Ohungarumlaut}{00A0}
\pdfglyphtounicode{Oi}{00A0}
\pdfglyphtounicode{Oinvertedbreve}{00A0}
\pdfglyphtounicode{Omacron}{00A0}
\pdfglyphtounicode{Omacronacute}{00A0}
\pdfglyphtounicode{Omacrongrave}{00A0}
\pdfglyphtounicode{Omega}{00A0}
\pdfglyphtounicode{Omegacyrillic}{00A0}
\pdfglyphtounicode{Omegagreek}{00A0}
\pdfglyphtounicode{Omegainv}{00A0}
\pdfglyphtounicode{Omegaroundcyrillic}{00A0}
\pdfglyphtounicode{Omegatitlocyrillic}{00A0}
\pdfglyphtounicode{Omegatonos}{00A0}
\pdfglyphtounicode{Omicron}{00A0}
\pdfglyphtounicode{Omicrontonos}{00A0}
\pdfglyphtounicode{Omonospace}{00A0}
\pdfglyphtounicode{Oneroman}{00A0}
\pdfglyphtounicode{Oogonek}{00A0}
\pdfglyphtounicode{Oogonekmacron}{00A0}
\pdfglyphtounicode{Oopen}{00A0}
\pdfglyphtounicode{Oslash}{00A0}
\pdfglyphtounicode{Oslashacute}{00A0}
\pdfglyphtounicode{Oslashsmall}{00A0}
\pdfglyphtounicode{Osmall}{00A0}
\pdfglyphtounicode{Ostrokeacute}{00A0}
\pdfglyphtounicode{Otcyrillic}{00A0}
\pdfglyphtounicode{Otilde}{00A0}
\pdfglyphtounicode{Otildeacute}{00A0}
\pdfglyphtounicode{Otildedieresis}{00A0}
\pdfglyphtounicode{Otildesmall}{00A0}
\pdfglyphtounicode{P}{00A0}
\pdfglyphtounicode{Pacute}{00A0}
\pdfglyphtounicode{Pcircle}{00A0}
\pdfglyphtounicode{Pdotaccent}{00A0}
\pdfglyphtounicode{Pecyrillic}{00A0}
\pdfglyphtounicode{Peharmenian}{00A0}
\pdfglyphtounicode{Pemiddlehookcyrillic}{00A0}
\pdfglyphtounicode{Phi}{00A0}
\pdfglyphtounicode{Phook}{00A0}
\pdfglyphtounicode{Pi}{00A0}
\pdfglyphtounicode{Piwrarmenian}{00A0}
\pdfglyphtounicode{Pmonospace}{00A0}
\pdfglyphtounicode{Psi}{00A0}
\pdfglyphtounicode{Psicyrillic}{00A0}
\pdfglyphtounicode{Psmall}{00A0}
\pdfglyphtounicode{Q}{00A0}
\pdfglyphtounicode{Qcircle}{00A0}
\pdfglyphtounicode{Qmonospace}{00A0}
\pdfglyphtounicode{Qsmall}{00A0}
\pdfglyphtounicode{R}{00A0}
\pdfglyphtounicode{Raarmenian}{00A0}
\pdfglyphtounicode{Racute}{00A0}
\pdfglyphtounicode{Rcaron}{00A0}
\pdfglyphtounicode{Rcedilla}{00A0}
\pdfglyphtounicode{Rcircle}{00A0}
\pdfglyphtounicode{Rcommaaccent}{00A0}
\pdfglyphtounicode{Rdblgrave}{00A0}
\pdfglyphtounicode{Rdotaccent}{00A0}
\pdfglyphtounicode{Rdotbelow}{00A0}
\pdfglyphtounicode{Rdotbelowmacron}{00A0}
\pdfglyphtounicode{Reharmenian}{00A0}
\pdfglyphtounicode{Rfractur}{00A0}
\pdfglyphtounicode{Rfraktur}{00A0}
\pdfglyphtounicode{Rho}{00A0}
\pdfglyphtounicode{Ringsmall}{00A0}
\pdfglyphtounicode{Rinvertedbreve}{00A0}
\pdfglyphtounicode{Rlinebelow}{00A0}
\pdfglyphtounicode{Rmonospace}{00A0}
\pdfglyphtounicode{Rsmall}{00A0}
\pdfglyphtounicode{Rsmallinverted}{00A0}
\pdfglyphtounicode{Rsmallinvertedsuperior}{00A0}
\pdfglyphtounicode{S}{00A0}
\pdfglyphtounicode{SF010000}{00A0}
\pdfglyphtounicode{SF020000}{00A0}
\pdfglyphtounicode{SF030000}{00A0}
\pdfglyphtounicode{SF040000}{00A0}
\pdfglyphtounicode{SF050000}{00A0}
\pdfglyphtounicode{SF060000}{00A0}
\pdfglyphtounicode{SF070000}{00A0}
\pdfglyphtounicode{SF080000}{00A0}
\pdfglyphtounicode{SF090000}{00A0}
\pdfglyphtounicode{SF100000}{00A0}
\pdfglyphtounicode{SF110000}{00A0}
\pdfglyphtounicode{SF190000}{00A0}
\pdfglyphtounicode{SF200000}{00A0}
\pdfglyphtounicode{SF210000}{00A0}
\pdfglyphtounicode{SF220000}{00A0}
\pdfglyphtounicode{SF230000}{00A0}
\pdfglyphtounicode{SF240000}{00A0}
\pdfglyphtounicode{SF250000}{00A0}
\pdfglyphtounicode{SF260000}{00A0}
\pdfglyphtounicode{SF270000}{00A0}
\pdfglyphtounicode{SF280000}{00A0}
\pdfglyphtounicode{SF360000}{00A0}
\pdfglyphtounicode{SF370000}{00A0}
\pdfglyphtounicode{SF380000}{00A0}
\pdfglyphtounicode{SF390000}{00A0}
\pdfglyphtounicode{SF400000}{00A0}
\pdfglyphtounicode{SF410000}{00A0}
\pdfglyphtounicode{SF420000}{00A0}
\pdfglyphtounicode{SF430000}{00A0}
\pdfglyphtounicode{SF440000}{00A0}
\pdfglyphtounicode{SF450000}{00A0}
\pdfglyphtounicode{SF460000}{00A0}
\pdfglyphtounicode{SF470000}{00A0}
\pdfglyphtounicode{SF480000}{00A0}
\pdfglyphtounicode{SF490000}{00A0}
\pdfglyphtounicode{SF500000}{00A0}
\pdfglyphtounicode{SF510000}{00A0}
\pdfglyphtounicode{SF520000}{00A0}
\pdfglyphtounicode{SF530000}{00A0}
\pdfglyphtounicode{SF540000}{00A0}
\pdfglyphtounicode{SS}{00A0}
\pdfglyphtounicode{SSsmall}{00A0}
\pdfglyphtounicode{Sacute}{00A0}
\pdfglyphtounicode{Sacutedotaccent}{00A0}
\pdfglyphtounicode{Sampigreek}{00A0}
\pdfglyphtounicode{Scaron}{00A0}
\pdfglyphtounicode{Scarondotaccent}{00A0}
\pdfglyphtounicode{Scaronsmall}{00A0}
\pdfglyphtounicode{Scedilla}{00A0}
\pdfglyphtounicode{Schwa}{00A0}
\pdfglyphtounicode{Schwacyrillic}{00A0}
\pdfglyphtounicode{Schwadieresiscyrillic}{00A0}
\pdfglyphtounicode{Scircle}{00A0}
\pdfglyphtounicode{Scircumflex}{00A0}
\pdfglyphtounicode{Scommaaccent}{00A0}
\pdfglyphtounicode{Sdotaccent}{00A0}
\pdfglyphtounicode{Sdotbelow}{00A0}
\pdfglyphtounicode{Sdotbelowdotaccent}{00A0}
\pdfglyphtounicode{Seharmenian}{00A0}
\pdfglyphtounicode{Sevenroman}{00A0}
\pdfglyphtounicode{Shaarmenian}{00A0}
\pdfglyphtounicode{Shacyrillic}{00A0}
\pdfglyphtounicode{Shchacyrillic}{00A0}
\pdfglyphtounicode{Sheicoptic}{00A0}
\pdfglyphtounicode{Shhacyrillic}{00A0}
\pdfglyphtounicode{Shimacoptic}{00A0}
\pdfglyphtounicode{Sigma}{00A0}
\pdfglyphtounicode{Sixroman}{00A0}
\pdfglyphtounicode{Smonospace}{00A0}
\pdfglyphtounicode{Softsigncyrillic}{00A0}
\pdfglyphtounicode{Ssmall}{00A0}
\pdfglyphtounicode{Stigmagreek}{00A0}
\pdfglyphtounicode{T}{00A0}
\pdfglyphtounicode{Tau}{00A0}
\pdfglyphtounicode{Tbar}{00A0}
\pdfglyphtounicode{Tcaron}{00A0}
\pdfglyphtounicode{Tcedilla}{00A0}
\pdfglyphtounicode{Tcircle}{00A0}
\pdfglyphtounicode{Tcircumflexbelow}{00A0}
\pdfglyphtounicode{Tcommaaccent}{00A0}
\pdfglyphtounicode{Tdotaccent}{00A0}
\pdfglyphtounicode{Tdotbelow}{00A0}
\pdfglyphtounicode{Tecyrillic}{00A0}
\pdfglyphtounicode{Tedescendercyrillic}{00A0}
\pdfglyphtounicode{Tenroman}{00A0}
\pdfglyphtounicode{Tetsecyrillic}{00A0}
\pdfglyphtounicode{Theta}{00A0}
\pdfglyphtounicode{Thook}{00A0}
\pdfglyphtounicode{Thorn}{00A0}
\pdfglyphtounicode{Thornsmall}{00A0}
\pdfglyphtounicode{Threeroman}{00A0}
\pdfglyphtounicode{Tildesmall}{00A0}
\pdfglyphtounicode{Tiwnarmenian}{00A0}
\pdfglyphtounicode{Tlinebelow}{00A0}
\pdfglyphtounicode{Tmonospace}{00A0}
\pdfglyphtounicode{Toarmenian}{00A0}
\pdfglyphtounicode{Tonefive}{00A0}
\pdfglyphtounicode{Tonesix}{00A0}
\pdfglyphtounicode{Tonetwo}{00A0}
\pdfglyphtounicode{Tretroflexhook}{00A0}
\pdfglyphtounicode{Tsecyrillic}{00A0}
\pdfglyphtounicode{Tshecyrillic}{00A0}
\pdfglyphtounicode{Tsmall}{00A0}
\pdfglyphtounicode{Twelveroman}{00A0}
\pdfglyphtounicode{Tworoman}{00A0}
\pdfglyphtounicode{U}{00A0}
\pdfglyphtounicode{Uacute}{00A0}
\pdfglyphtounicode{Uacutesmall}{00A0}
\pdfglyphtounicode{Ubreve}{00A0}
\pdfglyphtounicode{Ucaron}{00A0}
\pdfglyphtounicode{Ucircle}{00A0}
\pdfglyphtounicode{Ucircumflex}{00A0}
\pdfglyphtounicode{Ucircumflexbelow}{00A0}
\pdfglyphtounicode{Ucircumflexsmall}{00A0}
\pdfglyphtounicode{Ucyrillic}{00A0}
\pdfglyphtounicode{Udblacute}{00A0}
\pdfglyphtounicode{Udblgrave}{00A0}
\pdfglyphtounicode{Udieresis}{00A0}
\pdfglyphtounicode{Udieresisacute}{00A0}
\pdfglyphtounicode{Udieresisbelow}{00A0}
\pdfglyphtounicode{Udieresiscaron}{00A0}
\pdfglyphtounicode{Udieresiscyrillic}{00A0}
\pdfglyphtounicode{Udieresisgrave}{00A0}
\pdfglyphtounicode{Udieresismacron}{00A0}
\pdfglyphtounicode{Udieresissmall}{00A0}
\pdfglyphtounicode{Udotbelow}{00A0}
\pdfglyphtounicode{Ugrave}{00A0}
\pdfglyphtounicode{Ugravesmall}{00A0}
\pdfglyphtounicode{Uhookabove}{00A0}
\pdfglyphtounicode{Uhorn}{00A0}
\pdfglyphtounicode{Uhornacute}{00A0}
\pdfglyphtounicode{Uhorndotbelow}{00A0}
\pdfglyphtounicode{Uhorngrave}{00A0}
\pdfglyphtounicode{Uhornhookabove}{00A0}
\pdfglyphtounicode{Uhorntilde}{00A0}
\pdfglyphtounicode{Uhungarumlaut}{00A0}
\pdfglyphtounicode{Uhungarumlautcyrillic}{00A0}
\pdfglyphtounicode{Uinvertedbreve}{00A0}
\pdfglyphtounicode{Ukcyrillic}{00A0}
\pdfglyphtounicode{Umacron}{00A0}
\pdfglyphtounicode{Umacroncyrillic}{00A0}
\pdfglyphtounicode{Umacrondieresis}{00A0}
\pdfglyphtounicode{Umonospace}{00A0}
\pdfglyphtounicode{Uogonek}{00A0}
\pdfglyphtounicode{Upsilon}{00A0}
\pdfglyphtounicode{Upsilon1}{00A0}
\pdfglyphtounicode{Upsilonacutehooksymbolgreek}{00A0}
\pdfglyphtounicode{Upsilonafrican}{00A0}
\pdfglyphtounicode{Upsilondieresis}{00A0}
\pdfglyphtounicode{Upsilondieresishooksymbolgreek}{00A0}
\pdfglyphtounicode{Upsilonhooksymbol}{00A0}
\pdfglyphtounicode{Upsilontonos}{00A0}
\pdfglyphtounicode{Uring}{00A0}
\pdfglyphtounicode{Ushortcyrillic}{00A0}
\pdfglyphtounicode{Usmall}{00A0}
\pdfglyphtounicode{Ustraightcyrillic}{00A0}
\pdfglyphtounicode{Ustraightstrokecyrillic}{00A0}
\pdfglyphtounicode{Utilde}{00A0}
\pdfglyphtounicode{Utildeacute}{00A0}
\pdfglyphtounicode{Utildebelow}{00A0}
\pdfglyphtounicode{V}{00A0}
\pdfglyphtounicode{Vcircle}{00A0}
\pdfglyphtounicode{Vdotbelow}{00A0}
\pdfglyphtounicode{Vecyrillic}{00A0}
\pdfglyphtounicode{Vewarmenian}{00A0}
\pdfglyphtounicode{Vhook}{00A0}
\pdfglyphtounicode{Vmonospace}{00A0}
\pdfglyphtounicode{Voarmenian}{00A0}
\pdfglyphtounicode{Vsmall}{00A0}
\pdfglyphtounicode{Vtilde}{00A0}
\pdfglyphtounicode{W}{00A0}
\pdfglyphtounicode{Wacute}{00A0}
\pdfglyphtounicode{Wcircle}{00A0}
\pdfglyphtounicode{Wcircumflex}{00A0}
\pdfglyphtounicode{Wdieresis}{00A0}
\pdfglyphtounicode{Wdotaccent}{00A0}
\pdfglyphtounicode{Wdotbelow}{00A0}
\pdfglyphtounicode{Wgrave}{00A0}
\pdfglyphtounicode{Wmonospace}{00A0}
\pdfglyphtounicode{Wsmall}{00A0}
\pdfglyphtounicode{X}{00A0}
\pdfglyphtounicode{Xcircle}{00A0}
\pdfglyphtounicode{Xdieresis}{00A0}
\pdfglyphtounicode{Xdotaccent}{00A0}
\pdfglyphtounicode{Xeharmenian}{00A0}
\pdfglyphtounicode{Xi}{00A0}
\pdfglyphtounicode{Xmonospace}{00A0}
\pdfglyphtounicode{Xsmall}{00A0}
\pdfglyphtounicode{Y}{00A0}
\pdfglyphtounicode{Yacute}{00A0}
\pdfglyphtounicode{Yacutesmall}{00A0}
\pdfglyphtounicode{Yatcyrillic}{00A0}
\pdfglyphtounicode{Ycircle}{00A0}
\pdfglyphtounicode{Ycircumflex}{00A0}
\pdfglyphtounicode{Ydieresis}{00A0}
\pdfglyphtounicode{Ydieresissmall}{00A0}
\pdfglyphtounicode{Ydotaccent}{00A0}
\pdfglyphtounicode{Ydotbelow}{00A0}
\pdfglyphtounicode{Yen}{00A0}
\pdfglyphtounicode{Yericyrillic}{00A0}
\pdfglyphtounicode{Yerudieresiscyrillic}{00A0}
\pdfglyphtounicode{Ygrave}{00A0}
\pdfglyphtounicode{Yhook}{00A0}
\pdfglyphtounicode{Yhookabove}{00A0}
\pdfglyphtounicode{Yiarmenian}{00A0}
\pdfglyphtounicode{Yicyrillic}{00A0}
\pdfglyphtounicode{Yiwnarmenian}{00A0}
\pdfglyphtounicode{Ymonospace}{00A0}
\pdfglyphtounicode{Ysmall}{00A0}
\pdfglyphtounicode{Ytilde}{00A0}
\pdfglyphtounicode{Yusbigcyrillic}{00A0}
\pdfglyphtounicode{Yusbigiotifiedcyrillic}{00A0}
\pdfglyphtounicode{Yuslittlecyrillic}{00A0}
\pdfglyphtounicode{Yuslittleiotifiedcyrillic}{00A0}
\pdfglyphtounicode{Z}{00A0}
\pdfglyphtounicode{Zaarmenian}{00A0}
\pdfglyphtounicode{Zacute}{00A0}
\pdfglyphtounicode{Zcaron}{00A0}
\pdfglyphtounicode{Zcaronsmall}{00A0}
\pdfglyphtounicode{Zcircle}{00A0}
\pdfglyphtounicode{Zcircumflex}{00A0}
\pdfglyphtounicode{Zdot}{00A0}
\pdfglyphtounicode{Zdotaccent}{00A0}
\pdfglyphtounicode{Zdotbelow}{00A0}
\pdfglyphtounicode{Zecyrillic}{00A0}
\pdfglyphtounicode{Zedescendercyrillic}{00A0}
\pdfglyphtounicode{Zedieresiscyrillic}{00A0}
\pdfglyphtounicode{Zeta}{00A0}
\pdfglyphtounicode{Zhearmenian}{00A0}
\pdfglyphtounicode{Zhebrevecyrillic}{00A0}
\pdfglyphtounicode{Zhecyrillic}{00A0}
\pdfglyphtounicode{Zhedescendercyrillic}{00A0}
\pdfglyphtounicode{Zhedieresiscyrillic}{00A0}
\pdfglyphtounicode{Zlinebelow}{00A0}
\pdfglyphtounicode{Zmonospace}{00A0}
\pdfglyphtounicode{Zsmall}{00A0}
\pdfglyphtounicode{Zstroke}{00A0}
\pdfglyphtounicode{a}{00A0}
\pdfglyphtounicode{aabengali}{00A0}
\pdfglyphtounicode{aacute}{00A0}
\pdfglyphtounicode{aadeva}{00A0}
\pdfglyphtounicode{aagujarati}{00A0}
\pdfglyphtounicode{aagurmukhi}{00A0}
\pdfglyphtounicode{aamatragurmukhi}{00A0}
\pdfglyphtounicode{aarusquare}{00A0}
\pdfglyphtounicode{aavowelsignbengali}{00A0}
\pdfglyphtounicode{aavowelsigndeva}{00A0}
\pdfglyphtounicode{aavowelsigngujarati}{00A0}
\pdfglyphtounicode{abbreviationmarkarmenian}{00A0}
\pdfglyphtounicode{abbreviationsigndeva}{00A0}
\pdfglyphtounicode{abengali}{00A0}
\pdfglyphtounicode{abopomofo}{00A0}
\pdfglyphtounicode{abreve}{00A0}
\pdfglyphtounicode{abreveacute}{00A0}
\pdfglyphtounicode{abrevecyrillic}{00A0}
\pdfglyphtounicode{abrevedotbelow}{00A0}
\pdfglyphtounicode{abrevegrave}{00A0}
\pdfglyphtounicode{abrevehookabove}{00A0}
\pdfglyphtounicode{abrevetilde}{00A0}
\pdfglyphtounicode{acaron}{00A0}
\pdfglyphtounicode{acircle}{00A0}
\pdfglyphtounicode{acircumflex}{00A0}
\pdfglyphtounicode{acircumflexacute}{00A0}
\pdfglyphtounicode{acircumflexdotbelow}{00A0}
\pdfglyphtounicode{acircumflexgrave}{00A0}
\pdfglyphtounicode{acircumflexhookabove}{00A0}
\pdfglyphtounicode{acircumflextilde}{00A0}
\pdfglyphtounicode{acute}{00A0}
\pdfglyphtounicode{acutebelowcmb}{00A0}
\pdfglyphtounicode{acutecmb}{00A0}
\pdfglyphtounicode{acutecomb}{00A0}
\pdfglyphtounicode{acutedeva}{00A0}
\pdfglyphtounicode{acutelowmod}{00A0}
\pdfglyphtounicode{acutetonecmb}{00A0}
\pdfglyphtounicode{acyrillic}{00A0}
\pdfglyphtounicode{adblgrave}{00A0}
\pdfglyphtounicode{addakgurmukhi}{00A0}
\pdfglyphtounicode{adeva}{00A0}
\pdfglyphtounicode{adieresis}{00A0}
\pdfglyphtounicode{adieresiscyrillic}{00A0}
\pdfglyphtounicode{adieresismacron}{00A0}
\pdfglyphtounicode{adotbelow}{00A0}
\pdfglyphtounicode{adotmacron}{00A0}
\pdfglyphtounicode{ae}{00A0}
\pdfglyphtounicode{aeacute}{00A0}
\pdfglyphtounicode{aekorean}{00A0}
\pdfglyphtounicode{aemacron}{00A0}
\pdfglyphtounicode{afii00208}{00A0}
\pdfglyphtounicode{afii08941}{00A0}
\pdfglyphtounicode{afii10017}{00A0}
\pdfglyphtounicode{afii10018}{00A0}
\pdfglyphtounicode{afii10019}{00A0}
\pdfglyphtounicode{afii10020}{00A0}
\pdfglyphtounicode{afii10021}{00A0}
\pdfglyphtounicode{afii10022}{00A0}
\pdfglyphtounicode{afii10023}{00A0}
\pdfglyphtounicode{afii10024}{00A0}
\pdfglyphtounicode{afii10025}{00A0}
\pdfglyphtounicode{afii10026}{00A0}
\pdfglyphtounicode{afii10027}{00A0}
\pdfglyphtounicode{afii10028}{00A0}
\pdfglyphtounicode{afii10029}{00A0}
\pdfglyphtounicode{afii10030}{00A0}
\pdfglyphtounicode{afii10031}{00A0}
\pdfglyphtounicode{afii10032}{00A0}
\pdfglyphtounicode{afii10033}{00A0}
\pdfglyphtounicode{afii10034}{00A0}
\pdfglyphtounicode{afii10035}{00A0}
\pdfglyphtounicode{afii10036}{00A0}
\pdfglyphtounicode{afii10037}{00A0}
\pdfglyphtounicode{afii10038}{00A0}
\pdfglyphtounicode{afii10039}{00A0}
\pdfglyphtounicode{afii10040}{00A0}
\pdfglyphtounicode{afii10041}{00A0}
\pdfglyphtounicode{afii10042}{00A0}
\pdfglyphtounicode{afii10043}{00A0}
\pdfglyphtounicode{afii10044}{00A0}
\pdfglyphtounicode{afii10045}{00A0}
\pdfglyphtounicode{afii10046}{00A0}
\pdfglyphtounicode{afii10047}{00A0}
\pdfglyphtounicode{afii10048}{00A0}
\pdfglyphtounicode{afii10049}{00A0}
\pdfglyphtounicode{afii10050}{00A0}
\pdfglyphtounicode{afii10051}{00A0}
\pdfglyphtounicode{afii10052}{00A0}
\pdfglyphtounicode{afii10053}{00A0}
\pdfglyphtounicode{afii10054}{00A0}
\pdfglyphtounicode{afii10055}{00A0}
\pdfglyphtounicode{afii10056}{00A0}
\pdfglyphtounicode{afii10057}{00A0}
\pdfglyphtounicode{afii10058}{00A0}
\pdfglyphtounicode{afii10059}{00A0}
\pdfglyphtounicode{afii10060}{00A0}
\pdfglyphtounicode{afii10061}{00A0}
\pdfglyphtounicode{afii10062}{00A0}
\pdfglyphtounicode{afii10063}{00A0}
\pdfglyphtounicode{afii10064}{00A0}
\pdfglyphtounicode{afii10065}{00A0}
\pdfglyphtounicode{afii10066}{00A0}
\pdfglyphtounicode{afii10067}{00A0}
\pdfglyphtounicode{afii10068}{00A0}
\pdfglyphtounicode{afii10069}{00A0}
\pdfglyphtounicode{afii10070}{00A0}
\pdfglyphtounicode{afii10071}{00A0}
\pdfglyphtounicode{afii10072}{00A0}
\pdfglyphtounicode{afii10073}{00A0}
\pdfglyphtounicode{afii10074}{00A0}
\pdfglyphtounicode{afii10075}{00A0}
\pdfglyphtounicode{afii10076}{00A0}
\pdfglyphtounicode{afii10077}{00A0}
\pdfglyphtounicode{afii10078}{00A0}
\pdfglyphtounicode{afii10079}{00A0}
\pdfglyphtounicode{afii10080}{00A0}
\pdfglyphtounicode{afii10081}{00A0}
\pdfglyphtounicode{afii10082}{00A0}
\pdfglyphtounicode{afii10083}{00A0}
\pdfglyphtounicode{afii10084}{00A0}
\pdfglyphtounicode{afii10085}{00A0}
\pdfglyphtounicode{afii10086}{00A0}
\pdfglyphtounicode{afii10087}{00A0}
\pdfglyphtounicode{afii10088}{00A0}
\pdfglyphtounicode{afii10089}{00A0}
\pdfglyphtounicode{afii10090}{00A0}
\pdfglyphtounicode{afii10091}{00A0}
\pdfglyphtounicode{afii10092}{00A0}
\pdfglyphtounicode{afii10093}{00A0}
\pdfglyphtounicode{afii10094}{00A0}
\pdfglyphtounicode{afii10095}{00A0}
\pdfglyphtounicode{afii10096}{00A0}
\pdfglyphtounicode{afii10097}{00A0}
\pdfglyphtounicode{afii10098}{00A0}
\pdfglyphtounicode{afii10099}{00A0}
\pdfglyphtounicode{afii10100}{00A0}
\pdfglyphtounicode{afii10101}{00A0}
\pdfglyphtounicode{afii10102}{00A0}
\pdfglyphtounicode{afii10103}{00A0}
\pdfglyphtounicode{afii10104}{00A0}
\pdfglyphtounicode{afii10105}{00A0}
\pdfglyphtounicode{afii10106}{00A0}
\pdfglyphtounicode{afii10107}{00A0}
\pdfglyphtounicode{afii10108}{00A0}
\pdfglyphtounicode{afii10109}{00A0}
\pdfglyphtounicode{afii10110}{00A0}
\pdfglyphtounicode{afii10145}{00A0}
\pdfglyphtounicode{afii10146}{00A0}
\pdfglyphtounicode{afii10147}{00A0}
\pdfglyphtounicode{afii10148}{00A0}
\pdfglyphtounicode{afii10192}{00A0}
\pdfglyphtounicode{afii10193}{00A0}
\pdfglyphtounicode{afii10194}{00A0}
\pdfglyphtounicode{afii10195}{00A0}
\pdfglyphtounicode{afii10196}{00A0}
\pdfglyphtounicode{afii10831}{00A0}
\pdfglyphtounicode{afii10832}{00A0}
\pdfglyphtounicode{afii10846}{00A0}
\pdfglyphtounicode{afii299}{00A0}
\pdfglyphtounicode{afii300}{00A0}
\pdfglyphtounicode{afii301}{00A0}
\pdfglyphtounicode{afii57381}{00A0}
\pdfglyphtounicode{afii57388}{00A0}
\pdfglyphtounicode{afii57392}{00A0}
\pdfglyphtounicode{afii57393}{00A0}
\pdfglyphtounicode{afii57394}{00A0}
\pdfglyphtounicode{afii57395}{00A0}
\pdfglyphtounicode{afii57396}{00A0}
\pdfglyphtounicode{afii57397}{00A0}
\pdfglyphtounicode{afii57398}{00A0}
\pdfglyphtounicode{afii57399}{00A0}
\pdfglyphtounicode{afii57400}{00A0}
\pdfglyphtounicode{afii57401}{00A0}
\pdfglyphtounicode{afii57403}{00A0}
\pdfglyphtounicode{afii57407}{00A0}
\pdfglyphtounicode{afii57409}{00A0}
\pdfglyphtounicode{afii57410}{00A0}
\pdfglyphtounicode{afii57411}{00A0}
\pdfglyphtounicode{afii57412}{00A0}
\pdfglyphtounicode{afii57413}{00A0}
\pdfglyphtounicode{afii57414}{00A0}
\pdfglyphtounicode{afii57415}{00A0}
\pdfglyphtounicode{afii57416}{00A0}
\pdfglyphtounicode{afii57417}{00A0}
\pdfglyphtounicode{afii57418}{00A0}
\pdfglyphtounicode{afii57419}{00A0}
\pdfglyphtounicode{afii57420}{00A0}
\pdfglyphtounicode{afii57421}{00A0}
\pdfglyphtounicode{afii57422}{00A0}
\pdfglyphtounicode{afii57423}{00A0}
\pdfglyphtounicode{afii57424}{00A0}
\pdfglyphtounicode{afii57425}{00A0}
\pdfglyphtounicode{afii57426}{00A0}
\pdfglyphtounicode{afii57427}{00A0}
\pdfglyphtounicode{afii57428}{00A0}
\pdfglyphtounicode{afii57429}{00A0}
\pdfglyphtounicode{afii57430}{00A0}
\pdfglyphtounicode{afii57431}{00A0}
\pdfglyphtounicode{afii57432}{00A0}
\pdfglyphtounicode{afii57433}{00A0}
\pdfglyphtounicode{afii57434}{00A0}
\pdfglyphtounicode{afii57440}{00A0}
\pdfglyphtounicode{afii57441}{00A0}
\pdfglyphtounicode{afii57442}{00A0}
\pdfglyphtounicode{afii57443}{00A0}
\pdfglyphtounicode{afii57444}{00A0}
\pdfglyphtounicode{afii57445}{00A0}
\pdfglyphtounicode{afii57446}{00A0}
\pdfglyphtounicode{afii57448}{00A0}
\pdfglyphtounicode{afii57449}{00A0}
\pdfglyphtounicode{afii57450}{00A0}
\pdfglyphtounicode{afii57451}{00A0}
\pdfglyphtounicode{afii57452}{00A0}
\pdfglyphtounicode{afii57453}{00A0}
\pdfglyphtounicode{afii57454}{00A0}
\pdfglyphtounicode{afii57455}{00A0}
\pdfglyphtounicode{afii57456}{00A0}
\pdfglyphtounicode{afii57457}{00A0}
\pdfglyphtounicode{afii57458}{00A0}
\pdfglyphtounicode{afii57470}{00A0}
\pdfglyphtounicode{afii57505}{00A0}
\pdfglyphtounicode{afii57506}{00A0}
\pdfglyphtounicode{afii57507}{00A0}
\pdfglyphtounicode{afii57508}{00A0}
\pdfglyphtounicode{afii57509}{00A0}
\pdfglyphtounicode{afii57511}{00A0}
\pdfglyphtounicode{afii57512}{00A0}
\pdfglyphtounicode{afii57513}{00A0}
\pdfglyphtounicode{afii57514}{00A0}
\pdfglyphtounicode{afii57519}{00A0}
\pdfglyphtounicode{afii57534}{00A0}
\pdfglyphtounicode{afii57636}{00A0}
\pdfglyphtounicode{afii57645}{00A0}
\pdfglyphtounicode{afii57658}{00A0}
\pdfglyphtounicode{afii57664}{00A0}
\pdfglyphtounicode{afii57665}{00A0}
\pdfglyphtounicode{afii57666}{00A0}
\pdfglyphtounicode{afii57667}{00A0}
\pdfglyphtounicode{afii57668}{00A0}
\pdfglyphtounicode{afii57669}{00A0}
\pdfglyphtounicode{afii57670}{00A0}
\pdfglyphtounicode{afii57671}{00A0}
\pdfglyphtounicode{afii57672}{00A0}
\pdfglyphtounicode{afii57673}{00A0}
\pdfglyphtounicode{afii57674}{00A0}
\pdfglyphtounicode{afii57675}{00A0}
\pdfglyphtounicode{afii57676}{00A0}
\pdfglyphtounicode{afii57677}{00A0}
\pdfglyphtounicode{afii57678}{00A0}
\pdfglyphtounicode{afii57679}{00A0}
\pdfglyphtounicode{afii57680}{00A0}
\pdfglyphtounicode{afii57681}{00A0}
\pdfglyphtounicode{afii57682}{00A0}
\pdfglyphtounicode{afii57683}{00A0}
\pdfglyphtounicode{afii57684}{00A0}
\pdfglyphtounicode{afii57685}{00A0}
\pdfglyphtounicode{afii57686}{00A0}
\pdfglyphtounicode{afii57687}{00A0}
\pdfglyphtounicode{afii57688}{00A0}
\pdfglyphtounicode{afii57689}{00A0}
\pdfglyphtounicode{afii57690}{00A0}
\pdfglyphtounicode{afii57694}{00A0}
\pdfglyphtounicode{afii57695}{00A0}
\pdfglyphtounicode{afii57700}{00A0}
\pdfglyphtounicode{afii57705}{00A0}
\pdfglyphtounicode{afii57716}{00A0}
\pdfglyphtounicode{afii57717}{00A0}
\pdfglyphtounicode{afii57718}{00A0}
\pdfglyphtounicode{afii57723}{00A0}
\pdfglyphtounicode{afii57793}{00A0}
\pdfglyphtounicode{afii57794}{00A0}
\pdfglyphtounicode{afii57795}{00A0}
\pdfglyphtounicode{afii57796}{00A0}
\pdfglyphtounicode{afii57797}{00A0}
\pdfglyphtounicode{afii57798}{00A0}
\pdfglyphtounicode{afii57799}{00A0}
\pdfglyphtounicode{afii57800}{00A0}
\pdfglyphtounicode{afii57801}{00A0}
\pdfglyphtounicode{afii57802}{00A0}
\pdfglyphtounicode{afii57803}{00A0}
\pdfglyphtounicode{afii57804}{00A0}
\pdfglyphtounicode{afii57806}{00A0}
\pdfglyphtounicode{afii57807}{00A0}
\pdfglyphtounicode{afii57839}{00A0}
\pdfglyphtounicode{afii57841}{00A0}
\pdfglyphtounicode{afii57842}{00A0}
\pdfglyphtounicode{afii57929}{00A0}
\pdfglyphtounicode{afii61248}{00A0}
\pdfglyphtounicode{afii61289}{00A0}
\pdfglyphtounicode{afii61352}{00A0}
\pdfglyphtounicode{afii61573}{00A0}
\pdfglyphtounicode{afii61574}{00A0}
\pdfglyphtounicode{afii61575}{00A0}
\pdfglyphtounicode{afii61664}{00A0}
\pdfglyphtounicode{afii63167}{00A0}
\pdfglyphtounicode{afii64937}{00A0}
\pdfglyphtounicode{agrave}{00A0}
\pdfglyphtounicode{agujarati}{00A0}
\pdfglyphtounicode{agurmukhi}{00A0}
\pdfglyphtounicode{ahiragana}{00A0}
\pdfglyphtounicode{ahookabove}{00A0}
\pdfglyphtounicode{aibengali}{00A0}
\pdfglyphtounicode{aibopomofo}{00A0}
\pdfglyphtounicode{aideva}{00A0}
\pdfglyphtounicode{aiecyrillic}{00A0}
\pdfglyphtounicode{aigujarati}{00A0}
\pdfglyphtounicode{aigurmukhi}{00A0}
\pdfglyphtounicode{aimatragurmukhi}{00A0}
\pdfglyphtounicode{ainarabic}{00A0}
\pdfglyphtounicode{ainfinalarabic}{00A0}
\pdfglyphtounicode{aininitialarabic}{00A0}
\pdfglyphtounicode{ainmedialarabic}{00A0}
\pdfglyphtounicode{ainvertedbreve}{00A0}
\pdfglyphtounicode{aivowelsignbengali}{00A0}
\pdfglyphtounicode{aivowelsigndeva}{00A0}
\pdfglyphtounicode{aivowelsigngujarati}{00A0}
\pdfglyphtounicode{akatakana}{00A0}
\pdfglyphtounicode{akatakanahalfwidth}{00A0}
\pdfglyphtounicode{akorean}{00A0}
\pdfglyphtounicode{alef}{00A0}
\pdfglyphtounicode{alefarabic}{00A0}
\pdfglyphtounicode{alefdageshhebrew}{00A0}
\pdfglyphtounicode{aleffinalarabic}{00A0}
\pdfglyphtounicode{alefhamzaabovearabic}{00A0}
\pdfglyphtounicode{alefhamzaabovefinalarabic}{00A0}
\pdfglyphtounicode{alefhamzabelowarabic}{00A0}
\pdfglyphtounicode{alefhamzabelowfinalarabic}{00A0}
\pdfglyphtounicode{alefhebrew}{00A0}
\pdfglyphtounicode{aleflamedhebrew}{00A0}
\pdfglyphtounicode{alefmaddaabovearabic}{00A0}
\pdfglyphtounicode{alefmaddaabovefinalarabic}{00A0}
\pdfglyphtounicode{alefmaksuraarabic}{00A0}
\pdfglyphtounicode{alefmaksurafinalarabic}{00A0}
\pdfglyphtounicode{alefmaksurainitialarabic}{00A0}
\pdfglyphtounicode{alefmaksuramedialarabic}{00A0}
\pdfglyphtounicode{alefpatahhebrew}{00A0}
\pdfglyphtounicode{alefqamatshebrew}{00A0}
\pdfglyphtounicode{aleph}{00A0}
\pdfglyphtounicode{allequal}{00A0}
\pdfglyphtounicode{alpha}{00A0}
\pdfglyphtounicode{alphatonos}{00A0}
\pdfglyphtounicode{amacron}{00A0}
\pdfglyphtounicode{amonospace}{00A0}
\pdfglyphtounicode{ampersand}{00A0}
\pdfglyphtounicode{ampersandmonospace}{00A0}
\pdfglyphtounicode{ampersandsmall}{00A0}
\pdfglyphtounicode{amsquare}{00A0}
\pdfglyphtounicode{anbopomofo}{00A0}
\pdfglyphtounicode{angbopomofo}{00A0}
\pdfglyphtounicode{angbracketleft}{00A0}
\pdfglyphtounicode{angbracketright}{00A0}
\pdfglyphtounicode{angkhankhuthai}{00A0}
\pdfglyphtounicode{angle}{00A0}
\pdfglyphtounicode{anglebracketleft}{00A0}
\pdfglyphtounicode{anglebracketleftvertical}{00A0}
\pdfglyphtounicode{anglebracketright}{00A0}
\pdfglyphtounicode{anglebracketrightvertical}{00A0}
\pdfglyphtounicode{angleleft}{00A0}
\pdfglyphtounicode{angleright}{00A0}
\pdfglyphtounicode{angstrom}{00A0}
\pdfglyphtounicode{anoteleia}{00A0}
\pdfglyphtounicode{anticlockwise}{00A0}
\pdfglyphtounicode{anudattadeva}{00A0}
\pdfglyphtounicode{anusvarabengali}{00A0}
\pdfglyphtounicode{anusvaradeva}{00A0}
\pdfglyphtounicode{anusvaragujarati}{00A0}
\pdfglyphtounicode{aogonek}{00A0}
\pdfglyphtounicode{apaatosquare}{00A0}
\pdfglyphtounicode{aparen}{00A0}
\pdfglyphtounicode{apostrophearmenian}{00A0}
\pdfglyphtounicode{apostrophemod}{00A0}
\pdfglyphtounicode{apple}{00A0}
\pdfglyphtounicode{approaches}{00A0}
\pdfglyphtounicode{approxequal}{00A0}
\pdfglyphtounicode{approxequalorimage}{00A0}
\pdfglyphtounicode{approximatelyequal}{00A0}
\pdfglyphtounicode{approxorequal}{00A0}
\pdfglyphtounicode{araeaekorean}{00A0}
\pdfglyphtounicode{araeakorean}{00A0}
\pdfglyphtounicode{arc}{00A0}
\pdfglyphtounicode{archleftdown}{00A0}
\pdfglyphtounicode{archrightdown}{00A0}
\pdfglyphtounicode{arighthalfring}{00A0}
\pdfglyphtounicode{aring}{00A0}
\pdfglyphtounicode{aringacute}{00A0}
\pdfglyphtounicode{aringbelow}{00A0}
\pdfglyphtounicode{arrowboth}{00A0}
\pdfglyphtounicode{arrowbothv}{00A0}
\pdfglyphtounicode{arrowdashdown}{00A0}
\pdfglyphtounicode{arrowdashleft}{00A0}
\pdfglyphtounicode{arrowdashright}{00A0}
\pdfglyphtounicode{arrowdashup}{00A0}
\pdfglyphtounicode{arrowdblboth}{00A0}
\pdfglyphtounicode{arrowdblbothv}{00A0}
\pdfglyphtounicode{arrowdbldown}{00A0}
\pdfglyphtounicode{arrowdblleft}{00A0}
\pdfglyphtounicode{arrowdblright}{00A0}
\pdfglyphtounicode{arrowdblup}{00A0}
\pdfglyphtounicode{arrowdown}{00A0}
\pdfglyphtounicode{arrowdownleft}{00A0}
\pdfglyphtounicode{arrowdownright}{00A0}
\pdfglyphtounicode{arrowdownwhite}{00A0}
\pdfglyphtounicode{arrowheaddownmod}{00A0}
\pdfglyphtounicode{arrowheadleftmod}{00A0}
\pdfglyphtounicode{arrowheadrightmod}{00A0}
\pdfglyphtounicode{arrowheadupmod}{00A0}
\pdfglyphtounicode{arrowhorizex}{00A0}
\pdfglyphtounicode{arrowleft}{00A0}
\pdfglyphtounicode{arrowleftbothalf}{00A0}
\pdfglyphtounicode{arrowleftdbl}{00A0}
\pdfglyphtounicode{arrowleftdblstroke}{00A0}
\pdfglyphtounicode{arrowleftoverright}{00A0}
\pdfglyphtounicode{arrowlefttophalf}{00A0}
\pdfglyphtounicode{arrowleftwhite}{00A0}
\pdfglyphtounicode{arrownortheast}{00A0}
\pdfglyphtounicode{arrownorthwest}{00A0}
\pdfglyphtounicode{arrowparrleftright}{00A0}
\pdfglyphtounicode{arrowparrrightleft}{00A0}
\pdfglyphtounicode{arrowright}{00A0}
\pdfglyphtounicode{arrowrightbothalf}{00A0}
\pdfglyphtounicode{arrowrightdblstroke}{00A0}
\pdfglyphtounicode{arrowrightheavy}{00A0}
\pdfglyphtounicode{arrowrightoverleft}{00A0}
\pdfglyphtounicode{arrowrighttophalf}{00A0}
\pdfglyphtounicode{arrowrightwhite}{00A0}
\pdfglyphtounicode{arrowsoutheast}{00A0}
\pdfglyphtounicode{arrowsouthwest}{00A0}
\pdfglyphtounicode{arrowtableft}{00A0}
\pdfglyphtounicode{arrowtabright}{00A0}
\pdfglyphtounicode{arrowtailleft}{00A0}
\pdfglyphtounicode{arrowtailright}{00A0}
\pdfglyphtounicode{arrowtripleleft}{00A0}
\pdfglyphtounicode{arrowtripleright}{00A0}
\pdfglyphtounicode{arrowup}{00A0}
\pdfglyphtounicode{arrowupdn}{00A0}
\pdfglyphtounicode{arrowupdnbse}{00A0}
\pdfglyphtounicode{arrowupdownbase}{00A0}
\pdfglyphtounicode{arrowupleft}{00A0}
\pdfglyphtounicode{arrowupleftofdown}{00A0}
\pdfglyphtounicode{arrowupright}{00A0}
\pdfglyphtounicode{arrowupwhite}{00A0}
\pdfglyphtounicode{arrowvertex}{00A0}
\pdfglyphtounicode{asciicircum}{00A0}
\pdfglyphtounicode{asciicircummonospace}{00A0}
\pdfglyphtounicode{asciitilde}{00A0}
\pdfglyphtounicode{asciitildemonospace}{00A0}
\pdfglyphtounicode{ascript}{00A0}
\pdfglyphtounicode{ascriptturned}{00A0}
\pdfglyphtounicode{asmallhiragana}{00A0}
\pdfglyphtounicode{asmallkatakana}{00A0}
\pdfglyphtounicode{asmallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{asterisk}{00A0}
\pdfglyphtounicode{asteriskaltonearabic}{00A0}
\pdfglyphtounicode{asteriskarabic}{00A0}
\pdfglyphtounicode{asteriskcentered}{00A0}
\pdfglyphtounicode{asteriskmath}{00A0}
\pdfglyphtounicode{asteriskmonospace}{00A0}
\pdfglyphtounicode{asterisksmall}{00A0}
\pdfglyphtounicode{asterism}{00A0}
\pdfglyphtounicode{asuperior}{00A0}
\pdfglyphtounicode{asymptoticallyequal}{00A0}
\pdfglyphtounicode{at}{00A0}
\pdfglyphtounicode{atilde}{00A0}
\pdfglyphtounicode{atmonospace}{00A0}
\pdfglyphtounicode{atsmall}{00A0}
\pdfglyphtounicode{aturned}{00A0}
\pdfglyphtounicode{aubengali}{00A0}
\pdfglyphtounicode{aubopomofo}{00A0}
\pdfglyphtounicode{audeva}{00A0}
\pdfglyphtounicode{augujarati}{00A0}
\pdfglyphtounicode{augurmukhi}{00A0}
\pdfglyphtounicode{aulengthmarkbengali}{00A0}
\pdfglyphtounicode{aumatragurmukhi}{00A0}
\pdfglyphtounicode{auvowelsignbengali}{00A0}
\pdfglyphtounicode{auvowelsigndeva}{00A0}
\pdfglyphtounicode{auvowelsigngujarati}{00A0}
\pdfglyphtounicode{avagrahadeva}{00A0}
\pdfglyphtounicode{aybarmenian}{00A0}
\pdfglyphtounicode{ayin}{00A0}
\pdfglyphtounicode{ayinaltonehebrew}{00A0}
\pdfglyphtounicode{ayinhebrew}{00A0}
\pdfglyphtounicode{b}{00A0}
\pdfglyphtounicode{babengali}{00A0}
\pdfglyphtounicode{backslash}{00A0}
\pdfglyphtounicode{backslashmonospace}{00A0}
\pdfglyphtounicode{badeva}{00A0}
\pdfglyphtounicode{bagujarati}{00A0}
\pdfglyphtounicode{bagurmukhi}{00A0}
\pdfglyphtounicode{bahiragana}{00A0}
\pdfglyphtounicode{bahtthai}{00A0}
\pdfglyphtounicode{bakatakana}{00A0}
\pdfglyphtounicode{bar}{00A0}
\pdfglyphtounicode{bardbl}{00A0}
\pdfglyphtounicode{barmonospace}{00A0}
\pdfglyphtounicode{bbopomofo}{00A0}
\pdfglyphtounicode{bcircle}{00A0}
\pdfglyphtounicode{bdotaccent}{00A0}
\pdfglyphtounicode{bdotbelow}{00A0}
\pdfglyphtounicode{beamedsixteenthnotes}{00A0}
\pdfglyphtounicode{because}{00A0}
\pdfglyphtounicode{becyrillic}{00A0}
\pdfglyphtounicode{beharabic}{00A0}
\pdfglyphtounicode{behfinalarabic}{00A0}
\pdfglyphtounicode{behinitialarabic}{00A0}
\pdfglyphtounicode{behiragana}{00A0}
\pdfglyphtounicode{behmedialarabic}{00A0}
\pdfglyphtounicode{behmeeminitialarabic}{00A0}
\pdfglyphtounicode{behmeemisolatedarabic}{00A0}
\pdfglyphtounicode{behnoonfinalarabic}{00A0}
\pdfglyphtounicode{bekatakana}{00A0}
\pdfglyphtounicode{benarmenian}{00A0}
\pdfglyphtounicode{bet}{00A0}
\pdfglyphtounicode{beta}{00A0}
\pdfglyphtounicode{betasymbolgreek}{00A0}
\pdfglyphtounicode{betdagesh}{00A0}
\pdfglyphtounicode{betdageshhebrew}{00A0}
\pdfglyphtounicode{beth}{00A0}
\pdfglyphtounicode{bethebrew}{00A0}
\pdfglyphtounicode{betrafehebrew}{00A0}
\pdfglyphtounicode{between}{00A0}
\pdfglyphtounicode{bhabengali}{00A0}
\pdfglyphtounicode{bhadeva}{00A0}
\pdfglyphtounicode{bhagujarati}{00A0}
\pdfglyphtounicode{bhagurmukhi}{00A0}
\pdfglyphtounicode{bhook}{00A0}
\pdfglyphtounicode{bihiragana}{00A0}
\pdfglyphtounicode{bikatakana}{00A0}
\pdfglyphtounicode{bilabialclick}{00A0}
\pdfglyphtounicode{bindigurmukhi}{00A0}
\pdfglyphtounicode{birusquare}{00A0}
\pdfglyphtounicode{blackcircle}{00A0}
\pdfglyphtounicode{blackdiamond}{00A0}
\pdfglyphtounicode{blackdownpointingtriangle}{00A0}
\pdfglyphtounicode{blackleftpointingpointer}{00A0}
\pdfglyphtounicode{blackleftpointingtriangle}{00A0}
\pdfglyphtounicode{blacklenticularbracketleft}{00A0}
\pdfglyphtounicode{blacklenticularbracketleftvertical}{00A0}
\pdfglyphtounicode{blacklenticularbracketright}{00A0}
\pdfglyphtounicode{blacklenticularbracketrightvertical}{00A0}
\pdfglyphtounicode{blacklowerlefttriangle}{00A0}
\pdfglyphtounicode{blacklowerrighttriangle}{00A0}
\pdfglyphtounicode{blackrectangle}{00A0}
\pdfglyphtounicode{blackrightpointingpointer}{00A0}
\pdfglyphtounicode{blackrightpointingtriangle}{00A0}
\pdfglyphtounicode{blacksmallsquare}{00A0}
\pdfglyphtounicode{blacksmilingface}{00A0}
\pdfglyphtounicode{blacksquare}{00A0}
\pdfglyphtounicode{blackstar}{00A0}
\pdfglyphtounicode{blackupperlefttriangle}{00A0}
\pdfglyphtounicode{blackupperrighttriangle}{00A0}
\pdfglyphtounicode{blackuppointingsmalltriangle}{00A0}
\pdfglyphtounicode{blackuppointingtriangle}{00A0}
\pdfglyphtounicode{blank}{00A0}
\pdfglyphtounicode{blinebelow}{00A0}
\pdfglyphtounicode{block}{00A0}
\pdfglyphtounicode{bmonospace}{00A0}
\pdfglyphtounicode{bobaimaithai}{00A0}
\pdfglyphtounicode{bohiragana}{00A0}
\pdfglyphtounicode{bokatakana}{00A0}
\pdfglyphtounicode{bparen}{00A0}
\pdfglyphtounicode{bqsquare}{00A0}
\pdfglyphtounicode{braceex}{00A0}
\pdfglyphtounicode{braceleft}{00A0}
\pdfglyphtounicode{braceleftbt}{00A0}
\pdfglyphtounicode{braceleftmid}{00A0}
\pdfglyphtounicode{braceleftmonospace}{00A0}
\pdfglyphtounicode{braceleftsmall}{00A0}
\pdfglyphtounicode{bracelefttp}{00A0}
\pdfglyphtounicode{braceleftvertical}{00A0}
\pdfglyphtounicode{braceright}{00A0}
\pdfglyphtounicode{bracerightbt}{00A0}
\pdfglyphtounicode{bracerightmid}{00A0}
\pdfglyphtounicode{bracerightmonospace}{00A0}
\pdfglyphtounicode{bracerightsmall}{00A0}
\pdfglyphtounicode{bracerighttp}{00A0}
\pdfglyphtounicode{bracerightvertical}{00A0}
\pdfglyphtounicode{bracketleft}{00A0}
\pdfglyphtounicode{bracketleftbt}{00A0}
\pdfglyphtounicode{bracketleftex}{00A0}
\pdfglyphtounicode{bracketleftmonospace}{00A0}
\pdfglyphtounicode{bracketlefttp}{00A0}
\pdfglyphtounicode{bracketright}{00A0}
\pdfglyphtounicode{bracketrightbt}{00A0}
\pdfglyphtounicode{bracketrightex}{00A0}
\pdfglyphtounicode{bracketrightmonospace}{00A0}
\pdfglyphtounicode{bracketrighttp}{00A0}
\pdfglyphtounicode{breve}{00A0}
\pdfglyphtounicode{brevebelowcmb}{00A0}
\pdfglyphtounicode{brevecmb}{00A0}
\pdfglyphtounicode{breveinvertedbelowcmb}{00A0}
\pdfglyphtounicode{breveinvertedcmb}{00A0}
\pdfglyphtounicode{breveinverteddoublecmb}{00A0}
\pdfglyphtounicode{bridgebelowcmb}{00A0}
\pdfglyphtounicode{bridgeinvertedbelowcmb}{00A0}
\pdfglyphtounicode{brokenbar}{00A0}
\pdfglyphtounicode{bstroke}{00A0}
\pdfglyphtounicode{bsuperior}{00A0}
\pdfglyphtounicode{btopbar}{00A0}
\pdfglyphtounicode{buhiragana}{00A0}
\pdfglyphtounicode{bukatakana}{00A0}
\pdfglyphtounicode{bullet}{00A0}
\pdfglyphtounicode{bulletinverse}{00A0}
\pdfglyphtounicode{bulletoperator}{00A0}
\pdfglyphtounicode{bullseye}{00A0}
\pdfglyphtounicode{c}{00A0}
\pdfglyphtounicode{caarmenian}{00A0}
\pdfglyphtounicode{cabengali}{00A0}
\pdfglyphtounicode{cacute}{00A0}
\pdfglyphtounicode{cadeva}{00A0}
\pdfglyphtounicode{cagujarati}{00A0}
\pdfglyphtounicode{cagurmukhi}{00A0}
\pdfglyphtounicode{calsquare}{00A0}
\pdfglyphtounicode{candrabindubengali}{00A0}
\pdfglyphtounicode{candrabinducmb}{00A0}
\pdfglyphtounicode{candrabindudeva}{00A0}
\pdfglyphtounicode{candrabindugujarati}{00A0}
\pdfglyphtounicode{capslock}{00A0}
\pdfglyphtounicode{careof}{00A0}
\pdfglyphtounicode{caron}{00A0}
\pdfglyphtounicode{caronbelowcmb}{00A0}
\pdfglyphtounicode{caroncmb}{00A0}
\pdfglyphtounicode{carriagereturn}{00A0}
\pdfglyphtounicode{cbopomofo}{00A0}
\pdfglyphtounicode{ccaron}{00A0}
\pdfglyphtounicode{ccedilla}{00A0}
\pdfglyphtounicode{ccedillaacute}{00A0}
\pdfglyphtounicode{ccircle}{00A0}
\pdfglyphtounicode{ccircumflex}{00A0}
\pdfglyphtounicode{ccurl}{00A0}
\pdfglyphtounicode{cdot}{00A0}
\pdfglyphtounicode{cdotaccent}{00A0}
\pdfglyphtounicode{cdsquare}{00A0}
\pdfglyphtounicode{cedilla}{00A0}
\pdfglyphtounicode{cedillacmb}{00A0}
\pdfglyphtounicode{ceilingleft}{00A0}
\pdfglyphtounicode{ceilingright}{00A0}
\pdfglyphtounicode{cent}{00A0}
\pdfglyphtounicode{centigrade}{00A0}
\pdfglyphtounicode{centinferior}{00A0}
\pdfglyphtounicode{centmonospace}{00A0}
\pdfglyphtounicode{centoldstyle}{00A0}
\pdfglyphtounicode{centsuperior}{00A0}
\pdfglyphtounicode{chaarmenian}{00A0}
\pdfglyphtounicode{chabengali}{00A0}
\pdfglyphtounicode{chadeva}{00A0}
\pdfglyphtounicode{chagujarati}{00A0}
\pdfglyphtounicode{chagurmukhi}{00A0}
\pdfglyphtounicode{chbopomofo}{00A0}
\pdfglyphtounicode{cheabkhasiancyrillic}{00A0}
\pdfglyphtounicode{check}{00A0}
\pdfglyphtounicode{checkmark}{00A0}
\pdfglyphtounicode{checyrillic}{00A0}
\pdfglyphtounicode{chedescenderabkhasiancyrillic}{00A0}
\pdfglyphtounicode{chedescendercyrillic}{00A0}
\pdfglyphtounicode{chedieresiscyrillic}{00A0}
\pdfglyphtounicode{cheharmenian}{00A0}
\pdfglyphtounicode{chekhakassiancyrillic}{00A0}
\pdfglyphtounicode{cheverticalstrokecyrillic}{00A0}
\pdfglyphtounicode{chi}{00A0}
\pdfglyphtounicode{chieuchacirclekorean}{00A0}
\pdfglyphtounicode{chieuchaparenkorean}{00A0}
\pdfglyphtounicode{chieuchcirclekorean}{00A0}
\pdfglyphtounicode{chieuchkorean}{00A0}
\pdfglyphtounicode{chieuchparenkorean}{00A0}
\pdfglyphtounicode{chochangthai}{00A0}
\pdfglyphtounicode{chochanthai}{00A0}
\pdfglyphtounicode{chochingthai}{00A0}
\pdfglyphtounicode{chochoethai}{00A0}
\pdfglyphtounicode{chook}{00A0}
\pdfglyphtounicode{cieucacirclekorean}{00A0}
\pdfglyphtounicode{cieucaparenkorean}{00A0}
\pdfglyphtounicode{cieuccirclekorean}{00A0}
\pdfglyphtounicode{cieuckorean}{00A0}
\pdfglyphtounicode{cieucparenkorean}{00A0}
\pdfglyphtounicode{cieucuparenkorean}{00A0}
\pdfglyphtounicode{circle}{00A0}
\pdfglyphtounicode{circleR}{00A0}
\pdfglyphtounicode{circleS}{00A0}
\pdfglyphtounicode{circleasterisk}{00A0}
\pdfglyphtounicode{circlecopyrt}{00A0}
\pdfglyphtounicode{circledivide}{00A0}
\pdfglyphtounicode{circledot}{00A0}
\pdfglyphtounicode{circleequal}{00A0}
\pdfglyphtounicode{circleminus}{00A0}
\pdfglyphtounicode{circlemultiply}{00A0}
\pdfglyphtounicode{circleot}{00A0}
\pdfglyphtounicode{circleplus}{00A0}
\pdfglyphtounicode{circlepostalmark}{00A0}
\pdfglyphtounicode{circlering}{00A0}
\pdfglyphtounicode{circlewithlefthalfblack}{00A0}
\pdfglyphtounicode{circlewithrighthalfblack}{00A0}
\pdfglyphtounicode{circumflex}{00A0}
\pdfglyphtounicode{circumflexbelowcmb}{00A0}
\pdfglyphtounicode{circumflexcmb}{00A0}
\pdfglyphtounicode{clear}{00A0}
\pdfglyphtounicode{clickalveolar}{00A0}
\pdfglyphtounicode{clickdental}{00A0}
\pdfglyphtounicode{clicklateral}{00A0}
\pdfglyphtounicode{clickretroflex}{00A0}
\pdfglyphtounicode{clockwise}{00A0}
\pdfglyphtounicode{club}{00A0}
\pdfglyphtounicode{clubsuitblack}{00A0}
\pdfglyphtounicode{clubsuitwhite}{00A0}
\pdfglyphtounicode{cmcubedsquare}{00A0}
\pdfglyphtounicode{cmonospace}{00A0}
\pdfglyphtounicode{cmsquaredsquare}{00A0}
\pdfglyphtounicode{coarmenian}{00A0}
\pdfglyphtounicode{colon}{00A0}
\pdfglyphtounicode{colonmonetary}{00A0}
\pdfglyphtounicode{colonmonospace}{00A0}
\pdfglyphtounicode{colonsign}{00A0}
\pdfglyphtounicode{colonsmall}{00A0}
\pdfglyphtounicode{colontriangularhalfmod}{00A0}
\pdfglyphtounicode{colontriangularmod}{00A0}
\pdfglyphtounicode{comma}{00A0}
\pdfglyphtounicode{commaabovecmb}{00A0}
\pdfglyphtounicode{commaaboverightcmb}{00A0}
\pdfglyphtounicode{commaaccent}{00A0}
\pdfglyphtounicode{commaarabic}{00A0}
\pdfglyphtounicode{commaarmenian}{00A0}
\pdfglyphtounicode{commainferior}{00A0}
\pdfglyphtounicode{commamonospace}{00A0}
\pdfglyphtounicode{commareversedabovecmb}{00A0}
\pdfglyphtounicode{commareversedmod}{00A0}
\pdfglyphtounicode{commasmall}{00A0}
\pdfglyphtounicode{commasuperior}{00A0}
\pdfglyphtounicode{commaturnedabovecmb}{00A0}
\pdfglyphtounicode{commaturnedmod}{00A0}
\pdfglyphtounicode{compass}{00A0}
\pdfglyphtounicode{complement}{00A0}
\pdfglyphtounicode{compwordmark}{00A0}
\pdfglyphtounicode{congruent}{00A0}
\pdfglyphtounicode{contourintegral}{00A0}
\pdfglyphtounicode{control}{00A0}
\pdfglyphtounicode{controlACK}{00A0}
\pdfglyphtounicode{controlBEL}{00A0}
\pdfglyphtounicode{controlBS}{00A0}
\pdfglyphtounicode{controlCAN}{00A0}
\pdfglyphtounicode{controlCR}{00A0}
\pdfglyphtounicode{controlDC1}{00A0}
\pdfglyphtounicode{controlDC2}{00A0}
\pdfglyphtounicode{controlDC3}{00A0}
\pdfglyphtounicode{controlDC4}{00A0}
\pdfglyphtounicode{controlDEL}{00A0}
\pdfglyphtounicode{controlDLE}{00A0}
\pdfglyphtounicode{controlEM}{00A0}
\pdfglyphtounicode{controlENQ}{00A0}
\pdfglyphtounicode{controlEOT}{00A0}
\pdfglyphtounicode{controlESC}{00A0}
\pdfglyphtounicode{controlETB}{00A0}
\pdfglyphtounicode{controlETX}{00A0}
\pdfglyphtounicode{controlFF}{00A0}
\pdfglyphtounicode{controlFS}{00A0}
\pdfglyphtounicode{controlGS}{00A0}
\pdfglyphtounicode{controlHT}{00A0}
\pdfglyphtounicode{controlLF}{00A0}
\pdfglyphtounicode{controlNAK}{00A0}
\pdfglyphtounicode{controlRS}{00A0}
\pdfglyphtounicode{controlSI}{00A0}
\pdfglyphtounicode{controlSO}{00A0}
\pdfglyphtounicode{controlSOT}{00A0}
\pdfglyphtounicode{controlSTX}{00A0}
\pdfglyphtounicode{controlSUB}{00A0}
\pdfglyphtounicode{controlSYN}{00A0}
\pdfglyphtounicode{controlUS}{00A0}
\pdfglyphtounicode{controlVT}{00A0}
\pdfglyphtounicode{coproduct}{00A0}
\pdfglyphtounicode{copyright}{00A0}
\pdfglyphtounicode{copyrightsans}{00A0}
\pdfglyphtounicode{copyrightserif}{00A0}
\pdfglyphtounicode{cornerbracketleft}{00A0}
\pdfglyphtounicode{cornerbracketlefthalfwidth}{00A0}
\pdfglyphtounicode{cornerbracketleftvertical}{00A0}
\pdfglyphtounicode{cornerbracketright}{00A0}
\pdfglyphtounicode{cornerbracketrighthalfwidth}{00A0}
\pdfglyphtounicode{cornerbracketrightvertical}{00A0}
\pdfglyphtounicode{corporationsquare}{00A0}
\pdfglyphtounicode{cosquare}{00A0}
\pdfglyphtounicode{coverkgsquare}{00A0}
\pdfglyphtounicode{cparen}{00A0}
\pdfglyphtounicode{cruzeiro}{00A0}
\pdfglyphtounicode{cstretched}{00A0}
\pdfglyphtounicode{ct}{00A0}
\pdfglyphtounicode{curlyand}{00A0}
\pdfglyphtounicode{curlyleft}{00A0}
\pdfglyphtounicode{curlyor}{00A0}
\pdfglyphtounicode{curlyright}{00A0}
\pdfglyphtounicode{currency}{00A0}
\pdfglyphtounicode{cwm}{00A0}
\pdfglyphtounicode{cyrBreve}{00A0}
\pdfglyphtounicode{cyrFlex}{00A0}
\pdfglyphtounicode{cyrbreve}{00A0}
\pdfglyphtounicode{cyrflex}{00A0}
\pdfglyphtounicode{d}{00A0}
\pdfglyphtounicode{daarmenian}{00A0}
\pdfglyphtounicode{dabengali}{00A0}
\pdfglyphtounicode{dadarabic}{00A0}
\pdfglyphtounicode{dadeva}{00A0}
\pdfglyphtounicode{dadfinalarabic}{00A0}
\pdfglyphtounicode{dadinitialarabic}{00A0}
\pdfglyphtounicode{dadmedialarabic}{00A0}
\pdfglyphtounicode{dagesh}{00A0}
\pdfglyphtounicode{dageshhebrew}{00A0}
\pdfglyphtounicode{dagger}{00A0}
\pdfglyphtounicode{daggerdbl}{00A0}
\pdfglyphtounicode{dagujarati}{00A0}
\pdfglyphtounicode{dagurmukhi}{00A0}
\pdfglyphtounicode{dahiragana}{00A0}
\pdfglyphtounicode{dakatakana}{00A0}
\pdfglyphtounicode{dalarabic}{00A0}
\pdfglyphtounicode{dalet}{00A0}
\pdfglyphtounicode{daletdagesh}{00A0}
\pdfglyphtounicode{daletdageshhebrew}{00A0}
\pdfglyphtounicode{daleth}{00A0}
\pdfglyphtounicode{dalethatafpatah}{00A0}
\pdfglyphtounicode{dalethatafpatahhebrew}{00A0}
\pdfglyphtounicode{dalethatafsegol}{00A0}
\pdfglyphtounicode{dalethatafsegolhebrew}{00A0}
\pdfglyphtounicode{dalethebrew}{00A0}
\pdfglyphtounicode{dalethiriq}{00A0}
\pdfglyphtounicode{dalethiriqhebrew}{00A0}
\pdfglyphtounicode{daletholam}{00A0}
\pdfglyphtounicode{daletholamhebrew}{00A0}
\pdfglyphtounicode{daletpatah}{00A0}
\pdfglyphtounicode{daletpatahhebrew}{00A0}
\pdfglyphtounicode{daletqamats}{00A0}
\pdfglyphtounicode{daletqamatshebrew}{00A0}
\pdfglyphtounicode{daletqubuts}{00A0}
\pdfglyphtounicode{daletqubutshebrew}{00A0}
\pdfglyphtounicode{daletsegol}{00A0}
\pdfglyphtounicode{daletsegolhebrew}{00A0}
\pdfglyphtounicode{daletsheva}{00A0}
\pdfglyphtounicode{daletshevahebrew}{00A0}
\pdfglyphtounicode{dalettsere}{00A0}
\pdfglyphtounicode{dalettserehebrew}{00A0}
\pdfglyphtounicode{dalfinalarabic}{00A0}
\pdfglyphtounicode{dammaarabic}{00A0}
\pdfglyphtounicode{dammalowarabic}{00A0}
\pdfglyphtounicode{dammatanaltonearabic}{00A0}
\pdfglyphtounicode{dammatanarabic}{00A0}
\pdfglyphtounicode{danda}{00A0}
\pdfglyphtounicode{dargahebrew}{00A0}
\pdfglyphtounicode{dargalefthebrew}{00A0}
\pdfglyphtounicode{dasiapneumatacyrilliccmb}{00A0}
\pdfglyphtounicode{dbar}{00A0}
\pdfglyphtounicode{dblGrave}{00A0}
\pdfglyphtounicode{dblanglebracketleft}{00A0}
\pdfglyphtounicode{dblanglebracketleftvertical}{00A0}
\pdfglyphtounicode{dblanglebracketright}{00A0}
\pdfglyphtounicode{dblanglebracketrightvertical}{00A0}
\pdfglyphtounicode{dblarchinvertedbelowcmb}{00A0}
\pdfglyphtounicode{dblarrowdwn}{00A0}
\pdfglyphtounicode{dblarrowheadleft}{00A0}
\pdfglyphtounicode{dblarrowheadright}{00A0}
\pdfglyphtounicode{dblarrowleft}{00A0}
\pdfglyphtounicode{dblarrowright}{00A0}
\pdfglyphtounicode{dblarrowup}{00A0}
\pdfglyphtounicode{dblbracketleft}{00A0}
\pdfglyphtounicode{dblbracketright}{00A0}
\pdfglyphtounicode{dbldanda}{00A0}
\pdfglyphtounicode{dblgrave}{00A0}
\pdfglyphtounicode{dblgravecmb}{00A0}
\pdfglyphtounicode{dblintegral}{00A0}
\pdfglyphtounicode{dbllowline}{00A0}
\pdfglyphtounicode{dbllowlinecmb}{00A0}
\pdfglyphtounicode{dbloverlinecmb}{00A0}
\pdfglyphtounicode{dblprimemod}{00A0}
\pdfglyphtounicode{dblverticalbar}{00A0}
\pdfglyphtounicode{dblverticallineabovecmb}{00A0}
\pdfglyphtounicode{dbopomofo}{00A0}
\pdfglyphtounicode{dbsquare}{00A0}
\pdfglyphtounicode{dcaron}{00A0}
\pdfglyphtounicode{dcedilla}{00A0}
\pdfglyphtounicode{dcircle}{00A0}
\pdfglyphtounicode{dcircumflexbelow}{00A0}
\pdfglyphtounicode{dcroat}{00A0}
\pdfglyphtounicode{ddabengali}{00A0}
\pdfglyphtounicode{ddadeva}{00A0}
\pdfglyphtounicode{ddagujarati}{00A0}
\pdfglyphtounicode{ddagurmukhi}{00A0}
\pdfglyphtounicode{ddalarabic}{00A0}
\pdfglyphtounicode{ddalfinalarabic}{00A0}
\pdfglyphtounicode{dddhadeva}{00A0}
\pdfglyphtounicode{ddhabengali}{00A0}
\pdfglyphtounicode{ddhadeva}{00A0}
\pdfglyphtounicode{ddhagujarati}{00A0}
\pdfglyphtounicode{ddhagurmukhi}{00A0}
\pdfglyphtounicode{ddotaccent}{00A0}
\pdfglyphtounicode{ddotbelow}{00A0}
\pdfglyphtounicode{decimalseparatorarabic}{00A0}
\pdfglyphtounicode{decimalseparatorpersian}{00A0}
\pdfglyphtounicode{decyrillic}{00A0}
\pdfglyphtounicode{defines}{00A0}
\pdfglyphtounicode{degree}{00A0}
\pdfglyphtounicode{dehihebrew}{00A0}
\pdfglyphtounicode{dehiragana}{00A0}
\pdfglyphtounicode{deicoptic}{00A0}
\pdfglyphtounicode{dekatakana}{00A0}
\pdfglyphtounicode{deleteleft}{00A0}
\pdfglyphtounicode{deleteright}{00A0}
\pdfglyphtounicode{delta}{00A0}
\pdfglyphtounicode{deltaturned}{00A0}
\pdfglyphtounicode{denominatorminusonenumeratorbengali}{00A0}
\pdfglyphtounicode{dezh}{00A0}
\pdfglyphtounicode{dhabengali}{00A0}
\pdfglyphtounicode{dhadeva}{00A0}
\pdfglyphtounicode{dhagujarati}{00A0}
\pdfglyphtounicode{dhagurmukhi}{00A0}
\pdfglyphtounicode{dhook}{00A0}
\pdfglyphtounicode{dialytikatonos}{00A0}
\pdfglyphtounicode{dialytikatonoscmb}{00A0}
\pdfglyphtounicode{diamond}{00A0}
\pdfglyphtounicode{diamondmath}{00A0}
\pdfglyphtounicode{diamondsolid}{00A0}
\pdfglyphtounicode{diamondsuitwhite}{00A0}
\pdfglyphtounicode{dieresis}{00A0}
\pdfglyphtounicode{dieresisacute}{00A0}
\pdfglyphtounicode{dieresisbelowcmb}{00A0}
\pdfglyphtounicode{dieresiscmb}{00A0}
\pdfglyphtounicode{dieresisgrave}{00A0}
\pdfglyphtounicode{dieresistonos}{00A0}
\pdfglyphtounicode{difference}{00A0}
\pdfglyphtounicode{dihiragana}{00A0}
\pdfglyphtounicode{dikatakana}{00A0}
\pdfglyphtounicode{dittomark}{00A0}
\pdfglyphtounicode{divide}{00A0}
\pdfglyphtounicode{dividemultiply}{00A0}
\pdfglyphtounicode{divides}{00A0}
\pdfglyphtounicode{divisionslash}{00A0}
\pdfglyphtounicode{djecyrillic}{00A0}
\pdfglyphtounicode{dkshade}{00A0}
\pdfglyphtounicode{dlinebelow}{00A0}
\pdfglyphtounicode{dlsquare}{00A0}
\pdfglyphtounicode{dmacron}{00A0}
\pdfglyphtounicode{dmonospace}{00A0}
\pdfglyphtounicode{dnblock}{00A0}
\pdfglyphtounicode{dochadathai}{00A0}
\pdfglyphtounicode{dodekthai}{00A0}
\pdfglyphtounicode{dohiragana}{00A0}
\pdfglyphtounicode{dokatakana}{00A0}
\pdfglyphtounicode{dollar}{00A0}
\pdfglyphtounicode{dollarinferior}{00A0}
\pdfglyphtounicode{dollarmonospace}{00A0}
\pdfglyphtounicode{dollaroldstyle}{00A0}
\pdfglyphtounicode{dollarsmall}{00A0}
\pdfglyphtounicode{dollarsuperior}{00A0}
\pdfglyphtounicode{dong}{00A0}
\pdfglyphtounicode{dorusquare}{00A0}
\pdfglyphtounicode{dotaccent}{00A0}
\pdfglyphtounicode{dotaccentcmb}{00A0}
\pdfglyphtounicode{dotbelowcmb}{00A0}
\pdfglyphtounicode{dotbelowcomb}{00A0}
\pdfglyphtounicode{dotkatakana}{00A0}
\pdfglyphtounicode{dotlessi}{00A0}
\pdfglyphtounicode{dotlessj}{00A0}
\pdfglyphtounicode{dotlessjstrokehook}{00A0}
\pdfglyphtounicode{dotmath}{00A0}
\pdfglyphtounicode{dotplus}{00A0}
\pdfglyphtounicode{dottedcircle}{00A0}
\pdfglyphtounicode{doubleyodpatah}{00A0}
\pdfglyphtounicode{doubleyodpatahhebrew}{00A0}
\pdfglyphtounicode{downfall}{00A0}
\pdfglyphtounicode{downslope}{00A0}
\pdfglyphtounicode{downtackbelowcmb}{00A0}
\pdfglyphtounicode{downtackmod}{00A0}
\pdfglyphtounicode{dparen}{00A0}
\pdfglyphtounicode{dsuperior}{00A0}
\pdfglyphtounicode{dtail}{00A0}
\pdfglyphtounicode{dtopbar}{00A0}
\pdfglyphtounicode{duhiragana}{00A0}
\pdfglyphtounicode{dukatakana}{00A0}
\pdfglyphtounicode{dz}{00A0}
\pdfglyphtounicode{dzaltone}{00A0}
\pdfglyphtounicode{dzcaron}{00A0}
\pdfglyphtounicode{dzcurl}{00A0}
\pdfglyphtounicode{dzeabkhasiancyrillic}{00A0}
\pdfglyphtounicode{dzecyrillic}{00A0}
\pdfglyphtounicode{dzhecyrillic}{00A0}
\pdfglyphtounicode{e}{00A0}
\pdfglyphtounicode{eacute}{00A0}
\pdfglyphtounicode{earth}{00A0}
\pdfglyphtounicode{ebengali}{00A0}
\pdfglyphtounicode{ebopomofo}{00A0}
\pdfglyphtounicode{ebreve}{00A0}
\pdfglyphtounicode{ecandradeva}{00A0}
\pdfglyphtounicode{ecandragujarati}{00A0}
\pdfglyphtounicode{ecandravowelsigndeva}{00A0}
\pdfglyphtounicode{ecandravowelsigngujarati}{00A0}
\pdfglyphtounicode{ecaron}{00A0}
\pdfglyphtounicode{ecedillabreve}{00A0}
\pdfglyphtounicode{echarmenian}{00A0}
\pdfglyphtounicode{echyiwnarmenian}{00A0}
\pdfglyphtounicode{ecircle}{00A0}
\pdfglyphtounicode{ecircumflex}{00A0}
\pdfglyphtounicode{ecircumflexacute}{00A0}
\pdfglyphtounicode{ecircumflexbelow}{00A0}
\pdfglyphtounicode{ecircumflexdotbelow}{00A0}
\pdfglyphtounicode{ecircumflexgrave}{00A0}
\pdfglyphtounicode{ecircumflexhookabove}{00A0}
\pdfglyphtounicode{ecircumflextilde}{00A0}
\pdfglyphtounicode{ecyrillic}{00A0}
\pdfglyphtounicode{edblgrave}{00A0}
\pdfglyphtounicode{edeva}{00A0}
\pdfglyphtounicode{edieresis}{00A0}
\pdfglyphtounicode{edot}{00A0}
\pdfglyphtounicode{edotaccent}{00A0}
\pdfglyphtounicode{edotbelow}{00A0}
\pdfglyphtounicode{eegurmukhi}{00A0}
\pdfglyphtounicode{eematragurmukhi}{00A0}
\pdfglyphtounicode{efcyrillic}{00A0}
\pdfglyphtounicode{egrave}{00A0}
\pdfglyphtounicode{egujarati}{00A0}
\pdfglyphtounicode{eharmenian}{00A0}
\pdfglyphtounicode{ehbopomofo}{00A0}
\pdfglyphtounicode{ehiragana}{00A0}
\pdfglyphtounicode{ehookabove}{00A0}
\pdfglyphtounicode{eibopomofo}{00A0}
\pdfglyphtounicode{eight}{00A0}
\pdfglyphtounicode{eightarabic}{00A0}
\pdfglyphtounicode{eightbengali}{00A0}
\pdfglyphtounicode{eightcircle}{00A0}
\pdfglyphtounicode{eightcircleinversesansserif}{00A0}
\pdfglyphtounicode{eightdeva}{00A0}
\pdfglyphtounicode{eighteencircle}{00A0}
\pdfglyphtounicode{eighteenparen}{00A0}
\pdfglyphtounicode{eighteenperiod}{00A0}
\pdfglyphtounicode{eightgujarati}{00A0}
\pdfglyphtounicode{eightgurmukhi}{00A0}
\pdfglyphtounicode{eighthackarabic}{00A0}
\pdfglyphtounicode{eighthangzhou}{00A0}
\pdfglyphtounicode{eighthnotebeamed}{00A0}
\pdfglyphtounicode{eightideographicparen}{00A0}
\pdfglyphtounicode{eightinferior}{00A0}
\pdfglyphtounicode{eightmonospace}{00A0}
\pdfglyphtounicode{eightoldstyle}{00A0}
\pdfglyphtounicode{eightparen}{00A0}
\pdfglyphtounicode{eightperiod}{00A0}
\pdfglyphtounicode{eightpersian}{00A0}
\pdfglyphtounicode{eightroman}{00A0}
\pdfglyphtounicode{eightsuperior}{00A0}
\pdfglyphtounicode{eightthai}{00A0}
\pdfglyphtounicode{einvertedbreve}{00A0}
\pdfglyphtounicode{eiotifiedcyrillic}{00A0}
\pdfglyphtounicode{ekatakana}{00A0}
\pdfglyphtounicode{ekatakanahalfwidth}{00A0}
\pdfglyphtounicode{ekonkargurmukhi}{00A0}
\pdfglyphtounicode{ekorean}{00A0}
\pdfglyphtounicode{elcyrillic}{00A0}
\pdfglyphtounicode{element}{00A0}
\pdfglyphtounicode{elevencircle}{00A0}
\pdfglyphtounicode{elevenparen}{00A0}
\pdfglyphtounicode{elevenperiod}{00A0}
\pdfglyphtounicode{elevenroman}{00A0}
\pdfglyphtounicode{ellipsis}{00A0}
\pdfglyphtounicode{ellipsisvertical}{00A0}
\pdfglyphtounicode{emacron}{00A0}
\pdfglyphtounicode{emacronacute}{00A0}
\pdfglyphtounicode{emacrongrave}{00A0}
\pdfglyphtounicode{emcyrillic}{00A0}
\pdfglyphtounicode{emdash}{00A0}
\pdfglyphtounicode{emdashvertical}{00A0}
\pdfglyphtounicode{emonospace}{00A0}
\pdfglyphtounicode{emphasismarkarmenian}{00A0}
\pdfglyphtounicode{emptyset}{00A0}
\pdfglyphtounicode{enbopomofo}{00A0}
\pdfglyphtounicode{encyrillic}{00A0}
\pdfglyphtounicode{endash}{00A0}
\pdfglyphtounicode{endashvertical}{00A0}
\pdfglyphtounicode{endescendercyrillic}{00A0}
\pdfglyphtounicode{eng}{00A0}
\pdfglyphtounicode{engbopomofo}{00A0}
\pdfglyphtounicode{enghecyrillic}{00A0}
\pdfglyphtounicode{enhookcyrillic}{00A0}
\pdfglyphtounicode{enspace}{00A0}
\pdfglyphtounicode{eogonek}{00A0}
\pdfglyphtounicode{eokorean}{00A0}
\pdfglyphtounicode{eopen}{00A0}
\pdfglyphtounicode{eopenclosed}{00A0}
\pdfglyphtounicode{eopenreversed}{00A0}
\pdfglyphtounicode{eopenreversedclosed}{00A0}
\pdfglyphtounicode{eopenreversedhook}{00A0}
\pdfglyphtounicode{eparen}{00A0}
\pdfglyphtounicode{epsilon}{00A0}
\pdfglyphtounicode{epsilon1}{00A0}
\pdfglyphtounicode{epsiloninv}{00A0}
\pdfglyphtounicode{epsilontonos}{00A0}
\pdfglyphtounicode{equal}{00A0}
\pdfglyphtounicode{equaldotleftright}{00A0}
\pdfglyphtounicode{equaldotrightleft}{00A0}
\pdfglyphtounicode{equalmonospace}{00A0}
\pdfglyphtounicode{equalorfollows}{00A0}
\pdfglyphtounicode{equalorgreater}{00A0}
\pdfglyphtounicode{equalorless}{00A0}
\pdfglyphtounicode{equalorprecedes}{00A0}
\pdfglyphtounicode{equalorsimilar}{00A0}
\pdfglyphtounicode{equalsdots}{00A0}
\pdfglyphtounicode{equalsmall}{00A0}
\pdfglyphtounicode{equalsuperior}{00A0}
\pdfglyphtounicode{equivalence}{00A0}
\pdfglyphtounicode{equivasymptotic}{00A0}
\pdfglyphtounicode{erbopomofo}{00A0}
\pdfglyphtounicode{ercyrillic}{00A0}
\pdfglyphtounicode{ereversed}{00A0}
\pdfglyphtounicode{ereversedcyrillic}{00A0}
\pdfglyphtounicode{escyrillic}{00A0}
\pdfglyphtounicode{esdescendercyrillic}{00A0}
\pdfglyphtounicode{esh}{00A0}
\pdfglyphtounicode{eshcurl}{00A0}
\pdfglyphtounicode{eshortdeva}{00A0}
\pdfglyphtounicode{eshortvowelsigndeva}{00A0}
\pdfglyphtounicode{eshreversedloop}{00A0}
\pdfglyphtounicode{eshsquatreversed}{00A0}
\pdfglyphtounicode{esmallhiragana}{00A0}
\pdfglyphtounicode{esmallkatakana}{00A0}
\pdfglyphtounicode{esmallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{estimated}{00A0}
\pdfglyphtounicode{esuperior}{00A0}
\pdfglyphtounicode{eta}{00A0}
\pdfglyphtounicode{etarmenian}{00A0}
\pdfglyphtounicode{etatonos}{00A0}
\pdfglyphtounicode{eth}{00A0}
\pdfglyphtounicode{etilde}{00A0}
\pdfglyphtounicode{etildebelow}{00A0}
\pdfglyphtounicode{etnahtafoukhhebrew}{00A0}
\pdfglyphtounicode{etnahtafoukhlefthebrew}{00A0}
\pdfglyphtounicode{etnahtahebrew}{00A0}
\pdfglyphtounicode{etnahtalefthebrew}{00A0}
\pdfglyphtounicode{eturned}{00A0}
\pdfglyphtounicode{eukorean}{00A0}
\pdfglyphtounicode{euro}{00A0}
\pdfglyphtounicode{evowelsignbengali}{00A0}
\pdfglyphtounicode{evowelsigndeva}{00A0}
\pdfglyphtounicode{evowelsigngujarati}{00A0}
\pdfglyphtounicode{exclam}{00A0}
\pdfglyphtounicode{exclamarmenian}{00A0}
\pdfglyphtounicode{exclamdbl}{00A0}
\pdfglyphtounicode{exclamdown}{00A0}
\pdfglyphtounicode{exclamdownsmall}{00A0}
\pdfglyphtounicode{exclammonospace}{00A0}
\pdfglyphtounicode{exclamsmall}{00A0}
\pdfglyphtounicode{existential}{00A0}
\pdfglyphtounicode{ezh}{00A0}
\pdfglyphtounicode{ezhcaron}{00A0}
\pdfglyphtounicode{ezhcurl}{00A0}
\pdfglyphtounicode{ezhreversed}{00A0}
\pdfglyphtounicode{ezhtail}{00A0}
\pdfglyphtounicode{f}{00A0}
\pdfglyphtounicode{fadeva}{00A0}
\pdfglyphtounicode{fagurmukhi}{00A0}
\pdfglyphtounicode{fahrenheit}{00A0}
\pdfglyphtounicode{fathaarabic}{00A0}
\pdfglyphtounicode{fathalowarabic}{00A0}
\pdfglyphtounicode{fathatanarabic}{00A0}
\pdfglyphtounicode{fbopomofo}{00A0}
\pdfglyphtounicode{fcircle}{00A0}
\pdfglyphtounicode{fdotaccent}{00A0}
\pdfglyphtounicode{feharabic}{00A0}
\pdfglyphtounicode{feharmenian}{00A0}
\pdfglyphtounicode{fehfinalarabic}{00A0}
\pdfglyphtounicode{fehinitialarabic}{00A0}
\pdfglyphtounicode{fehmedialarabic}{00A0}
\pdfglyphtounicode{feicoptic}{00A0}
\pdfglyphtounicode{female}{00A0}
\pdfglyphtounicode{ff}{00A0}
\pdfglyphtounicode{ffi}{00A0}
\pdfglyphtounicode{ffl}{00A0}
\pdfglyphtounicode{fi}{00A0}
\pdfglyphtounicode{fifteencircle}{00A0}
\pdfglyphtounicode{fifteenparen}{00A0}
\pdfglyphtounicode{fifteenperiod}{00A0}
\pdfglyphtounicode{figuredash}{00A0}
\pdfglyphtounicode{filledbox}{00A0}
\pdfglyphtounicode{filledrect}{00A0}
\pdfglyphtounicode{finalkaf}{00A0}
\pdfglyphtounicode{finalkafdagesh}{00A0}
\pdfglyphtounicode{finalkafdageshhebrew}{00A0}
\pdfglyphtounicode{finalkafhebrew}{00A0}
\pdfglyphtounicode{finalkafqamats}{00A0}
\pdfglyphtounicode{finalkafqamatshebrew}{00A0}
\pdfglyphtounicode{finalkafsheva}{00A0}
\pdfglyphtounicode{finalkafshevahebrew}{00A0}
\pdfglyphtounicode{finalmem}{00A0}
\pdfglyphtounicode{finalmemhebrew}{00A0}
\pdfglyphtounicode{finalnun}{00A0}
\pdfglyphtounicode{finalnunhebrew}{00A0}
\pdfglyphtounicode{finalpe}{00A0}
\pdfglyphtounicode{finalpehebrew}{00A0}
\pdfglyphtounicode{finaltsadi}{00A0}
\pdfglyphtounicode{finaltsadihebrew}{00A0}
\pdfglyphtounicode{firsttonechinese}{00A0}
\pdfglyphtounicode{fisheye}{00A0}
\pdfglyphtounicode{fitacyrillic}{00A0}
\pdfglyphtounicode{five}{00A0}
\pdfglyphtounicode{fivearabic}{00A0}
\pdfglyphtounicode{fivebengali}{00A0}
\pdfglyphtounicode{fivecircle}{00A0}
\pdfglyphtounicode{fivecircleinversesansserif}{00A0}
\pdfglyphtounicode{fivedeva}{00A0}
\pdfglyphtounicode{fiveeighths}{00A0}
\pdfglyphtounicode{fivegujarati}{00A0}
\pdfglyphtounicode{fivegurmukhi}{00A0}
\pdfglyphtounicode{fivehackarabic}{00A0}
\pdfglyphtounicode{fivehangzhou}{00A0}
\pdfglyphtounicode{fiveideographicparen}{00A0}
\pdfglyphtounicode{fiveinferior}{00A0}
\pdfglyphtounicode{fivemonospace}{00A0}
\pdfglyphtounicode{fiveoldstyle}{00A0}
\pdfglyphtounicode{fiveparen}{00A0}
\pdfglyphtounicode{fiveperiod}{00A0}
\pdfglyphtounicode{fivepersian}{00A0}
\pdfglyphtounicode{fiveroman}{00A0}
\pdfglyphtounicode{fivesuperior}{00A0}
\pdfglyphtounicode{fivethai}{00A0}
\pdfglyphtounicode{fl}{00A0}
\pdfglyphtounicode{flat}{00A0}
\pdfglyphtounicode{floorleft}{00A0}
\pdfglyphtounicode{floorright}{00A0}
\pdfglyphtounicode{florin}{00A0}
\pdfglyphtounicode{fmonospace}{00A0}
\pdfglyphtounicode{fmsquare}{00A0}
\pdfglyphtounicode{fofanthai}{00A0}
\pdfglyphtounicode{fofathai}{00A0}
\pdfglyphtounicode{follownotdbleqv}{00A0}
\pdfglyphtounicode{follownotslnteql}{00A0}
\pdfglyphtounicode{followornoteqvlnt}{00A0}
\pdfglyphtounicode{follows}{00A0}
\pdfglyphtounicode{followsequal}{00A0}
\pdfglyphtounicode{followsorcurly}{00A0}
\pdfglyphtounicode{followsorequal}{00A0}
\pdfglyphtounicode{fongmanthai}{00A0}
\pdfglyphtounicode{forall}{00A0}
\pdfglyphtounicode{forces}{00A0}
\pdfglyphtounicode{forcesbar}{00A0}
\pdfglyphtounicode{fork}{00A0}
\pdfglyphtounicode{four}{00A0}
\pdfglyphtounicode{fourarabic}{00A0}
\pdfglyphtounicode{fourbengali}{00A0}
\pdfglyphtounicode{fourcircle}{00A0}
\pdfglyphtounicode{fourcircleinversesansserif}{00A0}
\pdfglyphtounicode{fourdeva}{00A0}
\pdfglyphtounicode{fourgujarati}{00A0}
\pdfglyphtounicode{fourgurmukhi}{00A0}
\pdfglyphtounicode{fourhackarabic}{00A0}
\pdfglyphtounicode{fourhangzhou}{00A0}
\pdfglyphtounicode{fourideographicparen}{00A0}
\pdfglyphtounicode{fourinferior}{00A0}
\pdfglyphtounicode{fourmonospace}{00A0}
\pdfglyphtounicode{fournumeratorbengali}{00A0}
\pdfglyphtounicode{fouroldstyle}{00A0}
\pdfglyphtounicode{fourparen}{00A0}
\pdfglyphtounicode{fourperiod}{00A0}
\pdfglyphtounicode{fourpersian}{00A0}
\pdfglyphtounicode{fourroman}{00A0}
\pdfglyphtounicode{foursuperior}{00A0}
\pdfglyphtounicode{fourteencircle}{00A0}
\pdfglyphtounicode{fourteenparen}{00A0}
\pdfglyphtounicode{fourteenperiod}{00A0}
\pdfglyphtounicode{fourthai}{00A0}
\pdfglyphtounicode{fourthtonechinese}{00A0}
\pdfglyphtounicode{fparen}{00A0}
\pdfglyphtounicode{fraction}{00A0}
\pdfglyphtounicode{franc}{00A0}
\pdfglyphtounicode{frown}{00A0}
\pdfglyphtounicode{g}{00A0}
\pdfglyphtounicode{gabengali}{00A0}
\pdfglyphtounicode{gacute}{00A0}
\pdfglyphtounicode{gadeva}{00A0}
\pdfglyphtounicode{gafarabic}{00A0}
\pdfglyphtounicode{gaffinalarabic}{00A0}
\pdfglyphtounicode{gafinitialarabic}{00A0}
\pdfglyphtounicode{gafmedialarabic}{00A0}
\pdfglyphtounicode{gagujarati}{00A0}
\pdfglyphtounicode{gagurmukhi}{00A0}
\pdfglyphtounicode{gahiragana}{00A0}
\pdfglyphtounicode{gakatakana}{00A0}
\pdfglyphtounicode{gamma}{00A0}
\pdfglyphtounicode{gammalatinsmall}{00A0}
\pdfglyphtounicode{gammasuperior}{00A0}
\pdfglyphtounicode{gangiacoptic}{00A0}
\pdfglyphtounicode{gbopomofo}{00A0}
\pdfglyphtounicode{gbreve}{00A0}
\pdfglyphtounicode{gcaron}{00A0}
\pdfglyphtounicode{gcedilla}{00A0}
\pdfglyphtounicode{gcircle}{00A0}
\pdfglyphtounicode{gcircumflex}{00A0}
\pdfglyphtounicode{gcommaaccent}{00A0}
\pdfglyphtounicode{gdot}{00A0}
\pdfglyphtounicode{gdotaccent}{00A0}
\pdfglyphtounicode{gecyrillic}{00A0}
\pdfglyphtounicode{gehiragana}{00A0}
\pdfglyphtounicode{gekatakana}{00A0}
\pdfglyphtounicode{geomequivalent}{00A0}
\pdfglyphtounicode{geometricallyequal}{00A0}
\pdfglyphtounicode{gereshaccenthebrew}{00A0}
\pdfglyphtounicode{gereshhebrew}{00A0}
\pdfglyphtounicode{gereshmuqdamhebrew}{00A0}
\pdfglyphtounicode{germandbls}{00A0}
\pdfglyphtounicode{gershayimaccenthebrew}{00A0}
\pdfglyphtounicode{gershayimhebrew}{00A0}
\pdfglyphtounicode{getamark}{00A0}
\pdfglyphtounicode{ghabengali}{00A0}
\pdfglyphtounicode{ghadarmenian}{00A0}
\pdfglyphtounicode{ghadeva}{00A0}
\pdfglyphtounicode{ghagujarati}{00A0}
\pdfglyphtounicode{ghagurmukhi}{00A0}
\pdfglyphtounicode{ghainarabic}{00A0}
\pdfglyphtounicode{ghainfinalarabic}{00A0}
\pdfglyphtounicode{ghaininitialarabic}{00A0}
\pdfglyphtounicode{ghainmedialarabic}{00A0}
\pdfglyphtounicode{ghemiddlehookcyrillic}{00A0}
\pdfglyphtounicode{ghestrokecyrillic}{00A0}
\pdfglyphtounicode{gheupturncyrillic}{00A0}
\pdfglyphtounicode{ghhadeva}{00A0}
\pdfglyphtounicode{ghhagurmukhi}{00A0}
\pdfglyphtounicode{ghook}{00A0}
\pdfglyphtounicode{ghzsquare}{00A0}
\pdfglyphtounicode{gihiragana}{00A0}
\pdfglyphtounicode{gikatakana}{00A0}
\pdfglyphtounicode{gimarmenian}{00A0}
\pdfglyphtounicode{gimel}{00A0}
\pdfglyphtounicode{gimeldagesh}{00A0}
\pdfglyphtounicode{gimeldageshhebrew}{00A0}
\pdfglyphtounicode{gimelhebrew}{00A0}
\pdfglyphtounicode{gjecyrillic}{00A0}
\pdfglyphtounicode{glottalinvertedstroke}{00A0}
\pdfglyphtounicode{glottalstop}{00A0}
\pdfglyphtounicode{glottalstopinverted}{00A0}
\pdfglyphtounicode{glottalstopmod}{00A0}
\pdfglyphtounicode{glottalstopreversed}{00A0}
\pdfglyphtounicode{glottalstopreversedmod}{00A0}
\pdfglyphtounicode{glottalstopreversedsuperior}{00A0}
\pdfglyphtounicode{glottalstopstroke}{00A0}
\pdfglyphtounicode{glottalstopstrokereversed}{00A0}
\pdfglyphtounicode{gmacron}{00A0}
\pdfglyphtounicode{gmonospace}{00A0}
\pdfglyphtounicode{gohiragana}{00A0}
\pdfglyphtounicode{gokatakana}{00A0}
\pdfglyphtounicode{gparen}{00A0}
\pdfglyphtounicode{gpasquare}{00A0}
\pdfglyphtounicode{gradient}{00A0}
\pdfglyphtounicode{grave}{00A0}
\pdfglyphtounicode{gravebelowcmb}{00A0}
\pdfglyphtounicode{gravecmb}{00A0}
\pdfglyphtounicode{gravecomb}{00A0}
\pdfglyphtounicode{gravedeva}{00A0}
\pdfglyphtounicode{gravelowmod}{00A0}
\pdfglyphtounicode{gravemonospace}{00A0}
\pdfglyphtounicode{gravetonecmb}{00A0}
\pdfglyphtounicode{greater}{00A0}
\pdfglyphtounicode{greaterdbleqlless}{00A0}
\pdfglyphtounicode{greaterdblequal}{00A0}
\pdfglyphtounicode{greaterdot}{00A0}
\pdfglyphtounicode{greaterequal}{00A0}
\pdfglyphtounicode{greaterequalorless}{00A0}
\pdfglyphtounicode{greaterlessequal}{00A0}
\pdfglyphtounicode{greatermonospace}{00A0}
\pdfglyphtounicode{greatermuch}{00A0}
\pdfglyphtounicode{greaternotdblequal}{00A0}
\pdfglyphtounicode{greaternotequal}{00A0}
\pdfglyphtounicode{greaterorapproxeql}{00A0}
\pdfglyphtounicode{greaterorequalslant}{00A0}
\pdfglyphtounicode{greaterorequivalent}{00A0}
\pdfglyphtounicode{greaterorless}{00A0}
\pdfglyphtounicode{greaterornotdbleql}{00A0}
\pdfglyphtounicode{greaterornotequal}{00A0}
\pdfglyphtounicode{greaterorsimilar}{00A0}
\pdfglyphtounicode{greateroverequal}{00A0}
\pdfglyphtounicode{greatersmall}{00A0}
\pdfglyphtounicode{gscript}{00A0}
\pdfglyphtounicode{gstroke}{00A0}
\pdfglyphtounicode{guhiragana}{00A0}
\pdfglyphtounicode{guillemotleft}{00A0}
\pdfglyphtounicode{guillemotright}{00A0}
\pdfglyphtounicode{guilsinglleft}{00A0}
\pdfglyphtounicode{guilsinglright}{00A0}
\pdfglyphtounicode{gukatakana}{00A0}
\pdfglyphtounicode{guramusquare}{00A0}
\pdfglyphtounicode{gysquare}{00A0}
\pdfglyphtounicode{h}{00A0}
\pdfglyphtounicode{haabkhasiancyrillic}{00A0}
\pdfglyphtounicode{haaltonearabic}{00A0}
\pdfglyphtounicode{habengali}{00A0}
\pdfglyphtounicode{hadescendercyrillic}{00A0}
\pdfglyphtounicode{hadeva}{00A0}
\pdfglyphtounicode{hagujarati}{00A0}
\pdfglyphtounicode{hagurmukhi}{00A0}
\pdfglyphtounicode{haharabic}{00A0}
\pdfglyphtounicode{hahfinalarabic}{00A0}
\pdfglyphtounicode{hahinitialarabic}{00A0}
\pdfglyphtounicode{hahiragana}{00A0}
\pdfglyphtounicode{hahmedialarabic}{00A0}
\pdfglyphtounicode{haitusquare}{00A0}
\pdfglyphtounicode{hakatakana}{00A0}
\pdfglyphtounicode{hakatakanahalfwidth}{00A0}
\pdfglyphtounicode{halantgurmukhi}{00A0}
\pdfglyphtounicode{hamzaarabic}{00A0}
\pdfglyphtounicode{hamzadammaarabic}{00A0}
\pdfglyphtounicode{hamzadammatanarabic}{00A0}
\pdfglyphtounicode{hamzafathaarabic}{00A0}
\pdfglyphtounicode{hamzafathatanarabic}{00A0}
\pdfglyphtounicode{hamzalowarabic}{00A0}
\pdfglyphtounicode{hamzalowkasraarabic}{00A0}
\pdfglyphtounicode{hamzalowkasratanarabic}{00A0}
\pdfglyphtounicode{hamzasukunarabic}{00A0}
\pdfglyphtounicode{hangulfiller}{00A0}
\pdfglyphtounicode{hardsigncyrillic}{00A0}
\pdfglyphtounicode{harpoondownleft}{00A0}
\pdfglyphtounicode{harpoondownright}{00A0}
\pdfglyphtounicode{harpoonleftbarbup}{00A0}
\pdfglyphtounicode{harpoonleftright}{00A0}
\pdfglyphtounicode{harpoonrightbarbup}{00A0}
\pdfglyphtounicode{harpoonrightleft}{00A0}
\pdfglyphtounicode{harpoonupleft}{00A0}
\pdfglyphtounicode{harpoonupright}{00A0}
\pdfglyphtounicode{hasquare}{00A0}
\pdfglyphtounicode{hatafpatah}{00A0}
\pdfglyphtounicode{hatafpatah16}{00A0}
\pdfglyphtounicode{hatafpatah23}{00A0}
\pdfglyphtounicode{hatafpatah2f}{00A0}
\pdfglyphtounicode{hatafpatahhebrew}{00A0}
\pdfglyphtounicode{hatafpatahnarrowhebrew}{00A0}
\pdfglyphtounicode{hatafpatahquarterhebrew}{00A0}
\pdfglyphtounicode{hatafpatahwidehebrew}{00A0}
\pdfglyphtounicode{hatafqamats}{00A0}
\pdfglyphtounicode{hatafqamats1b}{00A0}
\pdfglyphtounicode{hatafqamats28}{00A0}
\pdfglyphtounicode{hatafqamats34}{00A0}
\pdfglyphtounicode{hatafqamatshebrew}{00A0}
\pdfglyphtounicode{hatafqamatsnarrowhebrew}{00A0}
\pdfglyphtounicode{hatafqamatsquarterhebrew}{00A0}
\pdfglyphtounicode{hatafqamatswidehebrew}{00A0}
\pdfglyphtounicode{hatafsegol}{00A0}
\pdfglyphtounicode{hatafsegol17}{00A0}
\pdfglyphtounicode{hatafsegol24}{00A0}
\pdfglyphtounicode{hatafsegol30}{00A0}
\pdfglyphtounicode{hatafsegolhebrew}{00A0}
\pdfglyphtounicode{hatafsegolnarrowhebrew}{00A0}
\pdfglyphtounicode{hatafsegolquarterhebrew}{00A0}
\pdfglyphtounicode{hatafsegolwidehebrew}{00A0}
\pdfglyphtounicode{hbar}{00A0}
\pdfglyphtounicode{hbopomofo}{00A0}
\pdfglyphtounicode{hbrevebelow}{00A0}
\pdfglyphtounicode{hcedilla}{00A0}
\pdfglyphtounicode{hcircle}{00A0}
\pdfglyphtounicode{hcircumflex}{00A0}
\pdfglyphtounicode{hdieresis}{00A0}
\pdfglyphtounicode{hdotaccent}{00A0}
\pdfglyphtounicode{hdotbelow}{00A0}
\pdfglyphtounicode{he}{00A0}
\pdfglyphtounicode{heart}{00A0}
\pdfglyphtounicode{heartsuitblack}{00A0}
\pdfglyphtounicode{heartsuitwhite}{00A0}
\pdfglyphtounicode{hedagesh}{00A0}
\pdfglyphtounicode{hedageshhebrew}{00A0}
\pdfglyphtounicode{hehaltonearabic}{00A0}
\pdfglyphtounicode{heharabic}{00A0}
\pdfglyphtounicode{hehebrew}{00A0}
\pdfglyphtounicode{hehfinalaltonearabic}{00A0}
\pdfglyphtounicode{hehfinalalttwoarabic}{00A0}
\pdfglyphtounicode{hehfinalarabic}{00A0}
\pdfglyphtounicode{hehhamzaabovefinalarabic}{00A0}
\pdfglyphtounicode{hehhamzaaboveisolatedarabic}{00A0}
\pdfglyphtounicode{hehinitialaltonearabic}{00A0}
\pdfglyphtounicode{hehinitialarabic}{00A0}
\pdfglyphtounicode{hehiragana}{00A0}
\pdfglyphtounicode{hehmedialaltonearabic}{00A0}
\pdfglyphtounicode{hehmedialarabic}{00A0}
\pdfglyphtounicode{heiseierasquare}{00A0}
\pdfglyphtounicode{hekatakana}{00A0}
\pdfglyphtounicode{hekatakanahalfwidth}{00A0}
\pdfglyphtounicode{hekutaarusquare}{00A0}
\pdfglyphtounicode{henghook}{00A0}
\pdfglyphtounicode{herutusquare}{00A0}
\pdfglyphtounicode{het}{00A0}
\pdfglyphtounicode{hethebrew}{00A0}
\pdfglyphtounicode{hhook}{00A0}
\pdfglyphtounicode{hhooksuperior}{00A0}
\pdfglyphtounicode{hieuhacirclekorean}{00A0}
\pdfglyphtounicode{hieuhaparenkorean}{00A0}
\pdfglyphtounicode{hieuhcirclekorean}{00A0}
\pdfglyphtounicode{hieuhkorean}{00A0}
\pdfglyphtounicode{hieuhparenkorean}{00A0}
\pdfglyphtounicode{hihiragana}{00A0}
\pdfglyphtounicode{hikatakana}{00A0}
\pdfglyphtounicode{hikatakanahalfwidth}{00A0}
\pdfglyphtounicode{hiriq}{00A0}
\pdfglyphtounicode{hiriq14}{00A0}
\pdfglyphtounicode{hiriq21}{00A0}
\pdfglyphtounicode{hiriq2d}{00A0}
\pdfglyphtounicode{hiriqhebrew}{00A0}
\pdfglyphtounicode{hiriqnarrowhebrew}{00A0}
\pdfglyphtounicode{hiriqquarterhebrew}{00A0}
\pdfglyphtounicode{hiriqwidehebrew}{00A0}
\pdfglyphtounicode{hlinebelow}{00A0}
\pdfglyphtounicode{hmonospace}{00A0}
\pdfglyphtounicode{hoarmenian}{00A0}
\pdfglyphtounicode{hohipthai}{00A0}
\pdfglyphtounicode{hohiragana}{00A0}
\pdfglyphtounicode{hokatakana}{00A0}
\pdfglyphtounicode{hokatakanahalfwidth}{00A0}
\pdfglyphtounicode{holam}{00A0}
\pdfglyphtounicode{holam19}{00A0}
\pdfglyphtounicode{holam26}{00A0}
\pdfglyphtounicode{holam32}{00A0}
\pdfglyphtounicode{holamhebrew}{00A0}
\pdfglyphtounicode{holamnarrowhebrew}{00A0}
\pdfglyphtounicode{holamquarterhebrew}{00A0}
\pdfglyphtounicode{holamwidehebrew}{00A0}
\pdfglyphtounicode{honokhukthai}{00A0}
\pdfglyphtounicode{hookabovecomb}{00A0}
\pdfglyphtounicode{hookcmb}{00A0}
\pdfglyphtounicode{hookpalatalizedbelowcmb}{00A0}
\pdfglyphtounicode{hookretroflexbelowcmb}{00A0}
\pdfglyphtounicode{hoonsquare}{00A0}
\pdfglyphtounicode{horicoptic}{00A0}
\pdfglyphtounicode{horizontalbar}{00A0}
\pdfglyphtounicode{horncmb}{00A0}
\pdfglyphtounicode{hotsprings}{00A0}
\pdfglyphtounicode{house}{00A0}
\pdfglyphtounicode{hparen}{00A0}
\pdfglyphtounicode{hsuperior}{00A0}
\pdfglyphtounicode{hturned}{00A0}
\pdfglyphtounicode{huhiragana}{00A0}
\pdfglyphtounicode{huiitosquare}{00A0}
\pdfglyphtounicode{hukatakana}{00A0}
\pdfglyphtounicode{hukatakanahalfwidth}{00A0}
\pdfglyphtounicode{hungarumlaut}{00A0}
\pdfglyphtounicode{hungarumlautcmb}{00A0}
\pdfglyphtounicode{hv}{00A0}
\pdfglyphtounicode{hyphen}{00A0}
\pdfglyphtounicode{hyphenchar}{00A0}
\pdfglyphtounicode{hypheninferior}{00A0}
\pdfglyphtounicode{hyphenmonospace}{00A0}
\pdfglyphtounicode{hyphensmall}{00A0}
\pdfglyphtounicode{hyphensuperior}{00A0}
\pdfglyphtounicode{hyphentwo}{00A0}
\pdfglyphtounicode{i}{00A0}
\pdfglyphtounicode{iacute}{00A0}
\pdfglyphtounicode{iacyrillic}{00A0}
\pdfglyphtounicode{ibengali}{00A0}
\pdfglyphtounicode{ibopomofo}{00A0}
\pdfglyphtounicode{ibreve}{00A0}
\pdfglyphtounicode{icaron}{00A0}
\pdfglyphtounicode{icircle}{00A0}
\pdfglyphtounicode{icircumflex}{00A0}
\pdfglyphtounicode{icyrillic}{00A0}
\pdfglyphtounicode{idblgrave}{00A0}
\pdfglyphtounicode{ideographearthcircle}{00A0}
\pdfglyphtounicode{ideographfirecircle}{00A0}
\pdfglyphtounicode{ideographicallianceparen}{00A0}
\pdfglyphtounicode{ideographiccallparen}{00A0}
\pdfglyphtounicode{ideographiccentrecircle}{00A0}
\pdfglyphtounicode{ideographicclose}{00A0}
\pdfglyphtounicode{ideographiccomma}{00A0}
\pdfglyphtounicode{ideographiccommaleft}{00A0}
\pdfglyphtounicode{ideographiccongratulationparen}{00A0}
\pdfglyphtounicode{ideographiccorrectcircle}{00A0}
\pdfglyphtounicode{ideographicearthparen}{00A0}
\pdfglyphtounicode{ideographicenterpriseparen}{00A0}
\pdfglyphtounicode{ideographicexcellentcircle}{00A0}
\pdfglyphtounicode{ideographicfestivalparen}{00A0}
\pdfglyphtounicode{ideographicfinancialcircle}{00A0}
\pdfglyphtounicode{ideographicfinancialparen}{00A0}
\pdfglyphtounicode{ideographicfireparen}{00A0}
\pdfglyphtounicode{ideographichaveparen}{00A0}
\pdfglyphtounicode{ideographichighcircle}{00A0}
\pdfglyphtounicode{ideographiciterationmark}{00A0}
\pdfglyphtounicode{ideographiclaborcircle}{00A0}
\pdfglyphtounicode{ideographiclaborparen}{00A0}
\pdfglyphtounicode{ideographicleftcircle}{00A0}
\pdfglyphtounicode{ideographiclowcircle}{00A0}
\pdfglyphtounicode{ideographicmedicinecircle}{00A0}
\pdfglyphtounicode{ideographicmetalparen}{00A0}
\pdfglyphtounicode{ideographicmoonparen}{00A0}
\pdfglyphtounicode{ideographicnameparen}{00A0}
\pdfglyphtounicode{ideographicperiod}{00A0}
\pdfglyphtounicode{ideographicprintcircle}{00A0}
\pdfglyphtounicode{ideographicreachparen}{00A0}
\pdfglyphtounicode{ideographicrepresentparen}{00A0}
\pdfglyphtounicode{ideographicresourceparen}{00A0}
\pdfglyphtounicode{ideographicrightcircle}{00A0}
\pdfglyphtounicode{ideographicsecretcircle}{00A0}
\pdfglyphtounicode{ideographicselfparen}{00A0}
\pdfglyphtounicode{ideographicsocietyparen}{00A0}
\pdfglyphtounicode{ideographicspace}{00A0}
\pdfglyphtounicode{ideographicspecialparen}{00A0}
\pdfglyphtounicode{ideographicstockparen}{00A0}
\pdfglyphtounicode{ideographicstudyparen}{00A0}
\pdfglyphtounicode{ideographicsunparen}{00A0}
\pdfglyphtounicode{ideographicsuperviseparen}{00A0}
\pdfglyphtounicode{ideographicwaterparen}{00A0}
\pdfglyphtounicode{ideographicwoodparen}{00A0}
\pdfglyphtounicode{ideographiczero}{00A0}
\pdfglyphtounicode{ideographmetalcircle}{00A0}
\pdfglyphtounicode{ideographmooncircle}{00A0}
\pdfglyphtounicode{ideographnamecircle}{00A0}
\pdfglyphtounicode{ideographsuncircle}{00A0}
\pdfglyphtounicode{ideographwatercircle}{00A0}
\pdfglyphtounicode{ideographwoodcircle}{00A0}
\pdfglyphtounicode{ideva}{00A0}
\pdfglyphtounicode{idieresis}{00A0}
\pdfglyphtounicode{idieresisacute}{00A0}
\pdfglyphtounicode{idieresiscyrillic}{00A0}
\pdfglyphtounicode{idotbelow}{00A0}
\pdfglyphtounicode{iebrevecyrillic}{00A0}
\pdfglyphtounicode{iecyrillic}{00A0}
\pdfglyphtounicode{ieungacirclekorean}{00A0}
\pdfglyphtounicode{ieungaparenkorean}{00A0}
\pdfglyphtounicode{ieungcirclekorean}{00A0}
\pdfglyphtounicode{ieungkorean}{00A0}
\pdfglyphtounicode{ieungparenkorean}{00A0}
\pdfglyphtounicode{igrave}{00A0}
\pdfglyphtounicode{igujarati}{00A0}
\pdfglyphtounicode{igurmukhi}{00A0}
\pdfglyphtounicode{ihiragana}{00A0}
\pdfglyphtounicode{ihookabove}{00A0}
\pdfglyphtounicode{iibengali}{00A0}
\pdfglyphtounicode{iicyrillic}{00A0}
\pdfglyphtounicode{iideva}{00A0}
\pdfglyphtounicode{iigujarati}{00A0}
\pdfglyphtounicode{iigurmukhi}{00A0}
\pdfglyphtounicode{iimatragurmukhi}{00A0}
\pdfglyphtounicode{iinvertedbreve}{00A0}
\pdfglyphtounicode{iishortcyrillic}{00A0}
\pdfglyphtounicode{iivowelsignbengali}{00A0}
\pdfglyphtounicode{iivowelsigndeva}{00A0}
\pdfglyphtounicode{iivowelsigngujarati}{00A0}
\pdfglyphtounicode{ij}{00A0}
\pdfglyphtounicode{ikatakana}{00A0}
\pdfglyphtounicode{ikatakanahalfwidth}{00A0}
\pdfglyphtounicode{ikorean}{00A0}
\pdfglyphtounicode{ilde}{00A0}
\pdfglyphtounicode{iluyhebrew}{00A0}
\pdfglyphtounicode{imacron}{00A0}
\pdfglyphtounicode{imacroncyrillic}{00A0}
\pdfglyphtounicode{imageorapproximatelyequal}{00A0}
\pdfglyphtounicode{imatragurmukhi}{00A0}
\pdfglyphtounicode{imonospace}{00A0}
\pdfglyphtounicode{increment}{00A0}
\pdfglyphtounicode{infinity}{00A0}
\pdfglyphtounicode{iniarmenian}{00A0}
\pdfglyphtounicode{integerdivide}{00A0}
\pdfglyphtounicode{integral}{00A0}
\pdfglyphtounicode{integralbottom}{00A0}
\pdfglyphtounicode{integralbt}{00A0}
\pdfglyphtounicode{integralex}{00A0}
\pdfglyphtounicode{integraltop}{00A0}
\pdfglyphtounicode{integraltp}{00A0}
\pdfglyphtounicode{intercal}{00A0}
\pdfglyphtounicode{interrobang}{00A0}
\pdfglyphtounicode{interrobangdown}{00A0}
\pdfglyphtounicode{intersection}{00A0}
\pdfglyphtounicode{intersectiondbl}{00A0}
\pdfglyphtounicode{intersectionsq}{00A0}
\pdfglyphtounicode{intisquare}{00A0}
\pdfglyphtounicode{invbullet}{00A0}
\pdfglyphtounicode{invcircle}{00A0}
\pdfglyphtounicode{invsmileface}{00A0}
\pdfglyphtounicode{iocyrillic}{00A0}
\pdfglyphtounicode{iogonek}{00A0}
\pdfglyphtounicode{iota}{00A0}
\pdfglyphtounicode{iotadieresis}{00A0}
\pdfglyphtounicode{iotadieresistonos}{00A0}
\pdfglyphtounicode{iotalatin}{00A0}
\pdfglyphtounicode{iotatonos}{00A0}
\pdfglyphtounicode{iparen}{00A0}
\pdfglyphtounicode{irigurmukhi}{00A0}
\pdfglyphtounicode{ismallhiragana}{00A0}
\pdfglyphtounicode{ismallkatakana}{00A0}
\pdfglyphtounicode{ismallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{issharbengali}{00A0}
\pdfglyphtounicode{istroke}{00A0}
\pdfglyphtounicode{isuperior}{00A0}
\pdfglyphtounicode{iterationhiragana}{00A0}
\pdfglyphtounicode{iterationkatakana}{00A0}
\pdfglyphtounicode{itilde}{00A0}
\pdfglyphtounicode{itildebelow}{00A0}
\pdfglyphtounicode{iubopomofo}{00A0}
\pdfglyphtounicode{iucyrillic}{00A0}
\pdfglyphtounicode{ivowelsignbengali}{00A0}
\pdfglyphtounicode{ivowelsigndeva}{00A0}
\pdfglyphtounicode{ivowelsigngujarati}{00A0}
\pdfglyphtounicode{izhitsacyrillic}{00A0}
\pdfglyphtounicode{izhitsadblgravecyrillic}{00A0}
\pdfglyphtounicode{j}{00A0}
\pdfglyphtounicode{jaarmenian}{00A0}
\pdfglyphtounicode{jabengali}{00A0}
\pdfglyphtounicode{jadeva}{00A0}
\pdfglyphtounicode{jagujarati}{00A0}
\pdfglyphtounicode{jagurmukhi}{00A0}
\pdfglyphtounicode{jbopomofo}{00A0}
\pdfglyphtounicode{jcaron}{00A0}
\pdfglyphtounicode{jcircle}{00A0}
\pdfglyphtounicode{jcircumflex}{00A0}
\pdfglyphtounicode{jcrossedtail}{00A0}
\pdfglyphtounicode{jdotlessstroke}{00A0}
\pdfglyphtounicode{jecyrillic}{00A0}
\pdfglyphtounicode{jeemarabic}{00A0}
\pdfglyphtounicode{jeemfinalarabic}{00A0}
\pdfglyphtounicode{jeeminitialarabic}{00A0}
\pdfglyphtounicode{jeemmedialarabic}{00A0}
\pdfglyphtounicode{jeharabic}{00A0}
\pdfglyphtounicode{jehfinalarabic}{00A0}
\pdfglyphtounicode{jhabengali}{00A0}
\pdfglyphtounicode{jhadeva}{00A0}
\pdfglyphtounicode{jhagujarati}{00A0}
\pdfglyphtounicode{jhagurmukhi}{00A0}
\pdfglyphtounicode{jheharmenian}{00A0}
\pdfglyphtounicode{jis}{00A0}
\pdfglyphtounicode{jmonospace}{00A0}
\pdfglyphtounicode{jparen}{00A0}
\pdfglyphtounicode{jsuperior}{00A0}
\pdfglyphtounicode{k}{00A0}
\pdfglyphtounicode{kabashkircyrillic}{00A0}
\pdfglyphtounicode{kabengali}{00A0}
\pdfglyphtounicode{kacute}{00A0}
\pdfglyphtounicode{kacyrillic}{00A0}
\pdfglyphtounicode{kadescendercyrillic}{00A0}
\pdfglyphtounicode{kadeva}{00A0}
\pdfglyphtounicode{kaf}{00A0}
\pdfglyphtounicode{kafarabic}{00A0}
\pdfglyphtounicode{kafdagesh}{00A0}
\pdfglyphtounicode{kafdageshhebrew}{00A0}
\pdfglyphtounicode{kaffinalarabic}{00A0}
\pdfglyphtounicode{kafhebrew}{00A0}
\pdfglyphtounicode{kafinitialarabic}{00A0}
\pdfglyphtounicode{kafmedialarabic}{00A0}
\pdfglyphtounicode{kafrafehebrew}{00A0}
\pdfglyphtounicode{kagujarati}{00A0}
\pdfglyphtounicode{kagurmukhi}{00A0}
\pdfglyphtounicode{kahiragana}{00A0}
\pdfglyphtounicode{kahookcyrillic}{00A0}
\pdfglyphtounicode{kakatakana}{00A0}
\pdfglyphtounicode{kakatakanahalfwidth}{00A0}
\pdfglyphtounicode{kappa}{00A0}
\pdfglyphtounicode{kappasymbolgreek}{00A0}
\pdfglyphtounicode{kapyeounmieumkorean}{00A0}
\pdfglyphtounicode{kapyeounphieuphkorean}{00A0}
\pdfglyphtounicode{kapyeounpieupkorean}{00A0}
\pdfglyphtounicode{kapyeounssangpieupkorean}{00A0}
\pdfglyphtounicode{karoriisquare}{00A0}
\pdfglyphtounicode{kashidaautoarabic}{00A0}
\pdfglyphtounicode{kashidaautonosidebearingarabic}{00A0}
\pdfglyphtounicode{kasmallkatakana}{00A0}
\pdfglyphtounicode{kasquare}{00A0}
\pdfglyphtounicode{kasraarabic}{00A0}
\pdfglyphtounicode{kasratanarabic}{00A0}
\pdfglyphtounicode{kastrokecyrillic}{00A0}
\pdfglyphtounicode{katahiraprolongmarkhalfwidth}{00A0}
\pdfglyphtounicode{kaverticalstrokecyrillic}{00A0}
\pdfglyphtounicode{kbopomofo}{00A0}
\pdfglyphtounicode{kcalsquare}{00A0}
\pdfglyphtounicode{kcaron}{00A0}
\pdfglyphtounicode{kcedilla}{00A0}
\pdfglyphtounicode{kcircle}{00A0}
\pdfglyphtounicode{kcommaaccent}{00A0}
\pdfglyphtounicode{kdotbelow}{00A0}
\pdfglyphtounicode{keharmenian}{00A0}
\pdfglyphtounicode{kehiragana}{00A0}
\pdfglyphtounicode{kekatakana}{00A0}
\pdfglyphtounicode{kekatakanahalfwidth}{00A0}
\pdfglyphtounicode{kenarmenian}{00A0}
\pdfglyphtounicode{kesmallkatakana}{00A0}
\pdfglyphtounicode{kgreenlandic}{00A0}
\pdfglyphtounicode{khabengali}{00A0}
\pdfglyphtounicode{khacyrillic}{00A0}
\pdfglyphtounicode{khadeva}{00A0}
\pdfglyphtounicode{khagujarati}{00A0}
\pdfglyphtounicode{khagurmukhi}{00A0}
\pdfglyphtounicode{khaharabic}{00A0}
\pdfglyphtounicode{khahfinalarabic}{00A0}
\pdfglyphtounicode{khahinitialarabic}{00A0}
\pdfglyphtounicode{khahmedialarabic}{00A0}
\pdfglyphtounicode{kheicoptic}{00A0}
\pdfglyphtounicode{khhadeva}{00A0}
\pdfglyphtounicode{khhagurmukhi}{00A0}
\pdfglyphtounicode{khieukhacirclekorean}{00A0}
\pdfglyphtounicode{khieukhaparenkorean}{00A0}
\pdfglyphtounicode{khieukhcirclekorean}{00A0}
\pdfglyphtounicode{khieukhkorean}{00A0}
\pdfglyphtounicode{khieukhparenkorean}{00A0}
\pdfglyphtounicode{khokhaithai}{00A0}
\pdfglyphtounicode{khokhonthai}{00A0}
\pdfglyphtounicode{khokhuatthai}{00A0}
\pdfglyphtounicode{khokhwaithai}{00A0}
\pdfglyphtounicode{khomutthai}{00A0}
\pdfglyphtounicode{khook}{00A0}
\pdfglyphtounicode{khorakhangthai}{00A0}
\pdfglyphtounicode{khzsquare}{00A0}
\pdfglyphtounicode{kihiragana}{00A0}
\pdfglyphtounicode{kikatakana}{00A0}
\pdfglyphtounicode{kikatakanahalfwidth}{00A0}
\pdfglyphtounicode{kiroguramusquare}{00A0}
\pdfglyphtounicode{kiromeetorusquare}{00A0}
\pdfglyphtounicode{kirosquare}{00A0}
\pdfglyphtounicode{kiyeokacirclekorean}{00A0}
\pdfglyphtounicode{kiyeokaparenkorean}{00A0}
\pdfglyphtounicode{kiyeokcirclekorean}{00A0}
\pdfglyphtounicode{kiyeokkorean}{00A0}
\pdfglyphtounicode{kiyeokparenkorean}{00A0}
\pdfglyphtounicode{kiyeoksioskorean}{00A0}
\pdfglyphtounicode{kjecyrillic}{00A0}
\pdfglyphtounicode{klinebelow}{00A0}
\pdfglyphtounicode{klsquare}{00A0}
\pdfglyphtounicode{kmcubedsquare}{00A0}
\pdfglyphtounicode{kmonospace}{00A0}
\pdfglyphtounicode{kmsquaredsquare}{00A0}
\pdfglyphtounicode{kohiragana}{00A0}
\pdfglyphtounicode{kohmsquare}{00A0}
\pdfglyphtounicode{kokaithai}{00A0}
\pdfglyphtounicode{kokatakana}{00A0}
\pdfglyphtounicode{kokatakanahalfwidth}{00A0}
\pdfglyphtounicode{kooposquare}{00A0}
\pdfglyphtounicode{koppacyrillic}{00A0}
\pdfglyphtounicode{koreanstandardsymbol}{00A0}
\pdfglyphtounicode{koroniscmb}{00A0}
\pdfglyphtounicode{kparen}{00A0}
\pdfglyphtounicode{kpasquare}{00A0}
\pdfglyphtounicode{ksicyrillic}{00A0}
\pdfglyphtounicode{ktsquare}{00A0}
\pdfglyphtounicode{kturned}{00A0}
\pdfglyphtounicode{kuhiragana}{00A0}
\pdfglyphtounicode{kukatakana}{00A0}
\pdfglyphtounicode{kukatakanahalfwidth}{00A0}
\pdfglyphtounicode{kvsquare}{00A0}
\pdfglyphtounicode{kwsquare}{00A0}
\pdfglyphtounicode{l}{00A0}
\pdfglyphtounicode{labengali}{00A0}
\pdfglyphtounicode{lacute}{00A0}
\pdfglyphtounicode{ladeva}{00A0}
\pdfglyphtounicode{lagujarati}{00A0}
\pdfglyphtounicode{lagurmukhi}{00A0}
\pdfglyphtounicode{lakkhangyaothai}{00A0}
\pdfglyphtounicode{lamaleffinalarabic}{00A0}
\pdfglyphtounicode{lamalefhamzaabovefinalarabic}{00A0}
\pdfglyphtounicode{lamalefhamzaaboveisolatedarabic}{00A0}
\pdfglyphtounicode{lamalefhamzabelowfinalarabic}{00A0}
\pdfglyphtounicode{lamalefhamzabelowisolatedarabic}{00A0}
\pdfglyphtounicode{lamalefisolatedarabic}{00A0}
\pdfglyphtounicode{lamalefmaddaabovefinalarabic}{00A0}
\pdfglyphtounicode{lamalefmaddaaboveisolatedarabic}{00A0}
\pdfglyphtounicode{lamarabic}{00A0}
\pdfglyphtounicode{lambda}{00A0}
\pdfglyphtounicode{lambdastroke}{00A0}
\pdfglyphtounicode{lamed}{00A0}
\pdfglyphtounicode{lameddagesh}{00A0}
\pdfglyphtounicode{lameddageshhebrew}{00A0}
\pdfglyphtounicode{lamedhebrew}{00A0}
\pdfglyphtounicode{lamedholam}{00A0}
\pdfglyphtounicode{lamedholamdagesh}{00A0}
\pdfglyphtounicode{lamedholamdageshhebrew}{00A0}
\pdfglyphtounicode{lamedholamhebrew}{00A0}
\pdfglyphtounicode{lamfinalarabic}{00A0}
\pdfglyphtounicode{lamhahinitialarabic}{00A0}
\pdfglyphtounicode{laminitialarabic}{00A0}
\pdfglyphtounicode{lamjeeminitialarabic}{00A0}
\pdfglyphtounicode{lamkhahinitialarabic}{00A0}
\pdfglyphtounicode{lamlamhehisolatedarabic}{00A0}
\pdfglyphtounicode{lammedialarabic}{00A0}
\pdfglyphtounicode{lammeemhahinitialarabic}{00A0}
\pdfglyphtounicode{lammeeminitialarabic}{00A0}
\pdfglyphtounicode{lammeemjeeminitialarabic}{00A0}
\pdfglyphtounicode{lammeemkhahinitialarabic}{00A0}
\pdfglyphtounicode{largecircle}{00A0}
\pdfglyphtounicode{latticetop}{00A0}
\pdfglyphtounicode{lbar}{00A0}
\pdfglyphtounicode{lbelt}{00A0}
\pdfglyphtounicode{lbopomofo}{00A0}
\pdfglyphtounicode{lcaron}{00A0}
\pdfglyphtounicode{lcedilla}{00A0}
\pdfglyphtounicode{lcircle}{00A0}
\pdfglyphtounicode{lcircumflexbelow}{00A0}
\pdfglyphtounicode{lcommaaccent}{00A0}
\pdfglyphtounicode{ldot}{00A0}
\pdfglyphtounicode{ldotaccent}{00A0}
\pdfglyphtounicode{ldotbelow}{00A0}
\pdfglyphtounicode{ldotbelowmacron}{00A0}
\pdfglyphtounicode{leftangleabovecmb}{00A0}
\pdfglyphtounicode{lefttackbelowcmb}{00A0}
\pdfglyphtounicode{less}{00A0}
\pdfglyphtounicode{lessdbleqlgreater}{00A0}
\pdfglyphtounicode{lessdblequal}{00A0}
\pdfglyphtounicode{lessdot}{00A0}
\pdfglyphtounicode{lessequal}{00A0}
\pdfglyphtounicode{lessequalgreater}{00A0}
\pdfglyphtounicode{lessequalorgreater}{00A0}
\pdfglyphtounicode{lessmonospace}{00A0}
\pdfglyphtounicode{lessmuch}{00A0}
\pdfglyphtounicode{lessnotdblequal}{00A0}
\pdfglyphtounicode{lessnotequal}{00A0}
\pdfglyphtounicode{lessorapproxeql}{00A0}
\pdfglyphtounicode{lessorequalslant}{00A0}
\pdfglyphtounicode{lessorequivalent}{00A0}
\pdfglyphtounicode{lessorgreater}{00A0}
\pdfglyphtounicode{lessornotdbleql}{00A0}
\pdfglyphtounicode{lessornotequal}{00A0}
\pdfglyphtounicode{lessorsimilar}{00A0}
\pdfglyphtounicode{lessoverequal}{00A0}
\pdfglyphtounicode{lesssmall}{00A0}
\pdfglyphtounicode{lezh}{00A0}
\pdfglyphtounicode{lfblock}{00A0}
\pdfglyphtounicode{lhookretroflex}{00A0}
\pdfglyphtounicode{lira}{00A0}
\pdfglyphtounicode{liwnarmenian}{00A0}
\pdfglyphtounicode{lj}{00A0}
\pdfglyphtounicode{ljecyrillic}{00A0}
\pdfglyphtounicode{ll}{00A0}
\pdfglyphtounicode{lladeva}{00A0}
\pdfglyphtounicode{llagujarati}{00A0}
\pdfglyphtounicode{llinebelow}{00A0}
\pdfglyphtounicode{llladeva}{00A0}
\pdfglyphtounicode{llvocalicbengali}{00A0}
\pdfglyphtounicode{llvocalicdeva}{00A0}
\pdfglyphtounicode{llvocalicvowelsignbengali}{00A0}
\pdfglyphtounicode{llvocalicvowelsigndeva}{00A0}
\pdfglyphtounicode{lmiddletilde}{00A0}
\pdfglyphtounicode{lmonospace}{00A0}
\pdfglyphtounicode{lmsquare}{00A0}
\pdfglyphtounicode{lochulathai}{00A0}
\pdfglyphtounicode{logicaland}{00A0}
\pdfglyphtounicode{logicalnot}{00A0}
\pdfglyphtounicode{logicalnotreversed}{00A0}
\pdfglyphtounicode{logicalor}{00A0}
\pdfglyphtounicode{lolingthai}{00A0}
\pdfglyphtounicode{longdbls}{00A0}
\pdfglyphtounicode{longs}{00A0}
\pdfglyphtounicode{longsh}{00A0}
\pdfglyphtounicode{longsi}{00A0}
\pdfglyphtounicode{longsl}{00A0}
\pdfglyphtounicode{longst}{00A0}
\pdfglyphtounicode{lowlinecenterline}{00A0}
\pdfglyphtounicode{lowlinecmb}{00A0}
\pdfglyphtounicode{lowlinedashed}{00A0}
\pdfglyphtounicode{lozenge}{00A0}
\pdfglyphtounicode{lparen}{00A0}
\pdfglyphtounicode{lscript}{00A0}
\pdfglyphtounicode{lslash}{00A0}
\pdfglyphtounicode{lsquare}{00A0}
\pdfglyphtounicode{lsuperior}{00A0}
\pdfglyphtounicode{ltshade}{00A0}
\pdfglyphtounicode{luthai}{00A0}
\pdfglyphtounicode{lvocalicbengali}{00A0}
\pdfglyphtounicode{lvocalicdeva}{00A0}
\pdfglyphtounicode{lvocalicvowelsignbengali}{00A0}
\pdfglyphtounicode{lvocalicvowelsigndeva}{00A0}
\pdfglyphtounicode{lxsquare}{00A0}
\pdfglyphtounicode{m}{00A0}
\pdfglyphtounicode{mabengali}{00A0}
\pdfglyphtounicode{macron}{00A0}
\pdfglyphtounicode{macronbelowcmb}{00A0}
\pdfglyphtounicode{macroncmb}{00A0}
\pdfglyphtounicode{macronlowmod}{00A0}
\pdfglyphtounicode{macronmonospace}{00A0}
\pdfglyphtounicode{macute}{00A0}
\pdfglyphtounicode{madeva}{00A0}
\pdfglyphtounicode{magujarati}{00A0}
\pdfglyphtounicode{magurmukhi}{00A0}
\pdfglyphtounicode{mahapakhhebrew}{00A0}
\pdfglyphtounicode{mahapakhlefthebrew}{00A0}
\pdfglyphtounicode{mahiragana}{00A0}
\pdfglyphtounicode{maichattawalowleftthai}{00A0}
\pdfglyphtounicode{maichattawalowrightthai}{00A0}
\pdfglyphtounicode{maichattawathai}{00A0}
\pdfglyphtounicode{maichattawaupperleftthai}{00A0}
\pdfglyphtounicode{maieklowleftthai}{00A0}
\pdfglyphtounicode{maieklowrightthai}{00A0}
\pdfglyphtounicode{maiekthai}{00A0}
\pdfglyphtounicode{maiekupperleftthai}{00A0}
\pdfglyphtounicode{maihanakatleftthai}{00A0}
\pdfglyphtounicode{maihanakatthai}{00A0}
\pdfglyphtounicode{maitaikhuleftthai}{00A0}
\pdfglyphtounicode{maitaikhuthai}{00A0}
\pdfglyphtounicode{maitholowleftthai}{00A0}
\pdfglyphtounicode{maitholowrightthai}{00A0}
\pdfglyphtounicode{maithothai}{00A0}
\pdfglyphtounicode{maithoupperleftthai}{00A0}
\pdfglyphtounicode{maitrilowleftthai}{00A0}
\pdfglyphtounicode{maitrilowrightthai}{00A0}
\pdfglyphtounicode{maitrithai}{00A0}
\pdfglyphtounicode{maitriupperleftthai}{00A0}
\pdfglyphtounicode{maiyamokthai}{00A0}
\pdfglyphtounicode{makatakana}{00A0}
\pdfglyphtounicode{makatakanahalfwidth}{00A0}
\pdfglyphtounicode{male}{00A0}
\pdfglyphtounicode{maltesecross}{00A0}
\pdfglyphtounicode{mansyonsquare}{00A0}
\pdfglyphtounicode{maqafhebrew}{00A0}
\pdfglyphtounicode{mars}{00A0}
\pdfglyphtounicode{masoracirclehebrew}{00A0}
\pdfglyphtounicode{masquare}{00A0}
\pdfglyphtounicode{mbopomofo}{00A0}
\pdfglyphtounicode{mbsquare}{00A0}
\pdfglyphtounicode{mcircle}{00A0}
\pdfglyphtounicode{mcubedsquare}{00A0}
\pdfglyphtounicode{mdotaccent}{00A0}
\pdfglyphtounicode{mdotbelow}{00A0}
\pdfglyphtounicode{measuredangle}{00A0}
\pdfglyphtounicode{meemarabic}{00A0}
\pdfglyphtounicode{meemfinalarabic}{00A0}
\pdfglyphtounicode{meeminitialarabic}{00A0}
\pdfglyphtounicode{meemmedialarabic}{00A0}
\pdfglyphtounicode{meemmeeminitialarabic}{00A0}
\pdfglyphtounicode{meemmeemisolatedarabic}{00A0}
\pdfglyphtounicode{meetorusquare}{00A0}
\pdfglyphtounicode{mehiragana}{00A0}
\pdfglyphtounicode{meizierasquare}{00A0}
\pdfglyphtounicode{mekatakana}{00A0}
\pdfglyphtounicode{mekatakanahalfwidth}{00A0}
\pdfglyphtounicode{mem}{00A0}
\pdfglyphtounicode{memdagesh}{00A0}
\pdfglyphtounicode{memdageshhebrew}{00A0}
\pdfglyphtounicode{memhebrew}{00A0}
\pdfglyphtounicode{menarmenian}{00A0}
\pdfglyphtounicode{merkhahebrew}{00A0}
\pdfglyphtounicode{merkhakefulahebrew}{00A0}
\pdfglyphtounicode{merkhakefulalefthebrew}{00A0}
\pdfglyphtounicode{merkhalefthebrew}{00A0}
\pdfglyphtounicode{mhook}{00A0}
\pdfglyphtounicode{mhzsquare}{00A0}
\pdfglyphtounicode{middledotkatakanahalfwidth}{00A0}
\pdfglyphtounicode{middot}{00A0}
\pdfglyphtounicode{mieumacirclekorean}{00A0}
\pdfglyphtounicode{mieumaparenkorean}{00A0}
\pdfglyphtounicode{mieumcirclekorean}{00A0}
\pdfglyphtounicode{mieumkorean}{00A0}
\pdfglyphtounicode{mieumpansioskorean}{00A0}
\pdfglyphtounicode{mieumparenkorean}{00A0}
\pdfglyphtounicode{mieumpieupkorean}{00A0}
\pdfglyphtounicode{mieumsioskorean}{00A0}
\pdfglyphtounicode{mihiragana}{00A0}
\pdfglyphtounicode{mikatakana}{00A0}
\pdfglyphtounicode{mikatakanahalfwidth}{00A0}
\pdfglyphtounicode{minus}{00A0}
\pdfglyphtounicode{minusbelowcmb}{00A0}
\pdfglyphtounicode{minuscircle}{00A0}
\pdfglyphtounicode{minusmod}{00A0}
\pdfglyphtounicode{minusplus}{00A0}
\pdfglyphtounicode{minute}{00A0}
\pdfglyphtounicode{miribaarusquare}{00A0}
\pdfglyphtounicode{mirisquare}{00A0}
\pdfglyphtounicode{mlonglegturned}{00A0}
\pdfglyphtounicode{mlsquare}{00A0}
\pdfglyphtounicode{mmcubedsquare}{00A0}
\pdfglyphtounicode{mmonospace}{00A0}
\pdfglyphtounicode{mmsquaredsquare}{00A0}
\pdfglyphtounicode{mohiragana}{00A0}
\pdfglyphtounicode{mohmsquare}{00A0}
\pdfglyphtounicode{mokatakana}{00A0}
\pdfglyphtounicode{mokatakanahalfwidth}{00A0}
\pdfglyphtounicode{molsquare}{00A0}
\pdfglyphtounicode{momathai}{00A0}
\pdfglyphtounicode{moverssquare}{00A0}
\pdfglyphtounicode{moverssquaredsquare}{00A0}
\pdfglyphtounicode{mparen}{00A0}
\pdfglyphtounicode{mpasquare}{00A0}
\pdfglyphtounicode{mssquare}{00A0}
\pdfglyphtounicode{msuperior}{00A0}
\pdfglyphtounicode{mturned}{00A0}
\pdfglyphtounicode{mu}{00A0}
\pdfglyphtounicode{mu1}{00A0}
\pdfglyphtounicode{muasquare}{00A0}
\pdfglyphtounicode{muchgreater}{00A0}
\pdfglyphtounicode{muchless}{00A0}
\pdfglyphtounicode{mufsquare}{00A0}
\pdfglyphtounicode{mugreek}{00A0}
\pdfglyphtounicode{mugsquare}{00A0}
\pdfglyphtounicode{muhiragana}{00A0}
\pdfglyphtounicode{mukatakana}{00A0}
\pdfglyphtounicode{mukatakanahalfwidth}{00A0}
\pdfglyphtounicode{mulsquare}{00A0}
\pdfglyphtounicode{multicloseleft}{00A0}
\pdfglyphtounicode{multicloseright}{00A0}
\pdfglyphtounicode{multimap}{00A0}
\pdfglyphtounicode{multiopenleft}{00A0}
\pdfglyphtounicode{multiopenright}{00A0}
\pdfglyphtounicode{multiply}{00A0}
\pdfglyphtounicode{mumsquare}{00A0}
\pdfglyphtounicode{munahhebrew}{00A0}
\pdfglyphtounicode{munahlefthebrew}{00A0}
\pdfglyphtounicode{musicalnote}{00A0}
\pdfglyphtounicode{musicalnotedbl}{00A0}
\pdfglyphtounicode{musicflatsign}{00A0}
\pdfglyphtounicode{musicsharpsign}{00A0}
\pdfglyphtounicode{mussquare}{00A0}
\pdfglyphtounicode{muvsquare}{00A0}
\pdfglyphtounicode{muwsquare}{00A0}
\pdfglyphtounicode{mvmegasquare}{00A0}
\pdfglyphtounicode{mvsquare}{00A0}
\pdfglyphtounicode{mwmegasquare}{00A0}
\pdfglyphtounicode{mwsquare}{00A0}
\pdfglyphtounicode{n}{00A0}
\pdfglyphtounicode{nabengali}{00A0}
\pdfglyphtounicode{nabla}{00A0}
\pdfglyphtounicode{nacute}{00A0}
\pdfglyphtounicode{nadeva}{00A0}
\pdfglyphtounicode{nagujarati}{00A0}
\pdfglyphtounicode{nagurmukhi}{00A0}
\pdfglyphtounicode{nahiragana}{00A0}
\pdfglyphtounicode{nakatakana}{00A0}
\pdfglyphtounicode{nakatakanahalfwidth}{00A0}
\pdfglyphtounicode{nand}{00A0}
\pdfglyphtounicode{napostrophe}{00A0}
\pdfglyphtounicode{nasquare}{00A0}
\pdfglyphtounicode{natural}{00A0}
\pdfglyphtounicode{nbopomofo}{00A0}
\pdfglyphtounicode{nbspace}{00A0}
\pdfglyphtounicode{ncaron}{00A0}
\pdfglyphtounicode{ncedilla}{00A0}
\pdfglyphtounicode{ncircle}{00A0}
\pdfglyphtounicode{ncircumflexbelow}{00A0}
\pdfglyphtounicode{ncommaaccent}{00A0}
\pdfglyphtounicode{ndotaccent}{00A0}
\pdfglyphtounicode{ndotbelow}{00A0}
\pdfglyphtounicode{negationslash}{00A0}
\pdfglyphtounicode{nehiragana}{00A0}
\pdfglyphtounicode{nekatakana}{00A0}
\pdfglyphtounicode{nekatakanahalfwidth}{00A0}
\pdfglyphtounicode{newsheqelsign}{00A0}
\pdfglyphtounicode{nfsquare}{00A0}
\pdfglyphtounicode{ng}{00A0}
\pdfglyphtounicode{ngabengali}{00A0}
\pdfglyphtounicode{ngadeva}{00A0}
\pdfglyphtounicode{ngagujarati}{00A0}
\pdfglyphtounicode{ngagurmukhi}{00A0}
\pdfglyphtounicode{ngonguthai}{00A0}
\pdfglyphtounicode{nhiragana}{00A0}
\pdfglyphtounicode{nhookleft}{00A0}
\pdfglyphtounicode{nhookretroflex}{00A0}
\pdfglyphtounicode{nieunacirclekorean}{00A0}
\pdfglyphtounicode{nieunaparenkorean}{00A0}
\pdfglyphtounicode{nieuncieuckorean}{00A0}
\pdfglyphtounicode{nieuncirclekorean}{00A0}
\pdfglyphtounicode{nieunhieuhkorean}{00A0}
\pdfglyphtounicode{nieunkorean}{00A0}
\pdfglyphtounicode{nieunpansioskorean}{00A0}
\pdfglyphtounicode{nieunparenkorean}{00A0}
\pdfglyphtounicode{nieunsioskorean}{00A0}
\pdfglyphtounicode{nieuntikeutkorean}{00A0}
\pdfglyphtounicode{nihiragana}{00A0}
\pdfglyphtounicode{nikatakana}{00A0}
\pdfglyphtounicode{nikatakanahalfwidth}{00A0}
\pdfglyphtounicode{nikhahitleftthai}{00A0}
\pdfglyphtounicode{nikhahitthai}{00A0}
\pdfglyphtounicode{nine}{00A0}
\pdfglyphtounicode{ninearabic}{00A0}
\pdfglyphtounicode{ninebengali}{00A0}
\pdfglyphtounicode{ninecircle}{00A0}
\pdfglyphtounicode{ninecircleinversesansserif}{00A0}
\pdfglyphtounicode{ninedeva}{00A0}
\pdfglyphtounicode{ninegujarati}{00A0}
\pdfglyphtounicode{ninegurmukhi}{00A0}
\pdfglyphtounicode{ninehackarabic}{00A0}
\pdfglyphtounicode{ninehangzhou}{00A0}
\pdfglyphtounicode{nineideographicparen}{00A0}
\pdfglyphtounicode{nineinferior}{00A0}
\pdfglyphtounicode{ninemonospace}{00A0}
\pdfglyphtounicode{nineoldstyle}{00A0}
\pdfglyphtounicode{nineparen}{00A0}
\pdfglyphtounicode{nineperiod}{00A0}
\pdfglyphtounicode{ninepersian}{00A0}
\pdfglyphtounicode{nineroman}{00A0}
\pdfglyphtounicode{ninesuperior}{00A0}
\pdfglyphtounicode{nineteencircle}{00A0}
\pdfglyphtounicode{nineteenparen}{00A0}
\pdfglyphtounicode{nineteenperiod}{00A0}
\pdfglyphtounicode{ninethai}{00A0}
\pdfglyphtounicode{nj}{00A0}
\pdfglyphtounicode{njecyrillic}{00A0}
\pdfglyphtounicode{nkatakana}{00A0}
\pdfglyphtounicode{nkatakanahalfwidth}{00A0}
\pdfglyphtounicode{nlegrightlong}{00A0}
\pdfglyphtounicode{nlinebelow}{00A0}
\pdfglyphtounicode{nmonospace}{00A0}
\pdfglyphtounicode{nmsquare}{00A0}
\pdfglyphtounicode{nnabengali}{00A0}
\pdfglyphtounicode{nnadeva}{00A0}
\pdfglyphtounicode{nnagujarati}{00A0}
\pdfglyphtounicode{nnagurmukhi}{00A0}
\pdfglyphtounicode{nnnadeva}{00A0}
\pdfglyphtounicode{nohiragana}{00A0}
\pdfglyphtounicode{nokatakana}{00A0}
\pdfglyphtounicode{nokatakanahalfwidth}{00A0}
\pdfglyphtounicode{nonbreakingspace}{00A0}
\pdfglyphtounicode{nonenthai}{00A0}
\pdfglyphtounicode{nonuthai}{00A0}
\pdfglyphtounicode{noonarabic}{00A0}
\pdfglyphtounicode{noonfinalarabic}{00A0}
\pdfglyphtounicode{noonghunnaarabic}{00A0}
\pdfglyphtounicode{noonghunnafinalarabic}{00A0}
\pdfglyphtounicode{noonhehinitialarabic}{00A0}
\pdfglyphtounicode{nooninitialarabic}{00A0}
\pdfglyphtounicode{noonjeeminitialarabic}{00A0}
\pdfglyphtounicode{noonjeemisolatedarabic}{00A0}
\pdfglyphtounicode{noonmedialarabic}{00A0}
\pdfglyphtounicode{noonmeeminitialarabic}{00A0}
\pdfglyphtounicode{noonmeemisolatedarabic}{00A0}
\pdfglyphtounicode{noonnoonfinalarabic}{00A0}
\pdfglyphtounicode{notapproxequal}{00A0}
\pdfglyphtounicode{notarrowboth}{00A0}
\pdfglyphtounicode{notarrowleft}{00A0}
\pdfglyphtounicode{notarrowright}{00A0}
\pdfglyphtounicode{notbar}{00A0}
\pdfglyphtounicode{notcontains}{00A0}
\pdfglyphtounicode{notdblarrowboth}{00A0}
\pdfglyphtounicode{notdblarrowleft}{00A0}
\pdfglyphtounicode{notdblarrowright}{00A0}
\pdfglyphtounicode{notelement}{00A0}
\pdfglyphtounicode{notelementof}{00A0}
\pdfglyphtounicode{notequal}{00A0}
\pdfglyphtounicode{notexistential}{00A0}
\pdfglyphtounicode{notfollows}{00A0}
\pdfglyphtounicode{notfollowsoreql}{00A0}
\pdfglyphtounicode{notforces}{00A0}
\pdfglyphtounicode{notforcesextra}{00A0}
\pdfglyphtounicode{notgreater}{00A0}
\pdfglyphtounicode{notgreaterdblequal}{00A0}
\pdfglyphtounicode{notgreaterequal}{00A0}
\pdfglyphtounicode{notgreaternorequal}{00A0}
\pdfglyphtounicode{notgreaternorless}{00A0}
\pdfglyphtounicode{notgreaterorslnteql}{00A0}
\pdfglyphtounicode{notidentical}{00A0}
\pdfglyphtounicode{notless}{00A0}
\pdfglyphtounicode{notlessdblequal}{00A0}
\pdfglyphtounicode{notlessequal}{00A0}
\pdfglyphtounicode{notlessnorequal}{00A0}
\pdfglyphtounicode{notlessorslnteql}{00A0}
\pdfglyphtounicode{notparallel}{00A0}
\pdfglyphtounicode{notprecedes}{00A0}
\pdfglyphtounicode{notprecedesoreql}{00A0}
\pdfglyphtounicode{notsatisfies}{00A0}
\pdfglyphtounicode{notsimilar}{00A0}
\pdfglyphtounicode{notsubset}{00A0}
\pdfglyphtounicode{notsubseteql}{00A0}
\pdfglyphtounicode{notsubsetordbleql}{00A0}
\pdfglyphtounicode{notsubsetoreql}{00A0}
\pdfglyphtounicode{notsucceeds}{00A0}
\pdfglyphtounicode{notsuperset}{00A0}
\pdfglyphtounicode{notsuperseteql}{00A0}
\pdfglyphtounicode{notsupersetordbleql}{00A0}
\pdfglyphtounicode{notsupersetoreql}{00A0}
\pdfglyphtounicode{nottriangeqlleft}{00A0}
\pdfglyphtounicode{nottriangeqlright}{00A0}
\pdfglyphtounicode{nottriangleleft}{00A0}
\pdfglyphtounicode{nottriangleright}{00A0}
\pdfglyphtounicode{notturnstile}{00A0}
\pdfglyphtounicode{nowarmenian}{00A0}
\pdfglyphtounicode{nparen}{00A0}
\pdfglyphtounicode{nssquare}{00A0}
\pdfglyphtounicode{nsuperior}{00A0}
\pdfglyphtounicode{ntilde}{00A0}
\pdfglyphtounicode{nu}{00A0}
\pdfglyphtounicode{nuhiragana}{00A0}
\pdfglyphtounicode{nukatakana}{00A0}
\pdfglyphtounicode{nukatakanahalfwidth}{00A0}
\pdfglyphtounicode{nuktabengali}{00A0}
\pdfglyphtounicode{nuktadeva}{00A0}
\pdfglyphtounicode{nuktagujarati}{00A0}
\pdfglyphtounicode{nuktagurmukhi}{00A0}
\pdfglyphtounicode{numbersign}{00A0}
\pdfglyphtounicode{numbersignmonospace}{00A0}
\pdfglyphtounicode{numbersignsmall}{00A0}
\pdfglyphtounicode{numeralsigngreek}{00A0}
\pdfglyphtounicode{numeralsignlowergreek}{00A0}
\pdfglyphtounicode{numero}{00A0}
\pdfglyphtounicode{nun}{00A0}
\pdfglyphtounicode{nundagesh}{00A0}
\pdfglyphtounicode{nundageshhebrew}{00A0}
\pdfglyphtounicode{nunhebrew}{00A0}
\pdfglyphtounicode{nvsquare}{00A0}
\pdfglyphtounicode{nwsquare}{00A0}
\pdfglyphtounicode{nyabengali}{00A0}
\pdfglyphtounicode{nyadeva}{00A0}
\pdfglyphtounicode{nyagujarati}{00A0}
\pdfglyphtounicode{nyagurmukhi}{00A0}
\pdfglyphtounicode{o}{00A0}
\pdfglyphtounicode{oacute}{00A0}
\pdfglyphtounicode{oangthai}{00A0}
\pdfglyphtounicode{obarred}{00A0}
\pdfglyphtounicode{obarredcyrillic}{00A0}
\pdfglyphtounicode{obarreddieresiscyrillic}{00A0}
\pdfglyphtounicode{obengali}{00A0}
\pdfglyphtounicode{obopomofo}{00A0}
\pdfglyphtounicode{obreve}{00A0}
\pdfglyphtounicode{ocandradeva}{00A0}
\pdfglyphtounicode{ocandragujarati}{00A0}
\pdfglyphtounicode{ocandravowelsigndeva}{00A0}
\pdfglyphtounicode{ocandravowelsigngujarati}{00A0}
\pdfglyphtounicode{ocaron}{00A0}
\pdfglyphtounicode{ocircle}{00A0}
\pdfglyphtounicode{ocircumflex}{00A0}
\pdfglyphtounicode{ocircumflexacute}{00A0}
\pdfglyphtounicode{ocircumflexdotbelow}{00A0}
\pdfglyphtounicode{ocircumflexgrave}{00A0}
\pdfglyphtounicode{ocircumflexhookabove}{00A0}
\pdfglyphtounicode{ocircumflextilde}{00A0}
\pdfglyphtounicode{ocyrillic}{00A0}
\pdfglyphtounicode{odblacute}{00A0}
\pdfglyphtounicode{odblgrave}{00A0}
\pdfglyphtounicode{odeva}{00A0}
\pdfglyphtounicode{odieresis}{00A0}
\pdfglyphtounicode{odieresiscyrillic}{00A0}
\pdfglyphtounicode{odotbelow}{00A0}
\pdfglyphtounicode{oe}{00A0}
\pdfglyphtounicode{oekorean}{00A0}
\pdfglyphtounicode{ogonek}{00A0}
\pdfglyphtounicode{ogonekcmb}{00A0}
\pdfglyphtounicode{ograve}{00A0}
\pdfglyphtounicode{ogujarati}{00A0}
\pdfglyphtounicode{oharmenian}{00A0}
\pdfglyphtounicode{ohiragana}{00A0}
\pdfglyphtounicode{ohookabove}{00A0}
\pdfglyphtounicode{ohorn}{00A0}
\pdfglyphtounicode{ohornacute}{00A0}
\pdfglyphtounicode{ohorndotbelow}{00A0}
\pdfglyphtounicode{ohorngrave}{00A0}
\pdfglyphtounicode{ohornhookabove}{00A0}
\pdfglyphtounicode{ohorntilde}{00A0}
\pdfglyphtounicode{ohungarumlaut}{00A0}
\pdfglyphtounicode{oi}{00A0}
\pdfglyphtounicode{oinvertedbreve}{00A0}
\pdfglyphtounicode{okatakana}{00A0}
\pdfglyphtounicode{okatakanahalfwidth}{00A0}
\pdfglyphtounicode{okorean}{00A0}
\pdfglyphtounicode{olehebrew}{00A0}
\pdfglyphtounicode{omacron}{00A0}
\pdfglyphtounicode{omacronacute}{00A0}
\pdfglyphtounicode{omacrongrave}{00A0}
\pdfglyphtounicode{omdeva}{00A0}
\pdfglyphtounicode{omega}{00A0}
\pdfglyphtounicode{omega1}{00A0}
\pdfglyphtounicode{omegacyrillic}{00A0}
\pdfglyphtounicode{omegalatinclosed}{00A0}
\pdfglyphtounicode{omegaroundcyrillic}{00A0}
\pdfglyphtounicode{omegatitlocyrillic}{00A0}
\pdfglyphtounicode{omegatonos}{00A0}
\pdfglyphtounicode{omgujarati}{00A0}
\pdfglyphtounicode{omicron}{00A0}
\pdfglyphtounicode{omicrontonos}{00A0}
\pdfglyphtounicode{omonospace}{00A0}
\pdfglyphtounicode{one}{00A0}
\pdfglyphtounicode{onearabic}{00A0}
\pdfglyphtounicode{onebengali}{00A0}
\pdfglyphtounicode{onecircle}{00A0}
\pdfglyphtounicode{onecircleinversesansserif}{00A0}
\pdfglyphtounicode{onedeva}{00A0}
\pdfglyphtounicode{onedotenleader}{00A0}
\pdfglyphtounicode{oneeighth}{00A0}
\pdfglyphtounicode{onefitted}{00A0}
\pdfglyphtounicode{onegujarati}{00A0}
\pdfglyphtounicode{onegurmukhi}{00A0}
\pdfglyphtounicode{onehackarabic}{00A0}
\pdfglyphtounicode{onehalf}{00A0}
\pdfglyphtounicode{onehangzhou}{00A0}
\pdfglyphtounicode{oneideographicparen}{00A0}
\pdfglyphtounicode{oneinferior}{00A0}
\pdfglyphtounicode{onemonospace}{00A0}
\pdfglyphtounicode{onenumeratorbengali}{00A0}
\pdfglyphtounicode{oneoldstyle}{00A0}
\pdfglyphtounicode{oneparen}{00A0}
\pdfglyphtounicode{oneperiod}{00A0}
\pdfglyphtounicode{onepersian}{00A0}
\pdfglyphtounicode{onequarter}{00A0}
\pdfglyphtounicode{oneroman}{00A0}
\pdfglyphtounicode{onesuperior}{00A0}
\pdfglyphtounicode{onethai}{00A0}
\pdfglyphtounicode{onethird}{00A0}
\pdfglyphtounicode{oogonek}{00A0}
\pdfglyphtounicode{oogonekmacron}{00A0}
\pdfglyphtounicode{oogurmukhi}{00A0}
\pdfglyphtounicode{oomatragurmukhi}{00A0}
\pdfglyphtounicode{oopen}{00A0}
\pdfglyphtounicode{oparen}{00A0}
\pdfglyphtounicode{openbullet}{00A0}
\pdfglyphtounicode{option}{00A0}
\pdfglyphtounicode{ordfeminine}{00A0}
\pdfglyphtounicode{ordmasculine}{00A0}
\pdfglyphtounicode{orthogonal}{00A0}
\pdfglyphtounicode{orunderscore}{00A0}
\pdfglyphtounicode{oshortdeva}{00A0}
\pdfglyphtounicode{oshortvowelsigndeva}{00A0}
\pdfglyphtounicode{oslash}{00A0}
\pdfglyphtounicode{oslashacute}{00A0}
\pdfglyphtounicode{osmallhiragana}{00A0}
\pdfglyphtounicode{osmallkatakana}{00A0}
\pdfglyphtounicode{osmallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{ostrokeacute}{00A0}
\pdfglyphtounicode{osuperior}{00A0}
\pdfglyphtounicode{otcyrillic}{00A0}
\pdfglyphtounicode{otilde}{00A0}
\pdfglyphtounicode{otildeacute}{00A0}
\pdfglyphtounicode{otildedieresis}{00A0}
\pdfglyphtounicode{oubopomofo}{00A0}
\pdfglyphtounicode{overline}{00A0}
\pdfglyphtounicode{overlinecenterline}{00A0}
\pdfglyphtounicode{overlinecmb}{00A0}
\pdfglyphtounicode{overlinedashed}{00A0}
\pdfglyphtounicode{overlinedblwavy}{00A0}
\pdfglyphtounicode{overlinewavy}{00A0}
\pdfglyphtounicode{overscore}{00A0}
\pdfglyphtounicode{ovowelsignbengali}{00A0}
\pdfglyphtounicode{ovowelsigndeva}{00A0}
\pdfglyphtounicode{ovowelsigngujarati}{00A0}
\pdfglyphtounicode{owner}{00A0}
\pdfglyphtounicode{p}{00A0}
\pdfglyphtounicode{paampssquare}{00A0}
\pdfglyphtounicode{paasentosquare}{00A0}
\pdfglyphtounicode{pabengali}{00A0}
\pdfglyphtounicode{pacute}{00A0}
\pdfglyphtounicode{padeva}{00A0}
\pdfglyphtounicode{pagedown}{00A0}
\pdfglyphtounicode{pageup}{00A0}
\pdfglyphtounicode{pagujarati}{00A0}
\pdfglyphtounicode{pagurmukhi}{00A0}
\pdfglyphtounicode{pahiragana}{00A0}
\pdfglyphtounicode{paiyannoithai}{00A0}
\pdfglyphtounicode{pakatakana}{00A0}
\pdfglyphtounicode{palatalizationcyrilliccmb}{00A0}
\pdfglyphtounicode{palochkacyrillic}{00A0}
\pdfglyphtounicode{pansioskorean}{00A0}
\pdfglyphtounicode{paragraph}{00A0}
\pdfglyphtounicode{parallel}{00A0}
\pdfglyphtounicode{parenleft}{00A0}
\pdfglyphtounicode{parenleftaltonearabic}{00A0}
\pdfglyphtounicode{parenleftbt}{00A0}
\pdfglyphtounicode{parenleftex}{00A0}
\pdfglyphtounicode{parenleftinferior}{00A0}
\pdfglyphtounicode{parenleftmonospace}{00A0}
\pdfglyphtounicode{parenleftsmall}{00A0}
\pdfglyphtounicode{parenleftsuperior}{00A0}
\pdfglyphtounicode{parenlefttp}{00A0}
\pdfglyphtounicode{parenleftvertical}{00A0}
\pdfglyphtounicode{parenright}{00A0}
\pdfglyphtounicode{parenrightaltonearabic}{00A0}
\pdfglyphtounicode{parenrightbt}{00A0}
\pdfglyphtounicode{parenrightex}{00A0}
\pdfglyphtounicode{parenrightinferior}{00A0}
\pdfglyphtounicode{parenrightmonospace}{00A0}
\pdfglyphtounicode{parenrightsmall}{00A0}
\pdfglyphtounicode{parenrightsuperior}{00A0}
\pdfglyphtounicode{parenrighttp}{00A0}
\pdfglyphtounicode{parenrightvertical}{00A0}
\pdfglyphtounicode{partialdiff}{00A0}
\pdfglyphtounicode{paseqhebrew}{00A0}
\pdfglyphtounicode{pashtahebrew}{00A0}
\pdfglyphtounicode{pasquare}{00A0}
\pdfglyphtounicode{patah}{00A0}
\pdfglyphtounicode{patah11}{00A0}
\pdfglyphtounicode{patah1d}{00A0}
\pdfglyphtounicode{patah2a}{00A0}
\pdfglyphtounicode{patahhebrew}{00A0}
\pdfglyphtounicode{patahnarrowhebrew}{00A0}
\pdfglyphtounicode{patahquarterhebrew}{00A0}
\pdfglyphtounicode{patahwidehebrew}{00A0}
\pdfglyphtounicode{pazerhebrew}{00A0}
\pdfglyphtounicode{pbopomofo}{00A0}
\pdfglyphtounicode{pcircle}{00A0}
\pdfglyphtounicode{pdotaccent}{00A0}
\pdfglyphtounicode{pe}{00A0}
\pdfglyphtounicode{pecyrillic}{00A0}
\pdfglyphtounicode{pedagesh}{00A0}
\pdfglyphtounicode{pedageshhebrew}{00A0}
\pdfglyphtounicode{peezisquare}{00A0}
\pdfglyphtounicode{pefinaldageshhebrew}{00A0}
\pdfglyphtounicode{peharabic}{00A0}
\pdfglyphtounicode{peharmenian}{00A0}
\pdfglyphtounicode{pehebrew}{00A0}
\pdfglyphtounicode{pehfinalarabic}{00A0}
\pdfglyphtounicode{pehinitialarabic}{00A0}
\pdfglyphtounicode{pehiragana}{00A0}
\pdfglyphtounicode{pehmedialarabic}{00A0}
\pdfglyphtounicode{pekatakana}{00A0}
\pdfglyphtounicode{pemiddlehookcyrillic}{00A0}
\pdfglyphtounicode{perafehebrew}{00A0}
\pdfglyphtounicode{percent}{00A0}
\pdfglyphtounicode{percentarabic}{00A0}
\pdfglyphtounicode{percentmonospace}{00A0}
\pdfglyphtounicode{percentsmall}{00A0}
\pdfglyphtounicode{period}{00A0}
\pdfglyphtounicode{periodarmenian}{00A0}
\pdfglyphtounicode{periodcentered}{00A0}
\pdfglyphtounicode{periodhalfwidth}{00A0}
\pdfglyphtounicode{periodinferior}{00A0}
\pdfglyphtounicode{periodmonospace}{00A0}
\pdfglyphtounicode{periodsmall}{00A0}
\pdfglyphtounicode{periodsuperior}{00A0}
\pdfglyphtounicode{perispomenigreekcmb}{00A0}
\pdfglyphtounicode{perpcorrespond}{00A0}
\pdfglyphtounicode{perpendicular}{00A0}
\pdfglyphtounicode{pertenthousand}{00A0}
\pdfglyphtounicode{perthousand}{00A0}
\pdfglyphtounicode{peseta}{00A0}
\pdfglyphtounicode{pfsquare}{00A0}
\pdfglyphtounicode{phabengali}{00A0}
\pdfglyphtounicode{phadeva}{00A0}
\pdfglyphtounicode{phagujarati}{00A0}
\pdfglyphtounicode{phagurmukhi}{00A0}
\pdfglyphtounicode{phi}{00A0}
\pdfglyphtounicode{phi1}{00A0}
\pdfglyphtounicode{phieuphacirclekorean}{00A0}
\pdfglyphtounicode{phieuphaparenkorean}{00A0}
\pdfglyphtounicode{phieuphcirclekorean}{00A0}
\pdfglyphtounicode{phieuphkorean}{00A0}
\pdfglyphtounicode{phieuphparenkorean}{00A0}
\pdfglyphtounicode{philatin}{00A0}
\pdfglyphtounicode{phinthuthai}{00A0}
\pdfglyphtounicode{phisymbolgreek}{00A0}
\pdfglyphtounicode{phook}{00A0}
\pdfglyphtounicode{phophanthai}{00A0}
\pdfglyphtounicode{phophungthai}{00A0}
\pdfglyphtounicode{phosamphaothai}{00A0}
\pdfglyphtounicode{pi}{00A0}
\pdfglyphtounicode{pi1}{00A0}
\pdfglyphtounicode{pieupacirclekorean}{00A0}
\pdfglyphtounicode{pieupaparenkorean}{00A0}
\pdfglyphtounicode{pieupcieuckorean}{00A0}
\pdfglyphtounicode{pieupcirclekorean}{00A0}
\pdfglyphtounicode{pieupkiyeokkorean}{00A0}
\pdfglyphtounicode{pieupkorean}{00A0}
\pdfglyphtounicode{pieupparenkorean}{00A0}
\pdfglyphtounicode{pieupsioskiyeokkorean}{00A0}
\pdfglyphtounicode{pieupsioskorean}{00A0}
\pdfglyphtounicode{pieupsiostikeutkorean}{00A0}
\pdfglyphtounicode{pieupthieuthkorean}{00A0}
\pdfglyphtounicode{pieuptikeutkorean}{00A0}
\pdfglyphtounicode{pihiragana}{00A0}
\pdfglyphtounicode{pikatakana}{00A0}
\pdfglyphtounicode{pisymbolgreek}{00A0}
\pdfglyphtounicode{piwrarmenian}{00A0}
\pdfglyphtounicode{planckover2pi}{00A0}
\pdfglyphtounicode{planckover2pi1}{00A0}
\pdfglyphtounicode{plus}{00A0}
\pdfglyphtounicode{plusbelowcmb}{00A0}
\pdfglyphtounicode{pluscircle}{00A0}
\pdfglyphtounicode{plusminus}{00A0}
\pdfglyphtounicode{plusmod}{00A0}
\pdfglyphtounicode{plusmonospace}{00A0}
\pdfglyphtounicode{plussmall}{00A0}
\pdfglyphtounicode{plussuperior}{00A0}
\pdfglyphtounicode{pmonospace}{00A0}
\pdfglyphtounicode{pmsquare}{00A0}
\pdfglyphtounicode{pohiragana}{00A0}
\pdfglyphtounicode{pointingindexdownwhite}{00A0}
\pdfglyphtounicode{pointingindexleftwhite}{00A0}
\pdfglyphtounicode{pointingindexrightwhite}{00A0}
\pdfglyphtounicode{pointingindexupwhite}{00A0}
\pdfglyphtounicode{pokatakana}{00A0}
\pdfglyphtounicode{poplathai}{00A0}
\pdfglyphtounicode{postalmark}{00A0}
\pdfglyphtounicode{postalmarkface}{00A0}
\pdfglyphtounicode{pparen}{00A0}
\pdfglyphtounicode{precedenotdbleqv}{00A0}
\pdfglyphtounicode{precedenotslnteql}{00A0}
\pdfglyphtounicode{precedeornoteqvlnt}{00A0}
\pdfglyphtounicode{precedes}{00A0}
\pdfglyphtounicode{precedesequal}{00A0}
\pdfglyphtounicode{precedesorcurly}{00A0}
\pdfglyphtounicode{precedesorequal}{00A0}
\pdfglyphtounicode{prescription}{00A0}
\pdfglyphtounicode{prime}{00A0}
\pdfglyphtounicode{primemod}{00A0}
\pdfglyphtounicode{primereverse}{00A0}
\pdfglyphtounicode{primereversed}{00A0}
\pdfglyphtounicode{product}{00A0}
\pdfglyphtounicode{projective}{00A0}
\pdfglyphtounicode{prolongedkana}{00A0}
\pdfglyphtounicode{propellor}{00A0}
\pdfglyphtounicode{propersubset}{00A0}
\pdfglyphtounicode{propersuperset}{00A0}
\pdfglyphtounicode{proportion}{00A0}
\pdfglyphtounicode{proportional}{00A0}
\pdfglyphtounicode{psi}{00A0}
\pdfglyphtounicode{psicyrillic}{00A0}
\pdfglyphtounicode{psilipneumatacyrilliccmb}{00A0}
\pdfglyphtounicode{pssquare}{00A0}
\pdfglyphtounicode{puhiragana}{00A0}
\pdfglyphtounicode{pukatakana}{00A0}
\pdfglyphtounicode{punctdash}{00A0}
\pdfglyphtounicode{pvsquare}{00A0}
\pdfglyphtounicode{pwsquare}{00A0}
\pdfglyphtounicode{q}{00A0}
\pdfglyphtounicode{qadeva}{00A0}
\pdfglyphtounicode{qadmahebrew}{00A0}
\pdfglyphtounicode{qafarabic}{00A0}
\pdfglyphtounicode{qaffinalarabic}{00A0}
\pdfglyphtounicode{qafinitialarabic}{00A0}
\pdfglyphtounicode{qafmedialarabic}{00A0}
\pdfglyphtounicode{qamats}{00A0}
\pdfglyphtounicode{qamats10}{00A0}
\pdfglyphtounicode{qamats1a}{00A0}
\pdfglyphtounicode{qamats1c}{00A0}
\pdfglyphtounicode{qamats27}{00A0}
\pdfglyphtounicode{qamats29}{00A0}
\pdfglyphtounicode{qamats33}{00A0}
\pdfglyphtounicode{qamatsde}{00A0}
\pdfglyphtounicode{qamatshebrew}{00A0}
\pdfglyphtounicode{qamatsnarrowhebrew}{00A0}
\pdfglyphtounicode{qamatsqatanhebrew}{00A0}
\pdfglyphtounicode{qamatsqatannarrowhebrew}{00A0}
\pdfglyphtounicode{qamatsqatanquarterhebrew}{00A0}
\pdfglyphtounicode{qamatsqatanwidehebrew}{00A0}
\pdfglyphtounicode{qamatsquarterhebrew}{00A0}
\pdfglyphtounicode{qamatswidehebrew}{00A0}
\pdfglyphtounicode{qarneyparahebrew}{00A0}
\pdfglyphtounicode{qbopomofo}{00A0}
\pdfglyphtounicode{qcircle}{00A0}
\pdfglyphtounicode{qhook}{00A0}
\pdfglyphtounicode{qmonospace}{00A0}
\pdfglyphtounicode{qof}{00A0}
\pdfglyphtounicode{qofdagesh}{00A0}
\pdfglyphtounicode{qofdageshhebrew}{00A0}
\pdfglyphtounicode{qofhatafpatah}{00A0}
\pdfglyphtounicode{qofhatafpatahhebrew}{00A0}
\pdfglyphtounicode{qofhatafsegol}{00A0}
\pdfglyphtounicode{qofhatafsegolhebrew}{00A0}
\pdfglyphtounicode{qofhebrew}{00A0}
\pdfglyphtounicode{qofhiriq}{00A0}
\pdfglyphtounicode{qofhiriqhebrew}{00A0}
\pdfglyphtounicode{qofholam}{00A0}
\pdfglyphtounicode{qofholamhebrew}{00A0}
\pdfglyphtounicode{qofpatah}{00A0}
\pdfglyphtounicode{qofpatahhebrew}{00A0}
\pdfglyphtounicode{qofqamats}{00A0}
\pdfglyphtounicode{qofqamatshebrew}{00A0}
\pdfglyphtounicode{qofqubuts}{00A0}
\pdfglyphtounicode{qofqubutshebrew}{00A0}
\pdfglyphtounicode{qofsegol}{00A0}
\pdfglyphtounicode{qofsegolhebrew}{00A0}
\pdfglyphtounicode{qofsheva}{00A0}
\pdfglyphtounicode{qofshevahebrew}{00A0}
\pdfglyphtounicode{qoftsere}{00A0}
\pdfglyphtounicode{qoftserehebrew}{00A0}
\pdfglyphtounicode{qparen}{00A0}
\pdfglyphtounicode{quarternote}{00A0}
\pdfglyphtounicode{qubuts}{00A0}
\pdfglyphtounicode{qubuts18}{00A0}
\pdfglyphtounicode{qubuts25}{00A0}
\pdfglyphtounicode{qubuts31}{00A0}
\pdfglyphtounicode{qubutshebrew}{00A0}
\pdfglyphtounicode{qubutsnarrowhebrew}{00A0}
\pdfglyphtounicode{qubutsquarterhebrew}{00A0}
\pdfglyphtounicode{qubutswidehebrew}{00A0}
\pdfglyphtounicode{question}{00A0}
\pdfglyphtounicode{questionarabic}{00A0}
\pdfglyphtounicode{questionarmenian}{00A0}
\pdfglyphtounicode{questiondown}{00A0}
\pdfglyphtounicode{questiondownsmall}{00A0}
\pdfglyphtounicode{questiongreek}{00A0}
\pdfglyphtounicode{questionmonospace}{00A0}
\pdfglyphtounicode{questionsmall}{00A0}
\pdfglyphtounicode{quotedbl}{00A0}
\pdfglyphtounicode{quotedblbase}{00A0}
\pdfglyphtounicode{quotedblleft}{00A0}
\pdfglyphtounicode{quotedblmonospace}{00A0}
\pdfglyphtounicode{quotedblprime}{00A0}
\pdfglyphtounicode{quotedblprimereversed}{00A0}
\pdfglyphtounicode{quotedblright}{00A0}
\pdfglyphtounicode{quoteleft}{00A0}
\pdfglyphtounicode{quoteleftreversed}{00A0}
\pdfglyphtounicode{quotereversed}{00A0}
\pdfglyphtounicode{quoteright}{00A0}
\pdfglyphtounicode{quoterightn}{00A0}
\pdfglyphtounicode{quotesinglbase}{00A0}
\pdfglyphtounicode{quotesingle}{00A0}
\pdfglyphtounicode{quotesinglemonospace}{00A0}
\pdfglyphtounicode{r}{00A0}
\pdfglyphtounicode{raarmenian}{00A0}
\pdfglyphtounicode{rabengali}{00A0}
\pdfglyphtounicode{racute}{00A0}
\pdfglyphtounicode{radeva}{00A0}
\pdfglyphtounicode{radical}{00A0}
\pdfglyphtounicode{radicalex}{00A0}
\pdfglyphtounicode{radoverssquare}{00A0}
\pdfglyphtounicode{radoverssquaredsquare}{00A0}
\pdfglyphtounicode{radsquare}{00A0}
\pdfglyphtounicode{rafe}{00A0}
\pdfglyphtounicode{rafehebrew}{00A0}
\pdfglyphtounicode{ragujarati}{00A0}
\pdfglyphtounicode{ragurmukhi}{00A0}
\pdfglyphtounicode{rahiragana}{00A0}
\pdfglyphtounicode{rakatakana}{00A0}
\pdfglyphtounicode{rakatakanahalfwidth}{00A0}
\pdfglyphtounicode{ralowerdiagonalbengali}{00A0}
\pdfglyphtounicode{ramiddlediagonalbengali}{00A0}
\pdfglyphtounicode{ramshorn}{00A0}
\pdfglyphtounicode{rangedash}{00A0}
\pdfglyphtounicode{ratio}{00A0}
\pdfglyphtounicode{rbopomofo}{00A0}
\pdfglyphtounicode{rcaron}{00A0}
\pdfglyphtounicode{rcedilla}{00A0}
\pdfglyphtounicode{rcircle}{00A0}
\pdfglyphtounicode{rcommaaccent}{00A0}
\pdfglyphtounicode{rdblgrave}{00A0}
\pdfglyphtounicode{rdotaccent}{00A0}
\pdfglyphtounicode{rdotbelow}{00A0}
\pdfglyphtounicode{rdotbelowmacron}{00A0}
\pdfglyphtounicode{referencemark}{00A0}
\pdfglyphtounicode{reflexsubset}{00A0}
\pdfglyphtounicode{reflexsuperset}{00A0}
\pdfglyphtounicode{registered}{00A0}
\pdfglyphtounicode{registersans}{00A0}
\pdfglyphtounicode{registerserif}{00A0}
\pdfglyphtounicode{reharabic}{00A0}
\pdfglyphtounicode{reharmenian}{00A0}
\pdfglyphtounicode{rehfinalarabic}{00A0}
\pdfglyphtounicode{rehiragana}{00A0}
\pdfglyphtounicode{rehyehaleflamarabic}{00A0}
\pdfglyphtounicode{rekatakana}{00A0}
\pdfglyphtounicode{rekatakanahalfwidth}{00A0}
\pdfglyphtounicode{resh}{00A0}
\pdfglyphtounicode{reshdageshhebrew}{00A0}
\pdfglyphtounicode{reshhatafpatah}{00A0}
\pdfglyphtounicode{reshhatafpatahhebrew}{00A0}
\pdfglyphtounicode{reshhatafsegol}{00A0}
\pdfglyphtounicode{reshhatafsegolhebrew}{00A0}
\pdfglyphtounicode{reshhebrew}{00A0}
\pdfglyphtounicode{reshhiriq}{00A0}
\pdfglyphtounicode{reshhiriqhebrew}{00A0}
\pdfglyphtounicode{reshholam}{00A0}
\pdfglyphtounicode{reshholamhebrew}{00A0}
\pdfglyphtounicode{reshpatah}{00A0}
\pdfglyphtounicode{reshpatahhebrew}{00A0}
\pdfglyphtounicode{reshqamats}{00A0}
\pdfglyphtounicode{reshqamatshebrew}{00A0}
\pdfglyphtounicode{reshqubuts}{00A0}
\pdfglyphtounicode{reshqubutshebrew}{00A0}
\pdfglyphtounicode{reshsegol}{00A0}
\pdfglyphtounicode{reshsegolhebrew}{00A0}
\pdfglyphtounicode{reshsheva}{00A0}
\pdfglyphtounicode{reshshevahebrew}{00A0}
\pdfglyphtounicode{reshtsere}{00A0}
\pdfglyphtounicode{reshtserehebrew}{00A0}
\pdfglyphtounicode{revasymptequal}{00A0}
\pdfglyphtounicode{reversedtilde}{00A0}
\pdfglyphtounicode{reviahebrew}{00A0}
\pdfglyphtounicode{reviamugrashhebrew}{00A0}
\pdfglyphtounicode{revlogicalnot}{00A0}
\pdfglyphtounicode{revsimilar}{00A0}
\pdfglyphtounicode{rfishhook}{00A0}
\pdfglyphtounicode{rfishhookreversed}{00A0}
\pdfglyphtounicode{rhabengali}{00A0}
\pdfglyphtounicode{rhadeva}{00A0}
\pdfglyphtounicode{rho}{00A0}
\pdfglyphtounicode{rho1}{00A0}
\pdfglyphtounicode{rhook}{00A0}
\pdfglyphtounicode{rhookturned}{00A0}
\pdfglyphtounicode{rhookturnedsuperior}{00A0}
\pdfglyphtounicode{rhosymbolgreek}{00A0}
\pdfglyphtounicode{rhotichookmod}{00A0}
\pdfglyphtounicode{rieulacirclekorean}{00A0}
\pdfglyphtounicode{rieulaparenkorean}{00A0}
\pdfglyphtounicode{rieulcirclekorean}{00A0}
\pdfglyphtounicode{rieulhieuhkorean}{00A0}
\pdfglyphtounicode{rieulkiyeokkorean}{00A0}
\pdfglyphtounicode{rieulkiyeoksioskorean}{00A0}
\pdfglyphtounicode{rieulkorean}{00A0}
\pdfglyphtounicode{rieulmieumkorean}{00A0}
\pdfglyphtounicode{rieulpansioskorean}{00A0}
\pdfglyphtounicode{rieulparenkorean}{00A0}
\pdfglyphtounicode{rieulphieuphkorean}{00A0}
\pdfglyphtounicode{rieulpieupkorean}{00A0}
\pdfglyphtounicode{rieulpieupsioskorean}{00A0}
\pdfglyphtounicode{rieulsioskorean}{00A0}
\pdfglyphtounicode{rieulthieuthkorean}{00A0}
\pdfglyphtounicode{rieultikeutkorean}{00A0}
\pdfglyphtounicode{rieulyeorinhieuhkorean}{00A0}
\pdfglyphtounicode{rightangle}{00A0}
\pdfglyphtounicode{rightanglene}{00A0}
\pdfglyphtounicode{rightanglenw}{00A0}
\pdfglyphtounicode{rightanglese}{00A0}
\pdfglyphtounicode{rightanglesw}{00A0}
\pdfglyphtounicode{righttackbelowcmb}{00A0}
\pdfglyphtounicode{righttriangle}{00A0}
\pdfglyphtounicode{rihiragana}{00A0}
\pdfglyphtounicode{rikatakana}{00A0}
\pdfglyphtounicode{rikatakanahalfwidth}{00A0}
\pdfglyphtounicode{ring}{00A0}
\pdfglyphtounicode{ringbelowcmb}{00A0}
\pdfglyphtounicode{ringcmb}{00A0}
\pdfglyphtounicode{ringhalfleft}{00A0}
\pdfglyphtounicode{ringhalfleftarmenian}{00A0}
\pdfglyphtounicode{ringhalfleftbelowcmb}{00A0}
\pdfglyphtounicode{ringhalfleftcentered}{00A0}
\pdfglyphtounicode{ringhalfright}{00A0}
\pdfglyphtounicode{ringhalfrightbelowcmb}{00A0}
\pdfglyphtounicode{ringhalfrightcentered}{00A0}
\pdfglyphtounicode{ringinequal}{00A0}
\pdfglyphtounicode{rinvertedbreve}{00A0}
\pdfglyphtounicode{rittorusquare}{00A0}
\pdfglyphtounicode{rlinebelow}{00A0}
\pdfglyphtounicode{rlongleg}{00A0}
\pdfglyphtounicode{rlonglegturned}{00A0}
\pdfglyphtounicode{rmonospace}{00A0}
\pdfglyphtounicode{rohiragana}{00A0}
\pdfglyphtounicode{rokatakana}{00A0}
\pdfglyphtounicode{rokatakanahalfwidth}{00A0}
\pdfglyphtounicode{roruathai}{00A0}
\pdfglyphtounicode{rparen}{00A0}
\pdfglyphtounicode{rrabengali}{00A0}
\pdfglyphtounicode{rradeva}{00A0}
\pdfglyphtounicode{rragurmukhi}{00A0}
\pdfglyphtounicode{rreharabic}{00A0}
\pdfglyphtounicode{rrehfinalarabic}{00A0}
\pdfglyphtounicode{rrvocalicbengali}{00A0}
\pdfglyphtounicode{rrvocalicdeva}{00A0}
\pdfglyphtounicode{rrvocalicgujarati}{00A0}
\pdfglyphtounicode{rrvocalicvowelsignbengali}{00A0}
\pdfglyphtounicode{rrvocalicvowelsigndeva}{00A0}
\pdfglyphtounicode{rrvocalicvowelsigngujarati}{00A0}
\pdfglyphtounicode{rsuperior}{00A0}
\pdfglyphtounicode{rtblock}{00A0}
\pdfglyphtounicode{rturned}{00A0}
\pdfglyphtounicode{rturnedsuperior}{00A0}
\pdfglyphtounicode{ruhiragana}{00A0}
\pdfglyphtounicode{rukatakana}{00A0}
\pdfglyphtounicode{rukatakanahalfwidth}{00A0}
\pdfglyphtounicode{rupeemarkbengali}{00A0}
\pdfglyphtounicode{rupeesignbengali}{00A0}
\pdfglyphtounicode{rupiah}{00A0}
\pdfglyphtounicode{ruthai}{00A0}
\pdfglyphtounicode{rvocalicbengali}{00A0}
\pdfglyphtounicode{rvocalicdeva}{00A0}
\pdfglyphtounicode{rvocalicgujarati}{00A0}
\pdfglyphtounicode{rvocalicvowelsignbengali}{00A0}
\pdfglyphtounicode{rvocalicvowelsigndeva}{00A0}
\pdfglyphtounicode{rvocalicvowelsigngujarati}{00A0}
\pdfglyphtounicode{s}{00A0}
\pdfglyphtounicode{sabengali}{00A0}
\pdfglyphtounicode{sacute}{00A0}
\pdfglyphtounicode{sacutedotaccent}{00A0}
\pdfglyphtounicode{sadarabic}{00A0}
\pdfglyphtounicode{sadeva}{00A0}
\pdfglyphtounicode{sadfinalarabic}{00A0}
\pdfglyphtounicode{sadinitialarabic}{00A0}
\pdfglyphtounicode{sadmedialarabic}{00A0}
\pdfglyphtounicode{sagujarati}{00A0}
\pdfglyphtounicode{sagurmukhi}{00A0}
\pdfglyphtounicode{sahiragana}{00A0}
\pdfglyphtounicode{sakatakana}{00A0}
\pdfglyphtounicode{sakatakanahalfwidth}{00A0}
\pdfglyphtounicode{sallallahoualayhewasallamarabic}{00A0}
\pdfglyphtounicode{samekh}{00A0}
\pdfglyphtounicode{samekhdagesh}{00A0}
\pdfglyphtounicode{samekhdageshhebrew}{00A0}
\pdfglyphtounicode{samekhhebrew}{00A0}
\pdfglyphtounicode{saraaathai}{00A0}
\pdfglyphtounicode{saraaethai}{00A0}
\pdfglyphtounicode{saraaimaimalaithai}{00A0}
\pdfglyphtounicode{saraaimaimuanthai}{00A0}
\pdfglyphtounicode{saraamthai}{00A0}
\pdfglyphtounicode{saraathai}{00A0}
\pdfglyphtounicode{saraethai}{00A0}
\pdfglyphtounicode{saraiileftthai}{00A0}
\pdfglyphtounicode{saraiithai}{00A0}
\pdfglyphtounicode{saraileftthai}{00A0}
\pdfglyphtounicode{saraithai}{00A0}
\pdfglyphtounicode{saraothai}{00A0}
\pdfglyphtounicode{saraueeleftthai}{00A0}
\pdfglyphtounicode{saraueethai}{00A0}
\pdfglyphtounicode{saraueleftthai}{00A0}
\pdfglyphtounicode{sarauethai}{00A0}
\pdfglyphtounicode{sarauthai}{00A0}
\pdfglyphtounicode{sarauuthai}{00A0}
\pdfglyphtounicode{satisfies}{00A0}
\pdfglyphtounicode{sbopomofo}{00A0}
\pdfglyphtounicode{scaron}{00A0}
\pdfglyphtounicode{scarondotaccent}{00A0}
\pdfglyphtounicode{scedilla}{00A0}
\pdfglyphtounicode{schwa}{00A0}
\pdfglyphtounicode{schwacyrillic}{00A0}
\pdfglyphtounicode{schwadieresiscyrillic}{00A0}
\pdfglyphtounicode{schwahook}{00A0}
\pdfglyphtounicode{scircle}{00A0}
\pdfglyphtounicode{scircumflex}{00A0}
\pdfglyphtounicode{scommaaccent}{00A0}
\pdfglyphtounicode{sdotaccent}{00A0}
\pdfglyphtounicode{sdotbelow}{00A0}
\pdfglyphtounicode{sdotbelowdotaccent}{00A0}
\pdfglyphtounicode{seagullbelowcmb}{00A0}
\pdfglyphtounicode{second}{00A0}
\pdfglyphtounicode{secondtonechinese}{00A0}
\pdfglyphtounicode{section}{00A0}
\pdfglyphtounicode{seenarabic}{00A0}
\pdfglyphtounicode{seenfinalarabic}{00A0}
\pdfglyphtounicode{seeninitialarabic}{00A0}
\pdfglyphtounicode{seenmedialarabic}{00A0}
\pdfglyphtounicode{segol}{00A0}
\pdfglyphtounicode{segol13}{00A0}
\pdfglyphtounicode{segol1f}{00A0}
\pdfglyphtounicode{segol2c}{00A0}
\pdfglyphtounicode{segolhebrew}{00A0}
\pdfglyphtounicode{segolnarrowhebrew}{00A0}
\pdfglyphtounicode{segolquarterhebrew}{00A0}
\pdfglyphtounicode{segoltahebrew}{00A0}
\pdfglyphtounicode{segolwidehebrew}{00A0}
\pdfglyphtounicode{seharmenian}{00A0}
\pdfglyphtounicode{sehiragana}{00A0}
\pdfglyphtounicode{sekatakana}{00A0}
\pdfglyphtounicode{sekatakanahalfwidth}{00A0}
\pdfglyphtounicode{semicolon}{00A0}
\pdfglyphtounicode{semicolonarabic}{00A0}
\pdfglyphtounicode{semicolonmonospace}{00A0}
\pdfglyphtounicode{semicolonsmall}{00A0}
\pdfglyphtounicode{semivoicedmarkkana}{00A0}
\pdfglyphtounicode{semivoicedmarkkanahalfwidth}{00A0}
\pdfglyphtounicode{sentisquare}{00A0}
\pdfglyphtounicode{sentosquare}{00A0}
\pdfglyphtounicode{seven}{00A0}
\pdfglyphtounicode{sevenarabic}{00A0}
\pdfglyphtounicode{sevenbengali}{00A0}
\pdfglyphtounicode{sevencircle}{00A0}
\pdfglyphtounicode{sevencircleinversesansserif}{00A0}
\pdfglyphtounicode{sevendeva}{00A0}
\pdfglyphtounicode{seveneighths}{00A0}
\pdfglyphtounicode{sevengujarati}{00A0}
\pdfglyphtounicode{sevengurmukhi}{00A0}
\pdfglyphtounicode{sevenhackarabic}{00A0}
\pdfglyphtounicode{sevenhangzhou}{00A0}
\pdfglyphtounicode{sevenideographicparen}{00A0}
\pdfglyphtounicode{seveninferior}{00A0}
\pdfglyphtounicode{sevenmonospace}{00A0}
\pdfglyphtounicode{sevenoldstyle}{00A0}
\pdfglyphtounicode{sevenparen}{00A0}
\pdfglyphtounicode{sevenperiod}{00A0}
\pdfglyphtounicode{sevenpersian}{00A0}
\pdfglyphtounicode{sevenroman}{00A0}
\pdfglyphtounicode{sevensuperior}{00A0}
\pdfglyphtounicode{seventeencircle}{00A0}
\pdfglyphtounicode{seventeenparen}{00A0}
\pdfglyphtounicode{seventeenperiod}{00A0}
\pdfglyphtounicode{seventhai}{00A0}
\pdfglyphtounicode{sfthyphen}{00A0}
\pdfglyphtounicode{shaarmenian}{00A0}
\pdfglyphtounicode{shabengali}{00A0}
\pdfglyphtounicode{shacyrillic}{00A0}
\pdfglyphtounicode{shaddaarabic}{00A0}
\pdfglyphtounicode{shaddadammaarabic}{00A0}
\pdfglyphtounicode{shaddadammatanarabic}{00A0}
\pdfglyphtounicode{shaddafathaarabic}{00A0}
\pdfglyphtounicode{shaddafathatanarabic}{00A0}
\pdfglyphtounicode{shaddakasraarabic}{00A0}
\pdfglyphtounicode{shaddakasratanarabic}{00A0}
\pdfglyphtounicode{shade}{00A0}
\pdfglyphtounicode{shadedark}{00A0}
\pdfglyphtounicode{shadelight}{00A0}
\pdfglyphtounicode{shademedium}{00A0}
\pdfglyphtounicode{shadeva}{00A0}
\pdfglyphtounicode{shagujarati}{00A0}
\pdfglyphtounicode{shagurmukhi}{00A0}
\pdfglyphtounicode{shalshelethebrew}{00A0}
\pdfglyphtounicode{sharp}{00A0}
\pdfglyphtounicode{shbopomofo}{00A0}
\pdfglyphtounicode{shchacyrillic}{00A0}
\pdfglyphtounicode{sheenarabic}{00A0}
\pdfglyphtounicode{sheenfinalarabic}{00A0}
\pdfglyphtounicode{sheeninitialarabic}{00A0}
\pdfglyphtounicode{sheenmedialarabic}{00A0}
\pdfglyphtounicode{sheicoptic}{00A0}
\pdfglyphtounicode{sheqel}{00A0}
\pdfglyphtounicode{sheqelhebrew}{00A0}
\pdfglyphtounicode{sheva}{00A0}
\pdfglyphtounicode{sheva115}{00A0}
\pdfglyphtounicode{sheva15}{00A0}
\pdfglyphtounicode{sheva22}{00A0}
\pdfglyphtounicode{sheva2e}{00A0}
\pdfglyphtounicode{shevahebrew}{00A0}
\pdfglyphtounicode{shevanarrowhebrew}{00A0}
\pdfglyphtounicode{shevaquarterhebrew}{00A0}
\pdfglyphtounicode{shevawidehebrew}{00A0}
\pdfglyphtounicode{shhacyrillic}{00A0}
\pdfglyphtounicode{shiftleft}{00A0}
\pdfglyphtounicode{shiftright}{00A0}
\pdfglyphtounicode{shimacoptic}{00A0}
\pdfglyphtounicode{shin}{00A0}
\pdfglyphtounicode{shindagesh}{00A0}
\pdfglyphtounicode{shindageshhebrew}{00A0}
\pdfglyphtounicode{shindageshshindot}{00A0}
\pdfglyphtounicode{shindageshshindothebrew}{00A0}
\pdfglyphtounicode{shindageshsindot}{00A0}
\pdfglyphtounicode{shindageshsindothebrew}{00A0}
\pdfglyphtounicode{shindothebrew}{00A0}
\pdfglyphtounicode{shinhebrew}{00A0}
\pdfglyphtounicode{shinshindot}{00A0}
\pdfglyphtounicode{shinshindothebrew}{00A0}
\pdfglyphtounicode{shinsindot}{00A0}
\pdfglyphtounicode{shinsindothebrew}{00A0}
\pdfglyphtounicode{shook}{00A0}
\pdfglyphtounicode{sigma}{00A0}
\pdfglyphtounicode{sigma1}{00A0}
\pdfglyphtounicode{sigmafinal}{00A0}
\pdfglyphtounicode{sigmalunatesymbolgreek}{00A0}
\pdfglyphtounicode{sihiragana}{00A0}
\pdfglyphtounicode{sikatakana}{00A0}
\pdfglyphtounicode{sikatakanahalfwidth}{00A0}
\pdfglyphtounicode{siluqhebrew}{00A0}
\pdfglyphtounicode{siluqlefthebrew}{00A0}
\pdfglyphtounicode{similar}{00A0}
\pdfglyphtounicode{similarequal}{00A0}
\pdfglyphtounicode{sindothebrew}{00A0}
\pdfglyphtounicode{siosacirclekorean}{00A0}
\pdfglyphtounicode{siosaparenkorean}{00A0}
\pdfglyphtounicode{sioscieuckorean}{00A0}
\pdfglyphtounicode{sioscirclekorean}{00A0}
\pdfglyphtounicode{sioskiyeokkorean}{00A0}
\pdfglyphtounicode{sioskorean}{00A0}
\pdfglyphtounicode{siosnieunkorean}{00A0}
\pdfglyphtounicode{siosparenkorean}{00A0}
\pdfglyphtounicode{siospieupkorean}{00A0}
\pdfglyphtounicode{siostikeutkorean}{00A0}
\pdfglyphtounicode{six}{00A0}
\pdfglyphtounicode{sixarabic}{00A0}
\pdfglyphtounicode{sixbengali}{00A0}
\pdfglyphtounicode{sixcircle}{00A0}
\pdfglyphtounicode{sixcircleinversesansserif}{00A0}
\pdfglyphtounicode{sixdeva}{00A0}
\pdfglyphtounicode{sixgujarati}{00A0}
\pdfglyphtounicode{sixgurmukhi}{00A0}
\pdfglyphtounicode{sixhackarabic}{00A0}
\pdfglyphtounicode{sixhangzhou}{00A0}
\pdfglyphtounicode{sixideographicparen}{00A0}
\pdfglyphtounicode{sixinferior}{00A0}
\pdfglyphtounicode{sixmonospace}{00A0}
\pdfglyphtounicode{sixoldstyle}{00A0}
\pdfglyphtounicode{sixparen}{00A0}
\pdfglyphtounicode{sixperiod}{00A0}
\pdfglyphtounicode{sixpersian}{00A0}
\pdfglyphtounicode{sixroman}{00A0}
\pdfglyphtounicode{sixsuperior}{00A0}
\pdfglyphtounicode{sixteencircle}{00A0}
\pdfglyphtounicode{sixteencurrencydenominatorbengali}{00A0}
\pdfglyphtounicode{sixteenparen}{00A0}
\pdfglyphtounicode{sixteenperiod}{00A0}
\pdfglyphtounicode{sixthai}{00A0}
\pdfglyphtounicode{slash}{00A0}
\pdfglyphtounicode{slashmonospace}{00A0}
\pdfglyphtounicode{slong}{00A0}
\pdfglyphtounicode{slongdotaccent}{00A0}
\pdfglyphtounicode{slurabove}{00A0}
\pdfglyphtounicode{slurbelow}{00A0}
\pdfglyphtounicode{smile}{00A0}
\pdfglyphtounicode{smileface}{00A0}
\pdfglyphtounicode{smonospace}{00A0}
\pdfglyphtounicode{sofpasuqhebrew}{00A0}
\pdfglyphtounicode{softhyphen}{00A0}
\pdfglyphtounicode{softsigncyrillic}{00A0}
\pdfglyphtounicode{sohiragana}{00A0}
\pdfglyphtounicode{sokatakana}{00A0}
\pdfglyphtounicode{sokatakanahalfwidth}{00A0}
\pdfglyphtounicode{soliduslongoverlaycmb}{00A0}
\pdfglyphtounicode{solidusshortoverlaycmb}{00A0}
\pdfglyphtounicode{sorusithai}{00A0}
\pdfglyphtounicode{sosalathai}{00A0}
\pdfglyphtounicode{sosothai}{00A0}
\pdfglyphtounicode{sosuathai}{00A0}
\pdfglyphtounicode{space}{00A0}
\pdfglyphtounicode{spacehackarabic}{00A0}
\pdfglyphtounicode{spade}{00A0}
\pdfglyphtounicode{spadesuitblack}{00A0}
\pdfglyphtounicode{spadesuitwhite}{00A0}
\pdfglyphtounicode{sparen}{00A0}
\pdfglyphtounicode{sphericalangle}{00A0}
\pdfglyphtounicode{square}{00A0}
\pdfglyphtounicode{squarebelowcmb}{00A0}
\pdfglyphtounicode{squarecc}{00A0}
\pdfglyphtounicode{squarecm}{00A0}
\pdfglyphtounicode{squarediagonalcrosshatchfill}{00A0}
\pdfglyphtounicode{squaredot}{00A0}
\pdfglyphtounicode{squarehorizontalfill}{00A0}
\pdfglyphtounicode{squareimage}{00A0}
\pdfglyphtounicode{squarekg}{00A0}
\pdfglyphtounicode{squarekm}{00A0}
\pdfglyphtounicode{squarekmcapital}{00A0}
\pdfglyphtounicode{squareln}{00A0}
\pdfglyphtounicode{squarelog}{00A0}
\pdfglyphtounicode{squaremg}{00A0}
\pdfglyphtounicode{squaremil}{00A0}
\pdfglyphtounicode{squareminus}{00A0}
\pdfglyphtounicode{squaremm}{00A0}
\pdfglyphtounicode{squaremsquared}{00A0}
\pdfglyphtounicode{squaremultiply}{00A0}
\pdfglyphtounicode{squareoriginal}{00A0}
\pdfglyphtounicode{squareorthogonalcrosshatchfill}{00A0}
\pdfglyphtounicode{squareplus}{00A0}
\pdfglyphtounicode{squaresolid}{00A0}
\pdfglyphtounicode{squareupperlefttolowerrightfill}{00A0}
\pdfglyphtounicode{squareupperrighttolowerleftfill}{00A0}
\pdfglyphtounicode{squareverticalfill}{00A0}
\pdfglyphtounicode{squarewhitewithsmallblack}{00A0}
\pdfglyphtounicode{squiggleleftright}{00A0}
\pdfglyphtounicode{squiggleright}{00A0}
\pdfglyphtounicode{srsquare}{00A0}
\pdfglyphtounicode{ssabengali}{00A0}
\pdfglyphtounicode{ssadeva}{00A0}
\pdfglyphtounicode{ssagujarati}{00A0}
\pdfglyphtounicode{ssangcieuckorean}{00A0}
\pdfglyphtounicode{ssanghieuhkorean}{00A0}
\pdfglyphtounicode{ssangieungkorean}{00A0}
\pdfglyphtounicode{ssangkiyeokkorean}{00A0}
\pdfglyphtounicode{ssangnieunkorean}{00A0}
\pdfglyphtounicode{ssangpieupkorean}{00A0}
\pdfglyphtounicode{ssangsioskorean}{00A0}
\pdfglyphtounicode{ssangtikeutkorean}{00A0}
\pdfglyphtounicode{ssuperior}{00A0}
\pdfglyphtounicode{st}{00A0}
\pdfglyphtounicode{star}{00A0}
\pdfglyphtounicode{sterling}{00A0}
\pdfglyphtounicode{sterlingmonospace}{00A0}
\pdfglyphtounicode{strokelongoverlaycmb}{00A0}
\pdfglyphtounicode{strokeshortoverlaycmb}{00A0}
\pdfglyphtounicode{subset}{00A0}
\pdfglyphtounicode{subsetdbl}{00A0}
\pdfglyphtounicode{subsetdblequal}{00A0}
\pdfglyphtounicode{subsetnoteql}{00A0}
\pdfglyphtounicode{subsetnotequal}{00A0}
\pdfglyphtounicode{subsetorequal}{00A0}
\pdfglyphtounicode{subsetornotdbleql}{00A0}
\pdfglyphtounicode{subsetsqequal}{00A0}
\pdfglyphtounicode{succeeds}{00A0}
\pdfglyphtounicode{suchthat}{00A0}
\pdfglyphtounicode{suhiragana}{00A0}
\pdfglyphtounicode{sukatakana}{00A0}
\pdfglyphtounicode{sukatakanahalfwidth}{00A0}
\pdfglyphtounicode{sukunarabic}{00A0}
\pdfglyphtounicode{summation}{00A0}
\pdfglyphtounicode{sun}{00A0}
\pdfglyphtounicode{superset}{00A0}
\pdfglyphtounicode{supersetdbl}{00A0}
\pdfglyphtounicode{supersetdblequal}{00A0}
\pdfglyphtounicode{supersetnoteql}{00A0}
\pdfglyphtounicode{supersetnotequal}{00A0}
\pdfglyphtounicode{supersetorequal}{00A0}
\pdfglyphtounicode{supersetornotdbleql}{00A0}
\pdfglyphtounicode{supersetsqequal}{00A0}
\pdfglyphtounicode{svsquare}{00A0}
\pdfglyphtounicode{syouwaerasquare}{00A0}
\pdfglyphtounicode{t}{00A0}
\pdfglyphtounicode{tabengali}{00A0}
\pdfglyphtounicode{tackdown}{00A0}
\pdfglyphtounicode{tackleft}{00A0}
\pdfglyphtounicode{tadeva}{00A0}
\pdfglyphtounicode{tagujarati}{00A0}
\pdfglyphtounicode{tagurmukhi}{00A0}
\pdfglyphtounicode{taharabic}{00A0}
\pdfglyphtounicode{tahfinalarabic}{00A0}
\pdfglyphtounicode{tahinitialarabic}{00A0}
\pdfglyphtounicode{tahiragana}{00A0}
\pdfglyphtounicode{tahmedialarabic}{00A0}
\pdfglyphtounicode{taisyouerasquare}{00A0}
\pdfglyphtounicode{takatakana}{00A0}
\pdfglyphtounicode{takatakanahalfwidth}{00A0}
\pdfglyphtounicode{tatweelarabic}{00A0}
\pdfglyphtounicode{tau}{00A0}
\pdfglyphtounicode{tav}{00A0}
\pdfglyphtounicode{tavdages}{00A0}
\pdfglyphtounicode{tavdagesh}{00A0}
\pdfglyphtounicode{tavdageshhebrew}{00A0}
\pdfglyphtounicode{tavhebrew}{00A0}
\pdfglyphtounicode{tbar}{00A0}
\pdfglyphtounicode{tbopomofo}{00A0}
\pdfglyphtounicode{tcaron}{00A0}
\pdfglyphtounicode{tccurl}{00A0}
\pdfglyphtounicode{tcedilla}{00A0}
\pdfglyphtounicode{tcheharabic}{00A0}
\pdfglyphtounicode{tchehfinalarabic}{00A0}
\pdfglyphtounicode{tchehinitialarabic}{00A0}
\pdfglyphtounicode{tchehmedialarabic}{00A0}
\pdfglyphtounicode{tchehmeeminitialarabic}{00A0}
\pdfglyphtounicode{tcircle}{00A0}
\pdfglyphtounicode{tcircumflexbelow}{00A0}
\pdfglyphtounicode{tcommaaccent}{00A0}
\pdfglyphtounicode{tdieresis}{00A0}
\pdfglyphtounicode{tdotaccent}{00A0}
\pdfglyphtounicode{tdotbelow}{00A0}
\pdfglyphtounicode{tecyrillic}{00A0}
\pdfglyphtounicode{tedescendercyrillic}{00A0}
\pdfglyphtounicode{teharabic}{00A0}
\pdfglyphtounicode{tehfinalarabic}{00A0}
\pdfglyphtounicode{tehhahinitialarabic}{00A0}
\pdfglyphtounicode{tehhahisolatedarabic}{00A0}
\pdfglyphtounicode{tehinitialarabic}{00A0}
\pdfglyphtounicode{tehiragana}{00A0}
\pdfglyphtounicode{tehjeeminitialarabic}{00A0}
\pdfglyphtounicode{tehjeemisolatedarabic}{00A0}
\pdfglyphtounicode{tehmarbutaarabic}{00A0}
\pdfglyphtounicode{tehmarbutafinalarabic}{00A0}
\pdfglyphtounicode{tehmedialarabic}{00A0}
\pdfglyphtounicode{tehmeeminitialarabic}{00A0}
\pdfglyphtounicode{tehmeemisolatedarabic}{00A0}
\pdfglyphtounicode{tehnoonfinalarabic}{00A0}
\pdfglyphtounicode{tekatakana}{00A0}
\pdfglyphtounicode{tekatakanahalfwidth}{00A0}
\pdfglyphtounicode{telephone}{00A0}
\pdfglyphtounicode{telephoneblack}{00A0}
\pdfglyphtounicode{telishagedolahebrew}{00A0}
\pdfglyphtounicode{telishaqetanahebrew}{00A0}
\pdfglyphtounicode{tencircle}{00A0}
\pdfglyphtounicode{tenideographicparen}{00A0}
\pdfglyphtounicode{tenparen}{00A0}
\pdfglyphtounicode{tenperiod}{00A0}
\pdfglyphtounicode{tenroman}{00A0}
\pdfglyphtounicode{tesh}{00A0}
\pdfglyphtounicode{tet}{00A0}
\pdfglyphtounicode{tetdagesh}{00A0}
\pdfglyphtounicode{tetdageshhebrew}{00A0}
\pdfglyphtounicode{tethebrew}{00A0}
\pdfglyphtounicode{tetsecyrillic}{00A0}
\pdfglyphtounicode{tevirhebrew}{00A0}
\pdfglyphtounicode{tevirlefthebrew}{00A0}
\pdfglyphtounicode{tfm:cmbsy10/diamond}{00A0}
\pdfglyphtounicode{tfm:cmbsy10/heart}{00A0}
\pdfglyphtounicode{tfm:cmbsy5/diamond}{00A0}
\pdfglyphtounicode{tfm:cmbsy5/heart}{00A0}
\pdfglyphtounicode{tfm:cmbsy6/diamond}{00A0}
\pdfglyphtounicode{tfm:cmbsy6/heart}{00A0}
\pdfglyphtounicode{tfm:cmbsy7/diamond}{00A0}
\pdfglyphtounicode{tfm:cmbsy7/heart}{00A0}
\pdfglyphtounicode{tfm:cmbsy8/diamond}{00A0}
\pdfglyphtounicode{tfm:cmbsy8/heart}{00A0}
\pdfglyphtounicode{tfm:cmbsy9/diamond}{00A0}
\pdfglyphtounicode{tfm:cmbsy9/heart}{00A0}
\pdfglyphtounicode{tfm:cmmi10/phi}{00A0}
\pdfglyphtounicode{tfm:cmmi10/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmi12/phi}{00A0}
\pdfglyphtounicode{tfm:cmmi12/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmi5/phi}{00A0}
\pdfglyphtounicode{tfm:cmmi5/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmi6/phi}{00A0}
\pdfglyphtounicode{tfm:cmmi6/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmi7/phi}{00A0}
\pdfglyphtounicode{tfm:cmmi7/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmi8/phi}{00A0}
\pdfglyphtounicode{tfm:cmmi8/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmi9/phi}{00A0}
\pdfglyphtounicode{tfm:cmmi9/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmib10/phi}{00A0}
\pdfglyphtounicode{tfm:cmmib10/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmib5/phi}{00A0}
\pdfglyphtounicode{tfm:cmmib5/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmib6/phi}{00A0}
\pdfglyphtounicode{tfm:cmmib6/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmib7/phi}{00A0}
\pdfglyphtounicode{tfm:cmmib7/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmib8/phi}{00A0}
\pdfglyphtounicode{tfm:cmmib8/phi1}{00A0}
\pdfglyphtounicode{tfm:cmmib9/phi}{00A0}
\pdfglyphtounicode{tfm:cmmib9/phi1}{00A0}
\pdfglyphtounicode{tfm:cmsy10/diamond}{00A0}
\pdfglyphtounicode{tfm:cmsy10/heart}{00A0}
\pdfglyphtounicode{tfm:cmsy5/heart}{00A0}
\pdfglyphtounicode{tfm:cmsy6/diamond}{00A0}
\pdfglyphtounicode{tfm:cmsy6/heart}{00A0}
\pdfglyphtounicode{tfm:cmsy7/diamond}{00A0}
\pdfglyphtounicode{tfm:cmsy7/heart}{00A0}
\pdfglyphtounicode{tfm:cmsy8/diamond}{00A0}
\pdfglyphtounicode{tfm:cmsy8/heart}{00A0}
\pdfglyphtounicode{tfm:cmsy9/diamond}{00A0}
\pdfglyphtounicode{tfm:cmsy9/heart}{00A0}
\pdfglyphtounicode{tfm:eurb10/phi}{00A0}
\pdfglyphtounicode{tfm:eurb10/phi1}{00A0}
\pdfglyphtounicode{tfm:eurb5/phi}{00A0}
\pdfglyphtounicode{tfm:eurb5/phi1}{00A0}
\pdfglyphtounicode{tfm:eurb6/phi}{00A0}
\pdfglyphtounicode{tfm:eurb6/phi1}{00A0}
\pdfglyphtounicode{tfm:eurb7/phi}{00A0}
\pdfglyphtounicode{tfm:eurb7/phi1}{00A0}
\pdfglyphtounicode{tfm:eurb8/phi}{00A0}
\pdfglyphtounicode{tfm:eurb8/phi1}{00A0}
\pdfglyphtounicode{tfm:eurb9/phi}{00A0}
\pdfglyphtounicode{tfm:eurb9/phi1}{00A0}
\pdfglyphtounicode{tfm:eurm10/phi}{00A0}
\pdfglyphtounicode{tfm:eurm10/phi1}{00A0}
\pdfglyphtounicode{tfm:eurm5/phi}{00A0}
\pdfglyphtounicode{tfm:eurm5/phi1}{00A0}
\pdfglyphtounicode{tfm:eurm6/phi}{00A0}
\pdfglyphtounicode{tfm:eurm6/phi1}{00A0}
\pdfglyphtounicode{tfm:eurm7/phi}{00A0}
\pdfglyphtounicode{tfm:eurm7/phi1}{00A0}
\pdfglyphtounicode{tfm:eurm8/phi}{00A0}
\pdfglyphtounicode{tfm:eurm8/phi1}{00A0}
\pdfglyphtounicode{tfm:eurm9/phi}{00A0}
\pdfglyphtounicode{tfm:eurm9/phi1}{00A0}
\pdfglyphtounicode{tfm:fplmbi/phi}{00A0}
\pdfglyphtounicode{tfm:fplmbi/phi1}{00A0}
\pdfglyphtounicode{tfm:fplmri/phi}{00A0}
\pdfglyphtounicode{tfm:fplmri/phi1}{00A0}
\pdfglyphtounicode{tfm:lmbsy10/diamond}{00A0}
\pdfglyphtounicode{tfm:lmbsy10/heart}{00A0}
\pdfglyphtounicode{tfm:lmbsy5/diamond}{00A0}
\pdfglyphtounicode{tfm:lmbsy5/heart}{00A0}
\pdfglyphtounicode{tfm:lmbsy7/diamond}{00A0}
\pdfglyphtounicode{tfm:lmbsy7/heart}{00A0}
\pdfglyphtounicode{tfm:lmmi10/phi}{00A0}
\pdfglyphtounicode{tfm:lmmi10/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmi12/phi}{00A0}
\pdfglyphtounicode{tfm:lmmi12/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmi5/phi}{00A0}
\pdfglyphtounicode{tfm:lmmi5/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmi6/phi}{00A0}
\pdfglyphtounicode{tfm:lmmi6/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmi7/phi}{00A0}
\pdfglyphtounicode{tfm:lmmi7/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmi8/phi}{00A0}
\pdfglyphtounicode{tfm:lmmi8/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmi9/phi}{00A0}
\pdfglyphtounicode{tfm:lmmi9/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmib10/phi}{00A0}
\pdfglyphtounicode{tfm:lmmib10/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmib5/phi}{00A0}
\pdfglyphtounicode{tfm:lmmib5/phi1}{00A0}
\pdfglyphtounicode{tfm:lmmib7/phi}{00A0}
\pdfglyphtounicode{tfm:lmmib7/phi1}{00A0}
\pdfglyphtounicode{tfm:lmsy10/diamond}{00A0}
\pdfglyphtounicode{tfm:lmsy10/heart}{00A0}
\pdfglyphtounicode{tfm:lmsy5/diamond}{00A0}
\pdfglyphtounicode{tfm:lmsy5/heart}{00A0}
\pdfglyphtounicode{tfm:lmsy6/diamond}{00A0}
\pdfglyphtounicode{tfm:lmsy6/heart}{00A0}
\pdfglyphtounicode{tfm:lmsy7/diamond}{00A0}
\pdfglyphtounicode{tfm:lmsy7/heart}{00A0}
\pdfglyphtounicode{tfm:lmsy8/diamond}{00A0}
\pdfglyphtounicode{tfm:lmsy8/heart}{00A0}
\pdfglyphtounicode{tfm:lmsy9/diamond}{00A0}
\pdfglyphtounicode{tfm:lmsy9/heart}{00A0}
\pdfglyphtounicode{tfm:msam10/diamond}{00A0}
\pdfglyphtounicode{tfm:msam5/diamond}{00A0}
\pdfglyphtounicode{tfm:msam6/diamond}{00A0}
\pdfglyphtounicode{tfm:msam7/diamond}{00A0}
\pdfglyphtounicode{tfm:msam8/diamond}{00A0}
\pdfglyphtounicode{tfm:msam9/diamond}{00A0}
\pdfglyphtounicode{tfm:pxbmia/phi}{00A0}
\pdfglyphtounicode{tfm:pxbmia/phi1}{00A0}
\pdfglyphtounicode{tfm:pxbsy/diamond}{00A0}
\pdfglyphtounicode{tfm:pxbsy/heart}{00A0}
\pdfglyphtounicode{tfm:pxbsya/diamond}{00A0}
\pdfglyphtounicode{tfm:pxmia/phi}{00A0}
\pdfglyphtounicode{tfm:pxmia/phi1}{00A0}
\pdfglyphtounicode{tfm:pxsy/diamond}{00A0}
\pdfglyphtounicode{tfm:pxsy/heart}{00A0}
\pdfglyphtounicode{tfm:pxsya/diamond}{00A0}
\pdfglyphtounicode{tfm:pzdr/a1}{00A0}
\pdfglyphtounicode{tfm:pzdr/a10}{00A0}
\pdfglyphtounicode{tfm:pzdr/a100}{00A0}
\pdfglyphtounicode{tfm:pzdr/a101}{00A0}
\pdfglyphtounicode{tfm:pzdr/a102}{00A0}
\pdfglyphtounicode{tfm:pzdr/a103}{00A0}
\pdfglyphtounicode{tfm:pzdr/a104}{00A0}
\pdfglyphtounicode{tfm:pzdr/a105}{00A0}
\pdfglyphtounicode{tfm:pzdr/a106}{00A0}
\pdfglyphtounicode{tfm:pzdr/a107}{00A0}
\pdfglyphtounicode{tfm:pzdr/a108}{00A0}
\pdfglyphtounicode{tfm:pzdr/a109}{00A0}
\pdfglyphtounicode{tfm:pzdr/a11}{00A0}
\pdfglyphtounicode{tfm:pzdr/a110}{00A0}
\pdfglyphtounicode{tfm:pzdr/a111}{00A0}
\pdfglyphtounicode{tfm:pzdr/a112}{00A0}
\pdfglyphtounicode{tfm:pzdr/a117}{00A0}
\pdfglyphtounicode{tfm:pzdr/a118}{00A0}
\pdfglyphtounicode{tfm:pzdr/a119}{00A0}
\pdfglyphtounicode{tfm:pzdr/a12}{00A0}
\pdfglyphtounicode{tfm:pzdr/a120}{00A0}
\pdfglyphtounicode{tfm:pzdr/a121}{00A0}
\pdfglyphtounicode{tfm:pzdr/a122}{00A0}
\pdfglyphtounicode{tfm:pzdr/a123}{00A0}
\pdfglyphtounicode{tfm:pzdr/a124}{00A0}
\pdfglyphtounicode{tfm:pzdr/a125}{00A0}
\pdfglyphtounicode{tfm:pzdr/a126}{00A0}
\pdfglyphtounicode{tfm:pzdr/a127}{00A0}
\pdfglyphtounicode{tfm:pzdr/a128}{00A0}
\pdfglyphtounicode{tfm:pzdr/a129}{00A0}
\pdfglyphtounicode{tfm:pzdr/a13}{00A0}
\pdfglyphtounicode{tfm:pzdr/a130}{00A0}
\pdfglyphtounicode{tfm:pzdr/a131}{00A0}
\pdfglyphtounicode{tfm:pzdr/a132}{00A0}
\pdfglyphtounicode{tfm:pzdr/a133}{00A0}
\pdfglyphtounicode{tfm:pzdr/a134}{00A0}
\pdfglyphtounicode{tfm:pzdr/a135}{00A0}
\pdfglyphtounicode{tfm:pzdr/a136}{00A0}
\pdfglyphtounicode{tfm:pzdr/a137}{00A0}
\pdfglyphtounicode{tfm:pzdr/a138}{00A0}
\pdfglyphtounicode{tfm:pzdr/a139}{00A0}
\pdfglyphtounicode{tfm:pzdr/a14}{00A0}
\pdfglyphtounicode{tfm:pzdr/a140}{00A0}
\pdfglyphtounicode{tfm:pzdr/a141}{00A0}
\pdfglyphtounicode{tfm:pzdr/a142}{00A0}
\pdfglyphtounicode{tfm:pzdr/a143}{00A0}
\pdfglyphtounicode{tfm:pzdr/a144}{00A0}
\pdfglyphtounicode{tfm:pzdr/a145}{00A0}
\pdfglyphtounicode{tfm:pzdr/a146}{00A0}
\pdfglyphtounicode{tfm:pzdr/a147}{00A0}
\pdfglyphtounicode{tfm:pzdr/a148}{00A0}
\pdfglyphtounicode{tfm:pzdr/a149}{00A0}
\pdfglyphtounicode{tfm:pzdr/a15}{00A0}
\pdfglyphtounicode{tfm:pzdr/a150}{00A0}
\pdfglyphtounicode{tfm:pzdr/a151}{00A0}
\pdfglyphtounicode{tfm:pzdr/a152}{00A0}
\pdfglyphtounicode{tfm:pzdr/a153}{00A0}
\pdfglyphtounicode{tfm:pzdr/a154}{00A0}
\pdfglyphtounicode{tfm:pzdr/a155}{00A0}
\pdfglyphtounicode{tfm:pzdr/a156}{00A0}
\pdfglyphtounicode{tfm:pzdr/a157}{00A0}
\pdfglyphtounicode{tfm:pzdr/a158}{00A0}
\pdfglyphtounicode{tfm:pzdr/a159}{00A0}
\pdfglyphtounicode{tfm:pzdr/a16}{00A0}
\pdfglyphtounicode{tfm:pzdr/a160}{00A0}
\pdfglyphtounicode{tfm:pzdr/a161}{00A0}
\pdfglyphtounicode{tfm:pzdr/a162}{00A0}
\pdfglyphtounicode{tfm:pzdr/a163}{00A0}
\pdfglyphtounicode{tfm:pzdr/a164}{00A0}
\pdfglyphtounicode{tfm:pzdr/a165}{00A0}
\pdfglyphtounicode{tfm:pzdr/a166}{00A0}
\pdfglyphtounicode{tfm:pzdr/a167}{00A0}
\pdfglyphtounicode{tfm:pzdr/a168}{00A0}
\pdfglyphtounicode{tfm:pzdr/a169}{00A0}
\pdfglyphtounicode{tfm:pzdr/a17}{00A0}
\pdfglyphtounicode{tfm:pzdr/a170}{00A0}
\pdfglyphtounicode{tfm:pzdr/a171}{00A0}
\pdfglyphtounicode{tfm:pzdr/a172}{00A0}
\pdfglyphtounicode{tfm:pzdr/a173}{00A0}
\pdfglyphtounicode{tfm:pzdr/a174}{00A0}
\pdfglyphtounicode{tfm:pzdr/a175}{00A0}
\pdfglyphtounicode{tfm:pzdr/a176}{00A0}
\pdfglyphtounicode{tfm:pzdr/a177}{00A0}
\pdfglyphtounicode{tfm:pzdr/a178}{00A0}
\pdfglyphtounicode{tfm:pzdr/a179}{00A0}
\pdfglyphtounicode{tfm:pzdr/a18}{00A0}
\pdfglyphtounicode{tfm:pzdr/a180}{00A0}
\pdfglyphtounicode{tfm:pzdr/a181}{00A0}
\pdfglyphtounicode{tfm:pzdr/a182}{00A0}
\pdfglyphtounicode{tfm:pzdr/a183}{00A0}
\pdfglyphtounicode{tfm:pzdr/a184}{00A0}
\pdfglyphtounicode{tfm:pzdr/a185}{00A0}
\pdfglyphtounicode{tfm:pzdr/a186}{00A0}
\pdfglyphtounicode{tfm:pzdr/a187}{00A0}
\pdfglyphtounicode{tfm:pzdr/a188}{00A0}
\pdfglyphtounicode{tfm:pzdr/a189}{00A0}
\pdfglyphtounicode{tfm:pzdr/a19}{00A0}
\pdfglyphtounicode{tfm:pzdr/a190}{00A0}
\pdfglyphtounicode{tfm:pzdr/a191}{00A0}
\pdfglyphtounicode{tfm:pzdr/a192}{00A0}
\pdfglyphtounicode{tfm:pzdr/a193}{00A0}
\pdfglyphtounicode{tfm:pzdr/a194}{00A0}
\pdfglyphtounicode{tfm:pzdr/a195}{00A0}
\pdfglyphtounicode{tfm:pzdr/a196}{00A0}
\pdfglyphtounicode{tfm:pzdr/a197}{00A0}
\pdfglyphtounicode{tfm:pzdr/a198}{00A0}
\pdfglyphtounicode{tfm:pzdr/a199}{00A0}
\pdfglyphtounicode{tfm:pzdr/a2}{00A0}
\pdfglyphtounicode{tfm:pzdr/a20}{00A0}
\pdfglyphtounicode{tfm:pzdr/a200}{00A0}
\pdfglyphtounicode{tfm:pzdr/a201}{00A0}
\pdfglyphtounicode{tfm:pzdr/a202}{00A0}
\pdfglyphtounicode{tfm:pzdr/a203}{00A0}
\pdfglyphtounicode{tfm:pzdr/a204}{00A0}
\pdfglyphtounicode{tfm:pzdr/a205}{00A0}
\pdfglyphtounicode{tfm:pzdr/a206}{00A0}
\pdfglyphtounicode{tfm:pzdr/a21}{00A0}
\pdfglyphtounicode{tfm:pzdr/a22}{00A0}
\pdfglyphtounicode{tfm:pzdr/a23}{00A0}
\pdfglyphtounicode{tfm:pzdr/a24}{00A0}
\pdfglyphtounicode{tfm:pzdr/a25}{00A0}
\pdfglyphtounicode{tfm:pzdr/a26}{00A0}
\pdfglyphtounicode{tfm:pzdr/a27}{00A0}
\pdfglyphtounicode{tfm:pzdr/a28}{00A0}
\pdfglyphtounicode{tfm:pzdr/a29}{00A0}
\pdfglyphtounicode{tfm:pzdr/a3}{00A0}
\pdfglyphtounicode{tfm:pzdr/a30}{00A0}
\pdfglyphtounicode{tfm:pzdr/a31}{00A0}
\pdfglyphtounicode{tfm:pzdr/a32}{00A0}
\pdfglyphtounicode{tfm:pzdr/a33}{00A0}
\pdfglyphtounicode{tfm:pzdr/a34}{00A0}
\pdfglyphtounicode{tfm:pzdr/a35}{00A0}
\pdfglyphtounicode{tfm:pzdr/a36}{00A0}
\pdfglyphtounicode{tfm:pzdr/a37}{00A0}
\pdfglyphtounicode{tfm:pzdr/a38}{00A0}
\pdfglyphtounicode{tfm:pzdr/a39}{00A0}
\pdfglyphtounicode{tfm:pzdr/a4}{00A0}
\pdfglyphtounicode{tfm:pzdr/a40}{00A0}
\pdfglyphtounicode{tfm:pzdr/a41}{00A0}
\pdfglyphtounicode{tfm:pzdr/a42}{00A0}
\pdfglyphtounicode{tfm:pzdr/a43}{00A0}
\pdfglyphtounicode{tfm:pzdr/a44}{00A0}
\pdfglyphtounicode{tfm:pzdr/a45}{00A0}
\pdfglyphtounicode{tfm:pzdr/a46}{00A0}
\pdfglyphtounicode{tfm:pzdr/a47}{00A0}
\pdfglyphtounicode{tfm:pzdr/a48}{00A0}
\pdfglyphtounicode{tfm:pzdr/a49}{00A0}
\pdfglyphtounicode{tfm:pzdr/a5}{00A0}
\pdfglyphtounicode{tfm:pzdr/a50}{00A0}
\pdfglyphtounicode{tfm:pzdr/a51}{00A0}
\pdfglyphtounicode{tfm:pzdr/a52}{00A0}
\pdfglyphtounicode{tfm:pzdr/a53}{00A0}
\pdfglyphtounicode{tfm:pzdr/a54}{00A0}
\pdfglyphtounicode{tfm:pzdr/a55}{00A0}
\pdfglyphtounicode{tfm:pzdr/a56}{00A0}
\pdfglyphtounicode{tfm:pzdr/a57}{00A0}
\pdfglyphtounicode{tfm:pzdr/a58}{00A0}
\pdfglyphtounicode{tfm:pzdr/a59}{00A0}
\pdfglyphtounicode{tfm:pzdr/a6}{00A0}
\pdfglyphtounicode{tfm:pzdr/a60}{00A0}
\pdfglyphtounicode{tfm:pzdr/a61}{00A0}
\pdfglyphtounicode{tfm:pzdr/a62}{00A0}
\pdfglyphtounicode{tfm:pzdr/a63}{00A0}
\pdfglyphtounicode{tfm:pzdr/a64}{00A0}
\pdfglyphtounicode{tfm:pzdr/a65}{00A0}
\pdfglyphtounicode{tfm:pzdr/a66}{00A0}
\pdfglyphtounicode{tfm:pzdr/a67}{00A0}
\pdfglyphtounicode{tfm:pzdr/a68}{00A0}
\pdfglyphtounicode{tfm:pzdr/a69}{00A0}
\pdfglyphtounicode{tfm:pzdr/a7}{00A0}
\pdfglyphtounicode{tfm:pzdr/a70}{00A0}
\pdfglyphtounicode{tfm:pzdr/a71}{00A0}
\pdfglyphtounicode{tfm:pzdr/a72}{00A0}
\pdfglyphtounicode{tfm:pzdr/a73}{00A0}
\pdfglyphtounicode{tfm:pzdr/a74}{00A0}
\pdfglyphtounicode{tfm:pzdr/a75}{00A0}
\pdfglyphtounicode{tfm:pzdr/a76}{00A0}
\pdfglyphtounicode{tfm:pzdr/a77}{00A0}
\pdfglyphtounicode{tfm:pzdr/a78}{00A0}
\pdfglyphtounicode{tfm:pzdr/a79}{00A0}
\pdfglyphtounicode{tfm:pzdr/a8}{00A0}
\pdfglyphtounicode{tfm:pzdr/a81}{00A0}
\pdfglyphtounicode{tfm:pzdr/a82}{00A0}
\pdfglyphtounicode{tfm:pzdr/a83}{00A0}
\pdfglyphtounicode{tfm:pzdr/a84}{00A0}
\pdfglyphtounicode{tfm:pzdr/a85}{00A0}
\pdfglyphtounicode{tfm:pzdr/a86}{00A0}
\pdfglyphtounicode{tfm:pzdr/a87}{00A0}
\pdfglyphtounicode{tfm:pzdr/a88}{00A0}
\pdfglyphtounicode{tfm:pzdr/a89}{00A0}
\pdfglyphtounicode{tfm:pzdr/a9}{00A0}
\pdfglyphtounicode{tfm:pzdr/a90}{00A0}
\pdfglyphtounicode{tfm:pzdr/a91}{00A0}
\pdfglyphtounicode{tfm:pzdr/a92}{00A0}
\pdfglyphtounicode{tfm:pzdr/a93}{00A0}
\pdfglyphtounicode{tfm:pzdr/a94}{00A0}
\pdfglyphtounicode{tfm:pzdr/a95}{00A0}
\pdfglyphtounicode{tfm:pzdr/a96}{00A0}
\pdfglyphtounicode{tfm:pzdr/a97}{00A0}
\pdfglyphtounicode{tfm:pzdr/a98}{00A0}
\pdfglyphtounicode{tfm:pzdr/a99}{00A0}
\pdfglyphtounicode{tfm:rpxbmi/phi}{00A0}
\pdfglyphtounicode{tfm:rpxbmi/phi1}{00A0}
\pdfglyphtounicode{tfm:rpxmi/phi}{00A0}
\pdfglyphtounicode{tfm:rpxmi/phi1}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a1}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a10}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a100}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a101}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a102}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a103}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a104}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a105}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a106}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a107}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a108}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a109}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a11}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a110}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a111}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a112}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a117}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a118}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a119}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a12}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a120}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a121}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a122}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a123}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a124}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a125}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a126}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a127}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a128}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a129}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a13}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a130}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a131}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a132}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a133}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a134}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a135}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a136}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a137}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a138}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a139}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a14}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a140}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a141}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a142}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a143}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a144}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a145}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a146}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a147}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a148}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a149}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a15}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a150}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a151}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a152}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a153}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a154}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a155}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a156}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a157}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a158}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a159}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a16}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a160}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a161}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a162}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a163}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a164}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a165}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a166}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a167}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a168}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a169}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a17}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a170}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a171}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a172}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a173}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a174}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a175}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a176}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a177}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a178}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a179}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a18}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a180}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a181}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a182}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a183}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a184}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a185}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a186}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a187}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a188}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a189}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a19}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a190}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a191}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a192}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a193}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a194}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a195}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a196}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a197}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a198}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a199}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a2}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a20}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a200}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a201}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a202}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a203}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a204}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a205}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a206}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a21}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a22}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a23}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a24}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a25}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a26}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a27}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a28}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a29}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a3}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a30}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a31}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a32}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a33}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a34}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a35}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a36}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a37}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a38}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a39}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a4}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a40}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a41}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a42}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a43}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a44}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a45}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a46}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a47}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a48}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a49}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a5}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a50}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a51}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a52}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a53}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a54}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a55}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a56}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a57}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a58}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a59}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a6}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a60}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a61}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a62}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a63}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a64}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a65}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a66}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a67}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a68}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a69}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a7}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a70}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a71}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a72}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a73}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a74}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a75}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a76}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a77}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a78}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a79}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a8}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a81}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a82}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a83}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a84}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a85}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a86}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a87}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a88}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a89}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a9}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a90}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a91}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a92}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a93}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a94}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a95}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a96}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a97}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a98}{00A0}
\pdfglyphtounicode{tfm:rpzdr/a99}{00A0}
\pdfglyphtounicode{tfm:rtxbmi/phi}{00A0}
\pdfglyphtounicode{tfm:rtxbmi/phi1}{00A0}
\pdfglyphtounicode{tfm:rtxmi/phi}{00A0}
\pdfglyphtounicode{tfm:rtxmi/phi1}{00A0}
\pdfglyphtounicode{tfm:txbmia/phi}{00A0}
\pdfglyphtounicode{tfm:txbmia/phi1}{00A0}
\pdfglyphtounicode{tfm:txbsy/diamond}{00A0}
\pdfglyphtounicode{tfm:txbsy/heart}{00A0}
\pdfglyphtounicode{tfm:txbsya/diamond}{00A0}
\pdfglyphtounicode{tfm:txmia/phi}{00A0}
\pdfglyphtounicode{tfm:txmia/phi1}{00A0}
\pdfglyphtounicode{tfm:txsy/diamond}{00A0}
\pdfglyphtounicode{tfm:txsy/heart}{00A0}
\pdfglyphtounicode{tfm:txsya/diamond}{00A0}
\pdfglyphtounicode{tfm:zd/a1}{00A0}
\pdfglyphtounicode{tfm:zd/a10}{00A0}
\pdfglyphtounicode{tfm:zd/a100}{00A0}
\pdfglyphtounicode{tfm:zd/a101}{00A0}
\pdfglyphtounicode{tfm:zd/a102}{00A0}
\pdfglyphtounicode{tfm:zd/a103}{00A0}
\pdfglyphtounicode{tfm:zd/a104}{00A0}
\pdfglyphtounicode{tfm:zd/a105}{00A0}
\pdfglyphtounicode{tfm:zd/a106}{00A0}
\pdfglyphtounicode{tfm:zd/a107}{00A0}
\pdfglyphtounicode{tfm:zd/a108}{00A0}
\pdfglyphtounicode{tfm:zd/a109}{00A0}
\pdfglyphtounicode{tfm:zd/a11}{00A0}
\pdfglyphtounicode{tfm:zd/a110}{00A0}
\pdfglyphtounicode{tfm:zd/a111}{00A0}
\pdfglyphtounicode{tfm:zd/a112}{00A0}
\pdfglyphtounicode{tfm:zd/a117}{00A0}
\pdfglyphtounicode{tfm:zd/a118}{00A0}
\pdfglyphtounicode{tfm:zd/a119}{00A0}
\pdfglyphtounicode{tfm:zd/a12}{00A0}
\pdfglyphtounicode{tfm:zd/a120}{00A0}
\pdfglyphtounicode{tfm:zd/a121}{00A0}
\pdfglyphtounicode{tfm:zd/a122}{00A0}
\pdfglyphtounicode{tfm:zd/a123}{00A0}
\pdfglyphtounicode{tfm:zd/a124}{00A0}
\pdfglyphtounicode{tfm:zd/a125}{00A0}
\pdfglyphtounicode{tfm:zd/a126}{00A0}
\pdfglyphtounicode{tfm:zd/a127}{00A0}
\pdfglyphtounicode{tfm:zd/a128}{00A0}
\pdfglyphtounicode{tfm:zd/a129}{00A0}
\pdfglyphtounicode{tfm:zd/a13}{00A0}
\pdfglyphtounicode{tfm:zd/a130}{00A0}
\pdfglyphtounicode{tfm:zd/a131}{00A0}
\pdfglyphtounicode{tfm:zd/a132}{00A0}
\pdfglyphtounicode{tfm:zd/a133}{00A0}
\pdfglyphtounicode{tfm:zd/a134}{00A0}
\pdfglyphtounicode{tfm:zd/a135}{00A0}
\pdfglyphtounicode{tfm:zd/a136}{00A0}
\pdfglyphtounicode{tfm:zd/a137}{00A0}
\pdfglyphtounicode{tfm:zd/a138}{00A0}
\pdfglyphtounicode{tfm:zd/a139}{00A0}
\pdfglyphtounicode{tfm:zd/a14}{00A0}
\pdfglyphtounicode{tfm:zd/a140}{00A0}
\pdfglyphtounicode{tfm:zd/a141}{00A0}
\pdfglyphtounicode{tfm:zd/a142}{00A0}
\pdfglyphtounicode{tfm:zd/a143}{00A0}
\pdfglyphtounicode{tfm:zd/a144}{00A0}
\pdfglyphtounicode{tfm:zd/a145}{00A0}
\pdfglyphtounicode{tfm:zd/a146}{00A0}
\pdfglyphtounicode{tfm:zd/a147}{00A0}
\pdfglyphtounicode{tfm:zd/a148}{00A0}
\pdfglyphtounicode{tfm:zd/a149}{00A0}
\pdfglyphtounicode{tfm:zd/a15}{00A0}
\pdfglyphtounicode{tfm:zd/a150}{00A0}
\pdfglyphtounicode{tfm:zd/a151}{00A0}
\pdfglyphtounicode{tfm:zd/a152}{00A0}
\pdfglyphtounicode{tfm:zd/a153}{00A0}
\pdfglyphtounicode{tfm:zd/a154}{00A0}
\pdfglyphtounicode{tfm:zd/a155}{00A0}
\pdfglyphtounicode{tfm:zd/a156}{00A0}
\pdfglyphtounicode{tfm:zd/a157}{00A0}
\pdfglyphtounicode{tfm:zd/a158}{00A0}
\pdfglyphtounicode{tfm:zd/a159}{00A0}
\pdfglyphtounicode{tfm:zd/a16}{00A0}
\pdfglyphtounicode{tfm:zd/a160}{00A0}
\pdfglyphtounicode{tfm:zd/a161}{00A0}
\pdfglyphtounicode{tfm:zd/a162}{00A0}
\pdfglyphtounicode{tfm:zd/a163}{00A0}
\pdfglyphtounicode{tfm:zd/a164}{00A0}
\pdfglyphtounicode{tfm:zd/a165}{00A0}
\pdfglyphtounicode{tfm:zd/a166}{00A0}
\pdfglyphtounicode{tfm:zd/a167}{00A0}
\pdfglyphtounicode{tfm:zd/a168}{00A0}
\pdfglyphtounicode{tfm:zd/a169}{00A0}
\pdfglyphtounicode{tfm:zd/a17}{00A0}
\pdfglyphtounicode{tfm:zd/a170}{00A0}
\pdfglyphtounicode{tfm:zd/a171}{00A0}
\pdfglyphtounicode{tfm:zd/a172}{00A0}
\pdfglyphtounicode{tfm:zd/a173}{00A0}
\pdfglyphtounicode{tfm:zd/a174}{00A0}
\pdfglyphtounicode{tfm:zd/a175}{00A0}
\pdfglyphtounicode{tfm:zd/a176}{00A0}
\pdfglyphtounicode{tfm:zd/a177}{00A0}
\pdfglyphtounicode{tfm:zd/a178}{00A0}
\pdfglyphtounicode{tfm:zd/a179}{00A0}
\pdfglyphtounicode{tfm:zd/a18}{00A0}
\pdfglyphtounicode{tfm:zd/a180}{00A0}
\pdfglyphtounicode{tfm:zd/a181}{00A0}
\pdfglyphtounicode{tfm:zd/a182}{00A0}
\pdfglyphtounicode{tfm:zd/a183}{00A0}
\pdfglyphtounicode{tfm:zd/a184}{00A0}
\pdfglyphtounicode{tfm:zd/a185}{00A0}
\pdfglyphtounicode{tfm:zd/a186}{00A0}
\pdfglyphtounicode{tfm:zd/a187}{00A0}
\pdfglyphtounicode{tfm:zd/a188}{00A0}
\pdfglyphtounicode{tfm:zd/a189}{00A0}
\pdfglyphtounicode{tfm:zd/a19}{00A0}
\pdfglyphtounicode{tfm:zd/a190}{00A0}
\pdfglyphtounicode{tfm:zd/a191}{00A0}
\pdfglyphtounicode{tfm:zd/a192}{00A0}
\pdfglyphtounicode{tfm:zd/a193}{00A0}
\pdfglyphtounicode{tfm:zd/a194}{00A0}
\pdfglyphtounicode{tfm:zd/a195}{00A0}
\pdfglyphtounicode{tfm:zd/a196}{00A0}
\pdfglyphtounicode{tfm:zd/a197}{00A0}
\pdfglyphtounicode{tfm:zd/a198}{00A0}
\pdfglyphtounicode{tfm:zd/a199}{00A0}
\pdfglyphtounicode{tfm:zd/a2}{00A0}
\pdfglyphtounicode{tfm:zd/a20}{00A0}
\pdfglyphtounicode{tfm:zd/a200}{00A0}
\pdfglyphtounicode{tfm:zd/a201}{00A0}
\pdfglyphtounicode{tfm:zd/a202}{00A0}
\pdfglyphtounicode{tfm:zd/a203}{00A0}
\pdfglyphtounicode{tfm:zd/a204}{00A0}
\pdfglyphtounicode{tfm:zd/a205}{00A0}
\pdfglyphtounicode{tfm:zd/a206}{00A0}
\pdfglyphtounicode{tfm:zd/a21}{00A0}
\pdfglyphtounicode{tfm:zd/a22}{00A0}
\pdfglyphtounicode{tfm:zd/a23}{00A0}
\pdfglyphtounicode{tfm:zd/a24}{00A0}
\pdfglyphtounicode{tfm:zd/a25}{00A0}
\pdfglyphtounicode{tfm:zd/a26}{00A0}
\pdfglyphtounicode{tfm:zd/a27}{00A0}
\pdfglyphtounicode{tfm:zd/a28}{00A0}
\pdfglyphtounicode{tfm:zd/a29}{00A0}
\pdfglyphtounicode{tfm:zd/a3}{00A0}
\pdfglyphtounicode{tfm:zd/a30}{00A0}
\pdfglyphtounicode{tfm:zd/a31}{00A0}
\pdfglyphtounicode{tfm:zd/a32}{00A0}
\pdfglyphtounicode{tfm:zd/a33}{00A0}
\pdfglyphtounicode{tfm:zd/a34}{00A0}
\pdfglyphtounicode{tfm:zd/a35}{00A0}
\pdfglyphtounicode{tfm:zd/a36}{00A0}
\pdfglyphtounicode{tfm:zd/a37}{00A0}
\pdfglyphtounicode{tfm:zd/a38}{00A0}
\pdfglyphtounicode{tfm:zd/a39}{00A0}
\pdfglyphtounicode{tfm:zd/a4}{00A0}
\pdfglyphtounicode{tfm:zd/a40}{00A0}
\pdfglyphtounicode{tfm:zd/a41}{00A0}
\pdfglyphtounicode{tfm:zd/a42}{00A0}
\pdfglyphtounicode{tfm:zd/a43}{00A0}
\pdfglyphtounicode{tfm:zd/a44}{00A0}
\pdfglyphtounicode{tfm:zd/a45}{00A0}
\pdfglyphtounicode{tfm:zd/a46}{00A0}
\pdfglyphtounicode{tfm:zd/a47}{00A0}
\pdfglyphtounicode{tfm:zd/a48}{00A0}
\pdfglyphtounicode{tfm:zd/a49}{00A0}
\pdfglyphtounicode{tfm:zd/a5}{00A0}
\pdfglyphtounicode{tfm:zd/a50}{00A0}
\pdfglyphtounicode{tfm:zd/a51}{00A0}
\pdfglyphtounicode{tfm:zd/a52}{00A0}
\pdfglyphtounicode{tfm:zd/a53}{00A0}
\pdfglyphtounicode{tfm:zd/a54}{00A0}
\pdfglyphtounicode{tfm:zd/a55}{00A0}
\pdfglyphtounicode{tfm:zd/a56}{00A0}
\pdfglyphtounicode{tfm:zd/a57}{00A0}
\pdfglyphtounicode{tfm:zd/a58}{00A0}
\pdfglyphtounicode{tfm:zd/a59}{00A0}
\pdfglyphtounicode{tfm:zd/a6}{00A0}
\pdfglyphtounicode{tfm:zd/a60}{00A0}
\pdfglyphtounicode{tfm:zd/a61}{00A0}
\pdfglyphtounicode{tfm:zd/a62}{00A0}
\pdfglyphtounicode{tfm:zd/a63}{00A0}
\pdfglyphtounicode{tfm:zd/a64}{00A0}
\pdfglyphtounicode{tfm:zd/a65}{00A0}
\pdfglyphtounicode{tfm:zd/a66}{00A0}
\pdfglyphtounicode{tfm:zd/a67}{00A0}
\pdfglyphtounicode{tfm:zd/a68}{00A0}
\pdfglyphtounicode{tfm:zd/a69}{00A0}
\pdfglyphtounicode{tfm:zd/a7}{00A0}
\pdfglyphtounicode{tfm:zd/a70}{00A0}
\pdfglyphtounicode{tfm:zd/a71}{00A0}
\pdfglyphtounicode{tfm:zd/a72}{00A0}
\pdfglyphtounicode{tfm:zd/a73}{00A0}
\pdfglyphtounicode{tfm:zd/a74}{00A0}
\pdfglyphtounicode{tfm:zd/a75}{00A0}
\pdfglyphtounicode{tfm:zd/a76}{00A0}
\pdfglyphtounicode{tfm:zd/a77}{00A0}
\pdfglyphtounicode{tfm:zd/a78}{00A0}
\pdfglyphtounicode{tfm:zd/a79}{00A0}
\pdfglyphtounicode{tfm:zd/a8}{00A0}
\pdfglyphtounicode{tfm:zd/a81}{00A0}
\pdfglyphtounicode{tfm:zd/a82}{00A0}
\pdfglyphtounicode{tfm:zd/a83}{00A0}
\pdfglyphtounicode{tfm:zd/a84}{00A0}
\pdfglyphtounicode{tfm:zd/a85}{00A0}
\pdfglyphtounicode{tfm:zd/a86}{00A0}
\pdfglyphtounicode{tfm:zd/a87}{00A0}
\pdfglyphtounicode{tfm:zd/a88}{00A0}
\pdfglyphtounicode{tfm:zd/a89}{00A0}
\pdfglyphtounicode{tfm:zd/a9}{00A0}
\pdfglyphtounicode{tfm:zd/a90}{00A0}
\pdfglyphtounicode{tfm:zd/a91}{00A0}
\pdfglyphtounicode{tfm:zd/a92}{00A0}
\pdfglyphtounicode{tfm:zd/a93}{00A0}
\pdfglyphtounicode{tfm:zd/a94}{00A0}
\pdfglyphtounicode{tfm:zd/a95}{00A0}
\pdfglyphtounicode{tfm:zd/a96}{00A0}
\pdfglyphtounicode{tfm:zd/a97}{00A0}
\pdfglyphtounicode{tfm:zd/a98}{00A0}
\pdfglyphtounicode{tfm:zd/a99}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a1}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a10}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a100}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a101}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a102}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a103}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a104}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a105}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a106}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a107}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a108}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a109}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a11}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a110}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a111}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a112}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a117}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a118}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a119}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a12}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a120}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a121}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a122}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a123}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a124}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a125}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a126}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a127}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a128}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a129}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a13}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a130}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a131}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a132}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a133}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a134}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a135}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a136}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a137}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a138}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a139}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a14}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a140}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a141}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a142}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a143}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a144}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a145}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a146}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a147}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a148}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a149}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a15}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a150}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a151}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a152}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a153}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a154}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a155}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a156}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a157}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a158}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a159}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a16}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a160}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a161}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a162}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a163}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a164}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a165}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a166}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a167}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a168}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a169}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a17}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a170}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a171}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a172}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a173}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a174}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a175}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a176}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a177}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a178}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a179}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a18}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a180}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a181}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a182}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a183}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a184}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a185}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a186}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a187}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a188}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a189}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a19}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a190}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a191}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a192}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a193}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a194}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a195}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a196}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a197}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a198}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a199}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a2}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a20}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a200}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a201}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a202}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a203}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a204}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a205}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a206}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a21}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a22}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a23}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a24}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a25}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a26}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a27}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a28}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a29}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a3}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a30}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a31}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a32}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a33}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a34}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a35}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a36}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a37}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a38}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a39}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a4}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a40}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a41}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a42}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a43}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a44}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a45}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a46}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a47}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a48}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a49}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a5}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a50}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a51}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a52}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a53}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a54}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a55}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a56}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a57}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a58}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a59}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a6}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a60}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a61}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a62}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a63}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a64}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a65}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a66}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a67}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a68}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a69}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a7}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a70}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a71}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a72}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a73}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a74}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a75}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a76}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a77}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a78}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a79}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a8}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a81}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a82}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a83}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a84}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a85}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a86}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a87}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a88}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a89}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a9}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a90}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a91}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a92}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a93}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a94}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a95}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a96}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a97}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a98}{00A0}
\pdfglyphtounicode{tfm:zpzdr-reversed/a99}{00A0}
\pdfglyphtounicode{thabengali}{00A0}
\pdfglyphtounicode{thadeva}{00A0}
\pdfglyphtounicode{thagujarati}{00A0}
\pdfglyphtounicode{thagurmukhi}{00A0}
\pdfglyphtounicode{thalarabic}{00A0}
\pdfglyphtounicode{thalfinalarabic}{00A0}
\pdfglyphtounicode{thanthakhatlowleftthai}{00A0}
\pdfglyphtounicode{thanthakhatlowrightthai}{00A0}
\pdfglyphtounicode{thanthakhatthai}{00A0}
\pdfglyphtounicode{thanthakhatupperleftthai}{00A0}
\pdfglyphtounicode{theharabic}{00A0}
\pdfglyphtounicode{thehfinalarabic}{00A0}
\pdfglyphtounicode{thehinitialarabic}{00A0}
\pdfglyphtounicode{thehmedialarabic}{00A0}
\pdfglyphtounicode{thereexists}{00A0}
\pdfglyphtounicode{therefore}{00A0}
\pdfglyphtounicode{theta}{00A0}
\pdfglyphtounicode{theta1}{00A0}
\pdfglyphtounicode{thetasymbolgreek}{00A0}
\pdfglyphtounicode{thieuthacirclekorean}{00A0}
\pdfglyphtounicode{thieuthaparenkorean}{00A0}
\pdfglyphtounicode{thieuthcirclekorean}{00A0}
\pdfglyphtounicode{thieuthkorean}{00A0}
\pdfglyphtounicode{thieuthparenkorean}{00A0}
\pdfglyphtounicode{thirteencircle}{00A0}
\pdfglyphtounicode{thirteenparen}{00A0}
\pdfglyphtounicode{thirteenperiod}{00A0}
\pdfglyphtounicode{thonangmonthothai}{00A0}
\pdfglyphtounicode{thook}{00A0}
\pdfglyphtounicode{thophuthaothai}{00A0}
\pdfglyphtounicode{thorn}{00A0}
\pdfglyphtounicode{thothahanthai}{00A0}
\pdfglyphtounicode{thothanthai}{00A0}
\pdfglyphtounicode{thothongthai}{00A0}
\pdfglyphtounicode{thothungthai}{00A0}
\pdfglyphtounicode{thousandcyrillic}{00A0}
\pdfglyphtounicode{thousandsseparatorarabic}{00A0}
\pdfglyphtounicode{thousandsseparatorpersian}{00A0}
\pdfglyphtounicode{three}{00A0}
\pdfglyphtounicode{threearabic}{00A0}
\pdfglyphtounicode{threebengali}{00A0}
\pdfglyphtounicode{threecircle}{00A0}
\pdfglyphtounicode{threecircleinversesansserif}{00A0}
\pdfglyphtounicode{threedeva}{00A0}
\pdfglyphtounicode{threeeighths}{00A0}
\pdfglyphtounicode{threegujarati}{00A0}
\pdfglyphtounicode{threegurmukhi}{00A0}
\pdfglyphtounicode{threehackarabic}{00A0}
\pdfglyphtounicode{threehangzhou}{00A0}
\pdfglyphtounicode{threeideographicparen}{00A0}
\pdfglyphtounicode{threeinferior}{00A0}
\pdfglyphtounicode{threemonospace}{00A0}
\pdfglyphtounicode{threenumeratorbengali}{00A0}
\pdfglyphtounicode{threeoldstyle}{00A0}
\pdfglyphtounicode{threeparen}{00A0}
\pdfglyphtounicode{threeperiod}{00A0}
\pdfglyphtounicode{threepersian}{00A0}
\pdfglyphtounicode{threequarters}{00A0}
\pdfglyphtounicode{threequartersemdash}{00A0}
\pdfglyphtounicode{threeroman}{00A0}
\pdfglyphtounicode{threesuperior}{00A0}
\pdfglyphtounicode{threethai}{00A0}
\pdfglyphtounicode{thzsquare}{00A0}
\pdfglyphtounicode{tihiragana}{00A0}
\pdfglyphtounicode{tikatakana}{00A0}
\pdfglyphtounicode{tikatakanahalfwidth}{00A0}
\pdfglyphtounicode{tikeutacirclekorean}{00A0}
\pdfglyphtounicode{tikeutaparenkorean}{00A0}
\pdfglyphtounicode{tikeutcirclekorean}{00A0}
\pdfglyphtounicode{tikeutkorean}{00A0}
\pdfglyphtounicode{tikeutparenkorean}{00A0}
\pdfglyphtounicode{tilde}{00A0}
\pdfglyphtounicode{tildebelowcmb}{00A0}
\pdfglyphtounicode{tildecmb}{00A0}
\pdfglyphtounicode{tildecomb}{00A0}
\pdfglyphtounicode{tildedoublecmb}{00A0}
\pdfglyphtounicode{tildeoperator}{00A0}
\pdfglyphtounicode{tildeoverlaycmb}{00A0}
\pdfglyphtounicode{tildeverticalcmb}{00A0}
\pdfglyphtounicode{timescircle}{00A0}
\pdfglyphtounicode{tipehahebrew}{00A0}
\pdfglyphtounicode{tipehalefthebrew}{00A0}
\pdfglyphtounicode{tippigurmukhi}{00A0}
\pdfglyphtounicode{titlocyrilliccmb}{00A0}
\pdfglyphtounicode{tiwnarmenian}{00A0}
\pdfglyphtounicode{tlinebelow}{00A0}
\pdfglyphtounicode{tmonospace}{00A0}
\pdfglyphtounicode{toarmenian}{00A0}
\pdfglyphtounicode{tohiragana}{00A0}
\pdfglyphtounicode{tokatakana}{00A0}
\pdfglyphtounicode{tokatakanahalfwidth}{00A0}
\pdfglyphtounicode{tonebarextrahighmod}{00A0}
\pdfglyphtounicode{tonebarextralowmod}{00A0}
\pdfglyphtounicode{tonebarhighmod}{00A0}
\pdfglyphtounicode{tonebarlowmod}{00A0}
\pdfglyphtounicode{tonebarmidmod}{00A0}
\pdfglyphtounicode{tonefive}{00A0}
\pdfglyphtounicode{tonesix}{00A0}
\pdfglyphtounicode{tonetwo}{00A0}
\pdfglyphtounicode{tonos}{00A0}
\pdfglyphtounicode{tonsquare}{00A0}
\pdfglyphtounicode{topatakthai}{00A0}
\pdfglyphtounicode{tortoiseshellbracketleft}{00A0}
\pdfglyphtounicode{tortoiseshellbracketleftsmall}{00A0}
\pdfglyphtounicode{tortoiseshellbracketleftvertical}{00A0}
\pdfglyphtounicode{tortoiseshellbracketright}{00A0}
\pdfglyphtounicode{tortoiseshellbracketrightsmall}{00A0}
\pdfglyphtounicode{tortoiseshellbracketrightvertical}{00A0}
\pdfglyphtounicode{totaothai}{00A0}
\pdfglyphtounicode{tpalatalhook}{00A0}
\pdfglyphtounicode{tparen}{00A0}
\pdfglyphtounicode{trademark}{00A0}
\pdfglyphtounicode{trademarksans}{00A0}
\pdfglyphtounicode{trademarkserif}{00A0}
\pdfglyphtounicode{tretroflexhook}{00A0}
\pdfglyphtounicode{triagdn}{00A0}
\pdfglyphtounicode{triaglf}{00A0}
\pdfglyphtounicode{triagrt}{00A0}
\pdfglyphtounicode{triagup}{00A0}
\pdfglyphtounicode{triangle}{00A0}
\pdfglyphtounicode{triangledownsld}{00A0}
\pdfglyphtounicode{triangleinv}{00A0}
\pdfglyphtounicode{triangleleft}{00A0}
\pdfglyphtounicode{triangleleftequal}{00A0}
\pdfglyphtounicode{triangleleftsld}{00A0}
\pdfglyphtounicode{triangleright}{00A0}
\pdfglyphtounicode{trianglerightequal}{00A0}
\pdfglyphtounicode{trianglerightsld}{00A0}
\pdfglyphtounicode{trianglesolid}{00A0}
\pdfglyphtounicode{ts}{00A0}
\pdfglyphtounicode{tsadi}{00A0}
\pdfglyphtounicode{tsadidagesh}{00A0}
\pdfglyphtounicode{tsadidageshhebrew}{00A0}
\pdfglyphtounicode{tsadihebrew}{00A0}
\pdfglyphtounicode{tsecyrillic}{00A0}
\pdfglyphtounicode{tsere}{00A0}
\pdfglyphtounicode{tsere12}{00A0}
\pdfglyphtounicode{tsere1e}{00A0}
\pdfglyphtounicode{tsere2b}{00A0}
\pdfglyphtounicode{tserehebrew}{00A0}
\pdfglyphtounicode{tserenarrowhebrew}{00A0}
\pdfglyphtounicode{tserequarterhebrew}{00A0}
\pdfglyphtounicode{tserewidehebrew}{00A0}
\pdfglyphtounicode{tshecyrillic}{00A0}
\pdfglyphtounicode{tsuperior}{00A0}
\pdfglyphtounicode{ttabengali}{00A0}
\pdfglyphtounicode{ttadeva}{00A0}
\pdfglyphtounicode{ttagujarati}{00A0}
\pdfglyphtounicode{ttagurmukhi}{00A0}
\pdfglyphtounicode{tteharabic}{00A0}
\pdfglyphtounicode{ttehfinalarabic}{00A0}
\pdfglyphtounicode{ttehinitialarabic}{00A0}
\pdfglyphtounicode{ttehmedialarabic}{00A0}
\pdfglyphtounicode{tthabengali}{00A0}
\pdfglyphtounicode{tthadeva}{00A0}
\pdfglyphtounicode{tthagujarati}{00A0}
\pdfglyphtounicode{tthagurmukhi}{00A0}
\pdfglyphtounicode{tturned}{00A0}
\pdfglyphtounicode{tuhiragana}{00A0}
\pdfglyphtounicode{tukatakana}{00A0}
\pdfglyphtounicode{tukatakanahalfwidth}{00A0}
\pdfglyphtounicode{turnstileleft}{00A0}
\pdfglyphtounicode{turnstileright}{00A0}
\pdfglyphtounicode{tusmallhiragana}{00A0}
\pdfglyphtounicode{tusmallkatakana}{00A0}
\pdfglyphtounicode{tusmallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{twelvecircle}{00A0}
\pdfglyphtounicode{twelveparen}{00A0}
\pdfglyphtounicode{twelveperiod}{00A0}
\pdfglyphtounicode{twelveroman}{00A0}
\pdfglyphtounicode{twentycircle}{00A0}
\pdfglyphtounicode{twentyhangzhou}{00A0}
\pdfglyphtounicode{twentyparen}{00A0}
\pdfglyphtounicode{twentyperiod}{00A0}
\pdfglyphtounicode{two}{00A0}
\pdfglyphtounicode{twoarabic}{00A0}
\pdfglyphtounicode{twobengali}{00A0}
\pdfglyphtounicode{twocircle}{00A0}
\pdfglyphtounicode{twocircleinversesansserif}{00A0}
\pdfglyphtounicode{twodeva}{00A0}
\pdfglyphtounicode{twodotenleader}{00A0}
\pdfglyphtounicode{twodotleader}{00A0}
\pdfglyphtounicode{twodotleadervertical}{00A0}
\pdfglyphtounicode{twogujarati}{00A0}
\pdfglyphtounicode{twogurmukhi}{00A0}
\pdfglyphtounicode{twohackarabic}{00A0}
\pdfglyphtounicode{twohangzhou}{00A0}
\pdfglyphtounicode{twoideographicparen}{00A0}
\pdfglyphtounicode{twoinferior}{00A0}
\pdfglyphtounicode{twomonospace}{00A0}
\pdfglyphtounicode{twonumeratorbengali}{00A0}
\pdfglyphtounicode{twooldstyle}{00A0}
\pdfglyphtounicode{twoparen}{00A0}
\pdfglyphtounicode{twoperiod}{00A0}
\pdfglyphtounicode{twopersian}{00A0}
\pdfglyphtounicode{tworoman}{00A0}
\pdfglyphtounicode{twostroke}{00A0}
\pdfglyphtounicode{twosuperior}{00A0}
\pdfglyphtounicode{twothai}{00A0}
\pdfglyphtounicode{twothirds}{00A0}
\pdfglyphtounicode{u}{00A0}
\pdfglyphtounicode{uacute}{00A0}
\pdfglyphtounicode{ubar}{00A0}
\pdfglyphtounicode{ubengali}{00A0}
\pdfglyphtounicode{ubopomofo}{00A0}
\pdfglyphtounicode{ubreve}{00A0}
\pdfglyphtounicode{ucaron}{00A0}
\pdfglyphtounicode{ucircle}{00A0}
\pdfglyphtounicode{ucircumflex}{00A0}
\pdfglyphtounicode{ucircumflexbelow}{00A0}
\pdfglyphtounicode{ucyrillic}{00A0}
\pdfglyphtounicode{udattadeva}{00A0}
\pdfglyphtounicode{udblacute}{00A0}
\pdfglyphtounicode{udblgrave}{00A0}
\pdfglyphtounicode{udeva}{00A0}
\pdfglyphtounicode{udieresis}{00A0}
\pdfglyphtounicode{udieresisacute}{00A0}
\pdfglyphtounicode{udieresisbelow}{00A0}
\pdfglyphtounicode{udieresiscaron}{00A0}
\pdfglyphtounicode{udieresiscyrillic}{00A0}
\pdfglyphtounicode{udieresisgrave}{00A0}
\pdfglyphtounicode{udieresismacron}{00A0}
\pdfglyphtounicode{udotbelow}{00A0}
\pdfglyphtounicode{ugrave}{00A0}
\pdfglyphtounicode{ugujarati}{00A0}
\pdfglyphtounicode{ugurmukhi}{00A0}
\pdfglyphtounicode{uhiragana}{00A0}
\pdfglyphtounicode{uhookabove}{00A0}
\pdfglyphtounicode{uhorn}{00A0}
\pdfglyphtounicode{uhornacute}{00A0}
\pdfglyphtounicode{uhorndotbelow}{00A0}
\pdfglyphtounicode{uhorngrave}{00A0}
\pdfglyphtounicode{uhornhookabove}{00A0}
\pdfglyphtounicode{uhorntilde}{00A0}
\pdfglyphtounicode{uhungarumlaut}{00A0}
\pdfglyphtounicode{uhungarumlautcyrillic}{00A0}
\pdfglyphtounicode{uinvertedbreve}{00A0}
\pdfglyphtounicode{ukatakana}{00A0}
\pdfglyphtounicode{ukatakanahalfwidth}{00A0}
\pdfglyphtounicode{ukcyrillic}{00A0}
\pdfglyphtounicode{ukorean}{00A0}
\pdfglyphtounicode{umacron}{00A0}
\pdfglyphtounicode{umacroncyrillic}{00A0}
\pdfglyphtounicode{umacrondieresis}{00A0}
\pdfglyphtounicode{umatragurmukhi}{00A0}
\pdfglyphtounicode{umonospace}{00A0}
\pdfglyphtounicode{underscore}{00A0}
\pdfglyphtounicode{underscoredbl}{00A0}
\pdfglyphtounicode{underscoremonospace}{00A0}
\pdfglyphtounicode{underscorevertical}{00A0}
\pdfglyphtounicode{underscorewavy}{00A0}
\pdfglyphtounicode{union}{00A0}
\pdfglyphtounicode{uniondbl}{00A0}
\pdfglyphtounicode{unionmulti}{00A0}
\pdfglyphtounicode{unionsq}{00A0}
\pdfglyphtounicode{universal}{00A0}
\pdfglyphtounicode{uogonek}{00A0}
\pdfglyphtounicode{uparen}{00A0}
\pdfglyphtounicode{upblock}{00A0}
\pdfglyphtounicode{upperdothebrew}{00A0}
\pdfglyphtounicode{uprise}{00A0}
\pdfglyphtounicode{upsilon}{00A0}
\pdfglyphtounicode{upsilondieresis}{00A0}
\pdfglyphtounicode{upsilondieresistonos}{00A0}
\pdfglyphtounicode{upsilonlatin}{00A0}
\pdfglyphtounicode{upsilontonos}{00A0}
\pdfglyphtounicode{upslope}{00A0}
\pdfglyphtounicode{uptackbelowcmb}{00A0}
\pdfglyphtounicode{uptackmod}{00A0}
\pdfglyphtounicode{uragurmukhi}{00A0}
\pdfglyphtounicode{uring}{00A0}
\pdfglyphtounicode{ushortcyrillic}{00A0}
\pdfglyphtounicode{usmallhiragana}{00A0}
\pdfglyphtounicode{usmallkatakana}{00A0}
\pdfglyphtounicode{usmallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{ustraightcyrillic}{00A0}
\pdfglyphtounicode{ustraightstrokecyrillic}{00A0}
\pdfglyphtounicode{utilde}{00A0}
\pdfglyphtounicode{utildeacute}{00A0}
\pdfglyphtounicode{utildebelow}{00A0}
\pdfglyphtounicode{uubengali}{00A0}
\pdfglyphtounicode{uudeva}{00A0}
\pdfglyphtounicode{uugujarati}{00A0}
\pdfglyphtounicode{uugurmukhi}{00A0}
\pdfglyphtounicode{uumatragurmukhi}{00A0}
\pdfglyphtounicode{uuvowelsignbengali}{00A0}
\pdfglyphtounicode{uuvowelsigndeva}{00A0}
\pdfglyphtounicode{uuvowelsigngujarati}{00A0}
\pdfglyphtounicode{uvowelsignbengali}{00A0}
\pdfglyphtounicode{uvowelsigndeva}{00A0}
\pdfglyphtounicode{uvowelsigngujarati}{00A0}
\pdfglyphtounicode{v}{00A0}
\pdfglyphtounicode{vadeva}{00A0}
\pdfglyphtounicode{vagujarati}{00A0}
\pdfglyphtounicode{vagurmukhi}{00A0}
\pdfglyphtounicode{vakatakana}{00A0}
\pdfglyphtounicode{vav}{00A0}
\pdfglyphtounicode{vavdagesh}{00A0}
\pdfglyphtounicode{vavdagesh65}{00A0}
\pdfglyphtounicode{vavdageshhebrew}{00A0}
\pdfglyphtounicode{vavhebrew}{00A0}
\pdfglyphtounicode{vavholam}{00A0}
\pdfglyphtounicode{vavholamhebrew}{00A0}
\pdfglyphtounicode{vavvavhebrew}{00A0}
\pdfglyphtounicode{vavyodhebrew}{00A0}
\pdfglyphtounicode{vcircle}{00A0}
\pdfglyphtounicode{vdotbelow}{00A0}
\pdfglyphtounicode{vector}{00A0}
\pdfglyphtounicode{vecyrillic}{00A0}
\pdfglyphtounicode{veharabic}{00A0}
\pdfglyphtounicode{vehfinalarabic}{00A0}
\pdfglyphtounicode{vehinitialarabic}{00A0}
\pdfglyphtounicode{vehmedialarabic}{00A0}
\pdfglyphtounicode{vekatakana}{00A0}
\pdfglyphtounicode{venus}{00A0}
\pdfglyphtounicode{verticalbar}{00A0}
\pdfglyphtounicode{verticallineabovecmb}{00A0}
\pdfglyphtounicode{verticallinebelowcmb}{00A0}
\pdfglyphtounicode{verticallinelowmod}{00A0}
\pdfglyphtounicode{verticallinemod}{00A0}
\pdfglyphtounicode{vewarmenian}{00A0}
\pdfglyphtounicode{vhook}{00A0}
\pdfglyphtounicode{vikatakana}{00A0}
\pdfglyphtounicode{viramabengali}{00A0}
\pdfglyphtounicode{viramadeva}{00A0}
\pdfglyphtounicode{viramagujarati}{00A0}
\pdfglyphtounicode{visargabengali}{00A0}
\pdfglyphtounicode{visargadeva}{00A0}
\pdfglyphtounicode{visargagujarati}{00A0}
\pdfglyphtounicode{visiblespace}{00A0}
\pdfglyphtounicode{visualspace}{00A0}
\pdfglyphtounicode{vmonospace}{00A0}
\pdfglyphtounicode{voarmenian}{00A0}
\pdfglyphtounicode{voicediterationhiragana}{00A0}
\pdfglyphtounicode{voicediterationkatakana}{00A0}
\pdfglyphtounicode{voicedmarkkana}{00A0}
\pdfglyphtounicode{voicedmarkkanahalfwidth}{00A0}
\pdfglyphtounicode{vokatakana}{00A0}
\pdfglyphtounicode{vparen}{00A0}
\pdfglyphtounicode{vtilde}{00A0}
\pdfglyphtounicode{vturned}{00A0}
\pdfglyphtounicode{vuhiragana}{00A0}
\pdfglyphtounicode{vukatakana}{00A0}
\pdfglyphtounicode{w}{00A0}
\pdfglyphtounicode{wacute}{00A0}
\pdfglyphtounicode{waekorean}{00A0}
\pdfglyphtounicode{wahiragana}{00A0}
\pdfglyphtounicode{wakatakana}{00A0}
\pdfglyphtounicode{wakatakanahalfwidth}{00A0}
\pdfglyphtounicode{wakorean}{00A0}
\pdfglyphtounicode{wasmallhiragana}{00A0}
\pdfglyphtounicode{wasmallkatakana}{00A0}
\pdfglyphtounicode{wattosquare}{00A0}
\pdfglyphtounicode{wavedash}{00A0}
\pdfglyphtounicode{wavyunderscorevertical}{00A0}
\pdfglyphtounicode{wawarabic}{00A0}
\pdfglyphtounicode{wawfinalarabic}{00A0}
\pdfglyphtounicode{wawhamzaabovearabic}{00A0}
\pdfglyphtounicode{wawhamzaabovefinalarabic}{00A0}
\pdfglyphtounicode{wbsquare}{00A0}
\pdfglyphtounicode{wcircle}{00A0}
\pdfglyphtounicode{wcircumflex}{00A0}
\pdfglyphtounicode{wdieresis}{00A0}
\pdfglyphtounicode{wdotaccent}{00A0}
\pdfglyphtounicode{wdotbelow}{00A0}
\pdfglyphtounicode{wehiragana}{00A0}
\pdfglyphtounicode{weierstrass}{00A0}
\pdfglyphtounicode{wekatakana}{00A0}
\pdfglyphtounicode{wekorean}{00A0}
\pdfglyphtounicode{weokorean}{00A0}
\pdfglyphtounicode{wgrave}{00A0}
\pdfglyphtounicode{whitebullet}{00A0}
\pdfglyphtounicode{whitecircle}{00A0}
\pdfglyphtounicode{whitecircleinverse}{00A0}
\pdfglyphtounicode{whitecornerbracketleft}{00A0}
\pdfglyphtounicode{whitecornerbracketleftvertical}{00A0}
\pdfglyphtounicode{whitecornerbracketright}{00A0}
\pdfglyphtounicode{whitecornerbracketrightvertical}{00A0}
\pdfglyphtounicode{whitediamond}{00A0}
\pdfglyphtounicode{whitediamondcontainingblacksmalldiamond}{00A0}
\pdfglyphtounicode{whitedownpointingsmalltriangle}{00A0}
\pdfglyphtounicode{whitedownpointingtriangle}{00A0}
\pdfglyphtounicode{whiteleftpointingsmalltriangle}{00A0}
\pdfglyphtounicode{whiteleftpointingtriangle}{00A0}
\pdfglyphtounicode{whitelenticularbracketleft}{00A0}
\pdfglyphtounicode{whitelenticularbracketright}{00A0}
\pdfglyphtounicode{whiterightpointingsmalltriangle}{00A0}
\pdfglyphtounicode{whiterightpointingtriangle}{00A0}
\pdfglyphtounicode{whitesmallsquare}{00A0}
\pdfglyphtounicode{whitesmilingface}{00A0}
\pdfglyphtounicode{whitesquare}{00A0}
\pdfglyphtounicode{whitestar}{00A0}
\pdfglyphtounicode{whitetelephone}{00A0}
\pdfglyphtounicode{whitetortoiseshellbracketleft}{00A0}
\pdfglyphtounicode{whitetortoiseshellbracketright}{00A0}
\pdfglyphtounicode{whiteuppointingsmalltriangle}{00A0}
\pdfglyphtounicode{whiteuppointingtriangle}{00A0}
\pdfglyphtounicode{wihiragana}{00A0}
\pdfglyphtounicode{wikatakana}{00A0}
\pdfglyphtounicode{wikorean}{00A0}
\pdfglyphtounicode{wmonospace}{00A0}
\pdfglyphtounicode{wohiragana}{00A0}
\pdfglyphtounicode{wokatakana}{00A0}
\pdfglyphtounicode{wokatakanahalfwidth}{00A0}
\pdfglyphtounicode{won}{00A0}
\pdfglyphtounicode{wonmonospace}{00A0}
\pdfglyphtounicode{wowaenthai}{00A0}
\pdfglyphtounicode{wparen}{00A0}
\pdfglyphtounicode{wreathproduct}{00A0}
\pdfglyphtounicode{wring}{00A0}
\pdfglyphtounicode{wsuperior}{00A0}
\pdfglyphtounicode{wturned}{00A0}
\pdfglyphtounicode{wynn}{00A0}
\pdfglyphtounicode{x}{00A0}
\pdfglyphtounicode{xabovecmb}{00A0}
\pdfglyphtounicode{xbopomofo}{00A0}
\pdfglyphtounicode{xcircle}{00A0}
\pdfglyphtounicode{xdieresis}{00A0}
\pdfglyphtounicode{xdotaccent}{00A0}
\pdfglyphtounicode{xeharmenian}{00A0}
\pdfglyphtounicode{xi}{00A0}
\pdfglyphtounicode{xmonospace}{00A0}
\pdfglyphtounicode{xparen}{00A0}
\pdfglyphtounicode{xsuperior}{00A0}
\pdfglyphtounicode{y}{00A0}
\pdfglyphtounicode{yaadosquare}{00A0}
\pdfglyphtounicode{yabengali}{00A0}
\pdfglyphtounicode{yacute}{00A0}
\pdfglyphtounicode{yadeva}{00A0}
\pdfglyphtounicode{yaekorean}{00A0}
\pdfglyphtounicode{yagujarati}{00A0}
\pdfglyphtounicode{yagurmukhi}{00A0}
\pdfglyphtounicode{yahiragana}{00A0}
\pdfglyphtounicode{yakatakana}{00A0}
\pdfglyphtounicode{yakatakanahalfwidth}{00A0}
\pdfglyphtounicode{yakorean}{00A0}
\pdfglyphtounicode{yamakkanthai}{00A0}
\pdfglyphtounicode{yasmallhiragana}{00A0}
\pdfglyphtounicode{yasmallkatakana}{00A0}
\pdfglyphtounicode{yasmallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{yatcyrillic}{00A0}
\pdfglyphtounicode{ycircle}{00A0}
\pdfglyphtounicode{ycircumflex}{00A0}
\pdfglyphtounicode{ydieresis}{00A0}
\pdfglyphtounicode{ydotaccent}{00A0}
\pdfglyphtounicode{ydotbelow}{00A0}
\pdfglyphtounicode{yeharabic}{00A0}
\pdfglyphtounicode{yehbarreearabic}{00A0}
\pdfglyphtounicode{yehbarreefinalarabic}{00A0}
\pdfglyphtounicode{yehfinalarabic}{00A0}
\pdfglyphtounicode{yehhamzaabovearabic}{00A0}
\pdfglyphtounicode{yehhamzaabovefinalarabic}{00A0}
\pdfglyphtounicode{yehhamzaaboveinitialarabic}{00A0}
\pdfglyphtounicode{yehhamzaabovemedialarabic}{00A0}
\pdfglyphtounicode{yehinitialarabic}{00A0}
\pdfglyphtounicode{yehmedialarabic}{00A0}
\pdfglyphtounicode{yehmeeminitialarabic}{00A0}
\pdfglyphtounicode{yehmeemisolatedarabic}{00A0}
\pdfglyphtounicode{yehnoonfinalarabic}{00A0}
\pdfglyphtounicode{yehthreedotsbelowarabic}{00A0}
\pdfglyphtounicode{yekorean}{00A0}
\pdfglyphtounicode{yen}{00A0}
\pdfglyphtounicode{yenmonospace}{00A0}
\pdfglyphtounicode{yeokorean}{00A0}
\pdfglyphtounicode{yeorinhieuhkorean}{00A0}
\pdfglyphtounicode{yerahbenyomohebrew}{00A0}
\pdfglyphtounicode{yerahbenyomolefthebrew}{00A0}
\pdfglyphtounicode{yericyrillic}{00A0}
\pdfglyphtounicode{yerudieresiscyrillic}{00A0}
\pdfglyphtounicode{yesieungkorean}{00A0}
\pdfglyphtounicode{yesieungpansioskorean}{00A0}
\pdfglyphtounicode{yesieungsioskorean}{00A0}
\pdfglyphtounicode{yetivhebrew}{00A0}
\pdfglyphtounicode{ygrave}{00A0}
\pdfglyphtounicode{yhook}{00A0}
\pdfglyphtounicode{yhookabove}{00A0}
\pdfglyphtounicode{yiarmenian}{00A0}
\pdfglyphtounicode{yicyrillic}{00A0}
\pdfglyphtounicode{yikorean}{00A0}
\pdfglyphtounicode{yinyang}{00A0}
\pdfglyphtounicode{yiwnarmenian}{00A0}
\pdfglyphtounicode{ymonospace}{00A0}
\pdfglyphtounicode{yod}{00A0}
\pdfglyphtounicode{yoddagesh}{00A0}
\pdfglyphtounicode{yoddageshhebrew}{00A0}
\pdfglyphtounicode{yodhebrew}{00A0}
\pdfglyphtounicode{yodyodhebrew}{00A0}
\pdfglyphtounicode{yodyodpatahhebrew}{00A0}
\pdfglyphtounicode{yohiragana}{00A0}
\pdfglyphtounicode{yoikorean}{00A0}
\pdfglyphtounicode{yokatakana}{00A0}
\pdfglyphtounicode{yokatakanahalfwidth}{00A0}
\pdfglyphtounicode{yokorean}{00A0}
\pdfglyphtounicode{yosmallhiragana}{00A0}
\pdfglyphtounicode{yosmallkatakana}{00A0}
\pdfglyphtounicode{yosmallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{yotgreek}{00A0}
\pdfglyphtounicode{yoyaekorean}{00A0}
\pdfglyphtounicode{yoyakorean}{00A0}
\pdfglyphtounicode{yoyakthai}{00A0}
\pdfglyphtounicode{yoyingthai}{00A0}
\pdfglyphtounicode{yparen}{00A0}
\pdfglyphtounicode{ypogegrammeni}{00A0}
\pdfglyphtounicode{ypogegrammenigreekcmb}{00A0}
\pdfglyphtounicode{yr}{00A0}
\pdfglyphtounicode{yring}{00A0}
\pdfglyphtounicode{ysuperior}{00A0}
\pdfglyphtounicode{ytilde}{00A0}
\pdfglyphtounicode{yturned}{00A0}
\pdfglyphtounicode{yuhiragana}{00A0}
\pdfglyphtounicode{yuikorean}{00A0}
\pdfglyphtounicode{yukatakana}{00A0}
\pdfglyphtounicode{yukatakanahalfwidth}{00A0}
\pdfglyphtounicode{yukorean}{00A0}
\pdfglyphtounicode{yusbigcyrillic}{00A0}
\pdfglyphtounicode{yusbigiotifiedcyrillic}{00A0}
\pdfglyphtounicode{yuslittlecyrillic}{00A0}
\pdfglyphtounicode{yuslittleiotifiedcyrillic}{00A0}
\pdfglyphtounicode{yusmallhiragana}{00A0}
\pdfglyphtounicode{yusmallkatakana}{00A0}
\pdfglyphtounicode{yusmallkatakanahalfwidth}{00A0}
\pdfglyphtounicode{yuyekorean}{00A0}
\pdfglyphtounicode{yuyeokorean}{00A0}
\pdfglyphtounicode{yyabengali}{00A0}
\pdfglyphtounicode{yyadeva}{00A0}
\pdfglyphtounicode{z}{00A0}
\pdfglyphtounicode{zaarmenian}{00A0}
\pdfglyphtounicode{zacute}{00A0}
\pdfglyphtounicode{zadeva}{00A0}
\pdfglyphtounicode{zagurmukhi}{00A0}
\pdfglyphtounicode{zaharabic}{00A0}
\pdfglyphtounicode{zahfinalarabic}{00A0}
\pdfglyphtounicode{zahinitialarabic}{00A0}
\pdfglyphtounicode{zahiragana}{00A0}
\pdfglyphtounicode{zahmedialarabic}{00A0}
\pdfglyphtounicode{zainarabic}{00A0}
\pdfglyphtounicode{zainfinalarabic}{00A0}
\pdfglyphtounicode{zakatakana}{00A0}
\pdfglyphtounicode{zaqefgadolhebrew}{00A0}
\pdfglyphtounicode{zaqefqatanhebrew}{00A0}
\pdfglyphtounicode{zarqahebrew}{00A0}
\pdfglyphtounicode{zayin}{00A0}
\pdfglyphtounicode{zayindagesh}{00A0}
\pdfglyphtounicode{zayindageshhebrew}{00A0}
\pdfglyphtounicode{zayinhebrew}{00A0}
\pdfglyphtounicode{zbopomofo}{00A0}
\pdfglyphtounicode{zcaron}{00A0}
\pdfglyphtounicode{zcircle}{00A0}
\pdfglyphtounicode{zcircumflex}{00A0}
\pdfglyphtounicode{zcurl}{00A0}
\pdfglyphtounicode{zdot}{00A0}
\pdfglyphtounicode{zdotaccent}{00A0}
\pdfglyphtounicode{zdotbelow}{00A0}
\pdfglyphtounicode{zecyrillic}{00A0}
\pdfglyphtounicode{zedescendercyrillic}{00A0}
\pdfglyphtounicode{zedieresiscyrillic}{00A0}
\pdfglyphtounicode{zehiragana}{00A0}
\pdfglyphtounicode{zekatakana}{00A0}
\pdfglyphtounicode{zero}{00A0}
\pdfglyphtounicode{zeroarabic}{00A0}
\pdfglyphtounicode{zerobengali}{00A0}
\pdfglyphtounicode{zerodeva}{00A0}
\pdfglyphtounicode{zerogujarati}{00A0}
\pdfglyphtounicode{zerogurmukhi}{00A0}
\pdfglyphtounicode{zerohackarabic}{00A0}
\pdfglyphtounicode{zeroinferior}{00A0}
\pdfglyphtounicode{zeromonospace}{00A0}
\pdfglyphtounicode{zerooldstyle}{00A0}
\pdfglyphtounicode{zeropersian}{00A0}
\pdfglyphtounicode{zerosuperior}{00A0}
\pdfglyphtounicode{zerothai}{00A0}
\pdfglyphtounicode{zerowidthjoiner}{00A0}
\pdfglyphtounicode{zerowidthnonjoiner}{00A0}
\pdfglyphtounicode{zerowidthspace}{00A0}
\pdfglyphtounicode{zeta}{00A0}
\pdfglyphtounicode{zhbopomofo}{00A0}
\pdfglyphtounicode{zhearmenian}{00A0}
\pdfglyphtounicode{zhebrevecyrillic}{00A0}
\pdfglyphtounicode{zhecyrillic}{00A0}
\pdfglyphtounicode{zhedescendercyrillic}{00A0}
\pdfglyphtounicode{zhedieresiscyrillic}{00A0}
\pdfglyphtounicode{zihiragana}{00A0}
\pdfglyphtounicode{zikatakana}{00A0}
\pdfglyphtounicode{zinorhebrew}{00A0}
\pdfglyphtounicode{zlinebelow}{00A0}
\pdfglyphtounicode{zmonospace}{00A0}
\pdfglyphtounicode{zohiragana}{00A0}
\pdfglyphtounicode{zokatakana}{00A0}
\pdfglyphtounicode{zparen}{00A0}
\pdfglyphtounicode{zretroflexhook}{00A0}
\pdfglyphtounicode{zstroke}{00A0}
\pdfglyphtounicode{zuhiragana}{00A0}
\pdfglyphtounicode{zukatakana}{00A0}

